HAT-P-20b--HAT-P-23b: Four Massive Transiting Extrasolar Planets

We report the discovery of four relatively massive (2-7MJ) transiting extrasolar planets. HAT-P-20b orbits a V=11.339 K3 dwarf star with a period P=2.875317+/-0.000004d. The host star has a mass of 0.760+/-0.03 Msun, radius of 0.690+/-0.02 Rsun, Teff=4595+/-80 K, and metallicity [Fe/H]=+0.35+/-0.08. HAT-P-20b has a mass of 7.246+/-0.187 MJ, and radius of 0.867+/-0.033 RJ yielding a mean density of 13.78+/-1.50 gcm^-3 , which is the second highest value among all known exoplanets. HAT-P-21b orbits a V=11.685 G3 dwarf on an eccentric (e=0.2280+/-0.016) orbit, with a period of P=4.1244810+/-000007d. The host star has a mass of 0.95+/-0.04Msun, radius of 1.10+/-0.08Rsun, Teff=5588+/-80K, and [Fe/H]=+0.01+/-0.08. HAT-P-21b has a mass of 4.063+/-0.161MJ, and radius of 1.024+/-0.092RJ. HAT-P-22b orbits the V=9.732 G5 dwarf HD233731, with P=3.2122200+/-0.000009d. The host star has a mass of 0.92+/-0.03Msun, radius of 1.04+/-0.04Rsun, Teff=5302+/-80K, and metallicity of +0.24+/-0.08. The planet has a mass of 2.147+/-0.061 MJ, and compact radius of 1.080+/-0.058RJ. The host star also harbors an M-dwarf companion at a wide separation. Finally, HAT-P-23b orbits a V=12.432 G0 dwarf star, with a period P=1.212884+/-0.000002d. The host star has a mass of 1.13+/-0.04sun, radius of 1.20+/-0.07Rsun, Teff=5905+/-80K, and [Fe/H]=+0.15+/-0.04. The planetary companion has a mass of 2.090+/-0.111MJ, and radius of 1.368+/-0.090RJ (abridged).

==> HTR102-001_phfu_tab.tex <==
$ 54891.60570 $ & $   0.00028 $ & $   0.00069 $ & $   8.78803 $ & $ z$\\
$ 54891.60603 $ & $  -0.00100 $ & $   0.00069 $ & $   8.78658 $ & $ z$\\
$ 54891.60636 $ & $  -0.00189 $ & $   0.00069 $ & $   8.78541 $ & $ z$\\
$ 54891.60667 $ & $  -0.00138 $ & $   0.00069 $ & $   8.78514 $ & $ z$\\
$ 54891.60702 $ & $  -0.00237 $ & $   0.00069 $ & $   8.78534 $ & $ z$\\
$ 54891.60735 $ & $   0.00030 $ & $   0.00069 $ & $   8.78923 $ & $ z$\\
$ 54891.60767 $ & $   0.00404 $ & $   0.00069 $ & $   8.79234 $ & $ z$\\
$ 54891.60801 $ & $  -0.00170 $ & $   0.00069 $ & $   8.78696 $ & $ z$\\
$ 54891.60831 $ & $   0.00257 $ & $   0.00069 $ & $   8.79009 $ & $ z$\\
$ 54891.60865 $ & $  -0.00145 $ & $   0.00069 $ & $   8.78653 $ & $ z$\\
$ 54891.60899 $ & $  -0.00405 $ & $   0.00069 $ & $   8.78362 $ & $ z$\\
$ 54891.60930 $ & $  -0.00197 $ & $   0.00069 $ & $   8.78547 $ & $ z$\\
$ 54891.60964 $ & $  -0.00092 $ & $   0.00069 $ & $   8.78783 $ & $ z$\\
$ 54891.60997 $ & $  -0.00066 $ & $   0.00069 $ & $   8.78799 $ & $ z$\\
$ 54891.61033 $ & $  -0.00152 $ & $   0.00069 $ & $   8.78614 $ & $ z$\\
$ 54891.61064 $ & $  -0.00328 $ & $   0.00069 $ & $   8.78474 $ & $ z$\\
$ 54891.61099 $ & $  -0.00186 $ & $   0.00069 $ & $   8.78550 $ & $ z$\\
$ 54891.61130 $ & $   0.00002 $ & $   0.00069 $ & $   8.78768 $ & $ z$\\
$ 54891.61165 $ & $  -0.00016 $ & $   0.00069 $ & $   8.78857 $ & $ z$\\
$ 54891.61196 $ & $  -0.00155 $ & $   0.00069 $ & $   8.78621 $ & $ z$\\
$ 54891.61231 $ & $   0.00341 $ & $   0.00069 $ & $   8.79098 $ & $ z$\\
$ 54891.61261 $ & $   0.00360 $ & $   0.00069 $ & $   8.79165 $ & $ z$\\
$ 54891.61294 $ & $  -0.00062 $ & $   0.00069 $ & $   8.78729 $ & $ z$\\
$ 54891.61327 $ & $   0.00121 $ & $   0.00069 $ & $   8.79009 $ & $ z$\\
$ 54891.61360 $ & $   0.00114 $ & $   0.00069 $ & $   8.78900 $ & $ z$\\
$ 54891.61408 $ & $   0.00394 $ & $   0.00069 $ & $   8.79082 $ & $ z$\\
$ 54891.61441 $ & $   0.00167 $ & $   0.00069 $ & $   8.78818 $ & $ z$\\
$ 54891.61538 $ & $   0.00209 $ & $   0.00070 $ & $   8.79179 $ & $ z$\\
$ 54891.61570 $ & $   0.00298 $ & $   0.00069 $ & $   8.79138 $ & $ z$\\
$ 54891.61606 $ & $  -0.00062 $ & $   0.00069 $ & $   8.78689 $ & $ z$\\
$ 54891.61638 $ & $   0.00443 $ & $   0.00069 $ & $   8.79212 $ & $ z$\\
$ 54891.61672 $ & $  -0.00055 $ & $   0.00069 $ & $   8.78757 $ & $ z$\\
$ 54891.61706 $ & $   0.00003 $ & $   0.00069 $ & $   8.78805 $ & $ z$\\
$ 54891.61738 $ & $   0.00476 $ & $   0.00070 $ & $   8.79366 $ & $ z$\\
$ 54891.61772 $ & $   0.00738 $ & $   0.00069 $ & $   8.79538 $ & $ z$\\
$ 54891.61805 $ & $   0.00165 $ & $   0.00069 $ & $   8.78945 $ & $ z$\\
$ 54891.61840 $ & $   0.00381 $ & $   0.00069 $ & $   8.79106 $ & $ z$\\
$ 54891.61871 $ & $   0.00469 $ & $   0.00069 $ & $   8.79131 $ & $ z$\\
$ 54891.61905 $ & $   0.00251 $ & $   0.00070 $ & $   8.79130 $ & $ z$\\
$ 54891.61937 $ & $   0.00141 $ & $   0.00071 $ & $   8.79037 $ & $ z$\\
$ 54891.61971 $ & $   0.00226 $ & $   0.00070 $ & $   8.79143 $ & $ z$\\
$ 54891.62004 $ & $   0.00511 $ & $   0.00069 $ & $   8.79360 $ & $ z$\\
$ 54891.62038 $ & $   0.00412 $ & $   0.00069 $ & $   8.79188 $ & $ z$\\
$ 54891.62070 $ & $   0.00147 $ & $   0.00069 $ & $   8.79038 $ & $ z$\\
$ 54891.62103 $ & $   0.00350 $ & $   0.00069 $ & $   8.79176 $ & $ z$\\
$ 54891.62134 $ & $   0.00457 $ & $   0.00069 $ & $   8.79284 $ & $ z$\\
$ 54891.62167 $ & $   0.00685 $ & $   0.00069 $ & $   8.79336 $ & $ z$\\
$ 54891.62201 $ & $   0.00406 $ & $   0.00069 $ & $   8.79134 $ & $ z$\\
$ 54891.62237 $ & $   0.00340 $ & $   0.00069 $ & $   8.79093 $ & $ z$\\
$ 54891.62272 $ & $   0.00790 $ & $   0.00069 $ & $   8.79553 $ & $ z$\\
$ 54891.62304 $ & $   0.00895 $ & $   0.00069 $ & $   8.79687 $ & $ z$\\
$ 54891.62338 $ & $   0.01058 $ & $   0.00069 $ & $   8.79816 $ & $ z$\\
$ 54891.62372 $ & $   0.00875 $ & $   0.00069 $ & $   8.79592 $ & $ z$\\
$ 54891.62405 $ & $   0.00555 $ & $   0.00069 $ & $   8.79311 $ & $ z$\\
$ 54891.62439 $ & $   0.01335 $ & $   0.00070 $ & $   8.80242 $ & $ z$\\
$ 54891.62471 $ & $   0.00701 $ & $   0.00070 $ & $   8.79568 $ & $ z$\\
$ 54891.62505 $ & $   0.01063 $ & $   0.00070 $ & $   8.79915 $ & $ z$\\
$ 54891.62538 $ & $   0.01170 $ & $   0.00069 $ & $   8.79952 $ & $ z$\\
$ 54891.62571 $ & $   0.00479 $ & $   0.00070 $ & $   8.79273 $ & $ z$\\
$ 54891.62604 $ & $   0.00954 $ & $   0.00070 $ & $   8.79866 $ & $ z$\\
$ 54891.62638 $ & $   0.00675 $ & $   0.00069 $ & $   8.79486 $ & $ z$\\
$ 54891.62671 $ & $   0.00593 $ & $   0.00069 $ & $   8.79302 $ & $ z$\\
$ 54891.62702 $ & $   0.01361 $ & $   0.00069 $ & $   8.80152 $ & $ z$\\
$ 54891.62733 $ & $   0.01086 $ & $   0.00069 $ & $   8.79886 $ & $ z$\\
$ 54891.62769 $ & $   0.01304 $ & $   0.00069 $ & $   8.80028 $ & $ z$\\
$ 54891.62802 $ & $   0.00998 $ & $   0.00070 $ & $   8.79861 $ & $ z$\\
$ 54891.62835 $ & $   0.01231 $ & $   0.00070 $ & $   8.80078 $ & $ z$\\
$ 54891.62870 $ & $   0.01182 $ & $   0.00069 $ & $   8.79984 $ & $ z$\\
$ 54891.62906 $ & $   0.01035 $ & $   0.00069 $ & $   8.79853 $ & $ z$\\
$ 54891.62971 $ & $   0.01204 $ & $   0.00069 $ & $   8.79908 $ & $ z$\\
$ 54891.63003 $ & $   0.00761 $ & $   0.00069 $ & $   8.79451 $ & $ z$\\
$ 54891.63038 $ & $   0.01303 $ & $   0.00069 $ & $   8.80022 $ & $ z$\\
$ 54891.63074 $ & $   0.01134 $ & $   0.00069 $ & $   8.79913 $ & $ z$\\
$ 54891.63106 $ & $   0.00871 $ & $   0.00069 $ & $   8.79580 $ & $ z$\\
$ 54891.63138 $ & $   0.01490 $ & $   0.00069 $ & $   8.80167 $ & $ z$\\
$ 54891.63172 $ & $   0.01305 $ & $   0.00071 $ & $   8.80247 $ & $ z$\\
$ 54891.63206 $ & $   0.01243 $ & $   0.00069 $ & $   8.80097 $ & $ z$\\
$ 54891.63239 $ & $   0.01152 $ & $   0.00070 $ & $   8.79970 $ & $ z$\\
$ 54891.63274 $ & $   0.00991 $ & $   0.00069 $ & $   8.79865 $ & $ z$\\
$ 54891.63307 $ & $   0.01147 $ & $   0.00069 $ & $   8.79927 $ & $ z$\\
$ 54891.63340 $ & $   0.01595 $ & $   0.00069 $ & $   8.80316 $ & $ z$\\
$ 54891.63373 $ & $   0.01135 $ & $   0.00069 $ & $   8.79927 $ & $ z$\\
$ 54891.63407 $ & $   0.01424 $ & $   0.00069 $ & $   8.80134 $ & $ z$\\
$ 54891.63440 $ & $   0.01178 $ & $   0.00069 $ & $   8.79918 $ & $ z$\\
$ 54891.63473 $ & $   0.01338 $ & $   0.00069 $ & $   8.80057 $ & $ z$\\
$ 54891.63508 $ & $   0.01379 $ & $   0.00069 $ & $   8.79962 $ & $ z$\\
$ 54891.63539 $ & $   0.01206 $ & $   0.00069 $ & $   8.79939 $ & $ z$\\
$ 54891.63572 $ & $   0.01369 $ & $   0.00069 $ & $   8.80056 $ & $ z$\\
$ 54891.63606 $ & $   0.01245 $ & $   0.00069 $ & $   8.79836 $ & $ z$\\
$ 54891.63640 $ & $   0.01010 $ & $   0.00069 $ & $   8.79768 $ & $ z$\\
$ 54891.63672 $ & $   0.01391 $ & $   0.00069 $ & $   8.80084 $ & $ z$\\
$ 54891.63707 $ & $   0.01125 $ & $   0.00069 $ & $   8.79874 $ & $ z$\\
$ 54891.63739 $ & $   0.01819 $ & $   0.00069 $ & $   8.80505 $ & $ z$\\
$ 54891.63773 $ & $   0.01366 $ & $   0.00069 $ & $   8.80066 $ & $ z$\\
$ 54891.63806 $ & $   0.01474 $ & $   0.00069 $ & $   8.80235 $ & $ z$\\
$ 54891.63837 $ & $   0.01347 $ & $   0.00069 $ & $   8.80062 $ & $ z$\\
$ 54891.63871 $ & $   0.01535 $ & $   0.00069 $ & $   8.80239 $ & $ z$\\
$ 54891.63908 $ & $   0.01421 $ & $   0.00069 $ & $   8.80134 $ & $ z$\\
$ 54891.63940 $ & $   0.01262 $ & $   0.00069 $ & $   8.79904 $ & $ z$\\
$ 54891.63975 $ & $   0.01244 $ & $   0.00069 $ & $   8.79915 $ & $ z$\\
$ 54891.64009 $ & $   0.01368 $ & $   0.00069 $ & $   8.80041 $ & $ z$\\
$ 54891.64041 $ & $   0.01353 $ & $   0.00069 $ & $   8.80030 $ & $ z$\\
$ 54891.64074 $ & $   0.01531 $ & $   0.00069 $ & $   8.80201 $ & $ z$\\
$ 54891.64107 $ & $   0.01487 $ & $   0.00069 $ & $   8.80198 $ & $ z$\\
$ 54891.64141 $ & $   0.01126 $ & $   0.00069 $ & $   8.79873 $ & $ z$\\
$ 54891.64173 $ & $   0.01284 $ & $   0.00069 $ & $   8.80101 $ & $ z$\\
$ 54891.64208 $ & $   0.01534 $ & $   0.00069 $ & $   8.80204 $ & $ z$\\
$ 54891.64240 $ & $   0.01398 $ & $   0.00069 $ & $   8.80028 $ & $ z$\\
$ 54891.64271 $ & $   0.01468 $ & $   0.00069 $ & $   8.80104 $ & $ z$\\
$ 54891.64304 $ & $   0.01456 $ & $   0.00069 $ & $   8.80111 $ & $ z$\\
$ 54891.64337 $ & $   0.01323 $ & $   0.00069 $ & $   8.79985 $ & $ z$\\
$ 54891.64372 $ & $   0.01371 $ & $   0.00069 $ & $   8.80043 $ & $ z$\\
$ 54891.64405 $ & $   0.01122 $ & $   0.00069 $ & $   8.79802 $ & $ z$\\
$ 54891.64438 $ & $   0.01284 $ & $   0.00069 $ & $   8.80007 $ & $ z$\\
$ 54891.64472 $ & $   0.01702 $ & $   0.00069 $ & $   8.80432 $ & $ z$\\
$ 54891.64502 $ & $   0.01791 $ & $   0.00069 $ & $   8.80477 $ & $ z$\\
$ 54891.64534 $ & $   0.01014 $ & $   0.00069 $ & $   8.79614 $ & $ z$\\
$ 54891.64569 $ & $   0.01284 $ & $   0.00069 $ & $   8.79979 $ & $ z$\\
$ 54891.64603 $ & $   0.01477 $ & $   0.00069 $ & $   8.80121 $ & $ z$\\
$ 54891.64636 $ & $   0.01320 $ & $   0.00069 $ & $   8.79973 $ & $ z$\\
$ 54891.64667 $ & $   0.01388 $ & $   0.00069 $ & $   8.80116 $ & $ z$\\
$ 54891.64703 $ & $   0.01477 $ & $   0.00069 $ & $   8.80241 $ & $ z$\\
$ 54891.64740 $ & $   0.01264 $ & $   0.00068 $ & $   8.79888 $ & $ z$\\
$ 54891.64773 $ & $   0.01515 $ & $   0.00068 $ & $   8.80188 $ & $ z$\\
$ 54891.64807 $ & $   0.01236 $ & $   0.00068 $ & $   8.79986 $ & $ z$\\
$ 54891.64841 $ & $   0.01244 $ & $   0.00068 $ & $   8.79955 $ & $ z$\\
$ 54891.64874 $ & $   0.01734 $ & $   0.00068 $ & $   8.80449 $ & $ z$\\
$ 54891.64908 $ & $   0.01428 $ & $   0.00068 $ & $   8.80089 $ & $ z$\\
$ 54891.64940 $ & $   0.01330 $ & $   0.00068 $ & $   8.80045 $ & $ z$\\
$ 54891.64973 $ & $   0.01509 $ & $   0.00068 $ & $   8.80184 $ & $ z$\\
$ 54891.65006 $ & $   0.01096 $ & $   0.00068 $ & $   8.79776 $ & $ z$\\
$ 54891.65040 $ & $   0.01353 $ & $   0.00068 $ & $   8.80055 $ & $ z$\\
$ 54891.65072 $ & $   0.01430 $ & $   0.00068 $ & $   8.80123 $ & $ z$\\
$ 54891.65106 $ & $   0.01342 $ & $   0.00068 $ & $   8.79979 $ & $ z$\\
$ 54891.65138 $ & $   0.01394 $ & $   0.00068 $ & $   8.80096 $ & $ z$\\
$ 54891.65172 $ & $   0.01458 $ & $   0.00068 $ & $   8.80096 $ & $ z$\\
$ 54891.65206 $ & $   0.01165 $ & $   0.00068 $ & $   8.79845 $ & $ z$\\
$ 54891.65238 $ & $   0.01309 $ & $   0.00068 $ & $   8.79993 $ & $ z$\\
$ 54891.65273 $ & $   0.01586 $ & $   0.00068 $ & $   8.80220 $ & $ z$\\
$ 54891.65305 $ & $   0.01356 $ & $   0.00068 $ & $   8.80029 $ & $ z$\\
$ 54891.65337 $ & $   0.01254 $ & $   0.00068 $ & $   8.79865 $ & $ z$\\
$ 54891.65370 $ & $   0.01160 $ & $   0.00068 $ & $   8.79815 $ & $ z$\\
$ 54891.65406 $ & $   0.01340 $ & $   0.00068 $ & $   8.80026 $ & $ z$\\
$ 54891.65437 $ & $   0.01220 $ & $   0.00068 $ & $   8.79844 $ & $ z$\\
$ 54891.65471 $ & $   0.01358 $ & $   0.00068 $ & $   8.80045 $ & $ z$\\
$ 54891.65505 $ & $   0.01611 $ & $   0.00068 $ & $   8.80256 $ & $ z$\\
$ 54891.65539 $ & $   0.01532 $ & $   0.00068 $ & $   8.80133 $ & $ z$\\
$ 54891.65571 $ & $   0.01402 $ & $   0.00068 $ & $   8.80009 $ & $ z$\\
$ 54891.65605 $ & $   0.01180 $ & $   0.00068 $ & $   8.79795 $ & $ z$\\
$ 54891.65637 $ & $   0.01219 $ & $   0.00068 $ & $   8.79829 $ & $ z$\\
$ 54891.65671 $ & $   0.01334 $ & $   0.00068 $ & $   8.79981 $ & $ z$\\
$ 54891.65703 $ & $   0.01325 $ & $   0.00068 $ & $   8.79948 $ & $ z$\\
$ 54891.65738 $ & $   0.01464 $ & $   0.00068 $ & $   8.80060 $ & $ z$\\
$ 54891.65769 $ & $   0.01264 $ & $   0.00068 $ & $   8.80042 $ & $ z$\\
$ 54891.65804 $ & $   0.01431 $ & $   0.00068 $ & $   8.80124 $ & $ z$\\
$ 54891.65836 $ & $   0.01344 $ & $   0.00068 $ & $   8.80049 $ & $ z$\\
$ 54891.65870 $ & $   0.01197 $ & $   0.00068 $ & $   8.79872 $ & $ z$\\
$ 54891.65903 $ & $   0.01399 $ & $   0.00068 $ & $   8.80074 $ & $ z$\\
$ 54891.65937 $ & $   0.01144 $ & $   0.00068 $ & $   8.79849 $ & $ z$\\
$ 54891.65969 $ & $   0.01372 $ & $   0.00068 $ & $   8.80010 $ & $ z$\\
$ 54891.66002 $ & $   0.01405 $ & $   0.00068 $ & $   8.80087 $ & $ z$\\
$ 54891.66035 $ & $   0.01135 $ & $   0.00068 $ & $   8.79793 $ & $ z$\\
$ 54891.66069 $ & $   0.01281 $ & $   0.00068 $ & $   8.79972 $ & $ z$\\
$ 54891.66104 $ & $   0.01327 $ & $   0.00068 $ & $   8.79995 $ & $ z$\\
$ 54891.66136 $ & $   0.01502 $ & $   0.00068 $ & $   8.80133 $ & $ z$\\
$ 54891.66170 $ & $   0.01498 $ & $   0.00068 $ & $   8.80180 $ & $ z$\\
$ 54891.66203 $ & $   0.01616 $ & $   0.00068 $ & $   8.80286 $ & $ z$\\
$ 54891.66236 $ & $   0.01380 $ & $   0.00068 $ & $   8.80077 $ & $ z$\\
$ 54891.66268 $ & $   0.01468 $ & $   0.00068 $ & $   8.80162 $ & $ z$\\
$ 54891.66301 $ & $   0.01191 $ & $   0.00068 $ & $   8.79851 $ & $ z$\\
$ 54891.66336 $ & $   0.01730 $ & $   0.00068 $ & $   8.80325 $ & $ z$\\
$ 54891.66367 $ & $   0.01321 $ & $   0.00068 $ & $   8.80069 $ & $ z$\\
$ 54891.66414 $ & $   0.01443 $ & $   0.00068 $ & $   8.80098 $ & $ z$\\
$ 54891.66448 $ & $   0.01029 $ & $   0.00068 $ & $   8.79691 $ & $ z$\\
$ 54891.66480 $ & $   0.01225 $ & $   0.00068 $ & $   8.79891 $ & $ z$\\
$ 54891.66513 $ & $   0.01382 $ & $   0.00068 $ & $   8.80044 $ & $ z$\\
$ 54891.66546 $ & $   0.01374 $ & $   0.00068 $ & $   8.79985 $ & $ z$\\
$ 54891.66577 $ & $   0.01319 $ & $   0.00068 $ & $   8.79983 $ & $ z$\\
$ 54891.66611 $ & $   0.01424 $ & $   0.00068 $ & $   8.80114 $ & $ z$\\
$ 54891.66644 $ & $   0.01213 $ & $   0.00068 $ & $   8.79833 $ & $ z$\\
$ 54891.66676 $ & $   0.01181 $ & $   0.00068 $ & $   8.79858 $ & $ z$\\
$ 54891.66709 $ & $   0.01150 $ & $   0.00068 $ & $   8.79821 $ & $ z$\\
$ 54891.66740 $ & $   0.01326 $ & $   0.00068 $ & $   8.79983 $ & $ z$\\
$ 54891.66775 $ & $   0.01434 $ & $   0.00068 $ & $   8.80119 $ & $ z$\\
$ 54891.66807 $ & $   0.01483 $ & $   0.00068 $ & $   8.80131 $ & $ z$\\
$ 54891.66841 $ & $   0.01211 $ & $   0.00068 $ & $   8.79851 $ & $ z$\\
$ 54891.66873 $ & $   0.01313 $ & $   0.00068 $ & $   8.79953 $ & $ z$\\
$ 54891.66908 $ & $   0.01311 $ & $   0.00068 $ & $   8.79928 $ & $ z$\\
$ 54891.66939 $ & $   0.01165 $ & $   0.00068 $ & $   8.79834 $ & $ z$\\
$ 54891.66972 $ & $   0.01476 $ & $   0.00068 $ & $   8.80149 $ & $ z$\\
$ 54891.67004 $ & $   0.01362 $ & $   0.00068 $ & $   8.80132 $ & $ z$\\
$ 54891.67036 $ & $   0.01130 $ & $   0.00068 $ & $   8.79811 $ & $ z$\\
$ 54891.67070 $ & $   0.01413 $ & $   0.00068 $ & $   8.79986 $ & $ z$\\
$ 54891.67104 $ & $   0.01449 $ & $   0.00068 $ & $   8.80119 $ & $ z$\\
$ 54891.67137 $ & $   0.01240 $ & $   0.00068 $ & $   8.79881 $ & $ z$\\
$ 54891.67171 $ & $   0.01184 $ & $   0.00068 $ & $   8.79828 $ & $ z$\\
$ 54891.67203 $ & $   0.01587 $ & $   0.00068 $ & $   8.80264 $ & $ z$\\
$ 54891.67238 $ & $   0.01422 $ & $   0.00068 $ & $   8.80093 $ & $ z$\\
$ 54891.67270 $ & $   0.01486 $ & $   0.00068 $ & $   8.80096 $ & $ z$\\
$ 54891.67304 $ & $   0.01615 $ & $   0.00068 $ & $   8.80292 $ & $ z$\\
$ 54891.67336 $ & $   0.01314 $ & $   0.00068 $ & $   8.79931 $ & $ z$\\
$ 54891.67370 $ & $   0.01447 $ & $   0.00068 $ & $   8.80131 $ & $ z$\\
$ 54891.67402 $ & $   0.01091 $ & $   0.00068 $ & $   8.79699 $ & $ z$\\
$ 54891.67437 $ & $   0.01266 $ & $   0.00068 $ & $   8.79973 $ & $ z$\\
$ 54891.67468 $ & $   0.01258 $ & $   0.00068 $ & $   8.79891 $ & $ z$\\
$ 54891.67502 $ & $   0.01721 $ & $   0.00068 $ & $   8.80328 $ & $ z$\\
$ 54891.67534 $ & $   0.01362 $ & $   0.00068 $ & $   8.79947 $ & $ z$\\
$ 54891.67569 $ & $   0.01398 $ & $   0.00068 $ & $   8.80089 $ & $ z$\\
$ 54891.67599 $ & $   0.01250 $ & $   0.00068 $ & $   8.79969 $ & $ z$\\
$ 54891.67632 $ & $   0.01381 $ & $   0.00068 $ & $   8.80014 $ & $ z$\\
$ 54891.67665 $ & $   0.01561 $ & $   0.00068 $ & $   8.80175 $ & $ z$\\
$ 54891.67700 $ & $   0.01337 $ & $   0.00068 $ & $   8.80019 $ & $ z$\\
$ 54891.67732 $ & $   0.01398 $ & $   0.00068 $ & $   8.80104 $ & $ z$\\
$ 54891.67766 $ & $   0.01684 $ & $   0.00068 $ & $   8.80302 $ & $ z$\\
$ 54891.67799 $ & $   0.01253 $ & $   0.00068 $ & $   8.79829 $ & $ z$\\
$ 54891.67832 $ & $   0.01609 $ & $   0.00068 $ & $   8.80238 $ & $ z$\\
$ 54891.67866 $ & $   0.01288 $ & $   0.00068 $ & $   8.79902 $ & $ z$\\
$ 54891.67899 $ & $   0.01489 $ & $   0.00068 $ & $   8.80118 $ & $ z$\\
$ 54891.67930 $ & $   0.01632 $ & $   0.00068 $ & $   8.80207 $ & $ z$\\
$ 54891.67965 $ & $   0.01459 $ & $   0.00068 $ & $   8.80070 $ & $ z$\\
$ 54891.67997 $ & $   0.01534 $ & $   0.00068 $ & $   8.80165 $ & $ z$\\
$ 54891.68031 $ & $   0.01294 $ & $   0.00068 $ & $   8.79869 $ & $ z$\\
$ 54891.68078 $ & $   0.01514 $ & $   0.00068 $ & $   8.80107 $ & $ z$\\
$ 54891.68112 $ & $   0.01205 $ & $   0.00068 $ & $   8.79825 $ & $ z$\\
$ 54891.68144 $ & $   0.01247 $ & $   0.00067 $ & $   8.79842 $ & $ z$\\
$ 54891.68179 $ & $   0.01459 $ & $   0.00068 $ & $   8.80098 $ & $ z$\\
$ 54891.68211 $ & $   0.01593 $ & $   0.00068 $ & $   8.80246 $ & $ z$\\
$ 54891.68245 $ & $   0.01409 $ & $   0.00068 $ & $   8.80000 $ & $ z$\\
$ 54891.68278 $ & $   0.01358 $ & $   0.00068 $ & $   8.79979 $ & $ z$\\
$ 54891.68311 $ & $   0.01666 $ & $   0.00068 $ & $   8.80288 $ & $ z$\\
$ 54891.68344 $ & $   0.01539 $ & $   0.00067 $ & $   8.80154 $ & $ z$\\
$ 54891.68379 $ & $   0.01348 $ & $   0.00068 $ & $   8.79992 $ & $ z$\\
$ 54891.68411 $ & $   0.01183 $ & $   0.00067 $ & $   8.79735 $ & $ z$\\
$ 54891.68445 $ & $   0.01490 $ & $   0.00068 $ & $   8.80099 $ & $ z$\\
$ 54891.68477 $ & $   0.01497 $ & $   0.00068 $ & $   8.80159 $ & $ z$\\
$ 54891.68512 $ & $   0.01398 $ & $   0.00067 $ & $   8.79984 $ & $ z$\\
$ 54891.68546 $ & $   0.01312 $ & $   0.00068 $ & $   8.79960 $ & $ z$\\
$ 54891.68577 $ & $   0.01445 $ & $   0.00068 $ & $   8.80117 $ & $ z$\\
$ 54891.68609 $ & $   0.01338 $ & $   0.00068 $ & $   8.80007 $ & $ z$\\
$ 54891.68644 $ & $   0.01436 $ & $   0.00068 $ & $   8.80048 $ & $ z$\\
$ 54891.68678 $ & $   0.01408 $ & $   0.00068 $ & $   8.80093 $ & $ z$\\
$ 54891.68710 $ & $   0.01401 $ & $   0.00068 $ & $   8.80009 $ & $ z$\\
$ 54891.68744 $ & $   0.01339 $ & $   0.00068 $ & $   8.79941 $ & $ z$\\
$ 54891.68776 $ & $   0.01366 $ & $   0.00068 $ & $   8.79980 $ & $ z$\\
$ 54891.68810 $ & $   0.01490 $ & $   0.00068 $ & $   8.80123 $ & $ z$\\
$ 54891.68842 $ & $   0.01306 $ & $   0.00067 $ & $   8.79925 $ & $ z$\\
$ 54891.68875 $ & $   0.01482 $ & $   0.00068 $ & $   8.80157 $ & $ z$\\
$ 54891.68909 $ & $   0.01313 $ & $   0.00067 $ & $   8.80002 $ & $ z$\\
$ 54891.68941 $ & $   0.01379 $ & $   0.00067 $ & $   8.80028 $ & $ z$\\
$ 54891.68976 $ & $   0.01491 $ & $   0.00067 $ & $   8.80140 $ & $ z$\\
$ 54891.69007 $ & $   0.01161 $ & $   0.00067 $ & $   8.79812 $ & $ z$\\
$ 54891.69041 $ & $   0.01314 $ & $   0.00067 $ & $   8.79945 $ & $ z$\\
$ 54891.69076 $ & $   0.01470 $ & $   0.00067 $ & $   8.80127 $ & $ z$\\
$ 54891.69107 $ & $   0.01409 $ & $   0.00067 $ & $   8.80086 $ & $ z$\\
$ 54891.69139 $ & $   0.01153 $ & $   0.00068 $ & $   8.79841 $ & $ z$\\
$ 54891.69175 $ & $   0.01311 $ & $   0.00068 $ & $   8.79940 $ & $ z$\\
$ 54891.69206 $ & $   0.01435 $ & $   0.00067 $ & $   8.80014 $ & $ z$\\
$ 54891.69241 $ & $   0.01297 $ & $   0.00067 $ & $   8.79887 $ & $ z$\\
$ 54891.69274 $ & $   0.01499 $ & $   0.00067 $ & $   8.80142 $ & $ z$\\
$ 54891.69306 $ & $   0.01459 $ & $   0.00068 $ & $   8.80139 $ & $ z$\\
$ 54891.69340 $ & $   0.01419 $ & $   0.00067 $ & $   8.80082 $ & $ z$\\
$ 54891.69373 $ & $   0.01332 $ & $   0.00068 $ & $   8.79993 $ & $ z$\\
$ 54891.69407 $ & $   0.01186 $ & $   0.00067 $ & $   8.79810 $ & $ z$\\
$ 54891.69440 $ & $   0.01421 $ & $   0.00068 $ & $   8.79983 $ & $ z$\\
$ 54891.69474 $ & $   0.01387 $ & $   0.00068 $ & $   8.80026 $ & $ z$\\
$ 54891.69506 $ & $   0.01392 $ & $   0.00067 $ & $   8.80055 $ & $ z$\\
$ 54891.69537 $ & $   0.01511 $ & $   0.00067 $ & $   8.80116 $ & $ z$\\
$ 54891.69572 $ & $   0.01307 $ & $   0.00067 $ & $   8.79890 $ & $ z$\\
$ 54891.69605 $ & $   0.01295 $ & $   0.00067 $ & $   8.79955 $ & $ z$\\
$ 54891.69637 $ & $   0.01530 $ & $   0.00067 $ & $   8.80135 $ & $ z$\\
$ 54891.69669 $ & $   0.01381 $ & $   0.00067 $ & $   8.80004 $ & $ z$\\
$ 54891.69703 $ & $   0.01399 $ & $   0.00067 $ & $   8.80019 $ & $ z$\\
$ 54891.69742 $ & $   0.01416 $ & $   0.00067 $ & $   8.80021 $ & $ z$\\
$ 54891.69775 $ & $   0.01490 $ & $   0.00067 $ & $   8.80110 $ & $ z$\\
$ 54891.69807 $ & $   0.01331 $ & $   0.00067 $ & $   8.79962 $ & $ z$\\
$ 54891.69842 $ & $   0.01466 $ & $   0.00067 $ & $   8.80106 $ & $ z$\\
$ 54891.69873 $ & $   0.01666 $ & $   0.00067 $ & $   8.80302 $ & $ z$\\
$ 54891.69909 $ & $   0.01472 $ & $   0.00068 $ & $   8.80192 $ & $ z$\\
$ 54891.69943 $ & $   0.01358 $ & $   0.00068 $ & $   8.80007 $ & $ z$\\
$ 54891.69975 $ & $   0.01173 $ & $   0.00068 $ & $   8.79860 $ & $ z$\\
$ 54891.70011 $ & $   0.01423 $ & $   0.00068 $ & $   8.80118 $ & $ z$\\
$ 54891.70044 $ & $   0.01228 $ & $   0.00067 $ & $   8.79913 $ & $ z$\\
$ 54891.70077 $ & $   0.01333 $ & $   0.00068 $ & $   8.80098 $ & $ z$\\
$ 54891.70109 $ & $   0.01310 $ & $   0.00068 $ & $   8.79953 $ & $ z$\\
$ 54891.70143 $ & $   0.01137 $ & $   0.00068 $ & $   8.79793 $ & $ z$\\
$ 54891.70178 $ & $   0.01265 $ & $   0.00067 $ & $   8.79913 $ & $ z$\\
$ 54891.70212 $ & $   0.01324 $ & $   0.00068 $ & $   8.80061 $ & $ z$\\
$ 54891.70242 $ & $   0.01410 $ & $   0.00068 $ & $   8.80081 $ & $ z$\\
$ 54891.70276 $ & $   0.01431 $ & $   0.00068 $ & $   8.80119 $ & $ z$\\
$ 54891.70308 $ & $   0.01365 $ & $   0.00068 $ & $   8.80097 $ & $ z$\\
$ 54891.70342 $ & $   0.01464 $ & $   0.00069 $ & $   8.80264 $ & $ z$\\
$ 54891.70375 $ & $   0.01386 $ & $   0.00069 $ & $   8.80245 $ & $ z$\\
$ 54891.70408 $ & $   0.01394 $ & $   0.00068 $ & $   8.80129 $ & $ z$\\
$ 54891.70440 $ & $   0.01181 $ & $   0.00068 $ & $   8.79856 $ & $ z$\\
$ 54891.70475 $ & $   0.01037 $ & $   0.00068 $ & $   8.79730 $ & $ z$\\
$ 54891.70509 $ & $   0.01400 $ & $   0.00068 $ & $   8.80138 $ & $ z$\\
$ 54891.70542 $ & $   0.01298 $ & $   0.00068 $ & $   8.80064 $ & $ z$\\
$ 54891.70576 $ & $   0.01313 $ & $   0.00068 $ & $   8.80099 $ & $ z$\\
$ 54891.70609 $ & $   0.01332 $ & $   0.00068 $ & $   8.80126 $ & $ z$\\
$ 54891.70642 $ & $   0.01375 $ & $   0.00068 $ & $   8.80089 $ & $ z$\\
$ 54891.70675 $ & $   0.01101 $ & $   0.00068 $ & $   8.79851 $ & $ z$\\
$ 54891.70706 $ & $   0.01317 $ & $   0.00068 $ & $   8.80056 $ & $ z$\\
$ 54891.70741 $ & $   0.01362 $ & $   0.00068 $ & $   8.80033 $ & $ z$\\
$ 54891.70775 $ & $   0.01340 $ & $   0.00067 $ & $   8.79985 $ & $ z$\\
$ 54891.70807 $ & $   0.01262 $ & $   0.00068 $ & $   8.79982 $ & $ z$\\
$ 54891.70841 $ & $   0.01255 $ & $   0.00068 $ & $   8.79947 $ & $ z$\\
$ 54891.70875 $ & $   0.01519 $ & $   0.00068 $ & $   8.80211 $ & $ z$\\
$ 54891.70909 $ & $   0.01188 $ & $   0.00067 $ & $   8.79875 $ & $ z$\\
$ 54891.70943 $ & $   0.01377 $ & $   0.00067 $ & $   8.80065 $ & $ z$\\
$ 54891.70974 $ & $   0.01224 $ & $   0.00067 $ & $   8.79938 $ & $ z$\\
$ 54891.71007 $ & $   0.01263 $ & $   0.00068 $ & $   8.79950 $ & $ z$\\
$ 54891.71041 $ & $   0.01085 $ & $   0.00068 $ & $   8.79788 $ & $ z$\\
$ 54891.71073 $ & $   0.01365 $ & $   0.00067 $ & $   8.80055 $ & $ z$\\
$ 54891.71105 $ & $   0.01474 $ & $   0.00067 $ & $   8.80192 $ & $ z$\\
$ 54891.71137 $ & $   0.01220 $ & $   0.00067 $ & $   8.79920 $ & $ z$\\
$ 54891.71169 $ & $   0.01218 $ & $   0.00067 $ & $   8.79897 $ & $ z$\\
$ 54891.71204 $ & $   0.01404 $ & $   0.00067 $ & $   8.80099 $ & $ z$\\
$ 54891.71238 $ & $   0.01133 $ & $   0.00067 $ & $   8.79827 $ & $ z$\\
$ 54891.71270 $ & $   0.01021 $ & $   0.00067 $ & $   8.79711 $ & $ z$\\
$ 54891.71303 $ & $   0.01391 $ & $   0.00068 $ & $   8.80158 $ & $ z$\\
$ 54891.71335 $ & $   0.01185 $ & $   0.00068 $ & $   8.79877 $ & $ z$\\
$ 54891.71367 $ & $   0.01182 $ & $   0.00067 $ & $   8.79862 $ & $ z$\\
$ 54891.71404 $ & $   0.01286 $ & $   0.00067 $ & $   8.79996 $ & $ z$\\
$ 54891.71438 $ & $   0.01250 $ & $   0.00067 $ & $   8.79916 $ & $ z$\\
$ 54891.71469 $ & $   0.00966 $ & $   0.00067 $ & $   8.79650 $ & $ z$\\
$ 54891.71504 $ & $   0.01395 $ & $   0.00067 $ & $   8.80013 $ & $ z$\\
$ 54891.71539 $ & $   0.01330 $ & $   0.00068 $ & $   8.79997 $ & $ z$\\
$ 54891.71571 $ & $   0.01125 $ & $   0.00067 $ & $   8.79812 $ & $ z$\\
$ 54891.71605 $ & $   0.01142 $ & $   0.00067 $ & $   8.79785 $ & $ z$\\
$ 54891.71637 $ & $   0.01141 $ & $   0.00067 $ & $   8.79834 $ & $ z$\\
$ 54891.71671 $ & $   0.01190 $ & $   0.00067 $ & $   8.79861 $ & $ z$\\
$ 54891.71703 $ & $   0.01357 $ & $   0.00067 $ & $   8.80015 $ & $ z$\\
$ 54891.71737 $ & $   0.01252 $ & $   0.00067 $ & $   8.79834 $ & $ z$\\
$ 54891.71769 $ & $   0.00946 $ & $   0.00067 $ & $   8.79602 $ & $ z$\\
$ 54891.71803 $ & $   0.01105 $ & $   0.00067 $ & $   8.79791 $ & $ z$\\
$ 54891.71835 $ & $   0.01083 $ & $   0.00067 $ & $   8.79746 $ & $ z$\\
$ 54891.71869 $ & $   0.01070 $ & $   0.00067 $ & $   8.79664 $ & $ z$\\
$ 54891.71902 $ & $   0.01013 $ & $   0.00067 $ & $   8.79654 $ & $ z$\\
$ 54891.71936 $ & $   0.01048 $ & $   0.00067 $ & $   8.79697 $ & $ z$\\
$ 54891.71969 $ & $   0.01079 $ & $   0.00067 $ & $   8.79766 $ & $ z$\\
$ 54891.72002 $ & $   0.01135 $ & $   0.00067 $ & $   8.79806 $ & $ z$\\
$ 54891.72033 $ & $   0.01129 $ & $   0.00067 $ & $   8.79776 $ & $ z$\\
$ 54891.72066 $ & $   0.00994 $ & $   0.00067 $ & $   8.79631 $ & $ z$\\
$ 54891.72098 $ & $   0.01279 $ & $   0.00067 $ & $   8.79903 $ & $ z$\\
$ 54891.72131 $ & $   0.00923 $ & $   0.00067 $ & $   8.79518 $ & $ z$\\
$ 54891.72166 $ & $   0.00838 $ & $   0.00067 $ & $   8.79541 $ & $ z$\\
$ 54891.72198 $ & $   0.00819 $ & $   0.00067 $ & $   8.79477 $ & $ z$\\
$ 54891.72232 $ & $   0.00827 $ & $   0.00067 $ & $   8.79479 $ & $ z$\\
$ 54891.72264 $ & $   0.00921 $ & $   0.00067 $ & $   8.79562 $ & $ z$\\
$ 54891.72298 $ & $   0.00784 $ & $   0.00067 $ & $   8.79463 $ & $ z$\\
$ 54891.72330 $ & $   0.00576 $ & $   0.00067 $ & $   8.79230 $ & $ z$\\
$ 54891.72364 $ & $   0.00575 $ & $   0.00067 $ & $   8.79114 $ & $ z$\\
$ 54891.72399 $ & $   0.00683 $ & $   0.00068 $ & $   8.79360 $ & $ z$\\
$ 54891.72431 $ & $   0.00852 $ & $   0.00068 $ & $   8.79548 $ & $ z$\\
$ 54891.72463 $ & $   0.00519 $ & $   0.00068 $ & $   8.79106 $ & $ z$\\
$ 54891.72497 $ & $   0.00260 $ & $   0.00068 $ & $   8.78854 $ & $ z$\\
$ 54891.72530 $ & $   0.00908 $ & $   0.00067 $ & $   8.79563 $ & $ z$\\
$ 54891.72564 $ & $   0.00605 $ & $   0.00067 $ & $   8.79248 $ & $ z$\\
$ 54891.72600 $ & $   0.00410 $ & $   0.00067 $ & $   8.79083 $ & $ z$\\
$ 54891.72632 $ & $   0.00328 $ & $   0.00067 $ & $   8.78997 $ & $ z$\\
$ 54891.72667 $ & $   0.00566 $ & $   0.00067 $ & $   8.79273 $ & $ z$\\
$ 54891.72699 $ & $   0.00045 $ & $   0.00067 $ & $   8.78694 $ & $ z$\\
$ 54891.72732 $ & $   0.00426 $ & $   0.00067 $ & $   8.79077 $ & $ z$\\
$ 54891.72764 $ & $   0.00329 $ & $   0.00067 $ & $   8.79042 $ & $ z$\\
$ 54891.72798 $ & $   0.00316 $ & $   0.00067 $ & $   8.78984 $ & $ z$\\
$ 54891.72831 $ & $   0.00489 $ & $   0.00067 $ & $   8.79176 $ & $ z$\\
$ 54891.72865 $ & $   0.00321 $ & $   0.00067 $ & $   8.79048 $ & $ z$\\
$ 54891.72898 $ & $   0.00157 $ & $   0.00067 $ & $   8.78821 $ & $ z$\\
$ 54891.72932 $ & $   0.00025 $ & $   0.00067 $ & $   8.78674 $ & $ z$\\
$ 54891.72966 $ & $   0.00150 $ & $   0.00067 $ & $   8.78784 $ & $ z$\\
$ 54891.72998 $ & $  -0.00069 $ & $   0.00067 $ & $   8.78621 $ & $ z$\\
$ 54891.73033 $ & $   0.00236 $ & $   0.00067 $ & $   8.78893 $ & $ z$\\
$ 54891.73070 $ & $   0.00067 $ & $   0.00067 $ & $   8.78721 $ & $ z$\\
$ 54891.73102 $ & $   0.00178 $ & $   0.00067 $ & $   8.78890 $ & $ z$\\
$ 54891.73136 $ & $   0.00184 $ & $   0.00067 $ & $   8.78876 $ & $ z$\\
$ 54891.73168 $ & $   0.00185 $ & $   0.00067 $ & $   8.78827 $ & $ z$\\
$ 54891.73199 $ & $   0.00104 $ & $   0.00067 $ & $   8.78752 $ & $ z$\\
$ 54891.73231 $ & $   0.00069 $ & $   0.00067 $ & $   8.78756 $ & $ z$\\
$ 54891.73264 $ & $   0.00108 $ & $   0.00067 $ & $   8.78744 $ & $ z$\\
$ 54891.73299 $ & $   0.00146 $ & $   0.00066 $ & $   8.78735 $ & $ z$\\
$ 54891.73333 $ & $  -0.00058 $ & $   0.00066 $ & $   8.78571 $ & $ z$\\
$ 54891.73364 $ & $   0.00135 $ & $   0.00067 $ & $   8.78704 $ & $ z$\\
$ 54891.73397 $ & $   0.00006 $ & $   0.00067 $ & $   8.78657 $ & $ z$\\
$ 54891.73430 $ & $  -0.00007 $ & $   0.00067 $ & $   8.78670 $ & $ z$\\
$ 54891.73464 $ & $   0.00044 $ & $   0.00067 $ & $   8.78677 $ & $ z$\\
$ 54891.73497 $ & $  -0.00042 $ & $   0.00067 $ & $   8.78620 $ & $ z$\\
$ 54891.73532 $ & $   0.00012 $ & $   0.00067 $ & $   8.78711 $ & $ z$\\
$ 54891.73566 $ & $  -0.00050 $ & $   0.00067 $ & $   8.78590 $ & $ z$\\
$ 54891.73599 $ & $   0.00001 $ & $   0.00067 $ & $   8.78586 $ & $ z$\\
$ 54891.73632 $ & $   0.00038 $ & $   0.00067 $ & $   8.78651 $ & $ z$\\
$ 54891.73665 $ & $   0.00125 $ & $   0.00067 $ & $   8.78741 $ & $ z$\\
$ 54891.73699 $ & $   0.00096 $ & $   0.00067 $ & $   8.78700 $ & $ z$\\
$ 54891.73731 $ & $   0.00057 $ & $   0.00067 $ & $   8.78694 $ & $ z$\\
$ 54891.73765 $ & $   0.00270 $ & $   0.00067 $ & $   8.78979 $ & $ z$\\
$ 54891.73797 $ & $   0.00123 $ & $   0.00067 $ & $   8.78773 $ & $ z$\\
$ 54891.73829 $ & $   0.00040 $ & $   0.00067 $ & $   8.78672 $ & $ z$\\
$ 54891.73861 $ & $   0.00168 $ & $   0.00067 $ & $   8.78847 $ & $ z$\\
$ 54891.73895 $ & $  -0.00128 $ & $   0.00067 $ & $   8.78477 $ & $ z$\\
$ 54891.73930 $ & $   0.00178 $ & $   0.00067 $ & $   8.78837 $ & $ z$\\
$ 54891.73962 $ & $  -0.00015 $ & $   0.00067 $ & $   8.78639 $ & $ z$\\
$ 54891.73996 $ & $  -0.00067 $ & $   0.00067 $ & $   8.78565 $ & $ z$\\
$ 54891.74029 $ & $   0.00097 $ & $   0.00067 $ & $   8.78686 $ & $ z$\\
$ 54891.74064 $ & $  -0.00067 $ & $   0.00067 $ & $   8.78551 $ & $ z$\\
$ 54891.74098 $ & $  -0.00130 $ & $   0.00067 $ & $   8.78422 $ & $ z$\\
$ 54891.74131 $ & $   0.00058 $ & $   0.00067 $ & $   8.78671 $ & $ z$\\
$ 54891.74165 $ & $   0.00017 $ & $   0.00067 $ & $   8.78616 $ & $ z$\\
$ 54891.74199 $ & $   0.00145 $ & $   0.00067 $ & $   8.78744 $ & $ z$\\
$ 54891.74233 $ & $   0.00014 $ & $   0.00067 $ & $   8.78643 $ & $ z$\\
$ 54891.74265 $ & $  -0.00099 $ & $   0.00067 $ & $   8.78503 $ & $ z$\\
$ 54891.74300 $ & $   0.00028 $ & $   0.00067 $ & $   8.78649 $ & $ z$\\
$ 54891.74331 $ & $   0.00209 $ & $   0.00067 $ & $   8.78826 $ & $ z$\\
$ 54891.74366 $ & $  -0.00054 $ & $   0.00067 $ & $   8.78530 $ & $ z$\\
$ 54891.74398 $ & $   0.00070 $ & $   0.00067 $ & $   8.78683 $ & $ z$\\
$ 54891.74431 $ & $  -0.00180 $ & $   0.00067 $ & $   8.78455 $ & $ z$\\
$ 54891.74466 $ & $   0.00006 $ & $   0.00067 $ & $   8.78621 $ & $ z$\\
$ 54891.74499 $ & $  -0.00158 $ & $   0.00067 $ & $   8.78449 $ & $ z$\\
$ 54891.74532 $ & $  -0.00054 $ & $   0.00067 $ & $   8.78534 $ & $ z$\\
$ 54891.74564 $ & $  -0.00084 $ & $   0.00067 $ & $   8.78576 $ & $ z$\\
$ 54891.74598 $ & $  -0.00068 $ & $   0.00067 $ & $   8.78506 $ & $ z$\\
$ 54891.74630 $ & $  -0.00068 $ & $   0.00067 $ & $   8.78550 $ & $ z$\\
$ 54891.74665 $ & $   0.00124 $ & $   0.00067 $ & $   8.78734 $ & $ z$\\
$ 54891.74699 $ & $   0.00060 $ & $   0.00067 $ & $   8.78694 $ & $ z$\\
$ 54891.74740 $ & $   0.00029 $ & $   0.00067 $ & $   8.78611 $ & $ z$\\
$ 54891.74772 $ & $   0.00061 $ & $   0.00067 $ & $   8.78599 $ & $ z$\\
$ 54891.74805 $ & $   0.00009 $ & $   0.00067 $ & $   8.78632 $ & $ z$\\
$ 54891.74837 $ & $  -0.00060 $ & $   0.00067 $ & $   8.78583 $ & $ z$\\
$ 54891.74872 $ & $  -0.00161 $ & $   0.00067 $ & $   8.78419 $ & $ z$\\
$ 54891.74904 $ & $  -0.00133 $ & $   0.00067 $ & $   8.78496 $ & $ z$\\
$ 54891.74938 $ & $  -0.00022 $ & $   0.00067 $ & $   8.78540 $ & $ z$\\
$ 54891.74971 $ & $  -0.00056 $ & $   0.00067 $ & $   8.78563 $ & $ z$\\
$ 54891.75004 $ & $   0.00163 $ & $   0.00067 $ & $   8.78731 $ & $ z$\\
$ 54891.75039 $ & $   0.00109 $ & $   0.00067 $ & $   8.78751 $ & $ z$\\
$ 54891.75071 $ & $  -0.00035 $ & $   0.00067 $ & $   8.78558 $ & $ z$\\
$ 54891.75106 $ & $   0.00186 $ & $   0.00067 $ & $   8.78770 $ & $ z$\\
$ 54891.75140 $ & $   0.00123 $ & $   0.00067 $ & $   8.78766 $ & $ z$\\
$ 54891.75170 $ & $   0.00122 $ & $   0.00067 $ & $   8.78736 $ & $ z$\\
$ 54891.75205 $ & $   0.00339 $ & $   0.00067 $ & $   8.78875 $ & $ z$\\
$ 54891.75236 $ & $   0.00198 $ & $   0.00068 $ & $   8.78810 $ & $ z$\\
$ 54891.75271 $ & $  -0.00131 $ & $   0.00068 $ & $   8.78472 $ & $ z$\\
$ 54891.75305 $ & $   0.00201 $ & $   0.00068 $ & $   8.78825 $ & $ z$\\
$ 54891.75336 $ & $   0.00274 $ & $   0.00068 $ & $   8.78949 $ & $ z$\\
$ 54891.75371 $ & $   0.00058 $ & $   0.00067 $ & $   8.78688 $ & $ z$\\
$ 54891.75403 $ & $   0.00001 $ & $   0.00067 $ & $   8.78664 $ & $ z$\\
$ 54891.75437 $ & $  -0.00331 $ & $   0.00067 $ & $   8.78364 $ & $ z$\\
$ 54891.75471 $ & $  -0.00230 $ & $   0.00067 $ & $   8.78416 $ & $ z$\\
$ 54891.75503 $ & $   0.00246 $ & $   0.00067 $ & $   8.78862 $ & $ z$\\
$ 54891.75534 $ & $  -0.00241 $ & $   0.00067 $ & $   8.78462 $ & $ z$\\
$ 54891.75567 $ & $  -0.00201 $ & $   0.00067 $ & $   8.78431 $ & $ z$\\
$ 54891.75601 $ & $   0.00006 $ & $   0.00067 $ & $   8.78686 $ & $ z$\\
$ 54891.75633 $ & $  -0.00084 $ & $   0.00067 $ & $   8.78595 $ & $ z$\\
$ 54891.75667 $ & $  -0.00155 $ & $   0.00067 $ & $   8.78495 $ & $ z$\\
$ 54891.75699 $ & $   0.00034 $ & $   0.00067 $ & $   8.78698 $ & $ z$\\
$ 54891.75733 $ & $  -0.00132 $ & $   0.00067 $ & $   8.78530 $ & $ z$\\
$ 54891.75768 $ & $  -0.00026 $ & $   0.00067 $ & $   8.78660 $ & $ z$\\
$ 54891.75799 $ & $   0.00170 $ & $   0.00067 $ & $   8.78910 $ & $ z$\\
$ 54891.75834 $ & $  -0.00007 $ & $   0.00067 $ & $   8.78679 $ & $ z$\\
$ 54891.75866 $ & $   0.00012 $ & $   0.00067 $ & $   8.78739 $ & $ z$\\
$ 54891.75900 $ & $  -0.00132 $ & $   0.00067 $ & $   8.78622 $ & $ z$\\
$ 54891.75933 $ & $  -0.00003 $ & $   0.00067 $ & $   8.78635 $ & $ z$\\
$ 54891.75967 $ & $   0.00026 $ & $   0.00067 $ & $   8.78717 $ & $ z$\\
$ 54891.76000 $ & $  -0.00042 $ & $   0.00067 $ & $   8.78687 $ & $ z$\\
$ 54891.76034 $ & $  -0.00100 $ & $   0.00067 $ & $   8.78591 $ & $ z$\\
$ 54891.76065 $ & $  -0.00187 $ & $   0.00067 $ & $   8.78518 $ & $ z$\\
$ 54891.76099 $ & $  -0.00074 $ & $   0.00067 $ & $   8.78650 $ & $ z$\\
$ 54891.76133 $ & $  -0.00027 $ & $   0.00067 $ & $   8.78633 $ & $ z$\\
$ 54891.76165 $ & $  -0.00116 $ & $   0.00067 $ & $   8.78641 $ & $ z$\\
$ 54891.76199 $ & $  -0.00065 $ & $   0.00067 $ & $   8.78511 $ & $ z$\\
$ 54891.76232 $ & $  -0.00065 $ & $   0.00067 $ & $   8.78620 $ & $ z$\\
$ 54891.76266 $ & $   0.00057 $ & $   0.00067 $ & $   8.78764 $ & $ z$\\
$ 54891.76301 $ & $   0.00002 $ & $   0.00067 $ & $   8.78729 $ & $ z$\\
$ 54891.76334 $ & $  -0.00233 $ & $   0.00067 $ & $   8.78486 $ & $ z$\\
$ 54891.76368 $ & $   0.00021 $ & $   0.00067 $ & $   8.78718 $ & $ z$\\
$ 54891.76404 $ & $  -0.00011 $ & $   0.00067 $ & $   8.78685 $ & $ z$\\
$ 54891.76438 $ & $   0.00045 $ & $   0.00067 $ & $   8.78800 $ & $ z$\\
$ 54891.76471 $ & $  -0.00013 $ & $   0.00067 $ & $   8.78664 $ & $ z$\\
$ 54891.76505 $ & $  -0.00077 $ & $   0.00067 $ & $   8.78704 $ & $ z$\\
$ 54891.76536 $ & $  -0.00202 $ & $   0.00067 $ & $   8.78570 $ & $ z$\\
$ 54891.76571 $ & $   0.00085 $ & $   0.00067 $ & $   8.78790 $ & $ z$\\
$ 54891.76604 $ & $  -0.00122 $ & $   0.00067 $ & $   8.78570 $ & $ z$\\
$ 54891.76637 $ & $   0.00068 $ & $   0.00067 $ & $   8.78815 $ & $ z$\\
$ 54891.76669 $ & $  -0.00048 $ & $   0.00067 $ & $   8.78729 $ & $ z$\\
$ 54891.76704 $ & $   0.00025 $ & $   0.00067 $ & $   8.78729 $ & $ z$\\
$ 54891.76735 $ & $   0.00147 $ & $   0.00067 $ & $   8.78896 $ & $ z$\\
$ 54891.76769 $ & $   0.00005 $ & $   0.00067 $ & $   8.78699 $ & $ z$\\
$ 54891.76803 $ & $   0.00092 $ & $   0.00067 $ & $   8.78768 $ & $ z$\\
$ 54891.76835 $ & $  -0.00037 $ & $   0.00067 $ & $   8.78643 $ & $ z$\\
$ 54891.76869 $ & $   0.00307 $ & $   0.00067 $ & $   8.78953 $ & $ z$\\
$ 54891.76901 $ & $  -0.00042 $ & $   0.00067 $ & $   8.78619 $ & $ z$\\
$ 54891.76935 $ & $   0.00043 $ & $   0.00067 $ & $   8.78749 $ & $ z$\\
$ 54891.76969 $ & $  -0.00068 $ & $   0.00067 $ & $   8.78598 $ & $ z$\\
$ 54891.77004 $ & $   0.00044 $ & $   0.00067 $ & $   8.78733 $ & $ z$\\
$ 54891.77036 $ & $   0.00141 $ & $   0.00067 $ & $   8.78785 $ & $ z$\\
$ 54891.77070 $ & $  -0.00042 $ & $   0.00067 $ & $   8.78521 $ & $ z$\\
$ 54891.77102 $ & $  -0.00056 $ & $   0.00067 $ & $   8.78564 $ & $ z$\\
$ 54891.77137 $ & $  -0.00053 $ & $   0.00067 $ & $   8.78550 $ & $ z$\\
$ 54891.77169 $ & $   0.00102 $ & $   0.00067 $ & $   8.78771 $ & $ z$\\
$ 54891.77202 $ & $   0.00244 $ & $   0.00066 $ & $   8.78870 $ & $ z$\\
$ 54891.77233 $ & $  -0.00017 $ & $   0.00066 $ & $   8.78609 $ & $ z$\\
$ 54891.77266 $ & $  -0.00058 $ & $   0.00066 $ & $   8.78597 $ & $ z$\\
$ 54891.77300 $ & $   0.00029 $ & $   0.00066 $ & $   8.78668 $ & $ z$\\
$ 54891.77335 $ & $  -0.00048 $ & $   0.00066 $ & $   8.78670 $ & $ z$\\
$ 54891.77367 $ & $   0.00073 $ & $   0.00066 $ & $   8.78736 $ & $ z$\\
$ 54891.77400 $ & $  -0.00012 $ & $   0.00066 $ & $   8.78629 $ & $ z$\\
$ 54891.77433 $ & $  -0.00046 $ & $   0.00066 $ & $   8.78620 $ & $ z$\\
$ 54891.77467 $ & $  -0.00090 $ & $   0.00067 $ & $   8.78580 $ & $ z$\\
$ 54891.77499 $ & $   0.00035 $ & $   0.00067 $ & $   8.78688 $ & $ z$\\
$ 54891.77533 $ & $   0.00068 $ & $   0.00067 $ & $   8.78767 $ & $ z$\\
$ 54891.77567 $ & $   0.00133 $ & $   0.00067 $ & $   8.78740 $ & $ z$\\
$ 54891.77600 $ & $   0.00006 $ & $   0.00067 $ & $   8.78652 $ & $ z$\\
$ 54891.77635 $ & $   0.00045 $ & $   0.00067 $ & $   8.78745 $ & $ z$\\
$ 54891.77668 $ & $   0.00072 $ & $   0.00067 $ & $   8.78649 $ & $ z$\\
$ 54891.77700 $ & $  -0.00024 $ & $   0.00067 $ & $   8.78624 $ & $ z$\\
$ 54891.77734 $ & $   0.00056 $ & $   0.00067 $ & $   8.78649 $ & $ z$\\
$ 54891.77769 $ & $   0.00049 $ & $   0.00067 $ & $   8.78622 $ & $ z$\\
$ 54891.77805 $ & $  -0.00137 $ & $   0.00066 $ & $   8.78430 $ & $ z$\\
$ 54891.77836 $ & $  -0.00180 $ & $   0.00066 $ & $   8.78438 $ & $ z$\\
$ 54891.77871 $ & $  -0.00176 $ & $   0.00066 $ & $   8.78438 $ & $ z$\\
$ 54891.77904 $ & $  -0.00103 $ & $   0.00066 $ & $   8.78535 $ & $ z$\\
$ 54891.77938 $ & $  -0.00265 $ & $   0.00066 $ & $   8.78406 $ & $ z$\\
$ 54891.77970 $ & $  -0.00063 $ & $   0.00066 $ & $   8.78569 $ & $ z$\\
$ 54891.78003 $ & $   0.00192 $ & $   0.00066 $ & $   8.78785 $ & $ z$\\
$ 54891.78035 $ & $  -0.00167 $ & $   0.00066 $ & $   8.78487 $ & $ z$\\
$ 54891.78073 $ & $   0.00085 $ & $   0.00067 $ & $   8.78712 $ & $ z$\\
$ 54891.78106 $ & $   0.00049 $ & $   0.00067 $ & $   8.78668 $ & $ z$\\
$ 54891.78139 $ & $  -0.00034 $ & $   0.00067 $ & $   8.78622 $ & $ z$\\
$ 54891.78173 $ & $  -0.00032 $ & $   0.00067 $ & $   8.78644 $ & $ z$\\
$ 54891.78205 $ & $  -0.00138 $ & $   0.00066 $ & $   8.78573 $ & $ z$\\
$ 54891.78239 $ & $   0.00134 $ & $   0.00067 $ & $   8.78725 $ & $ z$\\
$ 54891.78272 $ & $   0.00019 $ & $   0.00067 $ & $   8.78747 $ & $ z$\\
$ 54952.63044 $ & $  -0.00069 $ & $   0.00064 $ & $   8.98403 $ & $ g$\\
$ 54952.63081 $ & $  -0.00283 $ & $   0.00064 $ & $   8.98301 $ & $ g$\\
$ 54952.63120 $ & $  -0.00089 $ & $   0.00064 $ & $   8.98577 $ & $ g$\\
$ 54952.63158 $ & $   0.00180 $ & $   0.00064 $ & $   8.98818 $ & $ g$\\
$ 54952.63199 $ & $   0.00311 $ & $   0.00064 $ & $   8.98966 $ & $ g$\\
$ 54952.63256 $ & $   0.00005 $ & $   0.00064 $ & $   8.98674 $ & $ g$\\
$ 54952.63294 $ & $   0.00281 $ & $   0.00064 $ & $   8.98883 $ & $ g$\\
$ 54952.63332 $ & $   0.00100 $ & $   0.00064 $ & $   8.98701 $ & $ g$\\
$ 54952.63370 $ & $   0.00245 $ & $   0.00064 $ & $   8.98789 $ & $ g$\\
$ 54952.63407 $ & $   0.00147 $ & $   0.00064 $ & $   8.98764 $ & $ g$\\
$ 54952.63469 $ & $  -0.00107 $ & $   0.00064 $ & $   8.98501 $ & $ g$\\
$ 54952.63507 $ & $   0.00013 $ & $   0.00064 $ & $   8.98659 $ & $ g$\\
$ 54952.63545 $ & $  -0.00006 $ & $   0.00064 $ & $   8.98582 $ & $ g$\\
$ 54952.63584 $ & $   0.00015 $ & $   0.00064 $ & $   8.98664 $ & $ g$\\
$ 54952.63622 $ & $   0.00108 $ & $   0.00064 $ & $   8.98752 $ & $ g$\\
$ 54952.63659 $ & $  -0.00004 $ & $   0.00064 $ & $   8.98642 $ & $ g$\\
$ 54952.63699 $ & $  -0.00251 $ & $   0.00064 $ & $   8.98309 $ & $ g$\\
$ 54952.63738 $ & $  -0.00062 $ & $   0.00064 $ & $   8.98418 $ & $ g$\\
$ 54952.63776 $ & $  -0.00286 $ & $   0.00064 $ & $   8.98291 $ & $ g$\\
$ 54952.63813 $ & $  -0.00250 $ & $   0.00064 $ & $   8.98344 $ & $ g$\\
$ 54952.63871 $ & $  -0.00045 $ & $   0.00064 $ & $   8.98456 $ & $ g$\\
$ 54952.63911 $ & $  -0.00078 $ & $   0.00064 $ & $   8.98561 $ & $ g$\\
$ 54952.63949 $ & $  -0.00084 $ & $   0.00064 $ & $   8.98447 $ & $ g$\\
$ 54952.63988 $ & $  -0.00255 $ & $   0.00064 $ & $   8.98303 $ & $ g$\\
$ 54952.64027 $ & $  -0.00293 $ & $   0.00064 $ & $   8.98343 $ & $ g$\\
$ 54952.64083 $ & $   0.00083 $ & $   0.00064 $ & $   8.98698 $ & $ g$\\
$ 54952.64122 $ & $  -0.00026 $ & $   0.00064 $ & $   8.98624 $ & $ g$\\
$ 54952.64162 $ & $  -0.00015 $ & $   0.00064 $ & $   8.98631 $ & $ g$\\
$ 54952.64201 $ & $  -0.00051 $ & $   0.00064 $ & $   8.98590 $ & $ g$\\
$ 54952.64242 $ & $  -0.00008 $ & $   0.00064 $ & $   8.98552 $ & $ g$\\
$ 54952.64301 $ & $   0.00153 $ & $   0.00064 $ & $   8.98666 $ & $ g$\\
$ 54952.64339 $ & $   0.00026 $ & $   0.00064 $ & $   8.98619 $ & $ g$\\
$ 54952.64378 $ & $  -0.00087 $ & $   0.00064 $ & $   8.98519 $ & $ g$\\
$ 54952.64457 $ & $   0.00159 $ & $   0.00064 $ & $   8.98755 $ & $ g$\\
$ 54952.64500 $ & $  -0.00069 $ & $   0.00064 $ & $   8.98614 $ & $ g$\\
$ 54952.64538 $ & $   0.00247 $ & $   0.00064 $ & $   8.98892 $ & $ g$\\
$ 54952.64576 $ & $  -0.00061 $ & $   0.00064 $ & $   8.98626 $ & $ g$\\
$ 54952.64615 $ & $   0.00299 $ & $   0.00064 $ & $   8.99028 $ & $ g$\\
$ 54952.64655 $ & $   0.00152 $ & $   0.00064 $ & $   8.98719 $ & $ g$\\
$ 54952.64699 $ & $  -0.00078 $ & $   0.00064 $ & $   8.98622 $ & $ g$\\
$ 54952.64737 $ & $  -0.00118 $ & $   0.00064 $ & $   8.98537 $ & $ g$\\
$ 54952.64776 $ & $   0.00183 $ & $   0.00064 $ & $   8.98798 $ & $ g$\\
$ 54952.64814 $ & $   0.00271 $ & $   0.00064 $ & $   8.98974 $ & $ g$\\
$ 54952.64853 $ & $   0.00129 $ & $   0.00064 $ & $   8.98786 $ & $ g$\\
$ 54952.64894 $ & $  -0.00018 $ & $   0.00064 $ & $   8.98598 $ & $ g$\\
$ 54952.64933 $ & $   0.00341 $ & $   0.00064 $ & $   8.99035 $ & $ g$\\
$ 54952.64971 $ & $   0.00182 $ & $   0.00064 $ & $   8.98834 $ & $ g$\\
$ 54952.65010 $ & $   0.00133 $ & $   0.00064 $ & $   8.98885 $ & $ g$\\
$ 54952.65049 $ & $   0.00226 $ & $   0.00064 $ & $   8.98856 $ & $ g$\\
$ 54952.65148 $ & $   0.00242 $ & $   0.00064 $ & $   8.98882 $ & $ g$\\
$ 54952.65188 $ & $   0.00218 $ & $   0.00064 $ & $   8.98754 $ & $ g$\\
$ 54952.65229 $ & $   0.00239 $ & $   0.00064 $ & $   8.98859 $ & $ g$\\
$ 54952.65268 $ & $   0.00163 $ & $   0.00064 $ & $   8.98810 $ & $ g$\\
$ 54952.65326 $ & $   0.00465 $ & $   0.00064 $ & $   8.99165 $ & $ g$\\
$ 54952.65364 $ & $   0.00283 $ & $   0.00064 $ & $   8.98900 $ & $ g$\\
$ 54952.65403 $ & $   0.00565 $ & $   0.00064 $ & $   8.99193 $ & $ g$\\
$ 54952.65441 $ & $   0.00437 $ & $   0.00064 $ & $   8.99092 $ & $ g$\\
$ 54952.65479 $ & $   0.00764 $ & $   0.00064 $ & $   8.99356 $ & $ g$\\
$ 54952.65522 $ & $   0.00370 $ & $   0.00064 $ & $   8.98998 $ & $ g$\\
$ 54952.65561 $ & $   0.00791 $ & $   0.00064 $ & $   8.99425 $ & $ g$\\
$ 54952.65600 $ & $   0.00817 $ & $   0.00064 $ & $   8.99530 $ & $ g$\\
$ 54952.65642 $ & $   0.00606 $ & $   0.00064 $ & $   8.99245 $ & $ g$\\
$ 54952.65680 $ & $   0.00663 $ & $   0.00064 $ & $   8.99448 $ & $ g$\\
$ 54952.65737 $ & $   0.00630 $ & $   0.00064 $ & $   8.99224 $ & $ g$\\
$ 54952.65775 $ & $   0.00754 $ & $   0.00064 $ & $   8.99361 $ & $ g$\\
$ 54952.65814 $ & $   0.00773 $ & $   0.00064 $ & $   8.99271 $ & $ g$\\
$ 54952.65855 $ & $   0.00648 $ & $   0.00064 $ & $   8.99276 $ & $ g$\\
$ 54952.65893 $ & $   0.00929 $ & $   0.00064 $ & $   8.99519 $ & $ g$\\
$ 54952.65937 $ & $   0.00933 $ & $   0.00064 $ & $   8.99498 $ & $ g$\\
$ 54952.65976 $ & $   0.01223 $ & $   0.00064 $ & $   8.99881 $ & $ g$\\
$ 54952.66016 $ & $   0.00905 $ & $   0.00064 $ & $   8.99626 $ & $ g$\\
$ 54952.66056 $ & $   0.00988 $ & $   0.00064 $ & $   8.99497 $ & $ g$\\
$ 54952.66096 $ & $   0.01082 $ & $   0.00064 $ & $   8.99657 $ & $ g$\\
$ 54952.66150 $ & $   0.00753 $ & $   0.00064 $ & $   8.99419 $ & $ g$\\
$ 54952.66187 $ & $   0.01291 $ & $   0.00064 $ & $   8.99789 $ & $ g$\\
$ 54952.66224 $ & $   0.01012 $ & $   0.00064 $ & $   8.99532 $ & $ g$\\
$ 54952.66262 $ & $   0.01018 $ & $   0.00064 $ & $   8.99703 $ & $ g$\\
$ 54952.66300 $ & $   0.00978 $ & $   0.00064 $ & $   8.99659 $ & $ g$\\
$ 54952.66341 $ & $   0.01032 $ & $   0.00064 $ & $   8.99552 $ & $ g$\\
$ 54952.66380 $ & $   0.00925 $ & $   0.00064 $ & $   8.99548 $ & $ g$\\
$ 54952.66420 $ & $   0.00879 $ & $   0.00064 $ & $   8.99403 $ & $ g$\\
$ 54952.66458 $ & $   0.00818 $ & $   0.00064 $ & $   8.99410 $ & $ g$\\
$ 54952.66496 $ & $   0.01011 $ & $   0.00064 $ & $   8.99663 $ & $ g$\\
$ 54952.66539 $ & $   0.01081 $ & $   0.00064 $ & $   8.99672 $ & $ g$\\
$ 54952.66577 $ & $   0.00983 $ & $   0.00064 $ & $   8.99604 $ & $ g$\\
$ 54952.66615 $ & $   0.01302 $ & $   0.00064 $ & $   8.99901 $ & $ g$\\
$ 54952.66655 $ & $   0.01311 $ & $   0.00064 $ & $   8.99842 $ & $ g$\\
$ 54952.66693 $ & $   0.01209 $ & $   0.00064 $ & $   8.99706 $ & $ g$\\
$ 54952.66751 $ & $   0.01067 $ & $   0.00064 $ & $   8.99721 $ & $ g$\\
$ 54952.66789 $ & $   0.01228 $ & $   0.00064 $ & $   8.99942 $ & $ g$\\
$ 54952.66828 $ & $   0.01118 $ & $   0.00064 $ & $   8.99710 $ & $ g$\\
$ 54952.66866 $ & $   0.01271 $ & $   0.00064 $ & $   8.99995 $ & $ g$\\
$ 54952.66907 $ & $   0.01503 $ & $   0.00064 $ & $   9.00184 $ & $ g$\\
$ 54952.66946 $ & $   0.01217 $ & $   0.00064 $ & $   8.99807 $ & $ g$\\
$ 54952.66986 $ & $   0.01120 $ & $   0.00064 $ & $   8.99787 $ & $ g$\\
$ 54952.67023 $ & $   0.01095 $ & $   0.00064 $ & $   8.99725 $ & $ g$\\
$ 54952.67062 $ & $   0.01504 $ & $   0.00064 $ & $   9.00175 $ & $ g$\\
$ 54952.67100 $ & $   0.01142 $ & $   0.00064 $ & $   8.99754 $ & $ g$\\
$ 54952.67158 $ & $   0.01244 $ & $   0.00064 $ & $   8.99933 $ & $ g$\\
$ 54952.67196 $ & $   0.01216 $ & $   0.00064 $ & $   8.99911 $ & $ g$\\
$ 54952.67234 $ & $   0.01623 $ & $   0.00064 $ & $   9.00142 $ & $ g$\\
$ 54952.67274 $ & $   0.01135 $ & $   0.00064 $ & $   8.99653 $ & $ g$\\
$ 54952.67312 $ & $   0.01443 $ & $   0.00064 $ & $   9.00147 $ & $ g$\\
$ 54952.67369 $ & $   0.01047 $ & $   0.00064 $ & $   8.99671 $ & $ g$\\
$ 54952.67408 $ & $   0.01470 $ & $   0.00064 $ & $   9.00090 $ & $ g$\\
$ 54952.67447 $ & $   0.01259 $ & $   0.00064 $ & $   8.99882 $ & $ g$\\
$ 54952.67486 $ & $   0.01265 $ & $   0.00064 $ & $   8.99977 $ & $ g$\\
$ 54952.67523 $ & $   0.01135 $ & $   0.00064 $ & $   8.99746 $ & $ g$\\
$ 54952.67584 $ & $   0.01453 $ & $   0.00064 $ & $   8.99994 $ & $ g$\\
$ 54952.67623 $ & $   0.01678 $ & $   0.00064 $ & $   9.00281 $ & $ g$\\
$ 54952.67663 $ & $   0.01643 $ & $   0.00064 $ & $   9.00224 $ & $ g$\\
$ 54952.67703 $ & $   0.01284 $ & $   0.00064 $ & $   8.99899 $ & $ g$\\
$ 54952.67742 $ & $   0.01618 $ & $   0.00065 $ & $   9.00317 $ & $ g$\\
$ 54952.67798 $ & $   0.01181 $ & $   0.00064 $ & $   8.99795 $ & $ g$\\
$ 54952.67836 $ & $   0.01423 $ & $   0.00064 $ & $   9.00116 $ & $ g$\\
$ 54952.67877 $ & $   0.01603 $ & $   0.00065 $ & $   9.00256 $ & $ g$\\
$ 54952.67915 $ & $   0.01621 $ & $   0.00065 $ & $   9.00296 $ & $ g$\\
$ 54952.67953 $ & $   0.01261 $ & $   0.00065 $ & $   8.99862 $ & $ g$\\
$ 54952.67996 $ & $   0.01317 $ & $   0.00064 $ & $   8.99888 $ & $ g$\\
$ 54952.68033 $ & $   0.01278 $ & $   0.00064 $ & $   8.99987 $ & $ g$\\
$ 54952.68071 $ & $   0.01471 $ & $   0.00065 $ & $   9.00064 $ & $ g$\\
$ 54952.68110 $ & $   0.01324 $ & $   0.00064 $ & $   9.00011 $ & $ g$\\
$ 54952.68151 $ & $   0.01411 $ & $   0.00065 $ & $   9.00060 $ & $ g$\\
$ 54952.68194 $ & $   0.01657 $ & $   0.00065 $ & $   9.00274 $ & $ g$\\
$ 54952.68233 $ & $   0.01379 $ & $   0.00065 $ & $   9.00129 $ & $ g$\\
$ 54952.68274 $ & $   0.01635 $ & $   0.00065 $ & $   9.00453 $ & $ g$\\
$ 54952.68312 $ & $   0.01516 $ & $   0.00064 $ & $   9.00219 $ & $ g$\\
$ 54952.68352 $ & $   0.01549 $ & $   0.00065 $ & $   9.00283 $ & $ g$\\
$ 54952.68411 $ & $   0.01234 $ & $   0.00064 $ & $   8.99936 $ & $ g$\\
$ 54952.68450 $ & $   0.01500 $ & $   0.00064 $ & $   9.00074 $ & $ g$\\
$ 54952.68488 $ & $   0.01471 $ & $   0.00064 $ & $   9.00227 $ & $ g$\\
$ 54952.68526 $ & $   0.01126 $ & $   0.00064 $ & $   8.99868 $ & $ g$\\
$ 54952.68563 $ & $   0.01414 $ & $   0.00065 $ & $   9.00117 $ & $ g$\\
$ 54952.68619 $ & $   0.01361 $ & $   0.00064 $ & $   9.00091 $ & $ g$\\
$ 54952.68657 $ & $   0.01314 $ & $   0.00064 $ & $   8.99947 $ & $ g$\\
$ 54952.68696 $ & $   0.01550 $ & $   0.00064 $ & $   9.00222 $ & $ g$\\
$ 54952.68735 $ & $   0.01522 $ & $   0.00064 $ & $   9.00148 $ & $ g$\\
$ 54952.68775 $ & $   0.01662 $ & $   0.00065 $ & $   9.00395 $ & $ g$\\
$ 54952.68819 $ & $   0.01553 $ & $   0.00064 $ & $   9.00200 $ & $ g$\\
$ 54952.68858 $ & $   0.01401 $ & $   0.00064 $ & $   8.99981 $ & $ g$\\
$ 54952.68897 $ & $   0.01649 $ & $   0.00064 $ & $   9.00258 $ & $ g$\\
$ 54952.68938 $ & $   0.01374 $ & $   0.00064 $ & $   9.00050 $ & $ g$\\
$ 54952.68976 $ & $   0.01807 $ & $   0.00065 $ & $   9.00471 $ & $ g$\\
$ 54952.69015 $ & $   0.01763 $ & $   0.00065 $ & $   9.00346 $ & $ g$\\
$ 54952.69055 $ & $   0.01479 $ & $   0.00064 $ & $   8.99999 $ & $ g$\\
$ 54952.69095 $ & $   0.01710 $ & $   0.00065 $ & $   9.00459 $ & $ g$\\
$ 54952.69134 $ & $   0.01679 $ & $   0.00064 $ & $   9.00274 $ & $ g$\\
$ 54952.69173 $ & $   0.01371 $ & $   0.00064 $ & $   9.00017 $ & $ g$\\
$ 54952.69216 $ & $   0.01472 $ & $   0.00064 $ & $   9.00227 $ & $ g$\\
$ 54952.69254 $ & $   0.01395 $ & $   0.00064 $ & $   9.00031 $ & $ g$\\
$ 54952.69293 $ & $   0.01599 $ & $   0.00065 $ & $   9.00177 $ & $ g$\\
$ 54952.69330 $ & $   0.01513 $ & $   0.00065 $ & $   9.00204 $ & $ g$\\
$ 54952.69368 $ & $   0.01397 $ & $   0.00064 $ & $   8.99971 $ & $ g$\\
$ 54952.69423 $ & $   0.01411 $ & $   0.00065 $ & $   9.00027 $ & $ g$\\
$ 54952.69461 $ & $   0.01566 $ & $   0.00065 $ & $   9.00264 $ & $ g$\\
$ 54952.69499 $ & $   0.01441 $ & $   0.00065 $ & $   9.00083 $ & $ g$\\
$ 54952.69540 $ & $   0.01451 $ & $   0.00065 $ & $   9.00039 $ & $ g$\\
$ 54952.69579 $ & $   0.01500 $ & $   0.00065 $ & $   9.00023 $ & $ g$\\
$ 54952.69620 $ & $   0.01613 $ & $   0.00065 $ & $   9.00300 $ & $ g$\\
$ 54952.69659 $ & $   0.01260 $ & $   0.00064 $ & $   8.99993 $ & $ g$\\
$ 54952.69697 $ & $   0.01444 $ & $   0.00065 $ & $   9.00052 $ & $ g$\\
$ 54952.69735 $ & $   0.01465 $ & $   0.00065 $ & $   9.00102 $ & $ g$\\
$ 54952.69774 $ & $   0.01423 $ & $   0.00065 $ & $   9.00118 $ & $ g$\\
$ 54952.69815 $ & $   0.01615 $ & $   0.00065 $ & $   9.00223 $ & $ g$\\
$ 54952.69852 $ & $   0.01544 $ & $   0.00065 $ & $   9.00162 $ & $ g$\\
$ 54952.69893 $ & $   0.01448 $ & $   0.00065 $ & $   9.00232 $ & $ g$\\
$ 54952.69931 $ & $   0.01647 $ & $   0.00065 $ & $   9.00218 $ & $ g$\\
$ 54952.69970 $ & $   0.01554 $ & $   0.00065 $ & $   9.00237 $ & $ g$\\
$ 54952.70014 $ & $   0.01442 $ & $   0.00065 $ & $   9.00142 $ & $ g$\\
$ 54952.70054 $ & $   0.01610 $ & $   0.00065 $ & $   9.00343 $ & $ g$\\
$ 54952.70092 $ & $   0.01449 $ & $   0.00065 $ & $   9.00167 $ & $ g$\\
$ 54952.70134 $ & $   0.01442 $ & $   0.00065 $ & $   9.00132 $ & $ g$\\
$ 54952.70173 $ & $   0.01799 $ & $   0.00065 $ & $   9.00504 $ & $ g$\\
$ 54952.70226 $ & $   0.01548 $ & $   0.00065 $ & $   9.00189 $ & $ g$\\
$ 54952.70265 $ & $   0.01747 $ & $   0.00065 $ & $   9.00430 $ & $ g$\\
$ 54952.70306 $ & $   0.01678 $ & $   0.00065 $ & $   9.00427 $ & $ g$\\
$ 54952.70345 $ & $   0.01535 $ & $   0.00065 $ & $   9.00305 $ & $ g$\\
$ 54952.70385 $ & $   0.01309 $ & $   0.00065 $ & $   9.00015 $ & $ g$\\
$ 54952.70429 $ & $   0.01433 $ & $   0.00065 $ & $   9.00009 $ & $ g$\\
$ 54952.70467 $ & $   0.01770 $ & $   0.00065 $ & $   9.00398 $ & $ g$\\
$ 54952.70507 $ & $   0.01187 $ & $   0.00065 $ & $   8.99858 $ & $ g$\\
$ 54952.70547 $ & $   0.01240 $ & $   0.00065 $ & $   8.99897 $ & $ g$\\
$ 54952.70586 $ & $   0.01354 $ & $   0.00065 $ & $   9.00015 $ & $ g$\\
$ 54952.70626 $ & $   0.01639 $ & $   0.00065 $ & $   9.00327 $ & $ g$\\
$ 54952.70665 $ & $   0.01609 $ & $   0.00065 $ & $   9.00283 $ & $ g$\\
$ 54952.70703 $ & $   0.01375 $ & $   0.00065 $ & $   9.00130 $ & $ g$\\
$ 54952.70742 $ & $   0.01706 $ & $   0.00065 $ & $   9.00534 $ & $ g$\\
$ 54952.70780 $ & $   0.01603 $ & $   0.00065 $ & $   9.00301 $ & $ g$\\
$ 54952.70823 $ & $   0.01762 $ & $   0.00065 $ & $   9.00311 $ & $ g$\\
$ 54952.70860 $ & $   0.01598 $ & $   0.00065 $ & $   9.00185 $ & $ g$\\
$ 54952.70900 $ & $   0.01474 $ & $   0.00065 $ & $   9.00228 $ & $ g$\\
$ 54952.70939 $ & $   0.01737 $ & $   0.00065 $ & $   9.00461 $ & $ g$\\
$ 54952.70978 $ & $   0.01627 $ & $   0.00065 $ & $   9.00198 $ & $ g$\\
$ 54952.71020 $ & $   0.01612 $ & $   0.00065 $ & $   9.00272 $ & $ g$\\
$ 54952.71059 $ & $   0.01577 $ & $   0.00065 $ & $   9.00383 $ & $ g$\\
$ 54952.71099 $ & $   0.01296 $ & $   0.00065 $ & $   9.00084 $ & $ g$\\
$ 54952.71138 $ & $   0.01525 $ & $   0.00065 $ & $   9.00116 $ & $ g$\\
$ 54952.71177 $ & $   0.01516 $ & $   0.00065 $ & $   9.00332 $ & $ g$\\
$ 54952.71273 $ & $   0.01789 $ & $   0.00065 $ & $   9.00455 $ & $ g$\\
$ 54952.71310 $ & $   0.01394 $ & $   0.00065 $ & $   9.00027 $ & $ g$\\
$ 54952.71350 $ & $   0.01482 $ & $   0.00065 $ & $   9.00227 $ & $ g$\\
$ 54952.71389 $ & $   0.01418 $ & $   0.00065 $ & $   9.00138 $ & $ g$\\
$ 54952.71429 $ & $   0.01368 $ & $   0.00065 $ & $   8.99998 $ & $ g$\\
$ 54952.71467 $ & $   0.01515 $ & $   0.00065 $ & $   9.00150 $ & $ g$\\
$ 54952.71507 $ & $   0.01450 $ & $   0.00065 $ & $   9.00149 $ & $ g$\\
$ 54952.71547 $ & $   0.01397 $ & $   0.00065 $ & $   9.00037 $ & $ g$\\
$ 54952.71587 $ & $   0.01407 $ & $   0.00065 $ & $   9.00130 $ & $ g$\\
$ 54952.71628 $ & $   0.01548 $ & $   0.00065 $ & $   9.00254 $ & $ g$\\
$ 54952.71688 $ & $   0.01560 $ & $   0.00065 $ & $   9.00116 $ & $ g$\\
$ 54952.71726 $ & $   0.01508 $ & $   0.00065 $ & $   9.00260 $ & $ g$\\
$ 54952.71764 $ & $   0.01725 $ & $   0.00065 $ & $   9.00542 $ & $ g$\\
$ 54952.71803 $ & $   0.01524 $ & $   0.00065 $ & $   9.00226 $ & $ g$\\
$ 54952.71842 $ & $   0.01190 $ & $   0.00065 $ & $   8.99977 $ & $ g$\\
$ 54952.71898 $ & $   0.01502 $ & $   0.00065 $ & $   9.00114 $ & $ g$\\
$ 54952.71937 $ & $   0.01417 $ & $   0.00065 $ & $   9.00113 $ & $ g$\\
$ 54952.71976 $ & $   0.01395 $ & $   0.00065 $ & $   9.00094 $ & $ g$\\
$ 54952.72016 $ & $   0.01788 $ & $   0.00065 $ & $   9.00585 $ & $ g$\\
$ 54952.72056 $ & $   0.01487 $ & $   0.00065 $ & $   9.00132 $ & $ g$\\
$ 54952.72099 $ & $   0.01451 $ & $   0.00065 $ & $   9.00218 $ & $ g$\\
$ 54952.72138 $ & $   0.01531 $ & $   0.00065 $ & $   9.00273 $ & $ g$\\
$ 54952.72177 $ & $   0.01326 $ & $   0.00065 $ & $   9.00075 $ & $ g$\\
$ 54952.72218 $ & $   0.01131 $ & $   0.00065 $ & $   8.99710 $ & $ g$\\
$ 54952.72257 $ & $   0.01641 $ & $   0.00065 $ & $   9.00429 $ & $ g$\\
$ 54952.72298 $ & $   0.01133 $ & $   0.00065 $ & $   8.99925 $ & $ g$\\
$ 54952.72336 $ & $   0.01620 $ & $   0.00065 $ & $   9.00423 $ & $ g$\\
$ 54952.72375 $ & $   0.01425 $ & $   0.00065 $ & $   9.00216 $ & $ g$\\
$ 54952.72415 $ & $   0.01388 $ & $   0.00065 $ & $   9.00123 $ & $ g$\\
$ 54952.72454 $ & $   0.01487 $ & $   0.00065 $ & $   9.00287 $ & $ g$\\
$ 54952.72498 $ & $   0.01178 $ & $   0.00065 $ & $   8.99827 $ & $ g$\\
$ 54952.72535 $ & $   0.01327 $ & $   0.00065 $ & $   9.00060 $ & $ g$\\
$ 54952.72575 $ & $   0.01346 $ & $   0.00065 $ & $   9.00223 $ & $ g$\\
$ 54952.72614 $ & $   0.01537 $ & $   0.00065 $ & $   9.00303 $ & $ g$\\
$ 54952.72653 $ & $   0.01142 $ & $   0.00065 $ & $   8.99777 $ & $ g$\\
$ 54952.72709 $ & $   0.01740 $ & $   0.00065 $ & $   9.00514 $ & $ g$\\
$ 54952.72748 $ & $   0.01471 $ & $   0.00065 $ & $   9.00197 $ & $ g$\\
$ 54952.72786 $ & $   0.01301 $ & $   0.00065 $ & $   9.00132 $ & $ g$\\
$ 54952.72824 $ & $   0.01554 $ & $   0.00065 $ & $   9.00368 $ & $ g$\\
$ 54952.72864 $ & $   0.01598 $ & $   0.00065 $ & $   9.00463 $ & $ g$\\
$ 54952.72921 $ & $   0.01507 $ & $   0.00065 $ & $   9.00148 $ & $ g$\\
$ 54952.72961 $ & $   0.01327 $ & $   0.00065 $ & $   9.00038 $ & $ g$\\
$ 54952.73001 $ & $   0.01079 $ & $   0.00065 $ & $   8.99789 $ & $ g$\\
$ 54952.73041 $ & $   0.01468 $ & $   0.00065 $ & $   9.00145 $ & $ g$\\
$ 54952.73080 $ & $   0.01209 $ & $   0.00065 $ & $   8.99940 $ & $ g$\\
$ 54952.73137 $ & $   0.01507 $ & $   0.00065 $ & $   9.00285 $ & $ g$\\
$ 54952.73177 $ & $   0.01454 $ & $   0.00065 $ & $   9.00251 $ & $ g$\\
$ 54952.73217 $ & $   0.01294 $ & $   0.00065 $ & $   9.00070 $ & $ g$\\
$ 54952.73256 $ & $   0.01669 $ & $   0.00065 $ & $   9.00459 $ & $ g$\\
$ 54952.73294 $ & $   0.01304 $ & $   0.00065 $ & $   9.00098 $ & $ g$\\
$ 54952.73348 $ & $   0.01187 $ & $   0.00065 $ & $   8.99941 $ & $ g$\\
$ 54952.73387 $ & $   0.01658 $ & $   0.00065 $ & $   9.00373 $ & $ g$\\
$ 54952.73427 $ & $   0.01228 $ & $   0.00065 $ & $   8.99960 $ & $ g$\\
$ 54952.73465 $ & $   0.01316 $ & $   0.00065 $ & $   9.00009 $ & $ g$\\
$ 54952.73507 $ & $   0.01450 $ & $   0.00065 $ & $   9.00279 $ & $ g$\\
$ 54952.73549 $ & $   0.01283 $ & $   0.00065 $ & $   9.00001 $ & $ g$\\
$ 54952.73588 $ & $   0.01327 $ & $   0.00065 $ & $   9.00099 $ & $ g$\\
$ 54952.73624 $ & $   0.01419 $ & $   0.00065 $ & $   9.00138 $ & $ g$\\
$ 54952.73663 $ & $   0.01558 $ & $   0.00065 $ & $   9.00184 $ & $ g$\\
$ 54952.73701 $ & $   0.01311 $ & $   0.00065 $ & $   9.00150 $ & $ g$\\
$ 54952.73762 $ & $   0.01214 $ & $   0.00065 $ & $   8.99997 $ & $ g$\\
$ 54952.73801 $ & $   0.01665 $ & $   0.00065 $ & $   9.00457 $ & $ g$\\
$ 54952.73840 $ & $   0.01126 $ & $   0.00065 $ & $   8.99892 $ & $ g$\\
$ 54952.73879 $ & $   0.01434 $ & $   0.00065 $ & $   9.00185 $ & $ g$\\
$ 54952.73918 $ & $   0.01222 $ & $   0.00065 $ & $   9.00021 $ & $ g$\\
$ 54952.73972 $ & $   0.01256 $ & $   0.00065 $ & $   9.00043 $ & $ g$\\
$ 54952.74011 $ & $   0.01100 $ & $   0.00065 $ & $   8.99779 $ & $ g$\\
$ 54952.74049 $ & $   0.01417 $ & $   0.00065 $ & $   9.00176 $ & $ g$\\
$ 54952.74089 $ & $   0.01288 $ & $   0.00065 $ & $   8.99970 $ & $ g$\\
$ 54952.74128 $ & $   0.01334 $ & $   0.00065 $ & $   9.00116 $ & $ g$\\
$ 54952.74170 $ & $   0.01363 $ & $   0.00065 $ & $   9.00084 $ & $ g$\\
$ 54952.74208 $ & $   0.01354 $ & $   0.00065 $ & $   9.00023 $ & $ g$\\
$ 54952.74247 $ & $   0.01489 $ & $   0.00065 $ & $   9.00319 $ & $ g$\\
$ 54952.74286 $ & $   0.01113 $ & $   0.00065 $ & $   8.99780 $ & $ g$\\
$ 54952.74325 $ & $   0.01271 $ & $   0.00065 $ & $   8.99893 $ & $ g$\\
$ 54952.74366 $ & $   0.01317 $ & $   0.00065 $ & $   9.00034 $ & $ g$\\
$ 54952.74403 $ & $   0.01469 $ & $   0.00065 $ & $   9.00238 $ & $ g$\\
$ 54952.74440 $ & $   0.01202 $ & $   0.00065 $ & $   8.99932 $ & $ g$\\
$ 54952.74478 $ & $   0.01048 $ & $   0.00065 $ & $   8.99735 $ & $ g$\\
$ 54952.74516 $ & $   0.00815 $ & $   0.00065 $ & $   8.99545 $ & $ g$\\
$ 54952.74560 $ & $   0.01117 $ & $   0.00065 $ & $   8.99683 $ & $ g$\\
$ 54952.74598 $ & $   0.00976 $ & $   0.00065 $ & $   8.99729 $ & $ g$\\
$ 54952.74639 $ & $   0.01164 $ & $   0.00065 $ & $   8.99827 $ & $ g$\\
$ 54952.74677 $ & $   0.01269 $ & $   0.00065 $ & $   9.00012 $ & $ g$\\
$ 54952.74718 $ & $   0.01264 $ & $   0.00065 $ & $   9.00005 $ & $ g$\\
$ 54952.74758 $ & $   0.01307 $ & $   0.00065 $ & $   8.99945 $ & $ g$\\
$ 54952.74797 $ & $   0.01118 $ & $   0.00065 $ & $   8.99761 $ & $ g$\\
$ 54952.74836 $ & $   0.01033 $ & $   0.00065 $ & $   8.99806 $ & $ g$\\
$ 54952.74873 $ & $   0.00876 $ & $   0.00065 $ & $   8.99506 $ & $ g$\\
$ 54952.74910 $ & $   0.01125 $ & $   0.00065 $ & $   8.99698 $ & $ g$\\
$ 54952.74954 $ & $   0.00813 $ & $   0.00065 $ & $   8.99410 $ & $ g$\\
$ 54952.74993 $ & $   0.00902 $ & $   0.00065 $ & $   8.99492 $ & $ g$\\
$ 54952.75032 $ & $   0.00698 $ & $   0.00065 $ & $   8.99357 $ & $ g$\\
$ 54952.75072 $ & $   0.01072 $ & $   0.00065 $ & $   8.99625 $ & $ g$\\
$ 54952.75111 $ & $   0.00978 $ & $   0.00065 $ & $   8.99722 $ & $ g$\\
$ 54952.75167 $ & $   0.00750 $ & $   0.00065 $ & $   8.99515 $ & $ g$\\
$ 54952.75206 $ & $   0.00637 $ & $   0.00065 $ & $   8.99347 $ & $ g$\\
$ 54952.75245 $ & $   0.01053 $ & $   0.00065 $ & $   8.99769 $ & $ g$\\
$ 54952.75286 $ & $   0.00730 $ & $   0.00065 $ & $   8.99338 $ & $ g$\\
$ 54952.75324 $ & $   0.00753 $ & $   0.00065 $ & $   8.99253 $ & $ g$\\
$ 54952.75367 $ & $   0.00660 $ & $   0.00065 $ & $   8.99258 $ & $ g$\\
$ 54952.75405 $ & $   0.00781 $ & $   0.00065 $ & $   8.99371 $ & $ g$\\
$ 54952.75442 $ & $   0.00931 $ & $   0.00065 $ & $   8.99534 $ & $ g$\\
$ 54952.75480 $ & $   0.00910 $ & $   0.00065 $ & $   8.99619 $ & $ g$\\
$ 54952.75520 $ & $   0.00719 $ & $   0.00065 $ & $   8.99413 $ & $ g$\\
$ 54952.75581 $ & $   0.00605 $ & $   0.00065 $ & $   8.99213 $ & $ g$\\
$ 54952.75619 $ & $   0.00840 $ & $   0.00065 $ & $   8.99524 $ & $ g$\\
$ 54952.75661 $ & $   0.00653 $ & $   0.00065 $ & $   8.99144 $ & $ g$\\
$ 54952.75699 $ & $   0.00262 $ & $   0.00065 $ & $   8.98822 $ & $ g$\\
$ 54952.75739 $ & $   0.00372 $ & $   0.00065 $ & $   8.99014 $ & $ g$\\
$ 54952.75800 $ & $   0.00634 $ & $   0.00065 $ & $   8.99267 $ & $ g$\\
$ 54952.75839 $ & $   0.00400 $ & $   0.00065 $ & $   8.99008 $ & $ g$\\
$ 54952.75880 $ & $   0.00305 $ & $   0.00065 $ & $   8.99080 $ & $ g$\\
$ 54952.75918 $ & $   0.00323 $ & $   0.00065 $ & $   8.98968 $ & $ g$\\
$ 54952.75958 $ & $   0.00087 $ & $   0.00065 $ & $   8.98667 $ & $ g$\\
$ 54952.76016 $ & $  -0.00045 $ & $   0.00065 $ & $   8.98600 $ & $ g$\\
$ 54952.76055 $ & $   0.00046 $ & $   0.00065 $ & $   8.98794 $ & $ g$\\
$ 54952.76095 $ & $   0.00116 $ & $   0.00065 $ & $   8.98743 $ & $ g$\\
$ 54952.76134 $ & $   0.00192 $ & $   0.00065 $ & $   8.98892 $ & $ g$\\
$ 54952.76174 $ & $   0.00133 $ & $   0.00065 $ & $   8.98812 $ & $ g$\\
$ 54952.76233 $ & $   0.00124 $ & $   0.00065 $ & $   8.98867 $ & $ g$\\
$ 54952.76272 $ & $   0.00352 $ & $   0.00065 $ & $   8.99005 $ & $ g$\\
$ 54952.76311 $ & $  -0.00153 $ & $   0.00065 $ & $   8.98578 $ & $ g$\\
$ 54952.76349 $ & $   0.00179 $ & $   0.00065 $ & $   8.98839 $ & $ g$\\
$ 54952.76388 $ & $   0.00117 $ & $   0.00065 $ & $   8.98825 $ & $ g$\\
$ 54952.76443 $ & $  -0.00191 $ & $   0.00065 $ & $   8.98318 $ & $ g$\\
$ 54952.76483 $ & $  -0.00084 $ & $   0.00065 $ & $   8.98535 $ & $ g$\\
$ 54952.76522 $ & $   0.00126 $ & $   0.00065 $ & $   8.98682 $ & $ g$\\
$ 54952.76560 $ & $  -0.00058 $ & $   0.00065 $ & $   8.98517 $ & $ g$\\
$ 54952.76598 $ & $   0.00145 $ & $   0.00065 $ & $   8.98829 $ & $ g$\\
$ 54952.76640 $ & $   0.00028 $ & $   0.00065 $ & $   8.98386 $ & $ g$\\
$ 54952.76715 $ & $   0.00082 $ & $   0.00065 $ & $   8.98704 $ & $ g$\\
$ 54952.76754 $ & $  -0.00216 $ & $   0.00065 $ & $   8.98447 $ & $ g$\\
$ 54952.76794 $ & $  -0.00030 $ & $   0.00065 $ & $   8.98583 $ & $ g$\\
$ 54952.76835 $ & $   0.00327 $ & $   0.00065 $ & $   8.99108 $ & $ g$\\
$ 54952.76876 $ & $  -0.00225 $ & $   0.00065 $ & $   8.98354 $ & $ g$\\
$ 54952.76915 $ & $   0.00189 $ & $   0.00065 $ & $   8.98871 $ & $ g$\\
$ 54952.76954 $ & $   0.00211 $ & $   0.00065 $ & $   8.98565 $ & $ g$\\
$ 54952.76992 $ & $  -0.00218 $ & $   0.00065 $ & $   8.98500 $ & $ g$\\
$ 54952.77051 $ & $  -0.00186 $ & $   0.00065 $ & $   8.98522 $ & $ g$\\
$ 54952.77090 $ & $  -0.00198 $ & $   0.00065 $ & $   8.98494 $ & $ g$\\
$ 54952.77128 $ & $  -0.00182 $ & $   0.00065 $ & $   8.98536 $ & $ g$\\
$ 54952.77166 $ & $  -0.00031 $ & $   0.00065 $ & $   8.98626 $ & $ g$\\
$ 54952.77207 $ & $  -0.00072 $ & $   0.00065 $ & $   8.98620 $ & $ g$\\
$ 54952.77247 $ & $   0.00067 $ & $   0.00065 $ & $   8.98621 $ & $ g$\\
$ 54952.77285 $ & $  -0.00188 $ & $   0.00065 $ & $   8.98524 $ & $ g$\\
$ 54952.77324 $ & $   0.00053 $ & $   0.00065 $ & $   8.98680 $ & $ g$\\
$ 54952.77363 $ & $   0.00007 $ & $   0.00065 $ & $   8.98566 $ & $ g$\\
$ 54952.77401 $ & $  -0.00032 $ & $   0.00065 $ & $   8.98572 $ & $ g$\\
$ 54952.77443 $ & $   0.00170 $ & $   0.00065 $ & $   8.98810 $ & $ g$\\
$ 54952.77481 $ & $  -0.00030 $ & $   0.00065 $ & $   8.98565 $ & $ g$\\
$ 54952.77518 $ & $   0.00242 $ & $   0.00065 $ & $   8.98769 $ & $ g$\\
$ 54952.77558 $ & $   0.00002 $ & $   0.00065 $ & $   8.98572 $ & $ g$\\


==> HTR102-001_phfu_tab_short.tex <==
$ 54891.60570 $ & $   0.00028 $ & $   0.00069 $ & $   8.78803 $ & $ z$\\
$ 54891.60603 $ & $  -0.00100 $ & $   0.00069 $ & $   8.78658 $ & $ z$\\
$ 54891.60636 $ & $  -0.00189 $ & $   0.00069 $ & $   8.78541 $ & $ z$\\
$ 54891.60667 $ & $  -0.00138 $ & $   0.00069 $ & $   8.78514 $ & $ z$\\
$ 54891.60702 $ & $  -0.00237 $ & $   0.00069 $ & $   8.78534 $ & $ z$\\
$ 54891.60735 $ & $   0.00030 $ & $   0.00069 $ & $   8.78923 $ & $ z$\\
$ 54891.60767 $ & $   0.00404 $ & $   0.00069 $ & $   8.79234 $ & $ z$\\
$ 54891.60801 $ & $  -0.00170 $ & $   0.00069 $ & $   8.78696 $ & $ z$\\
$ 54891.60831 $ & $   0.00257 $ & $   0.00069 $ & $   8.79009 $ & $ z$\\
$ 54891.60865 $ & $  -0.00145 $ & $   0.00069 $ & $   8.78653 $ & $ z$\\


==> HTR102-001_rvtable.tex <==
$ 928.94934 $ \dotfill & $   187.55 $ & $     1.12 $ & $    13.71 $ & $     4.73 $ & $     0.557 $ & $     0.002 $\\
$ 954.88137 $ \dotfill & $   284.38 $ & $     1.12 $ & $     7.07 $ & $     3.69 $ & $     0.556 $ & $     0.002 $\\
$ 954.88605 $ \dotfill & \nodata      & \nodata      & $    -2.17 $ & $     3.34 $ & $     0.554 $ & $     0.001 $\\
$ 955.79962 $ \dotfill & $    77.44 $ & $     1.46 $ & $     6.00 $ & $    13.88 $ & $     0.533 $ & $     0.008 $\\
$ 956.96383 $ \dotfill & $  -273.80 $ & $     1.30 $ & $     4.41 $ & $    10.92 $ & $     0.531 $ & $     0.005 $\\
$ 963.92157 $ \dotfill & $   -14.63 $ & $     1.33 $ & $    -0.17 $ & $     6.57 $ & $     0.570 $ & $     0.002 $\\
$ 983.82710 $ \dotfill & $   282.58 $ & $     0.98 $ & $     2.20 $ & $     3.79 $ & $     0.572 $ & $     0.003 $\\
$ 985.81064 $ \dotfill & $  -298.55 $ & $     1.14 $ & $    -2.81 $ & $     2.96 $ & $     0.560 $ & $     0.002 $\\
$ 986.84124 $ \dotfill & $   239.74 $ & $     1.39 $ & $    -7.48 $ & $     6.58 $ & $     0.553 $ & $     0.003 $\\
$ 988.83025 $ \dotfill & $  -300.15 $ & $     1.31 $ & $   -16.80 $ & $     8.24 $ & $     0.555 $ & $     0.002 $\\
$ 1191.14866 $ \dotfill & $  -326.24 $ & $     1.32 $ & $    -0.33 $ & $     5.00 $ & $     0.843 $ & $     0.003 $\\
$ 1193.10170 $ \dotfill & $   255.62 $ & $     1.30 $ & $    -8.71 $ & $     6.79 $ & $     0.835 $ & $     0.003 $\\
$ 1193.93435 $ \dotfill & $  -192.43 $ & $     1.38 $ & $     5.08 $ & $     5.27 $ & $     0.843 $ & $     0.004 $\\


==> HTR183-008_phfu_tab.tex <==
$ 54942.76369 $ & $   0.01133 $ & $   0.00088 $ & $  10.43700 $ & $ i$\\
$ 54942.76432 $ & $   0.01370 $ & $   0.00088 $ & $  10.43950 $ & $ i$\\
$ 54942.76495 $ & $   0.00989 $ & $   0.00088 $ & $  10.43550 $ & $ i$\\
$ 54942.76574 $ & $   0.00891 $ & $   0.00088 $ & $  10.43490 $ & $ i$\\
$ 54942.76637 $ & $   0.00974 $ & $   0.00088 $ & $  10.43570 $ & $ i$\\
$ 54942.76698 $ & $   0.01073 $ & $   0.00088 $ & $  10.43650 $ & $ i$\\
$ 54942.76779 $ & $   0.00961 $ & $   0.00088 $ & $  10.43480 $ & $ i$\\
$ 54942.76839 $ & $   0.00938 $ & $   0.00088 $ & $  10.43450 $ & $ i$\\
$ 54942.76902 $ & $   0.01249 $ & $   0.00088 $ & $  10.43800 $ & $ i$\\
$ 54942.76980 $ & $   0.01011 $ & $   0.00088 $ & $  10.43520 $ & $ i$\\
$ 54942.77042 $ & $   0.01268 $ & $   0.00088 $ & $  10.43750 $ & $ i$\\
$ 54942.77103 $ & $   0.01108 $ & $   0.00088 $ & $  10.43570 $ & $ i$\\
$ 54942.77184 $ & $   0.00941 $ & $   0.00088 $ & $  10.43420 $ & $ i$\\
$ 54942.77246 $ & $   0.00980 $ & $   0.00088 $ & $  10.43440 $ & $ i$\\
$ 54942.77309 $ & $   0.01061 $ & $   0.00088 $ & $  10.43550 $ & $ i$\\
$ 54942.77387 $ & $   0.01002 $ & $   0.00088 $ & $  10.43520 $ & $ i$\\
$ 54942.77450 $ & $   0.01023 $ & $   0.00088 $ & $  10.43540 $ & $ i$\\
$ 54942.77510 $ & $   0.01237 $ & $   0.00088 $ & $  10.43820 $ & $ i$\\
$ 54942.77591 $ & $   0.01234 $ & $   0.00088 $ & $  10.43700 $ & $ i$\\
$ 54942.77654 $ & $   0.01067 $ & $   0.00088 $ & $  10.43600 $ & $ i$\\
$ 54942.77715 $ & $   0.00883 $ & $   0.00088 $ & $  10.43420 $ & $ i$\\
$ 54942.77793 $ & $   0.01486 $ & $   0.00088 $ & $  10.43960 $ & $ i$\\
$ 54942.77854 $ & $   0.01159 $ & $   0.00088 $ & $  10.43610 $ & $ i$\\
$ 54942.77918 $ & $   0.01278 $ & $   0.00088 $ & $  10.43720 $ & $ i$\\
$ 54942.77999 $ & $   0.01119 $ & $   0.00088 $ & $  10.43630 $ & $ i$\\
$ 54942.78066 $ & $   0.01122 $ & $   0.00088 $ & $  10.43670 $ & $ i$\\
$ 54942.78127 $ & $   0.01260 $ & $   0.00088 $ & $  10.43680 $ & $ i$\\
$ 54942.78188 $ & $   0.00843 $ & $   0.00088 $ & $  10.43300 $ & $ i$\\
$ 54942.78268 $ & $   0.01008 $ & $   0.00088 $ & $  10.43470 $ & $ i$\\
$ 54942.78330 $ & $   0.00697 $ & $   0.00088 $ & $  10.43140 $ & $ i$\\
$ 54942.78393 $ & $   0.00889 $ & $   0.00088 $ & $  10.43340 $ & $ i$\\
$ 54942.78474 $ & $   0.01150 $ & $   0.00088 $ & $  10.43650 $ & $ i$\\
$ 54942.78536 $ & $   0.01123 $ & $   0.00088 $ & $  10.43630 $ & $ i$\\
$ 54942.78598 $ & $   0.01359 $ & $   0.00088 $ & $  10.43840 $ & $ i$\\
$ 54942.78678 $ & $   0.01186 $ & $   0.00088 $ & $  10.43630 $ & $ i$\\
$ 54942.78741 $ & $   0.01101 $ & $   0.00088 $ & $  10.43470 $ & $ i$\\
$ 54942.78803 $ & $   0.01008 $ & $   0.00088 $ & $  10.43460 $ & $ i$\\
$ 54942.78885 $ & $   0.00780 $ & $   0.00088 $ & $  10.43260 $ & $ i$\\
$ 54942.78947 $ & $   0.01058 $ & $   0.00088 $ & $  10.43550 $ & $ i$\\
$ 54942.79008 $ & $   0.00944 $ & $   0.00088 $ & $  10.43260 $ & $ i$\\
$ 54942.79087 $ & $   0.00995 $ & $   0.00088 $ & $  10.43440 $ & $ i$\\
$ 54942.79148 $ & $   0.01426 $ & $   0.00088 $ & $  10.43880 $ & $ i$\\
$ 54942.79212 $ & $   0.00930 $ & $   0.00088 $ & $  10.43350 $ & $ i$\\
$ 54942.79294 $ & $   0.01053 $ & $   0.00088 $ & $  10.43470 $ & $ i$\\
$ 54942.79355 $ & $   0.01266 $ & $   0.00088 $ & $  10.43700 $ & $ i$\\
$ 54942.79418 $ & $   0.01381 $ & $   0.00088 $ & $  10.43840 $ & $ i$\\
$ 54942.79499 $ & $   0.01099 $ & $   0.00088 $ & $  10.43540 $ & $ i$\\
$ 54942.79560 $ & $   0.00749 $ & $   0.00088 $ & $  10.43260 $ & $ i$\\
$ 54942.79622 $ & $   0.01101 $ & $   0.00088 $ & $  10.43450 $ & $ i$\\
$ 54942.79705 $ & $   0.00889 $ & $   0.00088 $ & $  10.43330 $ & $ i$\\
$ 54942.79775 $ & $   0.01124 $ & $   0.00088 $ & $  10.43600 $ & $ i$\\
$ 54942.79837 $ & $   0.01195 $ & $   0.00088 $ & $  10.43590 $ & $ i$\\
$ 54942.79898 $ & $   0.00981 $ & $   0.00088 $ & $  10.43430 $ & $ i$\\
$ 54942.79975 $ & $   0.01307 $ & $   0.00088 $ & $  10.43800 $ & $ i$\\
$ 54942.80038 $ & $   0.01244 $ & $   0.00088 $ & $  10.43710 $ & $ i$\\
$ 54942.80102 $ & $   0.01009 $ & $   0.00088 $ & $  10.43490 $ & $ i$\\
$ 54942.80181 $ & $   0.01052 $ & $   0.00088 $ & $  10.43510 $ & $ i$\\
$ 54942.80243 $ & $   0.01085 $ & $   0.00088 $ & $  10.43470 $ & $ i$\\
$ 54942.80305 $ & $   0.00887 $ & $   0.00088 $ & $  10.43360 $ & $ i$\\
$ 54942.80383 $ & $   0.01335 $ & $   0.00088 $ & $  10.43710 $ & $ i$\\
$ 54942.80445 $ & $   0.00800 $ & $   0.00088 $ & $  10.43230 $ & $ i$\\
$ 54942.80508 $ & $   0.00784 $ & $   0.00088 $ & $  10.43250 $ & $ i$\\
$ 54942.80589 $ & $   0.00838 $ & $   0.00088 $ & $  10.43260 $ & $ i$\\
$ 54942.80651 $ & $   0.00937 $ & $   0.00088 $ & $  10.43380 $ & $ i$\\
$ 54942.80714 $ & $   0.00842 $ & $   0.00088 $ & $  10.43320 $ & $ i$\\
$ 54942.80794 $ & $   0.01019 $ & $   0.00088 $ & $  10.43530 $ & $ i$\\
$ 54942.80855 $ & $   0.00953 $ & $   0.00088 $ & $  10.43490 $ & $ i$\\
$ 54942.80917 $ & $   0.00875 $ & $   0.00088 $ & $  10.43380 $ & $ i$\\
$ 54942.80997 $ & $   0.00997 $ & $   0.00088 $ & $  10.43490 $ & $ i$\\
$ 54942.81060 $ & $   0.00781 $ & $   0.00088 $ & $  10.43280 $ & $ i$\\
$ 54942.81121 $ & $   0.01215 $ & $   0.00088 $ & $  10.43680 $ & $ i$\\
$ 54942.81200 $ & $   0.01070 $ & $   0.00088 $ & $  10.43440 $ & $ i$\\
$ 54942.81260 $ & $   0.01073 $ & $   0.00088 $ & $  10.43560 $ & $ i$\\
$ 54942.81324 $ & $   0.01036 $ & $   0.00088 $ & $  10.43540 $ & $ i$\\
$ 54942.81406 $ & $   0.01118 $ & $   0.00088 $ & $  10.43520 $ & $ i$\\
$ 54942.81473 $ & $   0.01373 $ & $   0.00088 $ & $  10.43780 $ & $ i$\\
$ 54942.81534 $ & $   0.01105 $ & $   0.00088 $ & $  10.43580 $ & $ i$\\
$ 54942.81595 $ & $   0.01239 $ & $   0.00089 $ & $  10.43660 $ & $ i$\\
$ 54942.81674 $ & $   0.00994 $ & $   0.00089 $ & $  10.43400 $ & $ i$\\
$ 54942.81736 $ & $   0.00876 $ & $   0.00088 $ & $  10.43290 $ & $ i$\\
$ 54942.81796 $ & $   0.01178 $ & $   0.00088 $ & $  10.43660 $ & $ i$\\
$ 54942.81878 $ & $   0.01016 $ & $   0.00088 $ & $  10.43580 $ & $ i$\\
$ 54942.81941 $ & $   0.00958 $ & $   0.00088 $ & $  10.43430 $ & $ i$\\
$ 54942.82002 $ & $   0.01431 $ & $   0.00088 $ & $  10.43910 $ & $ i$\\
$ 54942.82082 $ & $   0.01010 $ & $   0.00088 $ & $  10.43440 $ & $ i$\\
$ 54942.82143 $ & $   0.01209 $ & $   0.00089 $ & $  10.43730 $ & $ i$\\
$ 54942.82204 $ & $   0.01038 $ & $   0.00088 $ & $  10.43510 $ & $ i$\\
$ 54942.82285 $ & $   0.01132 $ & $   0.00089 $ & $  10.43300 $ & $ i$\\
$ 54942.82348 $ & $   0.01026 $ & $   0.00088 $ & $  10.43540 $ & $ i$\\
$ 54942.82409 $ & $   0.00814 $ & $   0.00088 $ & $  10.43340 $ & $ i$\\
$ 54942.82487 $ & $   0.01259 $ & $   0.00088 $ & $  10.43710 $ & $ i$\\
$ 54942.82548 $ & $   0.01022 $ & $   0.00088 $ & $  10.43530 $ & $ i$\\
$ 54942.82609 $ & $   0.00952 $ & $   0.00088 $ & $  10.43360 $ & $ i$\\
$ 54942.82691 $ & $   0.00842 $ & $   0.00088 $ & $  10.43320 $ & $ i$\\
$ 54942.82753 $ & $   0.01008 $ & $   0.00088 $ & $  10.43530 $ & $ i$\\
$ 54942.82814 $ & $   0.01109 $ & $   0.00088 $ & $  10.43710 $ & $ i$\\
$ 54942.82892 $ & $   0.01332 $ & $   0.00089 $ & $  10.43820 $ & $ i$\\
$ 54942.82954 $ & $   0.01182 $ & $   0.00089 $ & $  10.43600 $ & $ i$\\
$ 54942.83016 $ & $   0.00848 $ & $   0.00089 $ & $  10.43320 $ & $ i$\\
$ 54942.83096 $ & $   0.00795 $ & $   0.00089 $ & $  10.43240 $ & $ i$\\
$ 54942.83160 $ & $   0.00863 $ & $   0.00089 $ & $  10.43350 $ & $ i$\\
$ 54942.83223 $ & $   0.00955 $ & $   0.00089 $ & $  10.43420 $ & $ i$\\
$ 54942.83284 $ & $   0.01012 $ & $   0.00089 $ & $  10.43540 $ & $ i$\\
$ 54942.83362 $ & $   0.01411 $ & $   0.00089 $ & $  10.43870 $ & $ i$\\
$ 54942.83425 $ & $   0.00900 $ & $   0.00089 $ & $  10.43350 $ & $ i$\\
$ 54942.83487 $ & $   0.01031 $ & $   0.00088 $ & $  10.43500 $ & $ i$\\
$ 54942.83568 $ & $   0.00784 $ & $   0.00088 $ & $  10.43350 $ & $ i$\\
$ 54942.83630 $ & $   0.00984 $ & $   0.00089 $ & $  10.43520 $ & $ i$\\
$ 54942.83693 $ & $   0.00806 $ & $   0.00089 $ & $  10.43250 $ & $ i$\\
$ 54942.83771 $ & $   0.00703 $ & $   0.00089 $ & $  10.43280 $ & $ i$\\
$ 54942.83833 $ & $   0.01119 $ & $   0.00089 $ & $  10.43680 $ & $ i$\\
$ 54942.83894 $ & $   0.00849 $ & $   0.00089 $ & $  10.43430 $ & $ i$\\
$ 54942.83975 $ & $   0.00860 $ & $   0.00089 $ & $  10.43470 $ & $ i$\\
$ 54942.84036 $ & $   0.00883 $ & $   0.00089 $ & $  10.43470 $ & $ i$\\
$ 54942.84100 $ & $   0.00816 $ & $   0.00089 $ & $  10.43330 $ & $ i$\\
$ 54942.84180 $ & $   0.00800 $ & $   0.00089 $ & $  10.43270 $ & $ i$\\
$ 54942.84240 $ & $   0.01099 $ & $   0.00089 $ & $  10.43640 $ & $ i$\\
$ 54942.84302 $ & $   0.00973 $ & $   0.00089 $ & $  10.43520 $ & $ i$\\
$ 54942.84384 $ & $   0.00902 $ & $   0.00089 $ & $  10.43460 $ & $ i$\\
$ 54942.84445 $ & $   0.00882 $ & $   0.00089 $ & $  10.43400 $ & $ i$\\
$ 54942.84508 $ & $   0.00963 $ & $   0.00089 $ & $  10.43490 $ & $ i$\\
$ 54942.84585 $ & $   0.00785 $ & $   0.00089 $ & $  10.43330 $ & $ i$\\
$ 54942.84646 $ & $   0.00978 $ & $   0.00089 $ & $  10.43550 $ & $ i$\\
$ 54942.84710 $ & $   0.00930 $ & $   0.00090 $ & $  10.43430 $ & $ i$\\
$ 54942.84791 $ & $   0.01079 $ & $   0.00089 $ & $  10.43720 $ & $ i$\\
$ 54942.84950 $ & $   0.00883 $ & $   0.00089 $ & $  10.43390 $ & $ i$\\
$ 54942.85012 $ & $   0.00959 $ & $   0.00089 $ & $  10.43400 $ & $ i$\\
$ 54942.85073 $ & $   0.00900 $ & $   0.00089 $ & $  10.43340 $ & $ i$\\
$ 54942.85153 $ & $   0.00789 $ & $   0.00089 $ & $  10.43340 $ & $ i$\\
$ 54942.85216 $ & $   0.00907 $ & $   0.00089 $ & $  10.43420 $ & $ i$\\
$ 54942.85276 $ & $   0.00482 $ & $   0.00089 $ & $  10.43130 $ & $ i$\\
$ 54942.85357 $ & $   0.00843 $ & $   0.00089 $ & $  10.43430 $ & $ i$\\
$ 54942.85419 $ & $   0.00543 $ & $   0.00089 $ & $  10.43150 $ & $ i$\\
$ 54942.85482 $ & $   0.00857 $ & $   0.00089 $ & $  10.43400 $ & $ i$\\
$ 54942.85560 $ & $   0.00845 $ & $   0.00089 $ & $  10.43440 $ & $ i$\\
$ 54942.85621 $ & $   0.00675 $ & $   0.00090 $ & $  10.43220 $ & $ i$\\
$ 54942.85682 $ & $   0.00693 $ & $   0.00090 $ & $  10.43240 $ & $ i$\\
$ 54942.85763 $ & $   0.00348 $ & $   0.00089 $ & $  10.42830 $ & $ i$\\
$ 54942.85827 $ & $   0.00570 $ & $   0.00089 $ & $  10.43090 $ & $ i$\\
$ 54942.85887 $ & $   0.00627 $ & $   0.00089 $ & $  10.43130 $ & $ i$\\
$ 54942.85966 $ & $   0.00723 $ & $   0.00089 $ & $  10.43200 $ & $ i$\\
$ 54942.86027 $ & $   0.00516 $ & $   0.00089 $ & $  10.43070 $ & $ i$\\
$ 54942.86091 $ & $   0.00478 $ & $   0.00089 $ & $  10.43000 $ & $ i$\\
$ 54942.86172 $ & $   0.00117 $ & $   0.00090 $ & $  10.42580 $ & $ i$\\
$ 54942.86233 $ & $   0.00354 $ & $   0.00089 $ & $  10.42910 $ & $ i$\\
$ 54942.86296 $ & $   0.00182 $ & $   0.00089 $ & $  10.42810 $ & $ i$\\
$ 54942.86374 $ & $   0.00388 $ & $   0.00089 $ & $  10.43010 $ & $ i$\\
$ 54942.86436 $ & $   0.00367 $ & $   0.00089 $ & $  10.42810 $ & $ i$\\
$ 54942.86498 $ & $   0.00263 $ & $   0.00089 $ & $  10.42870 $ & $ i$\\
$ 54942.86580 $ & $   0.00369 $ & $   0.00089 $ & $  10.42840 $ & $ i$\\
$ 54942.86644 $ & $  -0.00059 $ & $   0.00089 $ & $  10.42500 $ & $ i$\\
$ 54942.86705 $ & $   0.00137 $ & $   0.00089 $ & $  10.42690 $ & $ i$\\
$ 54942.86768 $ & $   0.00093 $ & $   0.00089 $ & $  10.42640 $ & $ i$\\
$ 54942.86846 $ & $   0.00283 $ & $   0.00089 $ & $  10.42880 $ & $ i$\\
$ 54942.86909 $ & $   0.00096 $ & $   0.00089 $ & $  10.42740 $ & $ i$\\
$ 54942.86970 $ & $   0.00049 $ & $   0.00089 $ & $  10.42640 $ & $ i$\\
$ 54942.87051 $ & $   0.00203 $ & $   0.00090 $ & $  10.42790 $ & $ i$\\
$ 54942.87114 $ & $  -0.00208 $ & $   0.00089 $ & $  10.42400 $ & $ i$\\
$ 54942.87175 $ & $   0.00149 $ & $   0.00089 $ & $  10.42750 $ & $ i$\\
$ 54942.87256 $ & $  -0.00153 $ & $   0.00089 $ & $  10.42430 $ & $ i$\\
$ 54942.87319 $ & $  -0.00466 $ & $   0.00089 $ & $  10.42060 $ & $ i$\\
$ 54942.87380 $ & $   0.00037 $ & $   0.00089 $ & $  10.42550 $ & $ i$\\
$ 54942.87463 $ & $  -0.00221 $ & $   0.00089 $ & $  10.42340 $ & $ i$\\
$ 54942.87525 $ & $   0.00334 $ & $   0.00090 $ & $  10.42880 $ & $ i$\\
$ 54942.87588 $ & $  -0.00169 $ & $   0.00090 $ & $  10.42390 $ & $ i$\\
$ 54942.87668 $ & $  -0.00075 $ & $   0.00089 $ & $  10.42520 $ & $ i$\\
$ 54942.87731 $ & $   0.00026 $ & $   0.00089 $ & $  10.42680 $ & $ i$\\
$ 54942.87793 $ & $  -0.00246 $ & $   0.00089 $ & $  10.42330 $ & $ i$\\
$ 54942.87875 $ & $   0.00057 $ & $   0.00089 $ & $  10.42670 $ & $ i$\\
$ 54942.87937 $ & $  -0.00246 $ & $   0.00089 $ & $  10.42370 $ & $ i$\\
$ 54942.87997 $ & $  -0.00004 $ & $   0.00089 $ & $  10.42640 $ & $ i$\\
$ 54942.88077 $ & $   0.00083 $ & $   0.00089 $ & $  10.42690 $ & $ i$\\
$ 54942.88139 $ & $  -0.00123 $ & $   0.00089 $ & $  10.42530 $ & $ i$\\
$ 54942.88201 $ & $  -0.00151 $ & $   0.00089 $ & $  10.42510 $ & $ i$\\
$ 54942.88265 $ & $   0.00030 $ & $   0.00089 $ & $  10.42650 $ & $ i$\\
$ 54942.88330 $ & $   0.00038 $ & $   0.00089 $ & $  10.42760 $ & $ i$\\
$ 54942.88391 $ & $  -0.00309 $ & $   0.00089 $ & $  10.42290 $ & $ i$\\
$ 54942.88454 $ & $  -0.00043 $ & $   0.00089 $ & $  10.42560 $ & $ i$\\
$ 54942.88533 $ & $  -0.00146 $ & $   0.00089 $ & $  10.42550 $ & $ i$\\
$ 54942.88595 $ & $   0.00280 $ & $   0.00089 $ & $  10.42940 $ & $ i$\\
$ 54942.88657 $ & $   0.00092 $ & $   0.00089 $ & $  10.42630 $ & $ i$\\
$ 54942.88740 $ & $   0.00161 $ & $   0.00089 $ & $  10.42810 $ & $ i$\\
$ 54942.88802 $ & $   0.00062 $ & $   0.00089 $ & $  10.42680 $ & $ i$\\
$ 54942.88865 $ & $   0.00012 $ & $   0.00089 $ & $  10.42640 $ & $ i$\\
$ 54942.88944 $ & $   0.00276 $ & $   0.00089 $ & $  10.42920 $ & $ i$\\
$ 54942.89006 $ & $   0.00021 $ & $   0.00089 $ & $  10.42710 $ & $ i$\\
$ 54942.89067 $ & $   0.00415 $ & $   0.00089 $ & $  10.43090 $ & $ i$\\
$ 54942.89147 $ & $  -0.00073 $ & $   0.00089 $ & $  10.42640 $ & $ i$\\
$ 54942.89209 $ & $   0.00079 $ & $   0.00089 $ & $  10.42750 $ & $ i$\\
$ 54942.89270 $ & $   0.00083 $ & $   0.00089 $ & $  10.42780 $ & $ i$\\
$ 54942.89349 $ & $  -0.00121 $ & $   0.00090 $ & $  10.42490 $ & $ i$\\
$ 54942.89412 $ & $   0.00076 $ & $   0.00090 $ & $  10.42740 $ & $ i$\\
$ 54942.89540 $ & $  -0.00046 $ & $   0.00089 $ & $  10.42700 $ & $ i$\\
$ 54942.89601 $ & $   0.00392 $ & $   0.00090 $ & $  10.43100 $ & $ i$\\
$ 54942.89665 $ & $   0.00210 $ & $   0.00090 $ & $  10.42880 $ & $ i$\\
$ 54942.89743 $ & $  -0.00259 $ & $   0.00089 $ & $  10.42520 $ & $ i$\\
$ 54942.89806 $ & $   0.00002 $ & $   0.00089 $ & $  10.42730 $ & $ i$\\
$ 54942.89868 $ & $   0.00039 $ & $   0.00090 $ & $  10.42710 $ & $ i$\\
$ 54942.89952 $ & $   0.00130 $ & $   0.00089 $ & $  10.42880 $ & $ i$\\
$ 54942.90020 $ & $  -0.00055 $ & $   0.00090 $ & $  10.42650 $ & $ i$\\
$ 54942.90082 $ & $   0.00000 $ & $   0.00089 $ & $  10.42710 $ & $ i$\\
$ 54942.90145 $ & $  -0.00007 $ & $   0.00090 $ & $  10.42690 $ & $ i$\\
$ 54942.90225 $ & $   0.00173 $ & $   0.00090 $ & $  10.42890 $ & $ i$\\
$ 54942.90286 $ & $   0.00024 $ & $   0.00089 $ & $  10.42740 $ & $ i$\\
$ 54942.90350 $ & $   0.00187 $ & $   0.00090 $ & $  10.42750 $ & $ i$\\
$ 54942.90432 $ & $  -0.00057 $ & $   0.00090 $ & $  10.42560 $ & $ i$\\
$ 54942.90494 $ & $  -0.00132 $ & $   0.00090 $ & $  10.42530 $ & $ i$\\
$ 54942.90557 $ & $  -0.00284 $ & $   0.00090 $ & $  10.42400 $ & $ i$\\
$ 54942.90637 $ & $  -0.00017 $ & $   0.00090 $ & $  10.42610 $ & $ i$\\
$ 54942.90699 $ & $  -0.00017 $ & $   0.00089 $ & $  10.42690 $ & $ i$\\
$ 54942.90762 $ & $   0.00185 $ & $   0.00090 $ & $  10.42810 $ & $ i$\\
$ 54942.90844 $ & $  -0.00010 $ & $   0.00090 $ & $  10.42790 $ & $ i$\\
$ 54942.90905 $ & $  -0.00504 $ & $   0.00090 $ & $  10.42180 $ & $ i$\\
$ 54942.90965 $ & $   0.00125 $ & $   0.00090 $ & $  10.42910 $ & $ i$\\
$ 54942.91045 $ & $  -0.00092 $ & $   0.00090 $ & $  10.42550 $ & $ i$\\
$ 54942.91107 $ & $   0.00006 $ & $   0.00091 $ & $  10.42720 $ & $ i$\\
$ 54942.91167 $ & $   0.00063 $ & $   0.00091 $ & $  10.42780 $ & $ i$\\
$ 54942.91249 $ & $  -0.00174 $ & $   0.00090 $ & $  10.42540 $ & $ i$\\
$ 54942.91310 $ & $   0.00136 $ & $   0.00090 $ & $  10.42930 $ & $ i$\\
$ 54942.91372 $ & $   0.00356 $ & $   0.00091 $ & $  10.42990 $ & $ i$\\
$ 54942.91450 $ & $   0.00071 $ & $   0.00092 $ & $  10.42820 $ & $ i$\\
$ 54942.91513 $ & $  -0.00015 $ & $   0.00091 $ & $  10.42610 $ & $ i$\\
$ 54942.91575 $ & $   0.00126 $ & $   0.00090 $ & $  10.42770 $ & $ i$\\
$ 54942.91656 $ & $   0.00208 $ & $   0.00090 $ & $  10.42900 $ & $ i$\\
$ 54942.91725 $ & $  -0.00388 $ & $   0.00090 $ & $  10.42220 $ & $ i$\\
$ 54942.91847 $ & $   0.00123 $ & $   0.00091 $ & $  10.42850 $ & $ i$\\
$ 54942.91926 $ & $  -0.00257 $ & $   0.00091 $ & $  10.42450 $ & $ i$\\
$ 54942.91987 $ & $  -0.00015 $ & $   0.00091 $ & $  10.42640 $ & $ i$\\
$ 54942.92050 $ & $   0.00041 $ & $   0.00091 $ & $  10.42630 $ & $ i$\\
$ 54942.92130 $ & $   0.00121 $ & $   0.00091 $ & $  10.42710 $ & $ i$\\
$ 54942.92192 $ & $  -0.00092 $ & $   0.00091 $ & $  10.42570 $ & $ i$\\
$ 54942.92255 $ & $   0.00008 $ & $   0.00092 $ & $  10.42560 $ & $ i$\\
$ 54942.92332 $ & $  -0.00064 $ & $   0.00091 $ & $  10.42550 $ & $ i$\\
$ 54942.92395 $ & $  -0.00075 $ & $   0.00093 $ & $  10.42570 $ & $ i$\\
$ 54942.92456 $ & $  -0.00099 $ & $   0.00091 $ & $  10.42540 $ & $ i$\\
$ 54942.92546 $ & $   0.00048 $ & $   0.00091 $ & $  10.42740 $ & $ i$\\
$ 54942.92610 $ & $  -0.00178 $ & $   0.00091 $ & $  10.42420 $ & $ i$\\
$ 54942.92671 $ & $   0.00041 $ & $   0.00091 $ & $  10.42700 $ & $ i$\\
$ 54942.92750 $ & $   0.00085 $ & $   0.00092 $ & $  10.42780 $ & $ i$\\
$ 54942.92810 $ & $  -0.00226 $ & $   0.00093 $ & $  10.42690 $ & $ i$\\
$ 54942.92873 $ & $  -0.00037 $ & $   0.00092 $ & $  10.42680 $ & $ i$\\
$ 55243.75880 $ & $  -0.00373 $ & $   0.00107 $ & $  10.47940 $ & $ i$\\
$ 55243.75929 $ & $   0.00463 $ & $   0.00107 $ & $  10.48860 $ & $ i$\\
$ 55243.76001 $ & $  -0.00073 $ & $   0.00106 $ & $  10.48320 $ & $ i$\\
$ 55243.76050 $ & $   0.00047 $ & $   0.00106 $ & $  10.48410 $ & $ i$\\
$ 55243.76119 $ & $  -0.00810 $ & $   0.00106 $ & $  10.47580 $ & $ i$\\
$ 55243.76198 $ & $  -0.00384 $ & $   0.00076 $ & $  10.47980 $ & $ i$\\
$ 55243.76302 $ & $  -0.00652 $ & $   0.00076 $ & $  10.47720 $ & $ i$\\
$ 55243.76403 $ & $  -0.00547 $ & $   0.00075 $ & $  10.47800 $ & $ i$\\
$ 55243.76506 $ & $  -0.00711 $ & $   0.00075 $ & $  10.47700 $ & $ i$\\
$ 55243.76576 $ & $  -0.00015 $ & $   0.00106 $ & $  10.48410 $ & $ i$\\
$ 55243.76627 $ & $   0.00010 $ & $   0.00107 $ & $  10.48380 $ & $ i$\\
$ 55243.76696 $ & $   0.00354 $ & $   0.00107 $ & $  10.48710 $ & $ i$\\
$ 55243.76746 $ & $  -0.00528 $ & $   0.00106 $ & $  10.47840 $ & $ i$\\
$ 55243.76814 $ & $  -0.00076 $ & $   0.00106 $ & $  10.48320 $ & $ i$\\
$ 55243.76864 $ & $  -0.00072 $ & $   0.00107 $ & $  10.48300 $ & $ i$\\
$ 55243.76933 $ & $   0.00176 $ & $   0.00106 $ & $  10.48610 $ & $ i$\\
$ 55243.76981 $ & $   0.00032 $ & $   0.00106 $ & $  10.48390 $ & $ i$\\
$ 55243.77049 $ & $  -0.00359 $ & $   0.00106 $ & $  10.47970 $ & $ i$\\
$ 55243.77098 $ & $   0.00284 $ & $   0.00106 $ & $  10.48690 $ & $ i$\\
$ 55243.77169 $ & $   0.00321 $ & $   0.00106 $ & $  10.48740 $ & $ i$\\
$ 55243.77220 $ & $   0.00170 $ & $   0.00107 $ & $  10.48570 $ & $ i$\\
$ 55243.77287 $ & $  -0.00104 $ & $   0.00106 $ & $  10.48300 $ & $ i$\\
$ 55243.77338 $ & $   0.00447 $ & $   0.00107 $ & $  10.48890 $ & $ i$\\
$ 55243.77405 $ & $  -0.00011 $ & $   0.00107 $ & $  10.48410 $ & $ i$\\
$ 55243.77456 $ & $  -0.00044 $ & $   0.00106 $ & $  10.48400 $ & $ i$\\
$ 55243.77523 $ & $  -0.00089 $ & $   0.00107 $ & $  10.48350 $ & $ i$\\
$ 55243.77574 $ & $  -0.00082 $ & $   0.00106 $ & $  10.48320 $ & $ i$\\
$ 55243.77642 $ & $   0.00603 $ & $   0.00106 $ & $  10.49050 $ & $ i$\\
$ 55243.77693 $ & $  -0.00206 $ & $   0.00107 $ & $  10.48130 $ & $ i$\\
$ 55243.77764 $ & $   0.00553 $ & $   0.00106 $ & $  10.49000 $ & $ i$\\
$ 55243.77815 $ & $  -0.00320 $ & $   0.00106 $ & $  10.48150 $ & $ i$\\
$ 55243.77882 $ & $   0.00208 $ & $   0.00106 $ & $  10.48630 $ & $ i$\\
$ 55243.77933 $ & $   0.00018 $ & $   0.00106 $ & $  10.48400 $ & $ i$\\
$ 55243.78001 $ & $  -0.00203 $ & $   0.00106 $ & $  10.48320 $ & $ i$\\
$ 55243.78051 $ & $  -0.00111 $ & $   0.00106 $ & $  10.48310 $ & $ i$\\
$ 55243.78119 $ & $   0.00720 $ & $   0.00106 $ & $  10.49060 $ & $ i$\\
$ 55243.78169 $ & $  -0.00417 $ & $   0.00106 $ & $  10.48040 $ & $ i$\\
$ 55243.78237 $ & $  -0.00050 $ & $   0.00107 $ & $  10.48340 $ & $ i$\\
$ 55243.78287 $ & $  -0.00015 $ & $   0.00106 $ & $  10.48420 $ & $ i$\\
$ 55243.78358 $ & $   0.00360 $ & $   0.00106 $ & $  10.48780 $ & $ i$\\
$ 55243.78408 $ & $   0.00400 $ & $   0.00106 $ & $  10.48830 $ & $ i$\\
$ 55243.78476 $ & $  -0.00091 $ & $   0.00106 $ & $  10.48280 $ & $ i$\\
$ 55243.78525 $ & $   0.00623 $ & $   0.00106 $ & $  10.49090 $ & $ i$\\
$ 55243.78594 $ & $   0.00131 $ & $   0.00106 $ & $  10.48540 $ & $ i$\\
$ 55243.78645 $ & $   0.00087 $ & $   0.00105 $ & $  10.48490 $ & $ i$\\
$ 55243.78711 $ & $   0.00231 $ & $   0.00105 $ & $  10.48680 $ & $ i$\\
$ 55243.78760 $ & $   0.00466 $ & $   0.00106 $ & $  10.48810 $ & $ i$\\
$ 55243.78827 $ & $  -0.00624 $ & $   0.00105 $ & $  10.47760 $ & $ i$\\
$ 55243.78877 $ & $   0.00053 $ & $   0.00106 $ & $  10.48430 $ & $ i$\\
$ 55243.78948 $ & $   0.00358 $ & $   0.00106 $ & $  10.48740 $ & $ i$\\
$ 55243.78998 $ & $   0.00429 $ & $   0.00105 $ & $  10.48800 $ & $ i$\\
$ 55243.79065 $ & $   0.00202 $ & $   0.00105 $ & $  10.48630 $ & $ i$\\
$ 55243.79113 $ & $   0.00472 $ & $   0.00106 $ & $  10.48860 $ & $ i$\\
$ 55243.79180 $ & $   0.00273 $ & $   0.00106 $ & $  10.48680 $ & $ i$\\
$ 55243.79231 $ & $  -0.00543 $ & $   0.00105 $ & $  10.47830 $ & $ i$\\
$ 55243.79299 $ & $   0.00085 $ & $   0.00105 $ & $  10.48450 $ & $ i$\\
$ 55243.79347 $ & $  -0.00247 $ & $   0.00106 $ & $  10.48120 $ & $ i$\\
$ 55243.79415 $ & $   0.00154 $ & $   0.00105 $ & $  10.48540 $ & $ i$\\
$ 55243.79464 $ & $   0.00024 $ & $   0.00105 $ & $  10.48490 $ & $ i$\\
$ 55243.79533 $ & $  -0.00200 $ & $   0.00106 $ & $  10.48160 $ & $ i$\\
$ 55243.79584 $ & $   0.00135 $ & $   0.00106 $ & $  10.48520 $ & $ i$\\
$ 55243.79652 $ & $   0.00338 $ & $   0.00105 $ & $  10.48660 $ & $ i$\\
$ 55243.79701 $ & $   0.00265 $ & $   0.00106 $ & $  10.48660 $ & $ i$\\
$ 55243.79771 $ & $   0.00184 $ & $   0.00105 $ & $  10.48610 $ & $ i$\\
$ 55243.79819 $ & $  -0.00090 $ & $   0.00105 $ & $  10.48250 $ & $ i$\\
$ 55243.79889 $ & $  -0.00114 $ & $   0.00106 $ & $  10.48210 $ & $ i$\\
$ 55243.79940 $ & $  -0.00534 $ & $   0.00106 $ & $  10.47850 $ & $ i$\\
$ 55243.80007 $ & $   0.00655 $ & $   0.00106 $ & $  10.49060 $ & $ i$\\
$ 55243.80058 $ & $  -0.00138 $ & $   0.00106 $ & $  10.48260 $ & $ i$\\
$ 55243.80128 $ & $   0.00507 $ & $   0.00105 $ & $  10.48870 $ & $ i$\\
$ 55243.80178 $ & $  -0.00315 $ & $   0.00106 $ & $  10.48100 $ & $ i$\\
$ 55243.80247 $ & $  -0.00340 $ & $   0.00105 $ & $  10.48080 $ & $ i$\\
$ 55243.80296 $ & $  -0.00442 $ & $   0.00106 $ & $  10.47960 $ & $ i$\\
$ 55243.80413 $ & $   0.00131 $ & $   0.00106 $ & $  10.48530 $ & $ i$\\
$ 55243.80481 $ & $  -0.00074 $ & $   0.00106 $ & $  10.48350 $ & $ i$\\
$ 55243.80531 $ & $  -0.00067 $ & $   0.00106 $ & $  10.48380 $ & $ i$\\
$ 55243.80600 $ & $  -0.00366 $ & $   0.00106 $ & $  10.48040 $ & $ i$\\
$ 55243.80650 $ & $   0.00083 $ & $   0.00106 $ & $  10.48540 $ & $ i$\\
$ 55243.80720 $ & $  -0.00046 $ & $   0.00105 $ & $  10.48350 $ & $ i$\\
$ 55243.80770 $ & $  -0.00045 $ & $   0.00105 $ & $  10.48350 $ & $ i$\\
$ 55243.80837 $ & $   0.00168 $ & $   0.00106 $ & $  10.48620 $ & $ i$\\
$ 55243.80955 $ & $   0.00244 $ & $   0.00106 $ & $  10.48680 $ & $ i$\\
$ 55243.81005 $ & $  -0.00287 $ & $   0.00106 $ & $  10.48190 $ & $ i$\\
$ 55243.81073 $ & $   0.00510 $ & $   0.00106 $ & $  10.48910 $ & $ i$\\
$ 55243.81123 $ & $  -0.00369 $ & $   0.00106 $ & $  10.48020 $ & $ i$\\
$ 55243.81191 $ & $   0.00006 $ & $   0.00106 $ & $  10.48490 $ & $ i$\\
$ 55243.81241 $ & $   0.00212 $ & $   0.00106 $ & $  10.48650 $ & $ i$\\
$ 55243.81310 $ & $   0.00234 $ & $   0.00106 $ & $  10.48720 $ & $ i$\\
$ 55243.81360 $ & $   0.00500 $ & $   0.00106 $ & $  10.48940 $ & $ i$\\
$ 55243.81427 $ & $   0.00986 $ & $   0.00106 $ & $  10.49440 $ & $ i$\\
$ 55243.81476 $ & $   0.00606 $ & $   0.00106 $ & $  10.49070 $ & $ i$\\
$ 55243.81543 $ & $   0.00565 $ & $   0.00106 $ & $  10.48960 $ & $ i$\\
$ 55243.81593 $ & $   0.00563 $ & $   0.00106 $ & $  10.48970 $ & $ i$\\
$ 55243.81662 $ & $   0.01139 $ & $   0.00106 $ & $  10.49600 $ & $ i$\\
$ 55243.81711 $ & $   0.00444 $ & $   0.00106 $ & $  10.48870 $ & $ i$\\
$ 55243.81777 $ & $   0.00625 $ & $   0.00105 $ & $  10.48990 $ & $ i$\\
$ 55243.81828 $ & $   0.00582 $ & $   0.00106 $ & $  10.48940 $ & $ i$\\
$ 55243.81897 $ & $   0.00656 $ & $   0.00106 $ & $  10.49080 $ & $ i$\\
$ 55243.81946 $ & $   0.00295 $ & $   0.00107 $ & $  10.48760 $ & $ i$\\
$ 55243.82013 $ & $   0.00724 $ & $   0.00106 $ & $  10.49150 $ & $ i$\\
$ 55243.82063 $ & $   0.00187 $ & $   0.00106 $ & $  10.48570 $ & $ i$\\
$ 55243.82128 $ & $   0.00056 $ & $   0.00106 $ & $  10.48460 $ & $ i$\\
$ 55243.82179 $ & $   0.00904 $ & $   0.00106 $ & $  10.49310 $ & $ i$\\
$ 55243.82248 $ & $   0.00204 $ & $   0.00106 $ & $  10.48640 $ & $ i$\\
$ 55243.82297 $ & $   0.00703 $ & $   0.00106 $ & $  10.49110 $ & $ i$\\
$ 55243.82366 $ & $   0.00873 $ & $   0.00106 $ & $  10.49320 $ & $ i$\\
$ 55243.82416 $ & $   0.00653 $ & $   0.00106 $ & $  10.49110 $ & $ i$\\
$ 55243.82471 $ & $   0.01226 $ & $   0.00105 $ & $  10.49690 $ & $ i$\\
$ 55243.82521 $ & $   0.01120 $ & $   0.00106 $ & $  10.49460 $ & $ i$\\
$ 55243.82588 $ & $   0.01056 $ & $   0.00106 $ & $  10.49410 $ & $ i$\\
$ 55243.82638 $ & $   0.01062 $ & $   0.00106 $ & $  10.49370 $ & $ i$\\
$ 55243.82705 $ & $   0.01383 $ & $   0.00106 $ & $  10.49770 $ & $ i$\\
$ 55243.82753 $ & $   0.01455 $ & $   0.00106 $ & $  10.49890 $ & $ i$\\
$ 55243.82821 $ & $   0.01136 $ & $   0.00106 $ & $  10.49440 $ & $ i$\\
$ 55243.82870 $ & $   0.00772 $ & $   0.00106 $ & $  10.49100 $ & $ i$\\
$ 55243.82936 $ & $   0.00250 $ & $   0.00106 $ & $  10.48690 $ & $ i$\\
$ 55243.82985 $ & $   0.00921 $ & $   0.00106 $ & $  10.49360 $ & $ i$\\
$ 55243.83056 $ & $   0.00922 $ & $   0.00106 $ & $  10.49310 $ & $ i$\\
$ 55243.83104 $ & $   0.00831 $ & $   0.00106 $ & $  10.49230 $ & $ i$\\
$ 55243.83170 $ & $   0.00768 $ & $   0.00106 $ & $  10.49160 $ & $ i$\\
$ 55243.83221 $ & $   0.00823 $ & $   0.00106 $ & $  10.49280 $ & $ i$\\
$ 55243.83288 $ & $   0.00848 $ & $   0.00106 $ & $  10.49240 $ & $ i$\\
$ 55243.83339 $ & $   0.01230 $ & $   0.00107 $ & $  10.49600 $ & $ i$\\
$ 55243.83407 $ & $   0.01475 $ & $   0.00106 $ & $  10.49880 $ & $ i$\\
$ 55243.83456 $ & $   0.00831 $ & $   0.00106 $ & $  10.49230 $ & $ i$\\
$ 55243.83523 $ & $   0.01123 $ & $   0.00106 $ & $  10.49520 $ & $ i$\\
$ 55243.83572 $ & $   0.00746 $ & $   0.00106 $ & $  10.49130 $ & $ i$\\
$ 55243.83641 $ & $   0.01428 $ & $   0.00107 $ & $  10.49800 $ & $ i$\\
$ 55243.83692 $ & $   0.01132 $ & $   0.00107 $ & $  10.49530 $ & $ i$\\
$ 55243.83760 $ & $   0.00835 $ & $   0.00106 $ & $  10.49200 $ & $ i$\\
$ 55243.83810 $ & $   0.00852 $ & $   0.00106 $ & $  10.49290 $ & $ i$\\
$ 55243.83878 $ & $   0.01302 $ & $   0.00107 $ & $  10.49720 $ & $ i$\\
$ 55243.83928 $ & $   0.01385 $ & $   0.00106 $ & $  10.49830 $ & $ i$\\
$ 55243.83994 $ & $   0.00879 $ & $   0.00107 $ & $  10.49350 $ & $ i$\\
$ 55243.84044 $ & $   0.01238 $ & $   0.00106 $ & $  10.49620 $ & $ i$\\
$ 55243.84111 $ & $   0.01256 $ & $   0.00106 $ & $  10.49750 $ & $ i$\\
$ 55243.84161 $ & $   0.01252 $ & $   0.00107 $ & $  10.49730 $ & $ i$\\
$ 55243.84231 $ & $   0.00774 $ & $   0.00106 $ & $  10.49200 $ & $ i$\\
$ 55243.84282 $ & $   0.01408 $ & $   0.00106 $ & $  10.49870 $ & $ i$\\
$ 55243.84348 $ & $   0.01987 $ & $   0.00106 $ & $  10.50490 $ & $ i$\\
$ 55243.84399 $ & $   0.01184 $ & $   0.00107 $ & $  10.49670 $ & $ i$\\
$ 55243.84466 $ & $   0.01193 $ & $   0.00106 $ & $  10.49640 $ & $ i$\\
$ 55243.84516 $ & $   0.01081 $ & $   0.00107 $ & $  10.49580 $ & $ i$\\
$ 55243.84568 $ & $   0.01838 $ & $   0.00107 $ & $  10.50350 $ & $ i$\\
$ 55243.84618 $ & $   0.01393 $ & $   0.00106 $ & $  10.49930 $ & $ i$\\
$ 55243.84686 $ & $   0.00748 $ & $   0.00106 $ & $  10.49190 $ & $ i$\\
$ 55243.84737 $ & $   0.01070 $ & $   0.00106 $ & $  10.49620 $ & $ i$\\
$ 55243.84808 $ & $   0.01283 $ & $   0.00106 $ & $  10.49770 $ & $ i$\\
$ 55243.84858 $ & $   0.01286 $ & $   0.00106 $ & $  10.49790 $ & $ i$\\
$ 55243.84926 $ & $   0.01091 $ & $   0.00107 $ & $  10.49560 $ & $ i$\\
$ 55243.84975 $ & $   0.01407 $ & $   0.00106 $ & $  10.49890 $ & $ i$\\
$ 55243.85042 $ & $   0.01197 $ & $   0.00106 $ & $  10.49690 $ & $ i$\\
$ 55243.85091 $ & $   0.01381 $ & $   0.00106 $ & $  10.49860 $ & $ i$\\
$ 55243.85161 $ & $   0.01339 $ & $   0.00106 $ & $  10.49800 $ & $ i$\\
$ 55243.85211 $ & $   0.00886 $ & $   0.00106 $ & $  10.49370 $ & $ i$\\
$ 55243.85279 $ & $   0.00931 $ & $   0.00106 $ & $  10.49340 $ & $ i$\\
$ 55243.85330 $ & $   0.01233 $ & $   0.00106 $ & $  10.49720 $ & $ i$\\
$ 55243.85399 $ & $   0.00789 $ & $   0.00106 $ & $  10.49290 $ & $ i$\\
$ 55243.85450 $ & $   0.00510 $ & $   0.00106 $ & $  10.48980 $ & $ i$\\
$ 55243.85519 $ & $   0.00913 $ & $   0.00106 $ & $  10.49350 $ & $ i$\\
$ 55243.85569 $ & $   0.01572 $ & $   0.00106 $ & $  10.50070 $ & $ i$\\
$ 55243.85637 $ & $   0.00380 $ & $   0.00106 $ & $  10.48850 $ & $ i$\\
$ 55243.85686 $ & $   0.00670 $ & $   0.00106 $ & $  10.49090 $ & $ i$\\
$ 55243.85753 $ & $   0.01026 $ & $   0.00106 $ & $  10.49480 $ & $ i$\\
$ 55243.85804 $ & $   0.01193 $ & $   0.00106 $ & $  10.49640 $ & $ i$\\
$ 55243.85873 $ & $   0.01120 $ & $   0.00106 $ & $  10.49560 $ & $ i$\\
$ 55243.85922 $ & $   0.00498 $ & $   0.00106 $ & $  10.48920 $ & $ i$\\
$ 55243.85993 $ & $   0.01826 $ & $   0.00106 $ & $  10.50210 $ & $ i$\\
$ 55243.86044 $ & $   0.00769 $ & $   0.00106 $ & $  10.49190 $ & $ i$\\
$ 55243.86111 $ & $   0.00638 $ & $   0.00106 $ & $  10.49070 $ & $ i$\\
$ 55243.86162 $ & $   0.01305 $ & $   0.00106 $ & $  10.49730 $ & $ i$\\
$ 55243.86230 $ & $   0.01024 $ & $   0.00106 $ & $  10.49530 $ & $ i$\\
$ 55243.86280 $ & $   0.01268 $ & $   0.00106 $ & $  10.49730 $ & $ i$\\
$ 55243.86350 $ & $   0.00775 $ & $   0.00105 $ & $  10.49220 $ & $ i$\\
$ 55243.86399 $ & $   0.00675 $ & $   0.00106 $ & $  10.49090 $ & $ i$\\
$ 55243.86468 $ & $   0.01126 $ & $   0.00106 $ & $  10.49560 $ & $ i$\\
$ 55243.86519 $ & $   0.00864 $ & $   0.00106 $ & $  10.49270 $ & $ i$\\
$ 55243.86588 $ & $   0.00829 $ & $   0.00106 $ & $  10.49340 $ & $ i$\\
$ 55243.86639 $ & $   0.00777 $ & $   0.00106 $ & $  10.49210 $ & $ i$\\
$ 55243.86707 $ & $   0.01320 $ & $   0.00106 $ & $  10.49820 $ & $ i$\\
$ 55243.86757 $ & $   0.01096 $ & $   0.00106 $ & $  10.49510 $ & $ i$\\
$ 55243.86825 $ & $   0.01236 $ & $   0.00106 $ & $  10.49660 $ & $ i$\\
$ 55243.86876 $ & $   0.01072 $ & $   0.00106 $ & $  10.49560 $ & $ i$\\
$ 55243.86942 $ & $   0.00642 $ & $   0.00106 $ & $  10.49060 $ & $ i$\\
$ 55243.86991 $ & $   0.00623 $ & $   0.00106 $ & $  10.49100 $ & $ i$\\
$ 55243.87043 $ & $   0.00954 $ & $   0.00106 $ & $  10.49410 $ & $ i$\\
$ 55243.87094 $ & $   0.00999 $ & $   0.00106 $ & $  10.49460 $ & $ i$\\
$ 55243.87166 $ & $   0.01380 $ & $   0.00106 $ & $  10.49820 $ & $ i$\\
$ 55243.87214 $ & $   0.00301 $ & $   0.00106 $ & $  10.48690 $ & $ i$\\
$ 55243.87280 $ & $   0.01131 $ & $   0.00106 $ & $  10.49600 $ & $ i$\\
$ 55243.87330 $ & $   0.00633 $ & $   0.00107 $ & $  10.49010 $ & $ i$\\
$ 55243.87399 $ & $   0.01300 $ & $   0.00106 $ & $  10.49710 $ & $ i$\\
$ 55243.87448 $ & $   0.01008 $ & $   0.00106 $ & $  10.49430 $ & $ i$\\
$ 55243.87516 $ & $   0.00815 $ & $   0.00106 $ & $  10.49290 $ & $ i$\\
$ 55243.87567 $ & $   0.01765 $ & $   0.00106 $ & $  10.50210 $ & $ i$\\
$ 55243.87634 $ & $   0.00686 $ & $   0.00107 $ & $  10.49150 $ & $ i$\\
$ 55243.87685 $ & $   0.00458 $ & $   0.00106 $ & $  10.48890 $ & $ i$\\
$ 55243.87755 $ & $   0.01049 $ & $   0.00106 $ & $  10.49500 $ & $ i$\\
$ 55243.87806 $ & $   0.01128 $ & $   0.00106 $ & $  10.49630 $ & $ i$\\
$ 55243.87874 $ & $   0.01257 $ & $   0.00106 $ & $  10.49730 $ & $ i$\\
$ 55243.87924 $ & $   0.01045 $ & $   0.00107 $ & $  10.49560 $ & $ i$\\
$ 55243.87991 $ & $   0.00570 $ & $   0.00106 $ & $  10.49030 $ & $ i$\\
$ 55243.88041 $ & $   0.01687 $ & $   0.00106 $ & $  10.50250 $ & $ i$\\
$ 55243.88108 $ & $   0.01057 $ & $   0.00106 $ & $  10.49590 $ & $ i$\\
$ 55243.88157 $ & $   0.00712 $ & $   0.00106 $ & $  10.49200 $ & $ i$\\
$ 55243.88226 $ & $   0.01293 $ & $   0.00107 $ & $  10.49730 $ & $ i$\\
$ 55243.88275 $ & $   0.00889 $ & $   0.00107 $ & $  10.49390 $ & $ i$\\
$ 55243.88347 $ & $   0.00883 $ & $   0.00107 $ & $  10.49350 $ & $ i$\\
$ 55243.88396 $ & $   0.01131 $ & $   0.00107 $ & $  10.49570 $ & $ i$\\
$ 55243.88462 $ & $   0.01524 $ & $   0.00107 $ & $  10.50070 $ & $ i$\\
$ 55243.88513 $ & $   0.01230 $ & $   0.00107 $ & $  10.49770 $ & $ i$\\
$ 55243.88581 $ & $   0.00939 $ & $   0.00107 $ & $  10.49480 $ & $ i$\\
$ 55243.88632 $ & $   0.01807 $ & $   0.00107 $ & $  10.50310 $ & $ i$\\
$ 55243.88700 $ & $   0.00746 $ & $   0.00106 $ & $  10.49330 $ & $ i$\\
$ 55243.88749 $ & $   0.00766 $ & $   0.00107 $ & $  10.49330 $ & $ i$\\
$ 55243.88816 $ & $   0.01210 $ & $   0.00106 $ & $  10.49770 $ & $ i$\\
$ 55243.88866 $ & $   0.00813 $ & $   0.00107 $ & $  10.49350 $ & $ i$\\
$ 55243.88936 $ & $   0.00521 $ & $   0.00106 $ & $  10.49070 $ & $ i$\\
$ 55243.88986 $ & $   0.00783 $ & $   0.00106 $ & $  10.49300 $ & $ i$\\
$ 55243.89054 $ & $   0.00758 $ & $   0.00107 $ & $  10.49300 $ & $ i$\\
$ 55243.89104 $ & $   0.01073 $ & $   0.00107 $ & $  10.49640 $ & $ i$\\
$ 55243.89171 $ & $   0.01348 $ & $   0.00107 $ & $  10.49840 $ & $ i$\\
$ 55243.89220 $ & $   0.01270 $ & $   0.00107 $ & $  10.49790 $ & $ i$\\
$ 55243.89288 $ & $   0.00969 $ & $   0.00106 $ & $  10.49500 $ & $ i$\\
$ 55243.89338 $ & $   0.00642 $ & $   0.00107 $ & $  10.49200 $ & $ i$\\
$ 55243.89404 $ & $   0.00825 $ & $   0.00107 $ & $  10.49340 $ & $ i$\\
$ 55243.89454 $ & $   0.01202 $ & $   0.00107 $ & $  10.49780 $ & $ i$\\
$ 55243.89524 $ & $   0.01470 $ & $   0.00107 $ & $  10.49940 $ & $ i$\\
$ 55243.89575 $ & $   0.01979 $ & $   0.00106 $ & $  10.50460 $ & $ i$\\
$ 55243.89644 $ & $   0.00575 $ & $   0.00107 $ & $  10.49090 $ & $ i$\\
$ 55243.89692 $ & $   0.00720 $ & $   0.00107 $ & $  10.49230 $ & $ i$\\
$ 55243.89761 $ & $   0.00839 $ & $   0.00107 $ & $  10.49440 $ & $ i$\\
$ 55243.89810 $ & $   0.00856 $ & $   0.00106 $ & $  10.49370 $ & $ i$\\
$ 55243.89876 $ & $   0.00945 $ & $   0.00107 $ & $  10.49440 $ & $ i$\\
$ 55243.89926 $ & $   0.01225 $ & $   0.00107 $ & $  10.49800 $ & $ i$\\
$ 55243.89992 $ & $   0.01407 $ & $   0.00106 $ & $  10.49890 $ & $ i$\\
$ 55243.90043 $ & $   0.00970 $ & $   0.00107 $ & $  10.49500 $ & $ i$\\
$ 55243.90114 $ & $   0.00658 $ & $   0.00106 $ & $  10.49200 $ & $ i$\\
$ 55243.90163 $ & $   0.00897 $ & $   0.00107 $ & $  10.49470 $ & $ i$\\
$ 55243.90230 $ & $   0.01292 $ & $   0.00106 $ & $  10.49810 $ & $ i$\\
$ 55243.90280 $ & $   0.01169 $ & $   0.00107 $ & $  10.49640 $ & $ i$\\
$ 55243.90347 $ & $   0.01227 $ & $   0.00106 $ & $  10.49710 $ & $ i$\\
$ 55243.90398 $ & $   0.01470 $ & $   0.00106 $ & $  10.49990 $ & $ i$\\
$ 55243.90465 $ & $   0.00618 $ & $   0.00107 $ & $  10.49170 $ & $ i$\\
$ 55243.90516 $ & $   0.01031 $ & $   0.00106 $ & $  10.49560 $ & $ i$\\
$ 55243.90585 $ & $   0.00756 $ & $   0.00106 $ & $  10.49280 $ & $ i$\\
$ 55243.90634 $ & $   0.01108 $ & $   0.00107 $ & $  10.49630 $ & $ i$\\
$ 55243.90706 $ & $   0.01112 $ & $   0.00106 $ & $  10.49640 $ & $ i$\\
$ 55243.90756 $ & $   0.01241 $ & $   0.00106 $ & $  10.49740 $ & $ i$\\
$ 55243.90823 $ & $   0.01160 $ & $   0.00106 $ & $  10.49680 $ & $ i$\\
$ 55243.90873 $ & $   0.00711 $ & $   0.00106 $ & $  10.49140 $ & $ i$\\
$ 55243.90942 $ & $   0.00966 $ & $   0.00106 $ & $  10.49450 $ & $ i$\\
$ 55243.90991 $ & $   0.01375 $ & $   0.00106 $ & $  10.49890 $ & $ i$\\
$ 55243.91058 $ & $   0.01252 $ & $   0.00106 $ & $  10.49680 $ & $ i$\\
$ 55243.91107 $ & $   0.01233 $ & $   0.00107 $ & $  10.49770 $ & $ i$\\
$ 55243.91174 $ & $   0.01084 $ & $   0.00106 $ & $  10.49670 $ & $ i$\\
$ 55243.91223 $ & $   0.01422 $ & $   0.00107 $ & $  10.49930 $ & $ i$\\
$ 55243.91295 $ & $   0.00824 $ & $   0.00106 $ & $  10.49330 $ & $ i$\\
$ 55243.91345 $ & $   0.00700 $ & $   0.00106 $ & $  10.49260 $ & $ i$\\
$ 55243.91413 $ & $   0.00997 $ & $   0.00106 $ & $  10.49560 $ & $ i$\\
$ 55243.91463 $ & $   0.00809 $ & $   0.00106 $ & $  10.49350 $ & $ i$\\
$ 55243.91533 $ & $   0.00576 $ & $   0.00107 $ & $  10.49120 $ & $ i$\\
$ 55243.91581 $ & $   0.01259 $ & $   0.00106 $ & $  10.49810 $ & $ i$\\
$ 55243.91648 $ & $   0.00352 $ & $   0.00106 $ & $  10.48870 $ & $ i$\\
$ 55243.91699 $ & $   0.00987 $ & $   0.00106 $ & $  10.49570 $ & $ i$\\
$ 55243.91766 $ & $   0.01163 $ & $   0.00106 $ & $  10.49670 $ & $ i$\\
$ 55243.91817 $ & $   0.00731 $ & $   0.00106 $ & $  10.49290 $ & $ i$\\
$ 55243.91888 $ & $   0.01700 $ & $   0.00106 $ & $  10.50330 $ & $ i$\\
$ 55243.91938 $ & $   0.01232 $ & $   0.00106 $ & $  10.49750 $ & $ i$\\
$ 55243.92005 $ & $   0.00911 $ & $   0.00106 $ & $  10.49400 $ & $ i$\\
$ 55243.92056 $ & $   0.00967 $ & $   0.00107 $ & $  10.49460 $ & $ i$\\
$ 55243.92123 $ & $   0.01389 $ & $   0.00106 $ & $  10.49920 $ & $ i$\\
$ 55243.92173 $ & $   0.01562 $ & $   0.00106 $ & $  10.50070 $ & $ i$\\
$ 55243.92240 $ & $   0.00373 $ & $   0.00106 $ & $  10.48900 $ & $ i$\\
$ 55243.92289 $ & $   0.01116 $ & $   0.00106 $ & $  10.49640 $ & $ i$\\
$ 55243.92355 $ & $   0.01320 $ & $   0.00107 $ & $  10.49830 $ & $ i$\\
$ 55243.92405 $ & $   0.00140 $ & $   0.00106 $ & $  10.48670 $ & $ i$\\
$ 55243.92476 $ & $   0.01184 $ & $   0.00106 $ & $  10.49690 $ & $ i$\\
$ 55243.92526 $ & $   0.01384 $ & $   0.00106 $ & $  10.49890 $ & $ i$\\
$ 55243.92594 $ & $   0.00969 $ & $   0.00106 $ & $  10.49490 $ & $ i$\\
$ 55243.92712 $ & $   0.01208 $ & $   0.00106 $ & $  10.49770 $ & $ i$\\
$ 55243.92763 $ & $   0.01707 $ & $   0.00106 $ & $  10.50200 $ & $ i$\\
$ 55243.92831 $ & $   0.01273 $ & $   0.00106 $ & $  10.49800 $ & $ i$\\
$ 55243.92880 $ & $   0.01143 $ & $   0.00106 $ & $  10.49650 $ & $ i$\\
$ 55243.92949 $ & $   0.00699 $ & $   0.00106 $ & $  10.49250 $ & $ i$\\
$ 55243.93000 $ & $   0.01335 $ & $   0.00106 $ & $  10.49890 $ & $ i$\\
$ 55243.93070 $ & $   0.00923 $ & $   0.00106 $ & $  10.49380 $ & $ i$\\
$ 55243.93119 $ & $   0.01071 $ & $   0.00106 $ & $  10.49590 $ & $ i$\\
$ 55243.93189 $ & $   0.00511 $ & $   0.00107 $ & $  10.49070 $ & $ i$\\
$ 55243.93239 $ & $   0.01002 $ & $   0.00106 $ & $  10.49530 $ & $ i$\\
$ 55243.93306 $ & $   0.01045 $ & $   0.00106 $ & $  10.49550 $ & $ i$\\
$ 55243.93355 $ & $   0.00727 $ & $   0.00106 $ & $  10.49250 $ & $ i$\\
$ 55243.93423 $ & $   0.00712 $ & $   0.00106 $ & $  10.49250 $ & $ i$\\
$ 55243.93473 $ & $   0.00776 $ & $   0.00106 $ & $  10.49280 $ & $ i$\\
$ 55243.93542 $ & $   0.00811 $ & $   0.00106 $ & $  10.49340 $ & $ i$\\
$ 55243.93592 $ & $   0.01188 $ & $   0.00106 $ & $  10.49720 $ & $ i$\\
$ 55243.93662 $ & $   0.00812 $ & $   0.00106 $ & $  10.49310 $ & $ i$\\
$ 55243.93712 $ & $   0.00774 $ & $   0.00106 $ & $  10.49400 $ & $ i$\\
$ 55243.93780 $ & $   0.00742 $ & $   0.00106 $ & $  10.49300 $ & $ i$\\
$ 55243.93830 $ & $   0.01287 $ & $   0.00107 $ & $  10.49820 $ & $ i$\\
$ 55243.93898 $ & $   0.00359 $ & $   0.00107 $ & $  10.48870 $ & $ i$\\
$ 55243.93949 $ & $   0.00981 $ & $   0.00106 $ & $  10.49530 $ & $ i$\\
$ 55243.94017 $ & $   0.00917 $ & $   0.00107 $ & $  10.49470 $ & $ i$\\
$ 55243.94066 $ & $   0.00127 $ & $   0.00107 $ & $  10.48650 $ & $ i$\\
$ 55243.94133 $ & $   0.00694 $ & $   0.00107 $ & $  10.49200 $ & $ i$\\
$ 55243.94183 $ & $   0.01026 $ & $   0.00107 $ & $  10.49560 $ & $ i$\\
$ 55243.94252 $ & $   0.01249 $ & $   0.00106 $ & $  10.49720 $ & $ i$\\
$ 55243.94301 $ & $   0.00222 $ & $   0.00106 $ & $  10.48790 $ & $ i$\\
$ 55243.94370 $ & $   0.00844 $ & $   0.00106 $ & $  10.49360 $ & $ i$\\
$ 55243.94421 $ & $   0.00873 $ & $   0.00106 $ & $  10.49450 $ & $ i$\\
$ 55243.94489 $ & $   0.00552 $ & $   0.00106 $ & $  10.49060 $ & $ i$\\
$ 55243.94539 $ & $   0.00371 $ & $   0.00106 $ & $  10.48890 $ & $ i$\\
$ 55243.94655 $ & $   0.00767 $ & $   0.00106 $ & $  10.49310 $ & $ i$\\
$ 55243.94770 $ & $   0.00021 $ & $   0.00107 $ & $  10.48550 $ & $ i$\\
$ 55243.94840 $ & $   0.00502 $ & $   0.00106 $ & $  10.49010 $ & $ i$\\
$ 55243.94890 $ & $   0.00399 $ & $   0.00106 $ & $  10.48980 $ & $ i$\\
$ 55243.94958 $ & $   0.00143 $ & $   0.00106 $ & $  10.48700 $ & $ i$\\
$ 55243.95008 $ & $   0.00174 $ & $   0.00107 $ & $  10.48680 $ & $ i$\\
$ 55243.95075 $ & $   0.00290 $ & $   0.00107 $ & $  10.48820 $ & $ i$\\
$ 55243.95125 $ & $  -0.00029 $ & $   0.00106 $ & $  10.48510 $ & $ i$\\
$ 55243.95192 $ & $  -0.00166 $ & $   0.00106 $ & $  10.48390 $ & $ i$\\
$ 55243.95242 $ & $   0.00101 $ & $   0.00106 $ & $  10.48610 $ & $ i$\\
$ 55243.95308 $ & $  -0.00576 $ & $   0.00107 $ & $  10.47990 $ & $ i$\\
$ 55243.95357 $ & $  -0.00002 $ & $   0.00107 $ & $  10.48540 $ & $ i$\\
$ 55243.95427 $ & $   0.00447 $ & $   0.00107 $ & $  10.49000 $ & $ i$\\
$ 55243.95477 $ & $  -0.00137 $ & $   0.00107 $ & $  10.48440 $ & $ i$\\
$ 55243.95530 $ & $  -0.00525 $ & $   0.00107 $ & $  10.48100 $ & $ i$\\
$ 55243.95580 $ & $   0.00059 $ & $   0.00106 $ & $  10.48580 $ & $ i$\\
$ 55243.95649 $ & $  -0.00817 $ & $   0.00106 $ & $  10.47770 $ & $ i$\\
$ 55243.95698 $ & $  -0.00195 $ & $   0.00107 $ & $  10.48370 $ & $ i$\\
$ 55243.95765 $ & $  -0.00187 $ & $   0.00107 $ & $  10.48330 $ & $ i$\\
$ 55243.95815 $ & $  -0.00666 $ & $   0.00107 $ & $  10.47850 $ & $ i$\\
$ 55243.95884 $ & $  -0.00406 $ & $   0.00107 $ & $  10.48120 $ & $ i$\\
$ 55243.95934 $ & $  -0.00234 $ & $   0.00107 $ & $  10.48330 $ & $ i$\\
$ 55243.96005 $ & $   0.00604 $ & $   0.00107 $ & $  10.49190 $ & $ i$\\
$ 55243.96056 $ & $   0.00002 $ & $   0.00106 $ & $  10.48550 $ & $ i$\\
$ 55243.96123 $ & $   0.00200 $ & $   0.00107 $ & $  10.48760 $ & $ i$\\
$ 55243.96174 $ & $  -0.00457 $ & $   0.00107 $ & $  10.48080 $ & $ i$\\
$ 55243.96242 $ & $   0.00421 $ & $   0.00107 $ & $  10.49000 $ & $ i$\\
$ 55243.96292 $ & $  -0.00018 $ & $   0.00107 $ & $  10.48510 $ & $ i$\\
$ 55243.96360 $ & $   0.00119 $ & $   0.00107 $ & $  10.48660 $ & $ i$\\
$ 55243.96410 $ & $  -0.00059 $ & $   0.00107 $ & $  10.48460 $ & $ i$\\
$ 55243.96478 $ & $   0.00021 $ & $   0.00107 $ & $  10.48610 $ & $ i$\\
$ 55243.96528 $ & $   0.00430 $ & $   0.00107 $ & $  10.48980 $ & $ i$\\
$ 55243.96600 $ & $  -0.00168 $ & $   0.00107 $ & $  10.48450 $ & $ i$\\
$ 55243.96651 $ & $   0.00020 $ & $   0.00107 $ & $  10.48560 $ & $ i$\\
$ 55243.96719 $ & $   0.00265 $ & $   0.00108 $ & $  10.48840 $ & $ i$\\
$ 55243.96769 $ & $  -0.00009 $ & $   0.00107 $ & $  10.48570 $ & $ i$\\
$ 55243.96836 $ & $   0.00765 $ & $   0.00107 $ & $  10.49300 $ & $ i$\\
$ 55243.96887 $ & $   0.00101 $ & $   0.00107 $ & $  10.48680 $ & $ i$\\
$ 55243.96955 $ & $   0.00249 $ & $   0.00107 $ & $  10.48790 $ & $ i$\\
$ 55243.97004 $ & $  -0.00162 $ & $   0.00107 $ & $  10.48460 $ & $ i$\\
$ 55243.97122 $ & $   0.00127 $ & $   0.00107 $ & $  10.48670 $ & $ i$\\
$ 55243.97191 $ & $  -0.00110 $ & $   0.00107 $ & $  10.48490 $ & $ i$\\
$ 55243.97241 $ & $  -0.00080 $ & $   0.00107 $ & $  10.48450 $ & $ i$\\
$ 55243.97359 $ & $  -0.00380 $ & $   0.00107 $ & $  10.48150 $ & $ i$\\
$ 55243.97427 $ & $   0.00105 $ & $   0.00108 $ & $  10.48700 $ & $ i$\\
$ 55243.97478 $ & $  -0.00207 $ & $   0.00107 $ & $  10.48340 $ & $ i$\\
$ 55243.97546 $ & $   0.00137 $ & $   0.00108 $ & $  10.48720 $ & $ i$\\
$ 55243.97595 $ & $  -0.00766 $ & $   0.00107 $ & $  10.47780 $ & $ i$\\
$ 55243.97663 $ & $  -0.00142 $ & $   0.00107 $ & $  10.48390 $ & $ i$\\
$ 55243.97713 $ & $  -0.00084 $ & $   0.00107 $ & $  10.48400 $ & $ i$\\
$ 55243.97780 $ & $   0.00432 $ & $   0.00107 $ & $  10.49020 $ & $ i$\\
$ 55243.97831 $ & $  -0.00565 $ & $   0.00107 $ & $  10.47990 $ & $ i$\\
$ 55243.97899 $ & $   0.00172 $ & $   0.00107 $ & $  10.48710 $ & $ i$\\
$ 55243.97949 $ & $  -0.00125 $ & $   0.00107 $ & $  10.48450 $ & $ i$\\
$ 55243.98016 $ & $   0.00049 $ & $   0.00108 $ & $  10.48640 $ & $ i$\\
$ 55243.98066 $ & $   0.00138 $ & $   0.00108 $ & $  10.48690 $ & $ i$\\
$ 55243.98133 $ & $  -0.00317 $ & $   0.00108 $ & $  10.48200 $ & $ i$\\
$ 55243.98184 $ & $   0.00413 $ & $   0.00107 $ & $  10.49020 $ & $ i$\\
$ 55243.98251 $ & $  -0.00271 $ & $   0.00107 $ & $  10.48350 $ & $ i$\\
$ 55243.98301 $ & $   0.00675 $ & $   0.00107 $ & $  10.49230 $ & $ i$\\
$ 55243.98369 $ & $   0.00104 $ & $   0.00107 $ & $  10.48680 $ & $ i$\\
$ 55243.98419 $ & $   0.00107 $ & $   0.00108 $ & $  10.48720 $ & $ i$\\
$ 55243.98487 $ & $  -0.00075 $ & $   0.00108 $ & $  10.48530 $ & $ i$\\
$ 55243.98538 $ & $  -0.00229 $ & $   0.00108 $ & $  10.48330 $ & $ i$\\
$ 55243.98605 $ & $  -0.00702 $ & $   0.00108 $ & $  10.47870 $ & $ i$\\
$ 55243.98655 $ & $   0.00071 $ & $   0.00108 $ & $  10.48660 $ & $ i$\\
$ 55243.98723 $ & $  -0.00055 $ & $   0.00108 $ & $  10.48530 $ & $ i$\\
$ 55243.98772 $ & $  -0.00977 $ & $   0.00108 $ & $  10.47670 $ & $ i$\\
$ 55243.98839 $ & $  -0.00761 $ & $   0.00109 $ & $  10.47930 $ & $ i$\\
$ 55243.98889 $ & $   0.00333 $ & $   0.00109 $ & $  10.48990 $ & $ i$\\
$ 55243.98957 $ & $  -0.00155 $ & $   0.00108 $ & $  10.48450 $ & $ i$\\
$ 55243.99008 $ & $   0.00612 $ & $   0.00109 $ & $  10.49330 $ & $ i$\\
$ 55243.99076 $ & $   0.00413 $ & $   0.00108 $ & $  10.49040 $ & $ i$\\
$ 55243.99127 $ & $   0.00374 $ & $   0.00108 $ & $  10.48980 $ & $ i$\\
$ 55243.99198 $ & $  -0.00165 $ & $   0.00108 $ & $  10.48430 $ & $ i$\\
$ 55243.99248 $ & $   0.00125 $ & $   0.00108 $ & $  10.48740 $ & $ i$\\
$ 55243.99318 $ & $  -0.00251 $ & $   0.00108 $ & $  10.48410 $ & $ i$\\
$ 55243.99369 $ & $  -0.00785 $ & $   0.00108 $ & $  10.47870 $ & $ i$\\
$ 55243.99436 $ & $  -0.00050 $ & $   0.00108 $ & $  10.48670 $ & $ i$\\
$ 55243.99486 $ & $  -0.00129 $ & $   0.00109 $ & $  10.48480 $ & $ i$\\
$ 55243.99558 $ & $  -0.00418 $ & $   0.00109 $ & $  10.48280 $ & $ i$\\
$ 55243.99608 $ & $  -0.00097 $ & $   0.00108 $ & $  10.48610 $ & $ i$\\
$ 55243.99676 $ & $   0.00705 $ & $   0.00109 $ & $  10.49320 $ & $ i$\\
$ 55243.99727 $ & $   0.00387 $ & $   0.00108 $ & $  10.49090 $ & $ i$\\
$ 55243.99794 $ & $   0.00519 $ & $   0.00109 $ & $  10.49200 $ & $ i$\\
$ 55243.99845 $ & $   0.00711 $ & $   0.00109 $ & $  10.49380 $ & $ i$\\
$ 55243.99912 $ & $   0.00060 $ & $   0.00108 $ & $  10.48710 $ & $ i$\\
$ 55243.99963 $ & $   0.00744 $ & $   0.00108 $ & $  10.49360 $ & $ i$\\
$ 55244.00031 $ & $  -0.00368 $ & $   0.00108 $ & $  10.48330 $ & $ i$\\
$ 55244.00082 $ & $   0.00533 $ & $   0.00108 $ & $  10.49230 $ & $ i$\\
$ 55244.00153 $ & $   0.00092 $ & $   0.00109 $ & $  10.48750 $ & $ i$\\
$ 55244.00203 $ & $  -0.00045 $ & $   0.00109 $ & $  10.48640 $ & $ i$\\
$ 55244.00271 $ & $   0.00480 $ & $   0.00108 $ & $  10.49150 $ & $ i$\\
$ 55244.00321 $ & $   0.00082 $ & $   0.00109 $ & $  10.48770 $ & $ i$\\
$ 55244.00389 $ & $   0.00164 $ & $   0.00109 $ & $  10.48890 $ & $ i$\\
$ 55244.00440 $ & $  -0.00001 $ & $   0.00108 $ & $  10.48710 $ & $ i$\\
$ 55247.88480 $ & $   0.01004 $ & $   0.00085 $ & $   9.01154 $ & $ i$\\
$ 55247.88516 $ & $   0.01359 $ & $   0.00087 $ & $   9.01467 $ & $ i$\\
$ 55247.88559 $ & $  -0.00347 $ & $   0.00084 $ & $   8.99808 $ & $ i$\\
$ 55247.88596 $ & $  -0.00440 $ & $   0.00089 $ & $   8.99780 $ & $ i$\\
$ 55247.88632 $ & $  -0.00647 $ & $   0.00086 $ & $   8.99521 $ & $ i$\\
$ 55247.88673 $ & $   0.00280 $ & $   0.00085 $ & $   9.00392 $ & $ i$\\
$ 55247.88708 $ & $  -0.00332 $ & $   0.00085 $ & $   8.99833 $ & $ i$\\
$ 55247.88743 $ & $   0.00080 $ & $   0.00086 $ & $   9.00371 $ & $ i$\\
$ 55247.88781 $ & $   0.00363 $ & $   0.00086 $ & $   9.00578 $ & $ i$\\
$ 55247.88821 $ & $  -0.00964 $ & $   0.00086 $ & $   8.99216 $ & $ i$\\
$ 55247.88859 $ & $   0.00753 $ & $   0.00087 $ & $   9.00942 $ & $ i$\\
$ 55247.88903 $ & $   0.00475 $ & $   0.00085 $ & $   9.00740 $ & $ i$\\
$ 55247.88973 $ & $   0.00893 $ & $   0.00085 $ & $   9.01136 $ & $ i$\\
$ 55247.89011 $ & $  -0.00341 $ & $   0.00084 $ & $   8.99824 $ & $ i$\\
$ 55247.89049 $ & $  -0.00735 $ & $   0.00085 $ & $   8.99400 $ & $ i$\\
$ 55247.89086 $ & $  -0.00339 $ & $   0.00087 $ & $   8.99796 $ & $ i$\\
$ 55247.89125 $ & $  -0.00214 $ & $   0.00086 $ & $   8.99873 $ & $ i$\\
$ 55247.89163 $ & $   0.00037 $ & $   0.00085 $ & $   9.00147 $ & $ i$\\
$ 55247.89239 $ & $   0.00120 $ & $   0.00089 $ & $   9.00269 $ & $ i$\\
$ 55247.89278 $ & $  -0.00029 $ & $   0.00084 $ & $   9.00048 $ & $ i$\\
$ 55247.89314 $ & $   0.00037 $ & $   0.00086 $ & $   9.00113 $ & $ i$\\
$ 55247.89350 $ & $   0.01290 $ & $   0.00088 $ & $   9.01497 $ & $ i$\\
$ 55247.89394 $ & $   0.00042 $ & $   0.00085 $ & $   9.00267 $ & $ i$\\
$ 55247.89434 $ & $   0.01297 $ & $   0.00088 $ & $   9.01532 $ & $ i$\\
$ 55247.89504 $ & $  -0.01163 $ & $   0.00088 $ & $   8.99063 $ & $ i$\\
$ 55247.89687 $ & $   0.00036 $ & $   0.00086 $ & $   9.00238 $ & $ i$\\
$ 55247.89759 $ & $   0.00490 $ & $   0.00087 $ & $   9.00657 $ & $ i$\\
$ 55247.89794 $ & $  -0.00130 $ & $   0.00086 $ & $   8.99954 $ & $ i$\\
$ 55247.89866 $ & $   0.00313 $ & $   0.00086 $ & $   9.00471 $ & $ i$\\
$ 55247.89938 $ & $  -0.00261 $ & $   0.00088 $ & $   8.99848 $ & $ i$\\
$ 55247.89973 $ & $  -0.00681 $ & $   0.00084 $ & $   8.99479 $ & $ i$\\
$ 55247.90050 $ & $  -0.00934 $ & $   0.00086 $ & $   8.99204 $ & $ i$\\
$ 55247.90085 $ & $   0.00809 $ & $   0.00086 $ & $   9.00991 $ & $ i$\\
$ 55247.90120 $ & $  -0.00403 $ & $   0.00086 $ & $   8.99789 $ & $ i$\\
$ 55247.90194 $ & $   0.01352 $ & $   0.00087 $ & $   9.01526 $ & $ i$\\
$ 55247.90231 $ & $   0.01154 $ & $   0.00087 $ & $   9.01342 $ & $ i$\\
$ 55247.90306 $ & $   0.00130 $ & $   0.00085 $ & $   9.00333 $ & $ i$\\
$ 55247.90346 $ & $   0.00138 $ & $   0.00085 $ & $   9.00334 $ & $ i$\\
$ 55247.90383 $ & $   0.00104 $ & $   0.00087 $ & $   9.00275 $ & $ i$\\
$ 55247.90419 $ & $  -0.01050 $ & $   0.00088 $ & $   8.99223 $ & $ i$\\
$ 55247.90529 $ & $   0.00831 $ & $   0.00088 $ & $   9.00940 $ & $ i$\\
$ 55247.90565 $ & $   0.00375 $ & $   0.00087 $ & $   9.00535 $ & $ i$\\
$ 55247.90599 $ & $  -0.00845 $ & $   0.00087 $ & $   8.99413 $ & $ i$\\
$ 55247.90634 $ & $   0.00591 $ & $   0.00087 $ & $   9.00760 $ & $ i$\\
$ 55247.90672 $ & $   0.00162 $ & $   0.00087 $ & $   9.00358 $ & $ i$\\
$ 55247.90709 $ & $  -0.01406 $ & $   0.00086 $ & $   8.98851 $ & $ i$\\
$ 55247.90744 $ & $   0.01500 $ & $   0.00088 $ & $   9.01690 $ & $ i$\\
$ 55247.90780 $ & $  -0.00364 $ & $   0.00088 $ & $   8.99849 $ & $ i$\\
$ 55247.91409 $ & $   0.00984 $ & $   0.00088 $ & $   9.01157 $ & $ i$\\
$ 55247.91445 $ & $   0.00852 $ & $   0.00087 $ & $   9.01138 $ & $ i$\\
$ 55247.91481 $ & $  -0.00318 $ & $   0.00085 $ & $   8.99881 $ & $ i$\\
$ 55247.91590 $ & $  -0.00778 $ & $   0.00087 $ & $   8.99413 $ & $ i$\\
$ 55247.91705 $ & $  -0.00780 $ & $   0.00087 $ & $   8.99416 $ & $ i$\\
$ 55247.91965 $ & $  -0.00389 $ & $   0.00087 $ & $   8.99880 $ & $ i$\\
$ 55247.92003 $ & $  -0.00505 $ & $   0.00086 $ & $   8.99816 $ & $ i$\\
$ 55247.92038 $ & $   0.01168 $ & $   0.00087 $ & $   9.01424 $ & $ i$\\
$ 55247.92073 $ & $   0.00366 $ & $   0.00088 $ & $   9.00580 $ & $ i$\\
$ 55247.92115 $ & $  -0.01213 $ & $   0.00087 $ & $   8.99013 $ & $ i$\\
$ 55247.92150 $ & $   0.01046 $ & $   0.00088 $ & $   9.01293 $ & $ i$\\
$ 55247.92189 $ & $  -0.00905 $ & $   0.00087 $ & $   8.99348 $ & $ i$\\
$ 55247.92223 $ & $  -0.00083 $ & $   0.00088 $ & $   9.00238 $ & $ i$\\
$ 55247.92294 $ & $  -0.00424 $ & $   0.00087 $ & $   8.99877 $ & $ i$\\
$ 55247.92442 $ & $   0.00852 $ & $   0.00087 $ & $   9.01200 $ & $ i$\\
$ 55247.92479 $ & $   0.00096 $ & $   0.00085 $ & $   9.00408 $ & $ i$\\
$ 55247.92514 $ & $  -0.00466 $ & $   0.00088 $ & $   8.99831 $ & $ i$\\
$ 55247.92548 $ & $   0.01052 $ & $   0.00087 $ & $   9.01329 $ & $ i$\\
$ 55247.92586 $ & $   0.00815 $ & $   0.00087 $ & $   9.01092 $ & $ i$\\
$ 55247.92623 $ & $   0.00977 $ & $   0.00086 $ & $   9.01261 $ & $ i$\\
$ 55247.92662 $ & $  -0.00259 $ & $   0.00087 $ & $   8.99949 $ & $ i$\\
$ 55247.92698 $ & $  -0.00914 $ & $   0.00086 $ & $   8.99410 $ & $ i$\\
$ 55247.92768 $ & $   0.00433 $ & $   0.00084 $ & $   9.00609 $ & $ i$\\
$ 55247.92806 $ & $   0.00184 $ & $   0.00085 $ & $   9.00383 $ & $ i$\\
$ 55247.92846 $ & $  -0.00522 $ & $   0.00087 $ & $   8.99907 $ & $ i$\\
$ 55247.92885 $ & $   0.00835 $ & $   0.00084 $ & $   9.01036 $ & $ i$\\
$ 55247.92998 $ & $  -0.00199 $ & $   0.00086 $ & $   9.00144 $ & $ i$\\
$ 55247.93034 $ & $   0.00008 $ & $   0.00085 $ & $   9.00123 $ & $ i$\\
$ 55247.93073 $ & $  -0.00633 $ & $   0.00086 $ & $   8.99608 $ & $ i$\\
$ 55247.93111 $ & $  -0.01061 $ & $   0.00087 $ & $   8.99301 $ & $ i$\\
$ 55247.93147 $ & $   0.00260 $ & $   0.00086 $ & $   9.00533 $ & $ i$\\
$ 55247.93185 $ & $   0.00374 $ & $   0.00084 $ & $   9.00545 $ & $ i$\\
$ 55247.93222 $ & $  -0.00894 $ & $   0.00085 $ & $   8.99351 $ & $ i$\\
$ 55247.93294 $ & $  -0.00525 $ & $   0.00087 $ & $   8.99833 $ & $ i$\\
$ 55247.93331 $ & $  -0.00225 $ & $   0.00086 $ & $   8.99954 $ & $ i$\\
$ 55247.93366 $ & $  -0.00030 $ & $   0.00084 $ & $   9.00145 $ & $ i$\\
$ 55247.93408 $ & $   0.00294 $ & $   0.00084 $ & $   9.00668 $ & $ i$\\
$ 55247.93449 $ & $   0.00021 $ & $   0.00084 $ & $   9.00245 $ & $ i$\\
$ 55247.93484 $ & $   0.00893 $ & $   0.00086 $ & $   9.01212 $ & $ i$\\
$ 55247.93522 $ & $   0.00126 $ & $   0.00086 $ & $   9.00459 $ & $ i$\\
$ 55247.93557 $ & $   0.01279 $ & $   0.00084 $ & $   9.01373 $ & $ i$\\
$ 55247.93592 $ & $  -0.00435 $ & $   0.00085 $ & $   8.99842 $ & $ i$\\
$ 55247.93630 $ & $   0.00523 $ & $   0.00085 $ & $   9.00742 $ & $ i$\\
$ 55247.93670 $ & $  -0.00253 $ & $   0.00085 $ & $   9.00025 $ & $ i$\\
$ 55247.93710 $ & $   0.00028 $ & $   0.00087 $ & $   9.00340 $ & $ i$\\
$ 55247.93747 $ & $   0.01256 $ & $   0.00087 $ & $   9.01520 $ & $ i$\\
$ 55247.93824 $ & $   0.00393 $ & $   0.00088 $ & $   9.00705 $ & $ i$\\
$ 55247.93859 $ & $   0.00800 $ & $   0.00086 $ & $   9.01080 $ & $ i$\\
$ 55247.93929 $ & $   0.00911 $ & $   0.00085 $ & $   9.01133 $ & $ i$\\
$ 55247.93967 $ & $   0.00380 $ & $   0.00086 $ & $   9.00756 $ & $ i$\\
$ 55247.94004 $ & $   0.00101 $ & $   0.00087 $ & $   9.00441 $ & $ i$\\
$ 55247.94043 $ & $   0.00338 $ & $   0.00086 $ & $   9.00603 $ & $ i$\\
$ 55247.94081 $ & $   0.00148 $ & $   0.00086 $ & $   9.00463 $ & $ i$\\
$ 55247.94119 $ & $   0.01288 $ & $   0.00088 $ & $   9.01557 $ & $ i$\\
$ 55247.94155 $ & $   0.01041 $ & $   0.00085 $ & $   9.01311 $ & $ i$\\
$ 55247.94195 $ & $   0.00465 $ & $   0.00086 $ & $   9.00832 $ & $ i$\\
$ 55247.94230 $ & $   0.00740 $ & $   0.00085 $ & $   9.01126 $ & $ i$\\
$ 55247.94265 $ & $  -0.00629 $ & $   0.00084 $ & $   8.99660 $ & $ i$\\
$ 55247.94300 $ & $   0.00410 $ & $   0.00086 $ & $   9.00746 $ & $ i$\\
$ 55247.94339 $ & $   0.00935 $ & $   0.00085 $ & $   9.01268 $ & $ i$\\
$ 55247.94411 $ & $   0.00578 $ & $   0.00085 $ & $   9.00905 $ & $ i$\\
$ 55247.94449 $ & $   0.00149 $ & $   0.00086 $ & $   9.00437 $ & $ i$\\
$ 55247.94488 $ & $  -0.00059 $ & $   0.00084 $ & $   9.00185 $ & $ i$\\
$ 55247.94524 $ & $  -0.00243 $ & $   0.00085 $ & $   9.00017 $ & $ i$\\
$ 55247.94564 $ & $   0.01779 $ & $   0.00084 $ & $   9.02003 $ & $ i$\\
$ 55247.94603 $ & $   0.00509 $ & $   0.00084 $ & $   9.00874 $ & $ i$\\
$ 55247.94639 $ & $  -0.00625 $ & $   0.00084 $ & $   8.99553 $ & $ i$\\
$ 55247.94679 $ & $   0.01064 $ & $   0.00085 $ & $   9.01360 $ & $ i$\\
$ 55247.94714 $ & $   0.00877 $ & $   0.00084 $ & $   9.01013 $ & $ i$\\
$ 55247.94754 $ & $   0.00570 $ & $   0.00084 $ & $   9.00839 $ & $ i$\\
$ 55247.94863 $ & $   0.01657 $ & $   0.00084 $ & $   9.01914 $ & $ i$\\
$ 55247.94898 $ & $   0.01631 $ & $   0.00084 $ & $   9.01837 $ & $ i$\\
$ 55247.94937 $ & $   0.00270 $ & $   0.00084 $ & $   9.00559 $ & $ i$\\
$ 55247.94973 $ & $   0.00206 $ & $   0.00084 $ & $   9.00518 $ & $ i$\\
$ 55247.95042 $ & $   0.00936 $ & $   0.00085 $ & $   9.01173 $ & $ i$\\
$ 55247.95080 $ & $   0.00897 $ & $   0.00088 $ & $   9.01133 $ & $ i$\\
$ 55247.95117 $ & $   0.01239 $ & $   0.00085 $ & $   9.01483 $ & $ i$\\
$ 55247.95156 $ & $   0.00458 $ & $   0.00086 $ & $   9.00783 $ & $ i$\\
$ 55247.95195 $ & $   0.00132 $ & $   0.00085 $ & $   9.00434 $ & $ i$\\
$ 55247.95232 $ & $   0.00528 $ & $   0.00085 $ & $   9.00721 $ & $ i$\\
$ 55247.95308 $ & $   0.01390 $ & $   0.00087 $ & $   9.01850 $ & $ i$\\
$ 55247.95343 $ & $   0.00166 $ & $   0.00086 $ & $   9.00452 $ & $ i$\\
$ 55247.95378 $ & $   0.00476 $ & $   0.00085 $ & $   9.00770 $ & $ i$\\
$ 55247.95417 $ & $   0.00380 $ & $   0.00087 $ & $   9.00690 $ & $ i$\\
$ 55247.95454 $ & $   0.01105 $ & $   0.00087 $ & $   9.01416 $ & $ i$\\
$ 55247.95497 $ & $   0.01377 $ & $   0.00085 $ & $   9.01628 $ & $ i$\\
$ 55247.95534 $ & $   0.00614 $ & $   0.00085 $ & $   9.00916 $ & $ i$\\
$ 55247.95571 $ & $   0.00118 $ & $   0.00086 $ & $   9.00518 $ & $ i$\\
$ 55247.95612 $ & $   0.01064 $ & $   0.00085 $ & $   9.01291 $ & $ i$\\
$ 55247.95647 $ & $   0.01537 $ & $   0.00085 $ & $   9.01835 $ & $ i$\\
$ 55247.95681 $ & $   0.01569 $ & $   0.00087 $ & $   9.01865 $ & $ i$\\
$ 55247.95723 $ & $   0.01979 $ & $   0.00087 $ & $   9.02330 $ & $ i$\\
$ 55247.95758 $ & $   0.00586 $ & $   0.00087 $ & $   9.00915 $ & $ i$\\
$ 55247.95832 $ & $   0.00824 $ & $   0.00087 $ & $   9.01232 $ & $ i$\\
$ 55247.95866 $ & $   0.00712 $ & $   0.00086 $ & $   9.01097 $ & $ i$\\
$ 55247.95944 $ & $   0.01970 $ & $   0.00088 $ & $   9.02429 $ & $ i$\\
$ 55247.95979 $ & $   0.01156 $ & $   0.00088 $ & $   9.01461 $ & $ i$\\
$ 55247.96014 $ & $   0.00745 $ & $   0.00085 $ & $   9.01130 $ & $ i$\\
$ 55247.96054 $ & $   0.01444 $ & $   0.00085 $ & $   9.01779 $ & $ i$\\
$ 55247.96091 $ & $   0.00264 $ & $   0.00086 $ & $   9.00687 $ & $ i$\\
$ 55247.96127 $ & $   0.01397 $ & $   0.00086 $ & $   9.01872 $ & $ i$\\
$ 55247.96163 $ & $  -0.00355 $ & $   0.00086 $ & $   8.99986 $ & $ i$\\
$ 55247.96197 $ & $   0.02698 $ & $   0.00087 $ & $   9.03109 $ & $ i$\\
$ 55247.96236 $ & $   0.02240 $ & $   0.00087 $ & $   9.02614 $ & $ i$\\
$ 55247.96273 $ & $   0.00692 $ & $   0.00086 $ & $   9.01112 $ & $ i$\\
$ 55247.96308 $ & $   0.01103 $ & $   0.00087 $ & $   9.01566 $ & $ i$\\
$ 55247.96346 $ & $   0.01798 $ & $   0.00086 $ & $   9.02074 $ & $ i$\\
$ 55247.96386 $ & $   0.01273 $ & $   0.00085 $ & $   9.01768 $ & $ i$\\
$ 55247.96422 $ & $   0.01321 $ & $   0.00085 $ & $   9.01738 $ & $ i$\\
$ 55247.96457 $ & $   0.00386 $ & $   0.00084 $ & $   9.00727 $ & $ i$\\
$ 55247.96493 $ & $   0.00229 $ & $   0.00084 $ & $   9.00575 $ & $ i$\\
$ 55247.96531 $ & $   0.01097 $ & $   0.00084 $ & $   9.01425 $ & $ i$\\
$ 55247.96567 $ & $   0.00970 $ & $   0.00084 $ & $   9.01280 $ & $ i$\\
$ 55247.96607 $ & $   0.00721 $ & $   0.00084 $ & $   9.01015 $ & $ i$\\
$ 55247.96645 $ & $   0.01066 $ & $   0.00084 $ & $   9.01357 $ & $ i$\\
$ 55247.96685 $ & $   0.00966 $ & $   0.00084 $ & $   9.01398 $ & $ i$\\
$ 55247.96794 $ & $   0.01078 $ & $   0.00084 $ & $   9.01412 $ & $ i$\\
$ 55247.96833 $ & $   0.00446 $ & $   0.00084 $ & $   9.01096 $ & $ i$\\
$ 55247.96869 $ & $  -0.00177 $ & $   0.00084 $ & $   9.00241 $ & $ i$\\
$ 55247.96912 $ & $   0.00324 $ & $   0.00084 $ & $   9.00733 $ & $ i$\\
$ 55247.96952 $ & $  -0.00795 $ & $   0.00084 $ & $   8.99623 $ & $ i$\\
$ 55247.96986 $ & $   0.00507 $ & $   0.00085 $ & $   9.00909 $ & $ i$\\
$ 55247.97025 $ & $   0.01260 $ & $   0.00084 $ & $   9.01664 $ & $ i$\\
$ 55247.97060 $ & $   0.00344 $ & $   0.00086 $ & $   9.00813 $ & $ i$\\
$ 55247.97095 $ & $   0.01524 $ & $   0.00085 $ & $   9.01963 $ & $ i$\\
$ 55247.97134 $ & $   0.01594 $ & $   0.00088 $ & $   9.01965 $ & $ i$\\
$ 55247.97170 $ & $   0.00943 $ & $   0.00087 $ & $   9.01388 $ & $ i$\\
$ 55247.97207 $ & $   0.00748 $ & $   0.00088 $ & $   9.01260 $ & $ i$\\
$ 55247.97242 $ & $   0.00156 $ & $   0.00088 $ & $   9.00622 $ & $ i$\\
$ 55247.97280 $ & $   0.00749 $ & $   0.00088 $ & $   9.01228 $ & $ i$\\
$ 55247.97390 $ & $   0.01523 $ & $   0.00088 $ & $   9.01980 $ & $ i$\\
$ 55247.97729 $ & $  -0.00265 $ & $   0.00088 $ & $   9.00205 $ & $ i$\\
$ 55247.97802 $ & $   0.00050 $ & $   0.00088 $ & $   9.00513 $ & $ i$\\
$ 55247.97945 $ & $   0.00033 $ & $   0.00088 $ & $   9.00537 $ & $ i$\\
$ 55247.98019 $ & $   0.02998 $ & $   0.00088 $ & $   9.03423 $ & $ i$\\
$ 55247.98057 $ & $   0.00971 $ & $   0.00087 $ & $   9.01413 $ & $ i$\\
$ 55247.98094 $ & $   0.01286 $ & $   0.00086 $ & $   9.01755 $ & $ i$\\
$ 55247.98129 $ & $   0.00878 $ & $   0.00086 $ & $   9.01303 $ & $ i$\\
$ 55247.98166 $ & $   0.00644 $ & $   0.00087 $ & $   9.01126 $ & $ i$\\
$ 55247.98203 $ & $   0.00756 $ & $   0.00086 $ & $   9.01208 $ & $ i$\\
$ 55247.98243 $ & $   0.00805 $ & $   0.00087 $ & $   9.01296 $ & $ i$\\
$ 55247.98280 $ & $   0.01035 $ & $   0.00088 $ & $   9.01530 $ & $ i$\\
$ 55247.98465 $ & $  -0.00074 $ & $   0.00087 $ & $   9.00422 $ & $ i$\\
$ 55247.98503 $ & $   0.01970 $ & $   0.00087 $ & $   9.02479 $ & $ i$\\
$ 55247.98539 $ & $   0.00766 $ & $   0.00087 $ & $   9.01237 $ & $ i$\\
$ 55247.98649 $ & $   0.02120 $ & $   0.00089 $ & $   9.02623 $ & $ i$\\
$ 55247.98684 $ & $  -0.00349 $ & $   0.00087 $ & $   9.00128 $ & $ i$\\
$ 55247.98723 $ & $   0.01510 $ & $   0.00089 $ & $   9.02048 $ & $ i$\\
$ 55247.98766 $ & $   0.00698 $ & $   0.00086 $ & $   9.01226 $ & $ i$\\
$ 55247.98801 $ & $   0.00762 $ & $   0.00088 $ & $   9.01215 $ & $ i$\\
$ 55247.98836 $ & $  -0.00140 $ & $   0.00085 $ & $   9.00304 $ & $ i$\\
$ 55247.98874 $ & $   0.00591 $ & $   0.00085 $ & $   9.01136 $ & $ i$\\
$ 55247.98991 $ & $   0.01228 $ & $   0.00086 $ & $   9.01709 $ & $ i$\\
$ 55247.99027 $ & $   0.00705 $ & $   0.00087 $ & $   9.01205 $ & $ i$\\
$ 55247.99066 $ & $   0.00554 $ & $   0.00085 $ & $   9.01094 $ & $ i$\\
$ 55247.99137 $ & $   0.01219 $ & $   0.00085 $ & $   9.01743 $ & $ i$\\
$ 55247.99179 $ & $   0.00702 $ & $   0.00086 $ & $   9.01273 $ & $ i$\\
$ 55247.99217 $ & $   0.00472 $ & $   0.00086 $ & $   9.01023 $ & $ i$\\
$ 55247.99252 $ & $   0.00867 $ & $   0.00086 $ & $   9.01394 $ & $ i$\\
$ 55247.99293 $ & $  -0.00047 $ & $   0.00085 $ & $   9.00472 $ & $ i$\\
$ 55247.99365 $ & $   0.01140 $ & $   0.00084 $ & $   9.01719 $ & $ i$\\
$ 55247.99439 $ & $   0.01247 $ & $   0.00084 $ & $   9.01847 $ & $ i$\\
$ 55247.99474 $ & $   0.00479 $ & $   0.00084 $ & $   9.01072 $ & $ i$\\
$ 55247.99555 $ & $   0.01742 $ & $   0.00085 $ & $   9.02235 $ & $ i$\\
$ 55247.99590 $ & $  -0.00578 $ & $   0.00084 $ & $   9.00050 $ & $ i$\\
$ 55247.99625 $ & $   0.02117 $ & $   0.00084 $ & $   9.02703 $ & $ i$\\
$ 55247.99663 $ & $   0.00842 $ & $   0.00084 $ & $   9.01532 $ & $ i$\\
$ 55247.99699 $ & $   0.01165 $ & $   0.00084 $ & $   9.01726 $ & $ i$\\
$ 55247.99736 $ & $  -0.00268 $ & $   0.00085 $ & $   9.00310 $ & $ i$\\
$ 55247.99774 $ & $   0.00659 $ & $   0.00084 $ & $   9.01050 $ & $ i$\\
$ 55247.99813 $ & $   0.02117 $ & $   0.00085 $ & $   9.02609 $ & $ i$\\
$ 55247.99889 $ & $   0.00511 $ & $   0.00084 $ & $   9.01163 $ & $ i$\\
$ 55247.99929 $ & $   0.00016 $ & $   0.00084 $ & $   9.00653 $ & $ i$\\
$ 55247.99966 $ & $   0.00471 $ & $   0.00084 $ & $   9.01046 $ & $ i$\\
$ 55248.00002 $ & $   0.01304 $ & $   0.00084 $ & $   9.01888 $ & $ i$\\
$ 55248.00038 $ & $   0.00414 $ & $   0.00084 $ & $   9.01007 $ & $ i$\\
$ 55248.00077 $ & $   0.02232 $ & $   0.00084 $ & $   9.02902 $ & $ i$\\
$ 55248.00115 $ & $   0.02257 $ & $   0.00085 $ & $   9.02774 $ & $ i$\\
$ 55248.00152 $ & $   0.01741 $ & $   0.00085 $ & $   9.02338 $ & $ i$\\
$ 55248.00188 $ & $   0.00884 $ & $   0.00084 $ & $   9.01514 $ & $ i$\\
$ 55248.00262 $ & $   0.00997 $ & $   0.00084 $ & $   9.01655 $ & $ i$\\
$ 55248.00297 $ & $   0.01557 $ & $   0.00084 $ & $   9.02156 $ & $ i$\\
$ 55248.00336 $ & $   0.00853 $ & $   0.00083 $ & $   9.01502 $ & $ i$\\
$ 55248.00372 $ & $   0.00013 $ & $   0.00083 $ & $   9.00671 $ & $ i$\\
$ 55248.00413 $ & $   0.01066 $ & $   0.00084 $ & $   9.01678 $ & $ i$\\
$ 55248.00487 $ & $   0.00766 $ & $   0.00083 $ & $   9.01351 $ & $ i$\\
$ 55248.00530 $ & $   0.00874 $ & $   0.00083 $ & $   9.01572 $ & $ i$\\
$ 55248.00566 $ & $   0.02329 $ & $   0.00083 $ & $   9.02947 $ & $ i$\\
$ 55248.00600 $ & $   0.01187 $ & $   0.00084 $ & $   9.01877 $ & $ i$\\
$ 55248.00639 $ & $   0.00766 $ & $   0.00083 $ & $   9.01319 $ & $ i$\\
$ 55248.00717 $ & $   0.01785 $ & $   0.00084 $ & $   9.02431 $ & $ i$\\
$ 55248.00758 $ & $   0.00814 $ & $   0.00084 $ & $   9.01403 $ & $ i$\\
$ 55248.00793 $ & $   0.00746 $ & $   0.00084 $ & $   9.01394 $ & $ i$\\
$ 55248.00832 $ & $   0.01472 $ & $   0.00084 $ & $   9.02067 $ & $ i$\\
$ 55248.00867 $ & $   0.01666 $ & $   0.00084 $ & $   9.02356 $ & $ i$\\
$ 55248.00901 $ & $   0.01246 $ & $   0.00084 $ & $   9.01853 $ & $ i$\\
$ 55248.00940 $ & $   0.00670 $ & $   0.00084 $ & $   9.01300 $ & $ i$\\
$ 55248.00979 $ & $   0.01098 $ & $   0.00084 $ & $   9.01714 $ & $ i$\\
$ 55248.01052 $ & $   0.01599 $ & $   0.00084 $ & $   9.02236 $ & $ i$\\
$ 55248.01172 $ & $   0.01263 $ & $   0.00084 $ & $   9.02083 $ & $ i$\\
$ 55248.01208 $ & $   0.01389 $ & $   0.00084 $ & $   9.02170 $ & $ i$\\
$ 55248.01247 $ & $   0.00683 $ & $   0.00084 $ & $   9.01439 $ & $ i$\\
$ 55248.01286 $ & $   0.01944 $ & $   0.00084 $ & $   9.02737 $ & $ i$\\
$ 55248.01323 $ & $   0.01692 $ & $   0.00083 $ & $   9.02430 $ & $ i$\\
$ 55248.01401 $ & $   0.00016 $ & $   0.00084 $ & $   9.00732 $ & $ i$\\
$ 55248.01587 $ & $   0.01395 $ & $   0.00084 $ & $   9.02049 $ & $ i$\\
$ 55248.01698 $ & $   0.00101 $ & $   0.00084 $ & $   9.00864 $ & $ i$\\
$ 55248.01734 $ & $   0.01374 $ & $   0.00084 $ & $   9.02210 $ & $ i$\\
$ 55248.01816 $ & $   0.00287 $ & $   0.00083 $ & $   9.01050 $ & $ i$\\
$ 55248.01851 $ & $   0.01209 $ & $   0.00083 $ & $   9.01969 $ & $ i$\\
$ 55248.01927 $ & $   0.01297 $ & $   0.00083 $ & $   9.02096 $ & $ i$\\
$ 55248.02002 $ & $   0.01616 $ & $   0.00084 $ & $   9.02408 $ & $ i$\\
$ 55248.02037 $ & $   0.01384 $ & $   0.00084 $ & $   9.02251 $ & $ i$\\
$ 55248.02077 $ & $   0.00373 $ & $   0.00084 $ & $   9.01157 $ & $ i$\\
$ 55248.02149 $ & $   0.00998 $ & $   0.00084 $ & $   9.01712 $ & $ i$\\
$ 55248.02184 $ & $   0.02000 $ & $   0.00084 $ & $   9.02702 $ & $ i$\\
$ 55248.02221 $ & $   0.01683 $ & $   0.00084 $ & $   9.02403 $ & $ i$\\
$ 55248.02264 $ & $   0.01090 $ & $   0.00084 $ & $   9.01818 $ & $ i$\\
$ 55248.02300 $ & $   0.00357 $ & $   0.00084 $ & $   9.01153 $ & $ i$\\
$ 55248.02338 $ & $   0.00652 $ & $   0.00086 $ & $   9.01353 $ & $ i$\\
$ 55248.02374 $ & $   0.02818 $ & $   0.00086 $ & $   9.03435 $ & $ i$\\
$ 55248.02409 $ & $   0.00887 $ & $   0.00085 $ & $   9.01588 $ & $ i$\\
$ 55248.02447 $ & $   0.02017 $ & $   0.00084 $ & $   9.02786 $ & $ i$\\
$ 55248.02483 $ & $   0.00919 $ & $   0.00085 $ & $   9.01730 $ & $ i$\\
$ 55248.02520 $ & $   0.00040 $ & $   0.00085 $ & $   9.00763 $ & $ i$\\
$ 55248.02561 $ & $   0.01558 $ & $   0.00084 $ & $   9.02268 $ & $ i$\\
$ 55248.02602 $ & $   0.00739 $ & $   0.00084 $ & $   9.01455 $ & $ i$\\
$ 55248.02637 $ & $   0.00430 $ & $   0.00084 $ & $   9.01217 $ & $ i$\\
$ 55248.02671 $ & $   0.02023 $ & $   0.00084 $ & $   9.02822 $ & $ i$\\
$ 55248.02745 $ & $   0.01829 $ & $   0.00084 $ & $   9.02519 $ & $ i$\\
$ 55248.02818 $ & $   0.02066 $ & $   0.00084 $ & $   9.02822 $ & $ i$\\
$ 55248.02858 $ & $   0.01176 $ & $   0.00086 $ & $   9.01885 $ & $ i$\\
$ 55248.02896 $ & $   0.00559 $ & $   0.00085 $ & $   9.01262 $ & $ i$\\
$ 55248.02931 $ & $   0.01062 $ & $   0.00085 $ & $   9.01818 $ & $ i$\\
$ 55248.02966 $ & $   0.01971 $ & $   0.00085 $ & $   9.02665 $ & $ i$\\
$ 55248.03007 $ & $   0.00795 $ & $   0.00084 $ & $   9.01593 $ & $ i$\\
$ 55248.03042 $ & $   0.00695 $ & $   0.00084 $ & $   9.01532 $ & $ i$\\
$ 55248.03077 $ & $   0.01389 $ & $   0.00084 $ & $   9.02251 $ & $ i$\\
$ 55248.03115 $ & $   0.02124 $ & $   0.00084 $ & $   9.02884 $ & $ i$\\
$ 55248.03154 $ & $   0.02232 $ & $   0.00084 $ & $   9.02865 $ & $ i$\\
$ 55248.03190 $ & $   0.02047 $ & $   0.00084 $ & $   9.02621 $ & $ i$\\
$ 55248.03226 $ & $   0.00998 $ & $   0.00083 $ & $   9.01745 $ & $ i$\\
$ 55248.03266 $ & $   0.00974 $ & $   0.00084 $ & $   9.01778 $ & $ i$\\
$ 55248.03305 $ & $   0.00272 $ & $   0.00084 $ & $   9.01147 $ & $ i$\\
$ 55248.03380 $ & $   0.00269 $ & $   0.00084 $ & $   9.01036 $ & $ i$\\
$ 55248.03416 $ & $   0.01847 $ & $   0.00085 $ & $   9.02631 $ & $ i$\\
$ 55248.03451 $ & $  -0.00080 $ & $   0.00087 $ & $   9.00567 $ & $ i$\\
$ 55248.03490 $ & $   0.01733 $ & $   0.00086 $ & $   9.02400 $ & $ i$\\
$ 55248.03526 $ & $   0.01263 $ & $   0.00086 $ & $   9.01957 $ & $ i$\\
$ 55248.03569 $ & $   0.00892 $ & $   0.00085 $ & $   9.01592 $ & $ i$\\
$ 55248.03709 $ & $   0.01921 $ & $   0.00084 $ & $   9.02668 $ & $ i$\\
$ 55248.03746 $ & $   0.02071 $ & $   0.00084 $ & $   9.02927 $ & $ i$\\
$ 55248.03782 $ & $   0.01617 $ & $   0.00084 $ & $   9.02394 $ & $ i$\\
$ 55248.03897 $ & $   0.00685 $ & $   0.00085 $ & $   9.01480 $ & $ i$\\
$ 55248.03936 $ & $   0.01739 $ & $   0.00084 $ & $   9.02574 $ & $ i$\\
$ 55248.03972 $ & $   0.01588 $ & $   0.00084 $ & $   9.02444 $ & $ i$\\
$ 55248.04008 $ & $  -0.00127 $ & $   0.00084 $ & $   9.00827 $ & $ i$\\
$ 55248.04050 $ & $   0.00564 $ & $   0.00084 $ & $   9.01418 $ & $ i$\\
$ 55248.04086 $ & $   0.01425 $ & $   0.00084 $ & $   9.02213 $ & $ i$\\
$ 55248.04124 $ & $  -0.00258 $ & $   0.00084 $ & $   9.00620 $ & $ i$\\
$ 55248.04163 $ & $   0.00638 $ & $   0.00084 $ & $   9.01494 $ & $ i$\\
$ 55248.04239 $ & $   0.01280 $ & $   0.00083 $ & $   9.02207 $ & $ i$\\
$ 55248.04315 $ & $   0.00564 $ & $   0.00083 $ & $   9.01477 $ & $ i$\\
$ 55248.04351 $ & $   0.01238 $ & $   0.00084 $ & $   9.02094 $ & $ i$\\
$ 55248.04388 $ & $   0.00126 $ & $   0.00084 $ & $   9.00888 $ & $ i$\\
$ 55248.04423 $ & $   0.01208 $ & $   0.00084 $ & $   9.02072 $ & $ i$\\
$ 55248.04458 $ & $   0.00774 $ & $   0.00084 $ & $   9.01551 $ & $ i$\\
$ 55248.04498 $ & $   0.01229 $ & $   0.00084 $ & $   9.02114 $ & $ i$\\
$ 55248.04533 $ & $   0.01377 $ & $   0.00084 $ & $   9.02208 $ & $ i$\\
$ 55248.04568 $ & $   0.01251 $ & $   0.00084 $ & $   9.02034 $ & $ i$\\
$ 55248.04603 $ & $   0.00832 $ & $   0.00084 $ & $   9.01611 $ & $ i$\\
$ 55248.04639 $ & $   0.00977 $ & $   0.00084 $ & $   9.01873 $ & $ i$\\
$ 55248.04679 $ & $   0.01868 $ & $   0.00084 $ & $   9.02761 $ & $ i$\\
$ 55248.04714 $ & $   0.01133 $ & $   0.00084 $ & $   9.01939 $ & $ i$\\
$ 55248.04750 $ & $   0.00438 $ & $   0.00084 $ & $   9.01245 $ & $ i$\\
$ 55248.04785 $ & $   0.01565 $ & $   0.00084 $ & $   9.02527 $ & $ i$\\
$ 55248.04823 $ & $   0.00550 $ & $   0.00084 $ & $   9.01455 $ & $ i$\\
$ 55248.04900 $ & $   0.01943 $ & $   0.00084 $ & $   9.02883 $ & $ i$\\
$ 55248.04936 $ & $   0.00731 $ & $   0.00083 $ & $   9.01690 $ & $ i$\\
$ 55248.04974 $ & $   0.00284 $ & $   0.00083 $ & $   9.01347 $ & $ i$\\
$ 55248.05012 $ & $   0.02260 $ & $   0.00084 $ & $   9.02996 $ & $ i$\\
$ 55248.05049 $ & $   0.01802 $ & $   0.00084 $ & $   9.02675 $ & $ i$\\
$ 55248.05087 $ & $   0.01230 $ & $   0.00084 $ & $   9.02084 $ & $ i$\\
$ 55248.05126 $ & $   0.01405 $ & $   0.00084 $ & $   9.02205 $ & $ i$\\
$ 55248.05162 $ & $   0.00652 $ & $   0.00084 $ & $   9.01526 $ & $ i$\\
$ 55248.05198 $ & $   0.00595 $ & $   0.00084 $ & $   9.01360 $ & $ i$\\
$ 55248.05238 $ & $  -0.00963 $ & $   0.00083 $ & $   8.99952 $ & $ i$\\
$ 55248.05274 $ & $   0.00833 $ & $   0.00083 $ & $   9.01842 $ & $ i$\\
$ 55248.05316 $ & $   0.01687 $ & $   0.00083 $ & $   9.02704 $ & $ i$\\
$ 55248.05353 $ & $  -0.00056 $ & $   0.00083 $ & $   9.01026 $ & $ i$\\
$ 55248.05463 $ & $   0.01084 $ & $   0.00083 $ & $   9.02089 $ & $ i$\\
$ 55248.05499 $ & $   0.01255 $ & $   0.00083 $ & $   9.02199 $ & $ i$\\
$ 55248.05574 $ & $   0.01733 $ & $   0.00083 $ & $   9.02378 $ & $ i$\\
$ 55248.05609 $ & $   0.00516 $ & $   0.00083 $ & $   9.01537 $ & $ i$\\
$ 55248.05648 $ & $   0.01046 $ & $   0.00084 $ & $   9.01912 $ & $ i$\\
$ 55248.05684 $ & $   0.01136 $ & $   0.00085 $ & $   9.01936 $ & $ i$\\
$ 55248.05720 $ & $   0.00863 $ & $   0.00084 $ & $   9.01670 $ & $ i$\\
$ 55248.05757 $ & $   0.01673 $ & $   0.00084 $ & $   9.02402 $ & $ i$\\
$ 55248.05795 $ & $   0.01004 $ & $   0.00083 $ & $   9.01791 $ & $ i$\\
$ 55248.05831 $ & $   0.01264 $ & $   0.00083 $ & $   9.02295 $ & $ i$\\
$ 55248.05901 $ & $   0.00636 $ & $   0.00083 $ & $   9.01622 $ & $ i$\\
$ 55248.05939 $ & $   0.00457 $ & $   0.00083 $ & $   9.01392 $ & $ i$\\
$ 55248.05975 $ & $   0.00793 $ & $   0.00084 $ & $   9.01681 $ & $ i$\\
$ 55248.06012 $ & $   0.01043 $ & $   0.00085 $ & $   9.01844 $ & $ i$\\
$ 55248.06050 $ & $   0.00739 $ & $   0.00085 $ & $   9.01502 $ & $ i$\\
$ 55248.06090 $ & $   0.00019 $ & $   0.00084 $ & $   9.00810 $ & $ i$\\
$ 55248.06130 $ & $   0.02066 $ & $   0.00084 $ & $   9.02847 $ & $ i$\\
$ 55248.06165 $ & $   0.00014 $ & $   0.00085 $ & $   9.00686 $ & $ i$\\
$ 55248.06205 $ & $   0.00519 $ & $   0.00085 $ & $   9.01307 $ & $ i$\\
$ 55248.06242 $ & $   0.01250 $ & $   0.00084 $ & $   9.02106 $ & $ i$\\
$ 55248.06278 $ & $   0.01459 $ & $   0.00084 $ & $   9.02361 $ & $ i$\\
$ 55248.06317 $ & $   0.01425 $ & $   0.00084 $ & $   9.02396 $ & $ i$\\
$ 55248.06352 $ & $   0.00882 $ & $   0.00084 $ & $   9.01776 $ & $ i$\\
$ 55248.06387 $ & $   0.00876 $ & $   0.00083 $ & $   9.01636 $ & $ i$\\
$ 55248.06457 $ & $   0.00912 $ & $   0.00084 $ & $   9.01782 $ & $ i$\\
$ 55248.06496 $ & $   0.00993 $ & $   0.00084 $ & $   9.01753 $ & $ i$\\
$ 55248.06535 $ & $   0.00281 $ & $   0.00083 $ & $   9.01266 $ & $ i$\\
$ 55248.06646 $ & $   0.00192 $ & $   0.00085 $ & $   9.00869 $ & $ i$\\
$ 55248.06686 $ & $   0.00422 $ & $   0.00085 $ & $   9.01145 $ & $ i$\\
$ 55248.06720 $ & $   0.01064 $ & $   0.00084 $ & $   9.01841 $ & $ i$\\
$ 55248.06758 $ & $  -0.00555 $ & $   0.00084 $ & $   9.00151 $ & $ i$\\
$ 55248.06793 $ & $   0.02112 $ & $   0.00084 $ & $   9.02806 $ & $ i$\\
$ 55248.06828 $ & $   0.00736 $ & $   0.00085 $ & $   9.01508 $ & $ i$\\
$ 55248.06863 $ & $   0.00670 $ & $   0.00084 $ & $   9.01533 $ & $ i$\\
$ 55248.06899 $ & $   0.00219 $ & $   0.00084 $ & $   9.00910 $ & $ i$\\
$ 55248.06936 $ & $   0.00841 $ & $   0.00083 $ & $   9.01762 $ & $ i$\\
$ 55248.06974 $ & $   0.00917 $ & $   0.00083 $ & $   9.01786 $ & $ i$\\
$ 55248.07045 $ & $  -0.00576 $ & $   0.00084 $ & $   9.00383 $ & $ i$\\
$ 55248.07083 $ & $   0.00938 $ & $   0.00083 $ & $   9.01846 $ & $ i$\\
$ 55248.07122 $ & $   0.00454 $ & $   0.00084 $ & $   9.01251 $ & $ i$\\
$ 55248.07158 $ & $   0.01235 $ & $   0.00083 $ & $   9.02139 $ & $ i$\\
$ 55248.07201 $ & $  -0.00356 $ & $   0.00083 $ & $   9.00620 $ & $ i$\\
$ 55248.07242 $ & $   0.00465 $ & $   0.00083 $ & $   9.01348 $ & $ i$\\
$ 55248.07277 $ & $  -0.00011 $ & $   0.00084 $ & $   9.00826 $ & $ i$\\
$ 55248.07315 $ & $   0.01208 $ & $   0.00084 $ & $   9.02046 $ & $ i$\\
$ 55248.07350 $ & $   0.00856 $ & $   0.00083 $ & $   9.01796 $ & $ i$\\
$ 55248.07385 $ & $   0.00380 $ & $   0.00083 $ & $   9.01275 $ & $ i$\\
$ 55248.07425 $ & $   0.00236 $ & $   0.00083 $ & $   9.00923 $ & $ i$\\
$ 55248.07461 $ & $  -0.00444 $ & $   0.00084 $ & $   9.00498 $ & $ i$\\
$ 55248.07616 $ & $   0.01026 $ & $   0.00084 $ & $   9.01853 $ & $ i$\\
$ 55248.07652 $ & $   0.00823 $ & $   0.00084 $ & $   9.01613 $ & $ i$\\
$ 55248.07687 $ & $   0.00290 $ & $   0.00084 $ & $   9.01029 $ & $ i$\\
$ 55248.07726 $ & $   0.00735 $ & $   0.00084 $ & $   9.01609 $ & $ i$\\
$ 55248.07762 $ & $  -0.00194 $ & $   0.00084 $ & $   9.00738 $ & $ i$\\
$ 55248.07798 $ & $  -0.00335 $ & $   0.00084 $ & $   9.00449 $ & $ i$\\
$ 55248.07874 $ & $  -0.01541 $ & $   0.00084 $ & $   8.99309 $ & $ i$\\
$ 55248.07946 $ & $  -0.00510 $ & $   0.00083 $ & $   9.00323 $ & $ i$\\
$ 55248.07990 $ & $   0.00347 $ & $   0.00083 $ & $   9.01238 $ & $ i$\\
$ 55248.08029 $ & $   0.00002 $ & $   0.00083 $ & $   9.00818 $ & $ i$\\
$ 55248.08065 $ & $   0.00217 $ & $   0.00084 $ & $   9.00845 $ & $ i$\\
$ 55248.08100 $ & $  -0.00643 $ & $   0.00083 $ & $   9.00192 $ & $ i$\\
$ 55248.08173 $ & $   0.00476 $ & $   0.00084 $ & $   9.01214 $ & $ i$\\
$ 55248.08209 $ & $   0.00370 $ & $   0.00085 $ & $   9.01006 $ & $ i$\\
$ 55248.08245 $ & $  -0.00675 $ & $   0.00084 $ & $   9.00046 $ & $ i$\\
$ 55248.08280 $ & $   0.00315 $ & $   0.00084 $ & $   9.01119 $ & $ i$\\
$ 55248.08315 $ & $   0.01182 $ & $   0.00084 $ & $   9.01854 $ & $ i$\\
$ 55248.08351 $ & $  -0.00897 $ & $   0.00084 $ & $   8.99883 $ & $ i$\\
$ 55248.08429 $ & $   0.00328 $ & $   0.00086 $ & $   9.00826 $ & $ i$\\
$ 55248.08465 $ & $  -0.00302 $ & $   0.00084 $ & $   9.00389 $ & $ i$\\
$ 55248.08503 $ & $   0.00581 $ & $   0.00084 $ & $   9.01275 $ & $ i$\\
$ 55248.08539 $ & $   0.01512 $ & $   0.00083 $ & $   9.02237 $ & $ i$\\
$ 55248.08575 $ & $   0.00478 $ & $   0.00084 $ & $   9.01217 $ & $ i$\\
$ 55248.08614 $ & $   0.00289 $ & $   0.00084 $ & $   9.01009 $ & $ i$\\
$ 55248.08684 $ & $   0.00628 $ & $   0.00084 $ & $   9.01376 $ & $ i$\\
$ 55248.08723 $ & $  -0.00180 $ & $   0.00084 $ & $   9.00454 $ & $ i$\\
$ 55248.08759 $ & $   0.01101 $ & $   0.00084 $ & $   9.01773 $ & $ i$\\
$ 55248.08795 $ & $   0.00478 $ & $   0.00084 $ & $   9.01129 $ & $ i$\\
$ 55248.08834 $ & $  -0.00082 $ & $   0.00084 $ & $   9.00676 $ & $ i$\\
$ 55248.08869 $ & $   0.00874 $ & $   0.00084 $ & $   9.01641 $ & $ i$\\
$ 55248.08905 $ & $  -0.00527 $ & $   0.00084 $ & $   9.00076 $ & $ i$\\
$ 55248.08979 $ & $  -0.00897 $ & $   0.00083 $ & $   8.99965 $ & $ i$\\
$ 55248.09015 $ & $  -0.00828 $ & $   0.00083 $ & $   8.99992 $ & $ i$\\
$ 55248.09054 $ & $   0.00804 $ & $   0.00083 $ & $   9.01572 $ & $ i$\\
$ 55248.09090 $ & $   0.00221 $ & $   0.00083 $ & $   9.00860 $ & $ i$\\
$ 55248.09125 $ & $  -0.00172 $ & $   0.00083 $ & $   9.00525 $ & $ i$\\
$ 55248.09164 $ & $   0.00757 $ & $   0.00083 $ & $   9.01601 $ & $ i$\\
$ 55248.09200 $ & $   0.01074 $ & $   0.00083 $ & $   9.01889 $ & $ i$\\
$ 55248.09236 $ & $  -0.00514 $ & $   0.00083 $ & $   9.00279 $ & $ i$\\
$ 55248.09275 $ & $  -0.00138 $ & $   0.00083 $ & $   9.00710 $ & $ i$\\
$ 55248.09310 $ & $   0.00061 $ & $   0.00083 $ & $   9.00770 $ & $ i$\\
$ 55248.09346 $ & $   0.00054 $ & $   0.00083 $ & $   9.00805 $ & $ i$\\
$ 55248.09384 $ & $  -0.00863 $ & $   0.00083 $ & $   8.99985 $ & $ i$\\
$ 55248.09420 $ & $  -0.01813 $ & $   0.00083 $ & $   8.99011 $ & $ i$\\
$ 55248.09460 $ & $   0.00115 $ & $   0.00083 $ & $   9.00971 $ & $ i$\\
$ 55248.09495 $ & $  -0.00727 $ & $   0.00083 $ & $   9.00082 $ & $ i$\\
$ 55248.09530 $ & $   0.00178 $ & $   0.00083 $ & $   9.00942 $ & $ i$\\
$ 55248.09569 $ & $   0.00348 $ & $   0.00083 $ & $   9.01114 $ & $ i$\\
$ 55248.09605 $ & $   0.00467 $ & $   0.00083 $ & $   9.01080 $ & $ i$\\
$ 55248.09681 $ & $   0.01011 $ & $   0.00084 $ & $   9.01699 $ & $ i$\\
$ 55248.09716 $ & $  -0.00652 $ & $   0.00084 $ & $   8.99978 $ & $ i$\\
$ 55248.09790 $ & $  -0.00354 $ & $   0.00084 $ & $   9.00310 $ & $ i$\\
$ 55248.09826 $ & $   0.00142 $ & $   0.00083 $ & $   9.00832 $ & $ i$\\
$ 55248.09862 $ & $  -0.00243 $ & $   0.00083 $ & $   9.00640 $ & $ i$\\
$ 55248.09901 $ & $  -0.00002 $ & $   0.00084 $ & $   9.00705 $ & $ i$\\
$ 55248.09936 $ & $   0.00124 $ & $   0.00084 $ & $   9.00888 $ & $ i$\\
$ 55248.09972 $ & $   0.00486 $ & $   0.00084 $ & $   9.00954 $ & $ i$\\
$ 55248.10010 $ & $   0.00476 $ & $   0.00084 $ & $   9.01143 $ & $ i$\\
$ 55248.10046 $ & $  -0.00530 $ & $   0.00083 $ & $   9.00338 $ & $ i$\\
$ 55248.10083 $ & $   0.00790 $ & $   0.00083 $ & $   9.01502 $ & $ i$\\
$ 55248.10192 $ & $   0.00184 $ & $   0.00083 $ & $   9.01023 $ & $ i$\\
$ 55248.10231 $ & $   0.01132 $ & $   0.00083 $ & $   9.01837 $ & $ i$\\
$ 55248.10267 $ & $   0.00514 $ & $   0.00083 $ & $   9.00995 $ & $ i$\\
$ 55248.10303 $ & $  -0.01122 $ & $   0.00083 $ & $   8.99752 $ & $ i$\\
$ 55248.10342 $ & $   0.01163 $ & $   0.00083 $ & $   9.02027 $ & $ i$\\
$ 55248.10377 $ & $   0.00607 $ & $   0.00084 $ & $   9.01293 $ & $ i$\\
$ 55248.10413 $ & $  -0.00872 $ & $   0.00084 $ & $   8.99711 $ & $ i$\\
$ 55248.10451 $ & $   0.01190 $ & $   0.00084 $ & $   9.01846 $ & $ i$\\
$ 55248.10487 $ & $   0.01216 $ & $   0.00084 $ & $   9.01911 $ & $ i$\\
$ 55248.10526 $ & $  -0.00705 $ & $   0.00084 $ & $   9.00055 $ & $ i$\\
$ 55248.10564 $ & $  -0.00148 $ & $   0.00084 $ & $   9.00492 $ & $ i$\\
$ 55248.10636 $ & $   0.00144 $ & $   0.00084 $ & $   9.00852 $ & $ i$\\
$ 55248.10674 $ & $  -0.00189 $ & $   0.00083 $ & $   9.00553 $ & $ i$\\
$ 55248.10710 $ & $   0.01086 $ & $   0.00084 $ & $   9.01822 $ & $ i$\\
$ 55248.10748 $ & $   0.00075 $ & $   0.00084 $ & $   9.00798 $ & $ i$\\
$ 55248.10784 $ & $   0.00324 $ & $   0.00084 $ & $   9.00949 $ & $ i$\\
$ 55248.10819 $ & $  -0.00457 $ & $   0.00084 $ & $   9.00211 $ & $ i$\\
$ 55248.10857 $ & $   0.00825 $ & $   0.00084 $ & $   9.01419 $ & $ i$\\
$ 55248.11039 $ & $   0.00721 $ & $   0.00083 $ & $   9.01334 $ & $ i$\\
$ 55248.11077 $ & $  -0.00020 $ & $   0.00084 $ & $   9.00695 $ & $ i$\\
$ 55248.11113 $ & $  -0.00552 $ & $   0.00084 $ & $   8.99992 $ & $ i$\\
$ 55248.11149 $ & $   0.00162 $ & $   0.00083 $ & $   9.00817 $ & $ i$\\
$ 55248.11189 $ & $  -0.00203 $ & $   0.00083 $ & $   9.00529 $ & $ i$\\
$ 55248.11224 $ & $  -0.00072 $ & $   0.00083 $ & $   9.00511 $ & $ i$\\
$ 55248.11260 $ & $  -0.00983 $ & $   0.00084 $ & $   8.99630 $ & $ i$\\
$ 55248.11298 $ & $  -0.00179 $ & $   0.00084 $ & $   9.00373 $ & $ i$\\
$ 55248.11334 $ & $   0.00456 $ & $   0.00084 $ & $   9.01062 $ & $ i$\\
$ 55248.11410 $ & $  -0.00274 $ & $   0.00084 $ & $   9.00213 $ & $ i$\\
$ 55248.11445 $ & $   0.00730 $ & $   0.00084 $ & $   9.01367 $ & $ i$\\
$ 55248.11480 $ & $  -0.00255 $ & $   0.00084 $ & $   9.00447 $ & $ i$\\
$ 55248.11555 $ & $  -0.00553 $ & $   0.00084 $ & $   9.00038 $ & $ i$\\
$ 55248.11591 $ & $  -0.00127 $ & $   0.00083 $ & $   9.00583 $ & $ i$\\
$ 55248.11630 $ & $   0.00806 $ & $   0.00084 $ & $   9.01116 $ & $ i$\\
$ 55248.11700 $ & $  -0.00582 $ & $   0.00083 $ & $   9.00043 $ & $ i$\\
$ 55248.11810 $ & $  -0.01404 $ & $   0.00084 $ & $   8.99196 $ & $ i$\\
$ 55248.11850 $ & $  -0.01029 $ & $   0.00084 $ & $   8.99724 $ & $ i$\\
$ 55248.11921 $ & $  -0.00268 $ & $   0.00085 $ & $   9.00239 $ & $ i$\\
$ 55248.11959 $ & $  -0.00237 $ & $   0.00085 $ & $   9.00273 $ & $ i$\\
$ 55248.11995 $ & $  -0.01405 $ & $   0.00085 $ & $   8.99090 $ & $ i$\\
$ 55248.12032 $ & $   0.00599 $ & $   0.00085 $ & $   9.01149 $ & $ i$\\
$ 55248.12070 $ & $   0.00568 $ & $   0.00084 $ & $   9.01193 $ & $ i$\\
$ 55248.12106 $ & $   0.00767 $ & $   0.00084 $ & $   9.01297 $ & $ i$\\
$ 55248.12141 $ & $   0.00252 $ & $   0.00084 $ & $   9.00822 $ & $ i$\\
$ 55248.12179 $ & $  -0.00687 $ & $   0.00084 $ & $   8.99877 $ & $ i$\\
$ 55248.12252 $ & $   0.00393 $ & $   0.00084 $ & $   9.00881 $ & $ i$\\
$ 55248.12291 $ & $   0.00081 $ & $   0.00084 $ & $   9.00612 $ & $ i$\\
$ 55248.12326 $ & $   0.00077 $ & $   0.00084 $ & $   9.00703 $ & $ i$\\
$ 55248.12362 $ & $  -0.01385 $ & $   0.00084 $ & $   8.99194 $ & $ i$\\
$ 55248.12436 $ & $  -0.00370 $ & $   0.00084 $ & $   9.00265 $ & $ i$\\
$ 55248.12473 $ & $  -0.00453 $ & $   0.00084 $ & $   9.00067 $ & $ i$\\
$ 55248.12511 $ & $  -0.00196 $ & $   0.00084 $ & $   9.00476 $ & $ i$\\
$ 55248.12547 $ & $  -0.00528 $ & $   0.00084 $ & $   9.00155 $ & $ i$\\
$ 55248.12582 $ & $  -0.00556 $ & $   0.00084 $ & $   9.00072 $ & $ i$\\
$ 55248.12657 $ & $   0.00055 $ & $   0.00084 $ & $   9.00651 $ & $ i$\\
$ 55248.12693 $ & $   0.00381 $ & $   0.00084 $ & $   9.00857 $ & $ i$\\
$ 55248.12732 $ & $  -0.00045 $ & $   0.00084 $ & $   9.00505 $ & $ i$\\
$ 55248.12767 $ & $  -0.00270 $ & $   0.00084 $ & $   9.00217 $ & $ i$\\
$ 55248.12803 $ & $  -0.00921 $ & $   0.00084 $ & $   8.99654 $ & $ i$\\
$ 55248.12841 $ & $  -0.00911 $ & $   0.00084 $ & $   8.99611 $ & $ i$\\
$ 55248.12914 $ & $  -0.00699 $ & $   0.00084 $ & $   8.99835 $ & $ i$\\


==> HTR183-008_phfu_tab_short.tex <==
$ 54942.76369 $ & $   0.01133 $ & $   0.00088 $ & $  10.43700 $ & $ i$\\
$ 54942.76432 $ & $   0.01370 $ & $   0.00088 $ & $  10.43950 $ & $ i$\\
$ 54942.76495 $ & $   0.00989 $ & $   0.00088 $ & $  10.43550 $ & $ i$\\
$ 54942.76574 $ & $   0.00891 $ & $   0.00088 $ & $  10.43490 $ & $ i$\\
$ 54942.76637 $ & $   0.00974 $ & $   0.00088 $ & $  10.43570 $ & $ i$\\
$ 54942.76698 $ & $   0.01073 $ & $   0.00088 $ & $  10.43650 $ & $ i$\\
$ 54942.76779 $ & $   0.00961 $ & $   0.00088 $ & $  10.43480 $ & $ i$\\
$ 54942.76839 $ & $   0.00938 $ & $   0.00088 $ & $  10.43450 $ & $ i$\\
$ 54942.76902 $ & $   0.01249 $ & $   0.00088 $ & $  10.43800 $ & $ i$\\
$ 54942.76980 $ & $   0.01011 $ & $   0.00088 $ & $  10.43520 $ & $ i$\\


==> HTR183-008_rvtable.tex <==
$ 954.91548 $ \dotfill & \nodata      & \nodata      & $     3.67 $ & $     5.10 $ & $     0.819 $ & $     0.002 $\\
$ 954.92307 $ \dotfill & $   221.51 $ & $     2.88 $ & $    -9.60 $ & $    13.62 $ & $     0.829 $ & $     0.003 $\\
$ 955.86532 $ \dotfill & $  -274.01 $ & $     2.48 $ & $    -8.08 $ & $     5.81 $ & $     0.823 $ & $     0.003 $\\
$ 955.98849 $ \dotfill & $  -314.29 $ & $     2.76 $ & $     7.51 $ & $    12.62 $ & $     0.855 $ & $     0.005 $\\
$ 957.00006 $ \dotfill & $  -378.18 $ & $     3.00 $ & $     2.88 $ & $     8.36 $ & $     0.866 $ & $     0.009 $\\
$ 963.95573 $ \dotfill & $  -197.70 $ & $     2.68 $ & $   -12.46 $ & $     5.48 $ & $     0.789 $ & $     0.003 $\\
$ 983.85638 $ \dotfill & $   212.70 $ & $     2.72 $ & $    -4.61 $ & $     3.33 $ & $     0.815 $ & $     0.003 $\\
$ 985.87988 $ \dotfill & $  -406.23 $ & $     2.46 $ & $     5.88 $ & $     4.95 $ & $     0.809 $ & $     0.003 $\\
$ 986.85645 $ \dotfill & $   509.76 $ & $     3.01 $ & $    -0.70 $ & $     7.24 $ & $     0.803 $ & $     0.005 $\\
$ 987.86480 $ \dotfill & $   270.66 $ & $     2.92 $ & $    -6.96 $ & $     4.20 $ & $     0.810 $ & $     0.004 $\\
$ 1174.14589 $ \dotfill & $  -145.85 $ & $     3.13 $ & $     0.01 $ & $     6.54 $ & $     0.833 $ & $     0.005 $\\
$ 1191.14119 $ \dotfill & $  -391.67 $ & $     2.75 $ & $     5.76 $ & $     5.16 $ & $     0.832 $ & $     0.005 $\\
$ 1192.12302 $ \dotfill & $  -457.57 $ & $     2.67 $ & $     7.04 $ & $     3.15 $ & $     0.809 $ & $     0.005 $\\
$ 1193.11001 $ \dotfill & $   496.07 $ & $     2.58 $ & $     2.50 $ & $     3.85 $ & $     0.794 $ & $     0.005 $\\
$ 1197.15057 $ \dotfill & $   459.61 $ & $     2.59 $ & $     9.69 $ & $     4.91 $ & $     0.777 $ & $     0.005 $\\
$ 1229.12322 $ \dotfill & $  -469.62 $ & $     2.81 $ & $    -2.53 $ & $     5.81 $ & $     0.821 $ & $     0.005 $\\


==> HTR267-010_phfu_tab.tex <==
$ 54902.59749 $ & $  -0.00169 $ & $   0.00075 $ & $  10.66286 $ & $ i$\\
$ 54902.59799 $ & $  -0.00139 $ & $   0.00075 $ & $  10.66200 $ & $ i$\\
$ 54902.59848 $ & $  -0.00469 $ & $   0.00075 $ & $  10.65893 $ & $ i$\\
$ 54902.59919 $ & $   0.00281 $ & $   0.00075 $ & $  10.66596 $ & $ i$\\
$ 54902.59970 $ & $  -0.00108 $ & $   0.00075 $ & $  10.66316 $ & $ i$\\
$ 54902.60020 $ & $   0.00141 $ & $   0.00075 $ & $  10.66524 $ & $ i$\\
$ 54902.60089 $ & $   0.00440 $ & $   0.00075 $ & $  10.66726 $ & $ i$\\
$ 54902.60139 $ & $   0.00040 $ & $   0.00075 $ & $  10.66424 $ & $ i$\\
$ 54902.60190 $ & $  -0.00064 $ & $   0.00075 $ & $  10.66234 $ & $ i$\\
$ 54902.60259 $ & $  -0.00009 $ & $   0.00075 $ & $  10.66388 $ & $ i$\\
$ 54902.60308 $ & $   0.00162 $ & $   0.00075 $ & $  10.66686 $ & $ i$\\
$ 54902.60359 $ & $  -0.00219 $ & $   0.00075 $ & $  10.66179 $ & $ i$\\
$ 54902.60426 $ & $  -0.00406 $ & $   0.00075 $ & $  10.66086 $ & $ i$\\
$ 54902.60476 $ & $   0.00169 $ & $   0.00075 $ & $  10.66507 $ & $ i$\\
$ 54902.60528 $ & $   0.00084 $ & $   0.00075 $ & $  10.66538 $ & $ i$\\
$ 54902.60597 $ & $  -0.00012 $ & $   0.00075 $ & $  10.66267 $ & $ i$\\
$ 54902.60648 $ & $   0.00136 $ & $   0.00075 $ & $  10.66555 $ & $ i$\\
$ 54902.60698 $ & $   0.00025 $ & $   0.00075 $ & $  10.66371 $ & $ i$\\
$ 54902.60768 $ & $  -0.00051 $ & $   0.00075 $ & $  10.66283 $ & $ i$\\
$ 54902.60818 $ & $  -0.00234 $ & $   0.00075 $ & $  10.66172 $ & $ i$\\
$ 54902.60869 $ & $   0.00054 $ & $   0.00075 $ & $  10.66438 $ & $ i$\\
$ 54902.60937 $ & $   0.00028 $ & $   0.00075 $ & $  10.66354 $ & $ i$\\
$ 54902.60988 $ & $   0.00236 $ & $   0.00075 $ & $  10.66471 $ & $ i$\\
$ 54902.61040 $ & $  -0.00247 $ & $   0.00075 $ & $  10.66124 $ & $ i$\\
$ 54902.61111 $ & $   0.00265 $ & $   0.00075 $ & $  10.66592 $ & $ i$\\
$ 54902.61161 $ & $  -0.00160 $ & $   0.00075 $ & $  10.66317 $ & $ i$\\
$ 54902.61211 $ & $  -0.00032 $ & $   0.00075 $ & $  10.66251 $ & $ i$\\
$ 54902.61279 $ & $   0.00135 $ & $   0.00075 $ & $  10.66455 $ & $ i$\\
$ 54902.61329 $ & $  -0.00082 $ & $   0.00075 $ & $  10.66183 $ & $ i$\\
$ 54902.61377 $ & $   0.00102 $ & $   0.00075 $ & $  10.66651 $ & $ i$\\
$ 54902.61449 $ & $  -0.00021 $ & $   0.00075 $ & $  10.66509 $ & $ i$\\
$ 54902.61498 $ & $  -0.00102 $ & $   0.00075 $ & $  10.66354 $ & $ i$\\
$ 54902.61547 $ & $   0.00066 $ & $   0.00075 $ & $  10.66554 $ & $ i$\\
$ 54902.61618 $ & $   0.00055 $ & $   0.00075 $ & $  10.66482 $ & $ i$\\
$ 54902.61667 $ & $  -0.00261 $ & $   0.00075 $ & $  10.66304 $ & $ i$\\
$ 54902.61717 $ & $   0.00044 $ & $   0.00075 $ & $  10.66498 $ & $ i$\\
$ 54902.61788 $ & $   0.00335 $ & $   0.00076 $ & $  10.66788 $ & $ i$\\
$ 54902.61838 $ & $  -0.00206 $ & $   0.00075 $ & $  10.66232 $ & $ i$\\
$ 54902.61890 $ & $  -0.00296 $ & $   0.00075 $ & $  10.66144 $ & $ i$\\
$ 54902.61958 $ & $  -0.00174 $ & $   0.00075 $ & $  10.66211 $ & $ i$\\
$ 54902.62009 $ & $   0.00117 $ & $   0.00075 $ & $  10.66518 $ & $ i$\\
$ 54902.62060 $ & $  -0.00013 $ & $   0.00075 $ & $  10.66509 $ & $ i$\\
$ 54902.62128 $ & $   0.00235 $ & $   0.00075 $ & $  10.66706 $ & $ i$\\
$ 54902.62178 $ & $   0.00123 $ & $   0.00075 $ & $  10.66551 $ & $ i$\\
$ 54902.62230 $ & $   0.00395 $ & $   0.00076 $ & $  10.66890 $ & $ i$\\
$ 54902.62300 $ & $   0.00338 $ & $   0.00075 $ & $  10.66686 $ & $ i$\\
$ 54902.62349 $ & $   0.00255 $ & $   0.00075 $ & $  10.66766 $ & $ i$\\
$ 54902.62400 $ & $   0.00446 $ & $   0.00075 $ & $  10.66818 $ & $ i$\\
$ 54902.62473 $ & $   0.00655 $ & $   0.00076 $ & $  10.67072 $ & $ i$\\
$ 54902.62523 $ & $   0.00701 $ & $   0.00076 $ & $  10.67046 $ & $ i$\\
$ 54902.62612 $ & $   0.00991 $ & $   0.00076 $ & $  10.67372 $ & $ i$\\
$ 54902.62661 $ & $   0.00754 $ & $   0.00075 $ & $  10.67230 $ & $ i$\\
$ 54902.62710 $ & $   0.00878 $ & $   0.00076 $ & $  10.67385 $ & $ i$\\
$ 54902.62779 $ & $   0.01020 $ & $   0.00076 $ & $  10.67484 $ & $ i$\\
$ 54902.62830 $ & $   0.00981 $ & $   0.00076 $ & $  10.67341 $ & $ i$\\
$ 54902.62881 $ & $   0.01215 $ & $   0.00076 $ & $  10.67621 $ & $ i$\\
$ 54902.62950 $ & $   0.01235 $ & $   0.00076 $ & $  10.67619 $ & $ i$\\
$ 54902.62999 $ & $   0.01513 $ & $   0.00076 $ & $  10.67921 $ & $ i$\\
$ 54902.63048 $ & $   0.01517 $ & $   0.00076 $ & $  10.67865 $ & $ i$\\
$ 54902.63119 $ & $   0.01364 $ & $   0.00076 $ & $  10.67775 $ & $ i$\\
$ 54902.63170 $ & $   0.01545 $ & $   0.00076 $ & $  10.67862 $ & $ i$\\
$ 54902.63220 $ & $   0.01631 $ & $   0.00076 $ & $  10.68097 $ & $ i$\\
$ 54902.63288 $ & $   0.01725 $ & $   0.00076 $ & $  10.67986 $ & $ i$\\
$ 54902.63339 $ & $   0.01514 $ & $   0.00076 $ & $  10.67910 $ & $ i$\\
$ 54902.63389 $ & $   0.01590 $ & $   0.00076 $ & $  10.67835 $ & $ i$\\
$ 54902.63457 $ & $   0.01587 $ & $   0.00076 $ & $  10.68062 $ & $ i$\\
$ 54902.63507 $ & $   0.01562 $ & $   0.00076 $ & $  10.67949 $ & $ i$\\
$ 54902.63559 $ & $   0.01961 $ & $   0.00076 $ & $  10.68451 $ & $ i$\\
$ 54902.63628 $ & $   0.01842 $ & $   0.00076 $ & $  10.68222 $ & $ i$\\
$ 54902.63678 $ & $   0.01757 $ & $   0.00076 $ & $  10.68223 $ & $ i$\\
$ 54902.63729 $ & $   0.01560 $ & $   0.00076 $ & $  10.67951 $ & $ i$\\
$ 54902.63798 $ & $   0.01787 $ & $   0.00076 $ & $  10.68155 $ & $ i$\\
$ 54902.63848 $ & $   0.01822 $ & $   0.00076 $ & $  10.68187 $ & $ i$\\
$ 54902.63899 $ & $   0.01882 $ & $   0.00076 $ & $  10.68345 $ & $ i$\\
$ 54902.63973 $ & $   0.01952 $ & $   0.00076 $ & $  10.68372 $ & $ i$\\
$ 54902.64022 $ & $   0.01749 $ & $   0.00076 $ & $  10.68134 $ & $ i$\\
$ 54902.64073 $ & $   0.01963 $ & $   0.00076 $ & $  10.68368 $ & $ i$\\
$ 54902.64144 $ & $   0.01896 $ & $   0.00076 $ & $  10.68236 $ & $ i$\\
$ 54902.64195 $ & $   0.01863 $ & $   0.00076 $ & $  10.68293 $ & $ i$\\
$ 54902.64245 $ & $   0.02085 $ & $   0.00076 $ & $  10.68483 $ & $ i$\\
$ 54902.64316 $ & $   0.01804 $ & $   0.00076 $ & $  10.68227 $ & $ i$\\
$ 54902.64365 $ & $   0.01737 $ & $   0.00076 $ & $  10.68168 $ & $ i$\\
$ 54902.64414 $ & $   0.01861 $ & $   0.00076 $ & $  10.68240 $ & $ i$\\
$ 54902.64482 $ & $   0.01852 $ & $   0.00076 $ & $  10.68289 $ & $ i$\\
$ 54902.64532 $ & $   0.02016 $ & $   0.00076 $ & $  10.68454 $ & $ i$\\
$ 54902.64583 $ & $   0.02106 $ & $   0.00076 $ & $  10.68480 $ & $ i$\\
$ 54902.64652 $ & $   0.01863 $ & $   0.00076 $ & $  10.68272 $ & $ i$\\
$ 54902.64702 $ & $   0.01856 $ & $   0.00076 $ & $  10.68234 $ & $ i$\\
$ 54902.64751 $ & $   0.02027 $ & $   0.00076 $ & $  10.68556 $ & $ i$\\
$ 54902.64820 $ & $   0.01996 $ & $   0.00076 $ & $  10.68376 $ & $ i$\\
$ 54902.64870 $ & $   0.02099 $ & $   0.00076 $ & $  10.68470 $ & $ i$\\
$ 54902.64921 $ & $   0.01846 $ & $   0.00076 $ & $  10.68299 $ & $ i$\\
$ 54902.64988 $ & $   0.02139 $ & $   0.00076 $ & $  10.68482 $ & $ i$\\
$ 54902.65039 $ & $   0.01722 $ & $   0.00076 $ & $  10.68207 $ & $ i$\\
$ 54902.65090 $ & $   0.01991 $ & $   0.00076 $ & $  10.68387 $ & $ i$\\
$ 54902.65158 $ & $   0.02086 $ & $   0.00077 $ & $  10.68511 $ & $ i$\\
$ 54902.65208 $ & $   0.01952 $ & $   0.00076 $ & $  10.68408 $ & $ i$\\
$ 54902.65259 $ & $   0.01891 $ & $   0.00076 $ & $  10.68326 $ & $ i$\\
$ 54902.65331 $ & $   0.02143 $ & $   0.00077 $ & $  10.68539 $ & $ i$\\
$ 54902.65380 $ & $   0.01914 $ & $   0.00076 $ & $  10.68131 $ & $ i$\\
$ 54902.65431 $ & $   0.02052 $ & $   0.00076 $ & $  10.68365 $ & $ i$\\
$ 54902.65482 $ & $   0.01673 $ & $   0.00076 $ & $  10.68264 $ & $ i$\\
$ 54902.65533 $ & $   0.02113 $ & $   0.00077 $ & $  10.68524 $ & $ i$\\
$ 54902.65602 $ & $   0.01869 $ & $   0.00076 $ & $  10.68379 $ & $ i$\\
$ 54902.65652 $ & $   0.01753 $ & $   0.00076 $ & $  10.68033 $ & $ i$\\
$ 54902.65704 $ & $   0.02060 $ & $   0.00076 $ & $  10.68415 $ & $ i$\\
$ 54902.65773 $ & $   0.02068 $ & $   0.00077 $ & $  10.68478 $ & $ i$\\
$ 54902.65824 $ & $   0.02160 $ & $   0.00077 $ & $  10.68611 $ & $ i$\\
$ 54902.65874 $ & $   0.02046 $ & $   0.00077 $ & $  10.68472 $ & $ i$\\
$ 54902.65943 $ & $   0.02072 $ & $   0.00077 $ & $  10.68576 $ & $ i$\\
$ 54902.65994 $ & $   0.02065 $ & $   0.00077 $ & $  10.68463 $ & $ i$\\
$ 54902.66043 $ & $   0.02160 $ & $   0.00077 $ & $  10.68609 $ & $ i$\\
$ 54902.66112 $ & $   0.01985 $ & $   0.00077 $ & $  10.68347 $ & $ i$\\
$ 54902.66163 $ & $   0.01873 $ & $   0.00076 $ & $  10.68292 $ & $ i$\\
$ 54902.66214 $ & $   0.01788 $ & $   0.00077 $ & $  10.68216 $ & $ i$\\
$ 54902.66283 $ & $   0.01749 $ & $   0.00077 $ & $  10.68165 $ & $ i$\\
$ 54902.66334 $ & $   0.01911 $ & $   0.00077 $ & $  10.68419 $ & $ i$\\
$ 54902.66384 $ & $   0.01874 $ & $   0.00077 $ & $  10.68411 $ & $ i$\\
$ 54902.66453 $ & $   0.01982 $ & $   0.00077 $ & $  10.68471 $ & $ i$\\
$ 54902.66503 $ & $   0.02202 $ & $   0.00077 $ & $  10.68643 $ & $ i$\\
$ 54902.66554 $ & $   0.01656 $ & $   0.00077 $ & $  10.68092 $ & $ i$\\
$ 54902.66623 $ & $   0.01870 $ & $   0.00077 $ & $  10.68368 $ & $ i$\\
$ 54902.66674 $ & $   0.02041 $ & $   0.00077 $ & $  10.68567 $ & $ i$\\
$ 54902.66724 $ & $   0.01992 $ & $   0.00077 $ & $  10.68354 $ & $ i$\\
$ 54902.66797 $ & $   0.01742 $ & $   0.00077 $ & $  10.68201 $ & $ i$\\
$ 54902.66845 $ & $   0.01682 $ & $   0.00077 $ & $  10.68155 $ & $ i$\\
$ 54902.66896 $ & $   0.01771 $ & $   0.00077 $ & $  10.68211 $ & $ i$\\
$ 54902.66966 $ & $   0.01790 $ & $   0.00077 $ & $  10.68118 $ & $ i$\\
$ 54902.67014 $ & $   0.01755 $ & $   0.00077 $ & $  10.68166 $ & $ i$\\
$ 54902.67064 $ & $   0.01758 $ & $   0.00077 $ & $  10.68190 $ & $ i$\\
$ 54902.67131 $ & $   0.01790 $ & $   0.00077 $ & $  10.68214 $ & $ i$\\
$ 54902.67182 $ & $   0.01880 $ & $   0.00077 $ & $  10.68291 $ & $ i$\\
$ 54902.67232 $ & $   0.01469 $ & $   0.00076 $ & $  10.67814 $ & $ i$\\
$ 54902.67299 $ & $   0.01682 $ & $   0.00077 $ & $  10.67990 $ & $ i$\\
$ 54902.67348 $ & $   0.01878 $ & $   0.00077 $ & $  10.68306 $ & $ i$\\
$ 54902.67399 $ & $   0.01795 $ & $   0.00077 $ & $  10.68263 $ & $ i$\\
$ 54902.67467 $ & $   0.01721 $ & $   0.00077 $ & $  10.68147 $ & $ i$\\
$ 54902.67518 $ & $   0.01951 $ & $   0.00077 $ & $  10.68427 $ & $ i$\\
$ 54902.67568 $ & $   0.02068 $ & $   0.00077 $ & $  10.68442 $ & $ i$\\
$ 54902.67636 $ & $   0.01561 $ & $   0.00077 $ & $  10.67995 $ & $ i$\\
$ 54902.67687 $ & $   0.01432 $ & $   0.00077 $ & $  10.67836 $ & $ i$\\
$ 54902.67738 $ & $   0.01430 $ & $   0.00077 $ & $  10.67889 $ & $ i$\\
$ 54902.67806 $ & $   0.01601 $ & $   0.00077 $ & $  10.68131 $ & $ i$\\
$ 54902.67857 $ & $   0.01892 $ & $   0.00077 $ & $  10.68245 $ & $ i$\\
$ 54902.67907 $ & $   0.01697 $ & $   0.00077 $ & $  10.68147 $ & $ i$\\
$ 54902.67974 $ & $   0.01467 $ & $   0.00077 $ & $  10.67887 $ & $ i$\\
$ 54902.68024 $ & $   0.01528 $ & $   0.00077 $ & $  10.67936 $ & $ i$\\
$ 54902.68075 $ & $   0.01610 $ & $   0.00076 $ & $  10.68041 $ & $ i$\\
$ 54902.68147 $ & $   0.01246 $ & $   0.00076 $ & $  10.67514 $ & $ i$\\
$ 54902.68196 $ & $   0.01636 $ & $   0.00077 $ & $  10.68091 $ & $ i$\\
$ 54902.68247 $ & $   0.01304 $ & $   0.00077 $ & $  10.67881 $ & $ i$\\
$ 54902.68297 $ & $   0.01376 $ & $   0.00076 $ & $  10.67802 $ & $ i$\\
$ 54902.68347 $ & $   0.01391 $ & $   0.00076 $ & $  10.67731 $ & $ i$\\
$ 54902.68416 $ & $   0.01301 $ & $   0.00076 $ & $  10.67696 $ & $ i$\\
$ 54902.68466 $ & $   0.01409 $ & $   0.00077 $ & $  10.67618 $ & $ i$\\
$ 54902.68517 $ & $   0.01210 $ & $   0.00077 $ & $  10.67751 $ & $ i$\\
$ 54902.68586 $ & $   0.01064 $ & $   0.00076 $ & $  10.67482 $ & $ i$\\
$ 54902.68637 $ & $   0.01160 $ & $   0.00077 $ & $  10.67539 $ & $ i$\\
$ 54902.68687 $ & $   0.00894 $ & $   0.00076 $ & $  10.67352 $ & $ i$\\
$ 54902.68758 $ & $   0.00615 $ & $   0.00076 $ & $  10.67136 $ & $ i$\\
$ 54902.68808 $ & $   0.00764 $ & $   0.00076 $ & $  10.67312 $ & $ i$\\
$ 54902.68859 $ & $   0.00383 $ & $   0.00076 $ & $  10.66858 $ & $ i$\\
$ 54902.68929 $ & $   0.00767 $ & $   0.00076 $ & $  10.67265 $ & $ i$\\
$ 54902.68980 $ & $   0.00842 $ & $   0.00076 $ & $  10.67308 $ & $ i$\\
$ 54902.69030 $ & $   0.00316 $ & $   0.00076 $ & $  10.66774 $ & $ i$\\
$ 54902.69100 $ & $   0.00169 $ & $   0.00076 $ & $  10.66638 $ & $ i$\\
$ 54902.69150 $ & $   0.00196 $ & $   0.00076 $ & $  10.66688 $ & $ i$\\
$ 54902.69202 $ & $   0.00305 $ & $   0.00076 $ & $  10.66821 $ & $ i$\\
$ 54902.69272 $ & $   0.00352 $ & $   0.00076 $ & $  10.66784 $ & $ i$\\
$ 54902.69322 $ & $   0.00494 $ & $   0.00076 $ & $  10.66957 $ & $ i$\\
$ 54902.69373 $ & $  -0.00270 $ & $   0.00076 $ & $  10.66157 $ & $ i$\\
$ 54902.69441 $ & $  -0.00088 $ & $   0.00076 $ & $  10.66408 $ & $ i$\\
$ 54902.69492 $ & $  -0.00161 $ & $   0.00076 $ & $  10.66405 $ & $ i$\\
$ 54902.69543 $ & $  -0.00178 $ & $   0.00076 $ & $  10.66259 $ & $ i$\\
$ 54902.69615 $ & $  -0.00036 $ & $   0.00076 $ & $  10.66498 $ & $ i$\\
$ 54902.69666 $ & $   0.00085 $ & $   0.00076 $ & $  10.66665 $ & $ i$\\
$ 54902.69716 $ & $   0.00031 $ & $   0.00076 $ & $  10.66516 $ & $ i$\\
$ 54902.69783 $ & $   0.00268 $ & $   0.00076 $ & $  10.66736 $ & $ i$\\
$ 54902.69833 $ & $   0.00302 $ & $   0.00076 $ & $  10.66745 $ & $ i$\\
$ 54902.69886 $ & $  -0.00029 $ & $   0.00076 $ & $  10.66411 $ & $ i$\\
$ 54902.69954 $ & $  -0.00062 $ & $   0.00076 $ & $  10.66409 $ & $ i$\\
$ 54902.70005 $ & $   0.00069 $ & $   0.00076 $ & $  10.66553 $ & $ i$\\
$ 54902.70056 $ & $  -0.00147 $ & $   0.00076 $ & $  10.66407 $ & $ i$\\
$ 54902.70128 $ & $   0.00155 $ & $   0.00076 $ & $  10.66600 $ & $ i$\\
$ 54902.70180 $ & $   0.00054 $ & $   0.00076 $ & $  10.66575 $ & $ i$\\
$ 54902.70231 $ & $   0.00144 $ & $   0.00076 $ & $  10.66733 $ & $ i$\\
$ 54902.70299 $ & $  -0.00061 $ & $   0.00076 $ & $  10.66392 $ & $ i$\\
$ 54902.70349 $ & $  -0.00294 $ & $   0.00076 $ & $  10.66153 $ & $ i$\\
$ 54902.70398 $ & $   0.00119 $ & $   0.00076 $ & $  10.66475 $ & $ i$\\
$ 54902.70468 $ & $   0.00151 $ & $   0.00076 $ & $  10.66653 $ & $ i$\\
$ 54902.70518 $ & $  -0.00079 $ & $   0.00076 $ & $  10.66393 $ & $ i$\\
$ 54902.70569 $ & $  -0.00059 $ & $   0.00076 $ & $  10.66267 $ & $ i$\\
$ 54902.70636 $ & $   0.00066 $ & $   0.00076 $ & $  10.66541 $ & $ i$\\
$ 54902.70685 $ & $   0.00260 $ & $   0.00076 $ & $  10.66714 $ & $ i$\\
$ 54902.70735 $ & $  -0.00203 $ & $   0.00076 $ & $  10.66305 $ & $ i$\\
$ 54902.70805 $ & $  -0.00015 $ & $   0.00076 $ & $  10.66546 $ & $ i$\\
$ 54902.70856 $ & $   0.00023 $ & $   0.00076 $ & $  10.66560 $ & $ i$\\
$ 54902.70906 $ & $   0.00028 $ & $   0.00076 $ & $  10.66575 $ & $ i$\\
$ 54902.70978 $ & $  -0.00062 $ & $   0.00076 $ & $  10.66483 $ & $ i$\\
$ 54902.71028 $ & $   0.00098 $ & $   0.00076 $ & $  10.66568 $ & $ i$\\
$ 54902.71079 $ & $  -0.00153 $ & $   0.00076 $ & $  10.66286 $ & $ i$\\
$ 54902.71130 $ & $   0.00183 $ & $   0.00076 $ & $  10.66645 $ & $ i$\\
$ 54902.71178 $ & $  -0.00260 $ & $   0.00076 $ & $  10.66352 $ & $ i$\\
$ 54902.71248 $ & $  -0.00256 $ & $   0.00076 $ & $  10.66147 $ & $ i$\\
$ 54902.71299 $ & $   0.00018 $ & $   0.00076 $ & $  10.66433 $ & $ i$\\
$ 54902.71349 $ & $   0.00060 $ & $   0.00076 $ & $  10.66594 $ & $ i$\\
$ 54902.71418 $ & $  -0.00070 $ & $   0.00076 $ & $  10.66377 $ & $ i$\\
$ 54902.71468 $ & $  -0.00019 $ & $   0.00076 $ & $  10.66592 $ & $ i$\\
$ 54902.71518 $ & $   0.00268 $ & $   0.00076 $ & $  10.66737 $ & $ i$\\
$ 54902.71587 $ & $  -0.00092 $ & $   0.00076 $ & $  10.66398 $ & $ i$\\
$ 54902.71638 $ & $   0.00163 $ & $   0.00076 $ & $  10.66751 $ & $ i$\\
$ 54902.71689 $ & $   0.00084 $ & $   0.00076 $ & $  10.66449 $ & $ i$\\
$ 54902.71757 $ & $  -0.00111 $ & $   0.00076 $ & $  10.66316 $ & $ i$\\
$ 54902.71807 $ & $  -0.00098 $ & $   0.00076 $ & $  10.66488 $ & $ i$\\
$ 54902.71859 $ & $  -0.00044 $ & $   0.00076 $ & $  10.66425 $ & $ i$\\
$ 54902.71928 $ & $  -0.00022 $ & $   0.00076 $ & $  10.66522 $ & $ i$\\
$ 54902.71978 $ & $   0.00085 $ & $   0.00076 $ & $  10.66543 $ & $ i$\\
$ 54902.72029 $ & $   0.00160 $ & $   0.00076 $ & $  10.66640 $ & $ i$\\
$ 54902.72099 $ & $  -0.00005 $ & $   0.00076 $ & $  10.66454 $ & $ i$\\
$ 54902.72148 $ & $   0.00489 $ & $   0.00076 $ & $  10.67057 $ & $ i$\\
$ 54902.72199 $ & $   0.00196 $ & $   0.00076 $ & $  10.66620 $ & $ i$\\
$ 54902.72269 $ & $   0.00047 $ & $   0.00076 $ & $  10.66569 $ & $ i$\\
$ 54902.72318 $ & $  -0.00138 $ & $   0.00076 $ & $  10.66349 $ & $ i$\\
$ 54902.72370 $ & $  -0.00137 $ & $   0.00076 $ & $  10.66290 $ & $ i$\\
$ 54902.72442 $ & $  -0.00062 $ & $   0.00076 $ & $  10.66387 $ & $ i$\\
$ 54902.72491 $ & $  -0.00206 $ & $   0.00076 $ & $  10.66395 $ & $ i$\\
$ 54902.72541 $ & $  -0.00091 $ & $   0.00076 $ & $  10.66429 $ & $ i$\\
$ 54902.72609 $ & $  -0.00183 $ & $   0.00076 $ & $  10.66278 $ & $ i$\\
$ 54902.72659 $ & $  -0.00117 $ & $   0.00076 $ & $  10.66406 $ & $ i$\\
$ 54902.72711 $ & $   0.00287 $ & $   0.00076 $ & $  10.66717 $ & $ i$\\
$ 54902.72779 $ & $   0.00176 $ & $   0.00076 $ & $  10.66725 $ & $ i$\\
$ 54902.72830 $ & $   0.00253 $ & $   0.00076 $ & $  10.66754 $ & $ i$\\
$ 54902.72879 $ & $  -0.00006 $ & $   0.00076 $ & $  10.66461 $ & $ i$\\
$ 54902.72948 $ & $   0.00066 $ & $   0.00076 $ & $  10.66621 $ & $ i$\\
$ 54902.72999 $ & $   0.00142 $ & $   0.00076 $ & $  10.66717 $ & $ i$\\
$ 54902.73049 $ & $   0.00241 $ & $   0.00076 $ & $  10.66790 $ & $ i$\\
$ 54902.73118 $ & $  -0.00155 $ & $   0.00076 $ & $  10.66344 $ & $ i$\\
$ 54902.73169 $ & $   0.00070 $ & $   0.00076 $ & $  10.66572 $ & $ i$\\
$ 54902.73220 $ & $   0.00383 $ & $   0.00076 $ & $  10.66920 $ & $ i$\\
$ 54902.73289 $ & $   0.00093 $ & $   0.00076 $ & $  10.66658 $ & $ i$\\
$ 54902.73338 $ & $  -0.00001 $ & $   0.00076 $ & $  10.66685 $ & $ i$\\
$ 54902.73388 $ & $   0.00125 $ & $   0.00076 $ & $  10.66548 $ & $ i$\\
$ 54902.73458 $ & $  -0.00057 $ & $   0.00076 $ & $  10.66525 $ & $ i$\\
$ 54902.73507 $ & $  -0.00229 $ & $   0.00076 $ & $  10.66438 $ & $ i$\\
$ 54902.73559 $ & $   0.00273 $ & $   0.00076 $ & $  10.66924 $ & $ i$\\
$ 54902.73678 $ & $  -0.00088 $ & $   0.00076 $ & $  10.66414 $ & $ i$\\
$ 54902.73726 $ & $   0.00051 $ & $   0.00076 $ & $  10.66618 $ & $ i$\\
$ 54902.73796 $ & $  -0.00043 $ & $   0.00076 $ & $  10.66586 $ & $ i$\\
$ 54902.73847 $ & $  -0.00049 $ & $   0.00076 $ & $  10.66473 $ & $ i$\\
$ 54902.73898 $ & $   0.00196 $ & $   0.00077 $ & $  10.66910 $ & $ i$\\
$ 54902.73949 $ & $  -0.00089 $ & $   0.00076 $ & $  10.66593 $ & $ i$\\
$ 54902.74069 $ & $   0.00214 $ & $   0.00077 $ & $  10.66827 $ & $ i$\\
$ 54902.74119 $ & $  -0.00191 $ & $   0.00076 $ & $  10.66337 $ & $ i$\\
$ 54902.74168 $ & $  -0.00068 $ & $   0.00076 $ & $  10.66430 $ & $ i$\\
$ 54902.74238 $ & $  -0.00040 $ & $   0.00076 $ & $  10.66423 $ & $ i$\\
$ 54902.74288 $ & $  -0.00451 $ & $   0.00076 $ & $  10.66081 $ & $ i$\\
$ 54902.74339 $ & $  -0.00083 $ & $   0.00076 $ & $  10.66552 $ & $ i$\\
$ 54902.74410 $ & $  -0.00190 $ & $   0.00076 $ & $  10.66571 $ & $ i$\\
$ 54902.74460 $ & $  -0.00181 $ & $   0.00076 $ & $  10.66314 $ & $ i$\\
$ 54902.74511 $ & $  -0.00330 $ & $   0.00076 $ & $  10.66330 $ & $ i$\\
$ 54902.74580 $ & $   0.00252 $ & $   0.00076 $ & $  10.66790 $ & $ i$\\
$ 54902.74629 $ & $  -0.00171 $ & $   0.00076 $ & $  10.66337 $ & $ i$\\
$ 54902.74680 $ & $  -0.00327 $ & $   0.00076 $ & $  10.66292 $ & $ i$\\
$ 54902.74754 $ & $   0.00178 $ & $   0.00076 $ & $  10.66726 $ & $ i$\\
$ 54902.74805 $ & $  -0.00109 $ & $   0.00076 $ & $  10.66554 $ & $ i$\\
$ 54902.74855 $ & $  -0.00067 $ & $   0.00076 $ & $  10.66514 $ & $ i$\\
$ 54902.74925 $ & $   0.00174 $ & $   0.00076 $ & $  10.66749 $ & $ i$\\
$ 54902.74974 $ & $   0.00417 $ & $   0.00076 $ & $  10.66916 $ & $ i$\\
$ 54902.75026 $ & $   0.00117 $ & $   0.00076 $ & $  10.66695 $ & $ i$\\
$ 54902.75096 $ & $   0.00104 $ & $   0.00076 $ & $  10.66693 $ & $ i$\\
$ 54902.75145 $ & $  -0.00125 $ & $   0.00076 $ & $  10.66507 $ & $ i$\\
$ 54902.75195 $ & $  -0.00044 $ & $   0.00076 $ & $  10.66553 $ & $ i$\\
$ 54902.75270 $ & $  -0.00430 $ & $   0.00076 $ & $  10.66019 $ & $ i$\\
$ 54902.75318 $ & $  -0.00289 $ & $   0.00076 $ & $  10.66335 $ & $ i$\\
$ 54902.75370 $ & $  -0.00036 $ & $   0.00076 $ & $  10.66578 $ & $ i$\\
$ 54902.75440 $ & $  -0.00201 $ & $   0.00076 $ & $  10.66350 $ & $ i$\\
$ 54902.75488 $ & $   0.00008 $ & $   0.00076 $ & $  10.66581 $ & $ i$\\
$ 54902.75538 $ & $  -0.00007 $ & $   0.00077 $ & $  10.66674 $ & $ i$\\
$ 54902.75609 $ & $   0.00079 $ & $   0.00076 $ & $  10.66795 $ & $ i$\\
$ 54902.75658 $ & $  -0.00264 $ & $   0.00076 $ & $  10.66222 $ & $ i$\\
$ 54902.75709 $ & $   0.00254 $ & $   0.00076 $ & $  10.67065 $ & $ i$\\
$ 54902.75779 $ & $   0.00258 $ & $   0.00076 $ & $  10.66885 $ & $ i$\\
$ 54902.75828 $ & $   0.00235 $ & $   0.00076 $ & $  10.66955 $ & $ i$\\
$ 54902.75878 $ & $   0.00060 $ & $   0.00077 $ & $  10.66688 $ & $ i$\\
$ 54902.75948 $ & $   0.00193 $ & $   0.00076 $ & $  10.66779 $ & $ i$\\
$ 54902.75997 $ & $  -0.00151 $ & $   0.00076 $ & $  10.66449 $ & $ i$\\
$ 54902.76048 $ & $   0.00183 $ & $   0.00076 $ & $  10.66832 $ & $ i$\\
$ 54902.76117 $ & $  -0.00409 $ & $   0.00076 $ & $  10.66173 $ & $ i$\\
$ 54902.76166 $ & $  -0.00023 $ & $   0.00076 $ & $  10.66520 $ & $ i$\\
$ 54902.76216 $ & $  -0.00063 $ & $   0.00076 $ & $  10.66570 $ & $ i$\\
$ 54902.76286 $ & $   0.00067 $ & $   0.00077 $ & $  10.66782 $ & $ i$\\
$ 54902.76335 $ & $  -0.00225 $ & $   0.00077 $ & $  10.66428 $ & $ i$\\
$ 54902.76386 $ & $  -0.00194 $ & $   0.00077 $ & $  10.66420 $ & $ i$\\
$ 54902.76506 $ & $  -0.00226 $ & $   0.00077 $ & $  10.66477 $ & $ i$\\
$ 54902.76555 $ & $   0.00129 $ & $   0.00077 $ & $  10.66968 $ & $ i$\\
$ 54902.76883 $ & $  -0.00088 $ & $   0.00076 $ & $  10.66570 $ & $ i$\\
$ 54902.76934 $ & $   0.00012 $ & $   0.00076 $ & $  10.66568 $ & $ i$\\
$ 54902.76985 $ & $  -0.00102 $ & $   0.00076 $ & $  10.66653 $ & $ i$\\
$ 54902.77054 $ & $  -0.00211 $ & $   0.00076 $ & $  10.66621 $ & $ i$\\
$ 54902.77104 $ & $  -0.00002 $ & $   0.00077 $ & $  10.66780 $ & $ i$\\
$ 54902.77154 $ & $  -0.00164 $ & $   0.00077 $ & $  10.66702 $ & $ i$\\
$ 54902.77223 $ & $   0.00286 $ & $   0.00077 $ & $  10.66884 $ & $ i$\\
$ 54902.77274 $ & $  -0.00442 $ & $   0.00076 $ & $  10.66060 $ & $ i$\\
$ 54902.77325 $ & $  -0.00170 $ & $   0.00076 $ & $  10.66590 $ & $ i$\\
$ 54902.77393 $ & $  -0.00269 $ & $   0.00076 $ & $  10.66694 $ & $ i$\\
$ 54902.77444 $ & $   0.00391 $ & $   0.00077 $ & $  10.67059 $ & $ i$\\
$ 54902.77495 $ & $   0.00126 $ & $   0.00077 $ & $  10.66892 $ & $ i$\\
$ 54902.77563 $ & $  -0.00055 $ & $   0.00078 $ & $  10.67207 $ & $ i$\\
$ 54902.77614 $ & $   0.00067 $ & $   0.00077 $ & $  10.67025 $ & $ i$\\
$ 54902.77666 $ & $   0.00027 $ & $   0.00076 $ & $  10.66750 $ & $ i$\\
$ 54902.77735 $ & $   0.00393 $ & $   0.00077 $ & $  10.67120 $ & $ i$\\
$ 54902.77786 $ & $  -0.00195 $ & $   0.00076 $ & $  10.66446 $ & $ i$\\
$ 54902.77835 $ & $  -0.00412 $ & $   0.00076 $ & $  10.66188 $ & $ i$\\
$ 54902.77905 $ & $   0.00009 $ & $   0.00076 $ & $  10.66641 $ & $ i$\\
$ 54902.77957 $ & $  -0.00197 $ & $   0.00076 $ & $  10.66492 $ & $ i$\\
$ 54902.78005 $ & $   0.00089 $ & $   0.00077 $ & $  10.66934 $ & $ i$\\
$ 54902.78077 $ & $   0.00070 $ & $   0.00077 $ & $  10.67148 $ & $ i$\\
$ 54902.78175 $ & $   0.00302 $ & $   0.00078 $ & $  10.67402 $ & $ i$\\
$ 54902.78298 $ & $  -0.00160 $ & $   0.00077 $ & $  10.66709 $ & $ i$\\
$ 54902.78348 $ & $   0.00128 $ & $   0.00076 $ & $  10.66896 $ & $ i$\\
$ 54902.78417 $ & $   0.00252 $ & $   0.00077 $ & $  10.67378 $ & $ i$\\
$ 54902.78519 $ & $   0.00262 $ & $   0.00076 $ & $  10.66982 $ & $ i$\\
$ 54902.78588 $ & $   0.00347 $ & $   0.00077 $ & $  10.67108 $ & $ i$\\
$ 54902.78637 $ & $  -0.00267 $ & $   0.00077 $ & $  10.66531 $ & $ i$\\
$ 54902.78686 $ & $  -0.00101 $ & $   0.00077 $ & $  10.66889 $ & $ i$\\
$ 54902.78753 $ & $   0.00180 $ & $   0.00076 $ & $  10.67074 $ & $ i$\\
$ 54902.78803 $ & $   0.00262 $ & $   0.00077 $ & $  10.66905 $ & $ i$\\
$ 54902.78854 $ & $  -0.00129 $ & $   0.00078 $ & $  10.66724 $ & $ i$\\
$ 54902.78923 $ & $   0.00186 $ & $   0.00077 $ & $  10.67325 $ & $ i$\\
$ 54902.78974 $ & $   0.00317 $ & $   0.00077 $ & $  10.67234 $ & $ i$\\
$ 54902.79025 $ & $   0.00117 $ & $   0.00076 $ & $  10.66779 $ & $ i$\\
$ 54902.79094 $ & $   0.00178 $ & $   0.00076 $ & $  10.66812 $ & $ i$\\
$ 54902.79144 $ & $  -0.00103 $ & $   0.00076 $ & $  10.66607 $ & $ i$\\
$ 54902.79194 $ & $  -0.00361 $ & $   0.00076 $ & $  10.66295 $ & $ i$\\
$ 54902.79262 $ & $  -0.00298 $ & $   0.00076 $ & $  10.66657 $ & $ i$\\
$ 54902.79313 $ & $  -0.00205 $ & $   0.00077 $ & $  10.66427 $ & $ i$\\
$ 54902.79364 $ & $  -0.00235 $ & $   0.00076 $ & $  10.66405 $ & $ i$\\
$ 54902.79433 $ & $   0.00256 $ & $   0.00078 $ & $  10.67414 $ & $ i$\\
$ 54902.79483 $ & $   0.00271 $ & $   0.00077 $ & $  10.67171 $ & $ i$\\
$ 54902.79535 $ & $  -0.00163 $ & $   0.00077 $ & $  10.66523 $ & $ i$\\
$ 54902.79607 $ & $  -0.00294 $ & $   0.00076 $ & $  10.66278 $ & $ i$\\
$ 54902.79658 $ & $  -0.00074 $ & $   0.00076 $ & $  10.66616 $ & $ i$\\
$ 54902.79708 $ & $  -0.00152 $ & $   0.00076 $ & $  10.66478 $ & $ i$\\
$ 54902.79759 $ & $  -0.00375 $ & $   0.00076 $ & $  10.66332 $ & $ i$\\
$ 54902.79878 $ & $  -0.00237 $ & $   0.00076 $ & $  10.66510 $ & $ i$\\
$ 54902.79929 $ & $   0.00186 $ & $   0.00077 $ & $  10.67062 $ & $ i$\\
$ 54902.79979 $ & $  -0.00086 $ & $   0.00076 $ & $  10.66534 $ & $ i$\\
$ 54902.80047 $ & $  -0.00145 $ & $   0.00076 $ & $  10.66686 $ & $ i$\\
$ 54902.80097 $ & $   0.00094 $ & $   0.00076 $ & $  10.66893 $ & $ i$\\
$ 54902.80149 $ & $  -0.00054 $ & $   0.00076 $ & $  10.66807 $ & $ i$\\
$ 54902.80218 $ & $   0.00392 $ & $   0.00076 $ & $  10.67118 $ & $ i$\\
$ 54902.80268 $ & $   0.00090 $ & $   0.00077 $ & $  10.66848 $ & $ i$\\
$ 54902.80315 $ & $   0.00355 $ & $   0.00077 $ & $  10.67292 $ & $ i$\\
$ 54902.80385 $ & $   0.00295 $ & $   0.00077 $ & $  10.67070 $ & $ i$\\
$ 54902.80435 $ & $  -0.00114 $ & $   0.00076 $ & $  10.66496 $ & $ i$\\
$ 54902.80484 $ & $   0.00332 $ & $   0.00077 $ & $  10.67356 $ & $ i$\\
$ 54902.80554 $ & $  -0.00410 $ & $   0.00076 $ & $  10.66255 $ & $ i$\\
$ 54902.80605 $ & $  -0.00195 $ & $   0.00076 $ & $  10.66422 $ & $ i$\\
$ 54902.80656 $ & $  -0.00044 $ & $   0.00076 $ & $  10.66442 $ & $ i$\\
$ 54902.80725 $ & $   0.00250 $ & $   0.00076 $ & $  10.66922 $ & $ i$\\
$ 54902.80776 $ & $   0.00052 $ & $   0.00076 $ & $  10.66690 $ & $ i$\\
$ 54902.80827 $ & $  -0.00261 $ & $   0.00076 $ & $  10.66501 $ & $ i$\\
$ 54902.80895 $ & $  -0.00145 $ & $   0.00076 $ & $  10.66804 $ & $ i$\\
$ 54902.80946 $ & $  -0.00078 $ & $   0.00076 $ & $  10.66650 $ & $ i$\\
$ 54902.80997 $ & $   0.00244 $ & $   0.00077 $ & $  10.67058 $ & $ i$\\
$ 54902.81068 $ & $   0.00275 $ & $   0.00077 $ & $  10.67002 $ & $ i$\\
$ 54902.81119 $ & $   0.00130 $ & $   0.00077 $ & $  10.67095 $ & $ i$\\
$ 54902.81169 $ & $  -0.00042 $ & $   0.00077 $ & $  10.66652 $ & $ i$\\
$ 54902.81240 $ & $  -0.00004 $ & $   0.00076 $ & $  10.66798 $ & $ i$\\
$ 54902.81290 $ & $   0.00191 $ & $   0.00076 $ & $  10.66839 $ & $ i$\\
$ 54902.81340 $ & $  -0.00015 $ & $   0.00076 $ & $  10.66670 $ & $ i$\\
$ 54902.81408 $ & $  -0.00032 $ & $   0.00076 $ & $  10.66664 $ & $ i$\\
$ 54902.81459 $ & $  -0.00302 $ & $   0.00076 $ & $  10.66427 $ & $ i$\\
$ 54902.81508 $ & $   0.00374 $ & $   0.00077 $ & $  10.66809 $ & $ i$\\
$ 54902.81629 $ & $   0.00354 $ & $   0.00078 $ & $  10.67380 $ & $ i$\\
$ 54902.81681 $ & $  -0.00004 $ & $   0.00076 $ & $  10.66700 $ & $ i$\\
$ 54902.81749 $ & $  -0.00131 $ & $   0.00077 $ & $  10.66665 $ & $ i$\\
$ 54902.81851 $ & $   0.00181 $ & $   0.00077 $ & $  10.67261 $ & $ i$\\
$ 54902.81921 $ & $   0.00136 $ & $   0.00077 $ & $  10.66921 $ & $ i$\\
$ 54902.81969 $ & $  -0.00422 $ & $   0.00076 $ & $  10.66246 $ & $ i$\\
$ 54902.82020 $ & $  -0.00248 $ & $   0.00076 $ & $  10.66451 $ & $ i$\\
$ 54902.82088 $ & $   0.00146 $ & $   0.00077 $ & $  10.67044 $ & $ i$\\
$ 54902.82138 $ & $   0.00084 $ & $   0.00078 $ & $  10.67143 $ & $ i$\\
$ 54902.82189 $ & $  -0.00059 $ & $   0.00076 $ & $  10.66604 $ & $ i$\\
$ 54902.82258 $ & $  -0.00014 $ & $   0.00076 $ & $  10.66568 $ & $ i$\\
$ 54902.82359 $ & $  -0.00186 $ & $   0.00076 $ & $  10.66605 $ & $ i$\\
$ 54902.82429 $ & $  -0.00018 $ & $   0.00076 $ & $  10.66536 $ & $ i$\\
$ 54902.82478 $ & $   0.00215 $ & $   0.00076 $ & $  10.66892 $ & $ i$\\
$ 54902.82530 $ & $   0.00129 $ & $   0.00076 $ & $  10.66867 $ & $ i$\\
$ 54902.82581 $ & $  -0.00204 $ & $   0.00076 $ & $  10.66621 $ & $ i$\\
$ 54902.82631 $ & $   0.00022 $ & $   0.00076 $ & $  10.66615 $ & $ i$\\
$ 54902.82699 $ & $  -0.00274 $ & $   0.00076 $ & $  10.66345 $ & $ i$\\
$ 54902.82750 $ & $  -0.00377 $ & $   0.00076 $ & $  10.66506 $ & $ i$\\
$ 54902.82800 $ & $  -0.00048 $ & $   0.00076 $ & $  10.66585 $ & $ i$\\
$ 54902.82918 $ & $   0.00279 $ & $   0.00076 $ & $  10.67005 $ & $ i$\\
$ 54902.82969 $ & $  -0.00099 $ & $   0.00076 $ & $  10.66592 $ & $ i$\\
$ 54902.83040 $ & $  -0.00113 $ & $   0.00076 $ & $  10.66682 $ & $ i$\\
$ 54902.83091 $ & $   0.00292 $ & $   0.00077 $ & $  10.67017 $ & $ i$\\
$ 54902.83140 $ & $   0.00403 $ & $   0.00077 $ & $  10.67133 $ & $ i$\\
$ 54902.83207 $ & $  -0.00294 $ & $   0.00076 $ & $  10.66544 $ & $ i$\\
$ 54902.83258 $ & $  -0.00067 $ & $   0.00076 $ & $  10.66832 $ & $ i$\\
$ 54902.83379 $ & $   0.00032 $ & $   0.00076 $ & $  10.66738 $ & $ i$\\
$ 54902.83429 $ & $   0.00212 $ & $   0.00076 $ & $  10.67004 $ & $ i$\\
$ 54902.83481 $ & $  -0.00210 $ & $   0.00076 $ & $  10.66460 $ & $ i$\\
$ 54902.83550 $ & $   0.00296 $ & $   0.00076 $ & $  10.66871 $ & $ i$\\
$ 54902.83600 $ & $  -0.00071 $ & $   0.00077 $ & $  10.66959 $ & $ i$\\
$ 55126.87477 $ & $  -0.00306 $ & $   0.00104 $ & $  10.66010 $ & $ i$\\
$ 55126.87514 $ & $   0.00434 $ & $   0.00104 $ & $  10.66545 $ & $ i$\\
$ 55126.87550 $ & $   0.00210 $ & $   0.00105 $ & $  10.66438 $ & $ i$\\
$ 55126.87606 $ & $  -0.00048 $ & $   0.00105 $ & $  10.66133 $ & $ i$\\
$ 55126.87643 $ & $  -0.00373 $ & $   0.00104 $ & $  10.65839 $ & $ i$\\
$ 55126.87679 $ & $  -0.00146 $ & $   0.00104 $ & $  10.66007 $ & $ i$\\
$ 55126.87733 $ & $   0.00324 $ & $   0.00104 $ & $  10.66629 $ & $ i$\\
$ 55126.87769 $ & $   0.00018 $ & $   0.00105 $ & $  10.66107 $ & $ i$\\
$ 55126.87859 $ & $  -0.00200 $ & $   0.00105 $ & $  10.66096 $ & $ i$\\
$ 55126.87895 $ & $  -0.00092 $ & $   0.00104 $ & $  10.66103 $ & $ i$\\
$ 55126.87931 $ & $   0.00257 $ & $   0.00105 $ & $  10.66357 $ & $ i$\\
$ 55126.87987 $ & $  -0.00290 $ & $   0.00104 $ & $  10.65713 $ & $ i$\\
$ 55126.88023 $ & $  -0.00359 $ & $   0.00104 $ & $  10.65684 $ & $ i$\\
$ 55126.88060 $ & $  -0.00172 $ & $   0.00104 $ & $  10.65974 $ & $ i$\\
$ 55126.88114 $ & $  -0.00135 $ & $   0.00104 $ & $  10.65976 $ & $ i$\\
$ 55126.88151 $ & $  -0.00038 $ & $   0.00105 $ & $  10.66151 $ & $ i$\\
$ 55126.88187 $ & $  -0.00229 $ & $   0.00105 $ & $  10.65926 $ & $ i$\\
$ 55126.88241 $ & $   0.00297 $ & $   0.00104 $ & $  10.66312 $ & $ i$\\
$ 55126.88277 $ & $   0.00004 $ & $   0.00105 $ & $  10.66040 $ & $ i$\\
$ 55126.88312 $ & $  -0.00114 $ & $   0.00105 $ & $  10.65871 $ & $ i$\\
$ 55126.88366 $ & $   0.00386 $ & $   0.00105 $ & $  10.66471 $ & $ i$\\
$ 55126.88439 $ & $   0.00316 $ & $   0.00105 $ & $  10.66431 $ & $ i$\\
$ 55126.88494 $ & $   0.00110 $ & $   0.00105 $ & $  10.66159 $ & $ i$\\
$ 55126.88530 $ & $   0.00263 $ & $   0.00105 $ & $  10.66217 $ & $ i$\\
$ 55126.88564 $ & $   0.00445 $ & $   0.00105 $ & $  10.66457 $ & $ i$\\
$ 55126.88622 $ & $  -0.00266 $ & $   0.00104 $ & $  10.65902 $ & $ i$\\
$ 55126.88672 $ & $   0.00427 $ & $   0.00105 $ & $  10.66275 $ & $ i$\\
$ 55126.88709 $ & $  -0.00326 $ & $   0.00104 $ & $  10.65790 $ & $ i$\\
$ 55126.88745 $ & $  -0.00054 $ & $   0.00104 $ & $  10.66014 $ & $ i$\\
$ 55126.88802 $ & $   0.00059 $ & $   0.00104 $ & $  10.66044 $ & $ i$\\
$ 55126.88839 $ & $   0.00429 $ & $   0.00105 $ & $  10.66431 $ & $ i$\\
$ 55126.88876 $ & $  -0.00088 $ & $   0.00105 $ & $  10.66034 $ & $ i$\\
$ 55126.88930 $ & $   0.00180 $ & $   0.00105 $ & $  10.66055 $ & $ i$\\
$ 55126.88966 $ & $   0.00050 $ & $   0.00105 $ & $  10.66118 $ & $ i$\\
$ 55126.89003 $ & $   0.00221 $ & $   0.00105 $ & $  10.66210 $ & $ i$\\
$ 55126.89060 $ & $   0.00096 $ & $   0.00104 $ & $  10.66182 $ & $ i$\\
$ 55126.89096 $ & $  -0.00114 $ & $   0.00104 $ & $  10.65943 $ & $ i$\\
$ 55126.89134 $ & $  -0.00019 $ & $   0.00105 $ & $  10.65972 $ & $ i$\\
$ 55126.89190 $ & $  -0.00233 $ & $   0.00104 $ & $  10.65817 $ & $ i$\\
$ 55126.89225 $ & $  -0.00161 $ & $   0.00104 $ & $  10.66002 $ & $ i$\\
$ 55126.89269 $ & $  -0.00148 $ & $   0.00104 $ & $  10.65779 $ & $ i$\\
$ 55126.89305 $ & $  -0.00257 $ & $   0.00104 $ & $  10.65737 $ & $ i$\\
$ 55126.89342 $ & $  -0.00221 $ & $   0.00104 $ & $  10.65758 $ & $ i$\\
$ 55126.89397 $ & $  -0.00164 $ & $   0.00104 $ & $  10.65868 $ & $ i$\\
$ 55126.89432 $ & $   0.00052 $ & $   0.00104 $ & $  10.66001 $ & $ i$\\
$ 55126.89468 $ & $   0.00253 $ & $   0.00105 $ & $  10.66332 $ & $ i$\\
$ 55126.89523 $ & $   0.00154 $ & $   0.00104 $ & $  10.66101 $ & $ i$\\
$ 55126.89559 $ & $  -0.00169 $ & $   0.00104 $ & $  10.65863 $ & $ i$\\
$ 55126.89594 $ & $   0.00136 $ & $   0.00104 $ & $  10.66155 $ & $ i$\\
$ 55126.89650 $ & $   0.00100 $ & $   0.00105 $ & $  10.66182 $ & $ i$\\
$ 55126.89688 $ & $   0.00152 $ & $   0.00104 $ & $  10.65954 $ & $ i$\\
$ 55126.89724 $ & $   0.00349 $ & $   0.00105 $ & $  10.66284 $ & $ i$\\
$ 55126.89780 $ & $   0.00329 $ & $   0.00105 $ & $  10.66337 $ & $ i$\\
$ 55126.89817 $ & $   0.00238 $ & $   0.00105 $ & $  10.66284 $ & $ i$\\
$ 55126.89853 $ & $   0.00429 $ & $   0.00105 $ & $  10.66411 $ & $ i$\\
$ 55126.89912 $ & $   0.00753 $ & $   0.00105 $ & $  10.66691 $ & $ i$\\
$ 55126.89949 $ & $   0.00849 $ & $   0.00105 $ & $  10.66806 $ & $ i$\\
$ 55126.89984 $ & $   0.00694 $ & $   0.00105 $ & $  10.66722 $ & $ i$\\
$ 55126.90041 $ & $   0.00686 $ & $   0.00105 $ & $  10.66695 $ & $ i$\\
$ 55126.90078 $ & $   0.01063 $ & $   0.00105 $ & $  10.66996 $ & $ i$\\
$ 55126.90115 $ & $   0.00391 $ & $   0.00104 $ & $  10.66169 $ & $ i$\\
$ 55126.90171 $ & $   0.01037 $ & $   0.00105 $ & $  10.67095 $ & $ i$\\
$ 55126.90208 $ & $   0.01273 $ & $   0.00105 $ & $  10.67021 $ & $ i$\\
$ 55126.90245 $ & $   0.00859 $ & $   0.00105 $ & $  10.66810 $ & $ i$\\
$ 55126.90301 $ & $   0.00926 $ & $   0.00105 $ & $  10.66827 $ & $ i$\\
$ 55126.90336 $ & $   0.01297 $ & $   0.00105 $ & $  10.67187 $ & $ i$\\
$ 55126.90375 $ & $   0.00953 $ & $   0.00105 $ & $  10.66688 $ & $ i$\\
$ 55126.90430 $ & $   0.01403 $ & $   0.00105 $ & $  10.67230 $ & $ i$\\
$ 55126.90467 $ & $   0.01102 $ & $   0.00105 $ & $  10.66993 $ & $ i$\\
$ 55126.90503 $ & $   0.01151 $ & $   0.00105 $ & $  10.66937 $ & $ i$\\
$ 55126.90559 $ & $   0.01723 $ & $   0.00105 $ & $  10.67559 $ & $ i$\\
$ 55126.90596 $ & $   0.01470 $ & $   0.00105 $ & $  10.67351 $ & $ i$\\
$ 55126.90634 $ & $   0.01281 $ & $   0.00105 $ & $  10.67125 $ & $ i$\\
$ 55126.90689 $ & $   0.01695 $ & $   0.00105 $ & $  10.67399 $ & $ i$\\
$ 55126.90725 $ & $   0.01391 $ & $   0.00105 $ & $  10.67235 $ & $ i$\\
$ 55126.90764 $ & $   0.01536 $ & $   0.00105 $ & $  10.67424 $ & $ i$\\
$ 55126.90818 $ & $   0.01497 $ & $   0.00105 $ & $  10.67121 $ & $ i$\\
$ 55126.90854 $ & $   0.01788 $ & $   0.00105 $ & $  10.67685 $ & $ i$\\
$ 55126.90891 $ & $   0.01341 $ & $   0.00105 $ & $  10.67162 $ & $ i$\\
$ 55126.90949 $ & $   0.01875 $ & $   0.00105 $ & $  10.67581 $ & $ i$\\
$ 55126.90986 $ & $   0.01455 $ & $   0.00105 $ & $  10.67286 $ & $ i$\\
$ 55126.91022 $ & $   0.01672 $ & $   0.00105 $ & $  10.67492 $ & $ i$\\
$ 55126.91077 $ & $   0.01695 $ & $   0.00105 $ & $  10.67383 $ & $ i$\\
$ 55126.91113 $ & $   0.01639 $ & $   0.00105 $ & $  10.67401 $ & $ i$\\
$ 55126.91153 $ & $   0.01673 $ & $   0.00105 $ & $  10.67588 $ & $ i$\\
$ 55126.91206 $ & $   0.01945 $ & $   0.00106 $ & $  10.67826 $ & $ i$\\
$ 55126.91242 $ & $   0.01788 $ & $   0.00105 $ & $  10.67635 $ & $ i$\\
$ 55126.91280 $ & $   0.01775 $ & $   0.00105 $ & $  10.67616 $ & $ i$\\
$ 55126.91339 $ & $   0.01461 $ & $   0.00105 $ & $  10.67488 $ & $ i$\\
$ 55126.91376 $ & $   0.01928 $ & $   0.00105 $ & $  10.67638 $ & $ i$\\
$ 55126.91413 $ & $   0.01564 $ & $   0.00105 $ & $  10.67384 $ & $ i$\\
$ 55126.91466 $ & $   0.02040 $ & $   0.00106 $ & $  10.67763 $ & $ i$\\
$ 55126.91503 $ & $   0.01730 $ & $   0.00106 $ & $  10.67532 $ & $ i$\\
$ 55126.91540 $ & $   0.01502 $ & $   0.00105 $ & $  10.67367 $ & $ i$\\
$ 55126.91597 $ & $   0.01869 $ & $   0.00106 $ & $  10.67671 $ & $ i$\\
$ 55126.91633 $ & $   0.02007 $ & $   0.00105 $ & $  10.67757 $ & $ i$\\
$ 55126.91669 $ & $   0.01899 $ & $   0.00105 $ & $  10.67650 $ & $ i$\\
$ 55126.91724 $ & $   0.02025 $ & $   0.00105 $ & $  10.67668 $ & $ i$\\
$ 55126.91759 $ & $   0.01817 $ & $   0.00105 $ & $  10.67551 $ & $ i$\\
$ 55126.91796 $ & $   0.02130 $ & $   0.00105 $ & $  10.67917 $ & $ i$\\
$ 55126.91852 $ & $   0.02008 $ & $   0.00106 $ & $  10.67803 $ & $ i$\\
$ 55126.91887 $ & $   0.02052 $ & $   0.00106 $ & $  10.67700 $ & $ i$\\
$ 55126.91922 $ & $   0.02120 $ & $   0.00106 $ & $  10.67860 $ & $ i$\\
$ 55126.91975 $ & $   0.01761 $ & $   0.00105 $ & $  10.67538 $ & $ i$\\
$ 55126.92014 $ & $   0.01784 $ & $   0.00105 $ & $  10.67665 $ & $ i$\\
$ 55126.92049 $ & $   0.02128 $ & $   0.00106 $ & $  10.67857 $ & $ i$\\
$ 55126.92106 $ & $   0.02220 $ & $   0.00106 $ & $  10.68074 $ & $ i$\\
$ 55126.92141 $ & $   0.02254 $ & $   0.00106 $ & $  10.68001 $ & $ i$\\
$ 55126.92176 $ & $   0.01941 $ & $   0.00105 $ & $  10.67670 $ & $ i$\\
$ 55126.92230 $ & $   0.02376 $ & $   0.00106 $ & $  10.68154 $ & $ i$\\
$ 55126.92267 $ & $   0.02223 $ & $   0.00106 $ & $  10.67888 $ & $ i$\\
$ 55126.92303 $ & $   0.01985 $ & $   0.00106 $ & $  10.67865 $ & $ i$\\
$ 55126.92357 $ & $   0.01717 $ & $   0.00105 $ & $  10.67526 $ & $ i$\\
$ 55126.92395 $ & $   0.01931 $ & $   0.00105 $ & $  10.67469 $ & $ i$\\
$ 55126.92433 $ & $   0.01525 $ & $   0.00105 $ & $  10.67321 $ & $ i$\\
$ 55126.92488 $ & $   0.02313 $ & $   0.00106 $ & $  10.68128 $ & $ i$\\
$ 55126.92526 $ & $   0.01991 $ & $   0.00106 $ & $  10.67789 $ & $ i$\\
$ 55126.92562 $ & $   0.01833 $ & $   0.00105 $ & $  10.67537 $ & $ i$\\
$ 55126.92618 $ & $   0.02040 $ & $   0.00106 $ & $  10.67880 $ & $ i$\\
$ 55126.92654 $ & $   0.01725 $ & $   0.00105 $ & $  10.67643 $ & $ i$\\
$ 55126.92691 $ & $   0.01816 $ & $   0.00105 $ & $  10.67516 $ & $ i$\\
$ 55126.92746 $ & $   0.01911 $ & $   0.00106 $ & $  10.67700 $ & $ i$\\
$ 55126.92782 $ & $   0.02147 $ & $   0.00106 $ & $  10.67831 $ & $ i$\\
$ 55126.92819 $ & $   0.01802 $ & $   0.00105 $ & $  10.67407 $ & $ i$\\
$ 55126.92875 $ & $   0.02061 $ & $   0.00106 $ & $  10.67806 $ & $ i$\\
$ 55126.92911 $ & $   0.02218 $ & $   0.00106 $ & $  10.67849 $ & $ i$\\
$ 55126.92945 $ & $   0.01910 $ & $   0.00106 $ & $  10.67746 $ & $ i$\\
$ 55126.93001 $ & $   0.02017 $ & $   0.00106 $ & $  10.67682 $ & $ i$\\
$ 55126.93038 $ & $   0.02281 $ & $   0.00106 $ & $  10.67977 $ & $ i$\\
$ 55126.93076 $ & $   0.01898 $ & $   0.00106 $ & $  10.67588 $ & $ i$\\
$ 55126.93132 $ & $   0.02014 $ & $   0.00105 $ & $  10.67699 $ & $ i$\\
$ 55126.93169 $ & $   0.01565 $ & $   0.00105 $ & $  10.67286 $ & $ i$\\
$ 55126.93206 $ & $   0.01915 $ & $   0.00105 $ & $  10.67604 $ & $ i$\\
$ 55126.93260 $ & $   0.02146 $ & $   0.00106 $ & $  10.67732 $ & $ i$\\
$ 55126.93299 $ & $   0.01763 $ & $   0.00105 $ & $  10.67569 $ & $ i$\\
$ 55126.93334 $ & $   0.01554 $ & $   0.00105 $ & $  10.67366 $ & $ i$\\
$ 55126.93391 $ & $   0.02198 $ & $   0.00106 $ & $  10.67901 $ & $ i$\\
$ 55126.93428 $ & $   0.02010 $ & $   0.00106 $ & $  10.67637 $ & $ i$\\
$ 55126.93465 $ & $   0.01943 $ & $   0.00106 $ & $  10.67592 $ & $ i$\\
$ 55126.93520 $ & $   0.01994 $ & $   0.00105 $ & $  10.67580 $ & $ i$\\
$ 55126.93555 $ & $   0.01821 $ & $   0.00105 $ & $  10.67526 $ & $ i$\\
$ 55126.93593 $ & $   0.01976 $ & $   0.00105 $ & $  10.67564 $ & $ i$\\
$ 55126.93650 $ & $   0.01998 $ & $   0.00106 $ & $  10.67699 $ & $ i$\\
$ 55126.93687 $ & $   0.01964 $ & $   0.00106 $ & $  10.67761 $ & $ i$\\
$ 55126.93724 $ & $   0.01990 $ & $   0.00106 $ & $  10.67682 $ & $ i$\\
$ 55126.93781 $ & $   0.01710 $ & $   0.00105 $ & $  10.67430 $ & $ i$\\
$ 55126.93818 $ & $   0.02020 $ & $   0.00105 $ & $  10.67608 $ & $ i$\\
$ 55126.93856 $ & $   0.01789 $ & $   0.00105 $ & $  10.67423 $ & $ i$\\
$ 55126.93912 $ & $   0.02204 $ & $   0.00106 $ & $  10.67769 $ & $ i$\\
$ 55126.93949 $ & $   0.01762 $ & $   0.00105 $ & $  10.67566 $ & $ i$\\
$ 55126.93984 $ & $   0.02143 $ & $   0.00105 $ & $  10.67715 $ & $ i$\\
$ 55126.94042 $ & $   0.01782 $ & $   0.00105 $ & $  10.67520 $ & $ i$\\
$ 55126.94079 $ & $   0.02072 $ & $   0.00106 $ & $  10.67754 $ & $ i$\\
$ 55126.94115 $ & $   0.01878 $ & $   0.00105 $ & $  10.67522 $ & $ i$\\
$ 55126.94170 $ & $   0.01675 $ & $   0.00105 $ & $  10.67289 $ & $ i$\\
$ 55126.94206 $ & $   0.01931 $ & $   0.00105 $ & $  10.67609 $ & $ i$\\
$ 55126.94243 $ & $   0.01442 $ & $   0.00105 $ & $  10.67114 $ & $ i$\\
$ 55126.94296 $ & $   0.01564 $ & $   0.00105 $ & $  10.67121 $ & $ i$\\
$ 55126.94332 $ & $   0.01665 $ & $   0.00105 $ & $  10.67319 $ & $ i$\\
$ 55126.94368 $ & $   0.01739 $ & $   0.00106 $ & $  10.67460 $ & $ i$\\
$ 55126.94425 $ & $   0.01712 $ & $   0.00106 $ & $  10.67398 $ & $ i$\\
$ 55126.94461 $ & $   0.01511 $ & $   0.00105 $ & $  10.67159 $ & $ i$\\
$ 55126.94497 $ & $   0.01822 $ & $   0.00106 $ & $  10.67356 $ & $ i$\\
$ 55126.94552 $ & $   0.01530 $ & $   0.00105 $ & $  10.67110 $ & $ i$\\
$ 55126.94588 $ & $   0.01920 $ & $   0.00105 $ & $  10.67474 $ & $ i$\\
$ 55126.94625 $ & $   0.01642 $ & $   0.00105 $ & $  10.67222 $ & $ i$\\
$ 55126.94679 $ & $   0.02200 $ & $   0.00106 $ & $  10.67816 $ & $ i$\\
$ 55126.94716 $ & $   0.01864 $ & $   0.00105 $ & $  10.67553 $ & $ i$\\
$ 55126.94755 $ & $   0.01969 $ & $   0.00106 $ & $  10.67707 $ & $ i$\\
$ 55126.94810 $ & $   0.01707 $ & $   0.00105 $ & $  10.67271 $ & $ i$\\
$ 55126.94846 $ & $   0.01735 $ & $   0.00105 $ & $  10.67366 $ & $ i$\\
$ 55126.94883 $ & $   0.01618 $ & $   0.00105 $ & $  10.67234 $ & $ i$\\
$ 55126.94939 $ & $   0.01814 $ & $   0.00105 $ & $  10.67448 $ & $ i$\\
$ 55126.94975 $ & $   0.01729 $ & $   0.00105 $ & $  10.67340 $ & $ i$\\
$ 55126.95010 $ & $   0.01518 $ & $   0.00105 $ & $  10.67088 $ & $ i$\\
$ 55126.95066 $ & $   0.02144 $ & $   0.00106 $ & $  10.67824 $ & $ i$\\
$ 55126.95101 $ & $   0.01751 $ & $   0.00105 $ & $  10.67401 $ & $ i$\\
$ 55126.95137 $ & $   0.01567 $ & $   0.00105 $ & $  10.67247 $ & $ i$\\
$ 55126.95192 $ & $   0.01926 $ & $   0.00106 $ & $  10.67586 $ & $ i$\\
$ 55126.95228 $ & $   0.01783 $ & $   0.00105 $ & $  10.67409 $ & $ i$\\
$ 55126.95265 $ & $   0.01939 $ & $   0.00105 $ & $  10.67659 $ & $ i$\\
$ 55126.95318 $ & $   0.01555 $ & $   0.00105 $ & $  10.67259 $ & $ i$\\
$ 55126.95354 $ & $   0.01537 $ & $   0.00105 $ & $  10.67142 $ & $ i$\\
$ 55126.95391 $ & $   0.01698 $ & $   0.00105 $ & $  10.67387 $ & $ i$\\
$ 55126.95448 $ & $   0.01606 $ & $   0.00105 $ & $  10.67184 $ & $ i$\\
$ 55126.95483 $ & $   0.01994 $ & $   0.00105 $ & $  10.67597 $ & $ i$\\
$ 55126.95519 $ & $   0.01632 $ & $   0.00105 $ & $  10.67282 $ & $ i$\\
$ 55126.95577 $ & $   0.01454 $ & $   0.00105 $ & $  10.66987 $ & $ i$\\
$ 55126.95614 $ & $   0.01521 $ & $   0.00105 $ & $  10.67211 $ & $ i$\\
$ 55126.95706 $ & $   0.01333 $ & $   0.00105 $ & $  10.67051 $ & $ i$\\
$ 55126.95742 $ & $   0.01506 $ & $   0.00105 $ & $  10.67269 $ & $ i$\\
$ 55126.95778 $ & $   0.01537 $ & $   0.00105 $ & $  10.67189 $ & $ i$\\
$ 55126.95832 $ & $   0.01352 $ & $   0.00105 $ & $  10.66887 $ & $ i$\\
$ 55126.95869 $ & $   0.01160 $ & $   0.00105 $ & $  10.66950 $ & $ i$\\
$ 55126.95905 $ & $   0.00745 $ & $   0.00105 $ & $  10.66511 $ & $ i$\\
$ 55126.95960 $ & $   0.00932 $ & $   0.00105 $ & $  10.66630 $ & $ i$\\
$ 55126.95997 $ & $   0.01217 $ & $   0.00105 $ & $  10.66955 $ & $ i$\\
$ 55126.96034 $ & $   0.01111 $ & $   0.00105 $ & $  10.66776 $ & $ i$\\
$ 55126.96089 $ & $   0.01188 $ & $   0.00105 $ & $  10.66809 $ & $ i$\\
$ 55126.96126 $ & $   0.00788 $ & $   0.00105 $ & $  10.66544 $ & $ i$\\
$ 55126.96162 $ & $   0.01103 $ & $   0.00105 $ & $  10.66941 $ & $ i$\\
$ 55126.96219 $ & $   0.00570 $ & $   0.00104 $ & $  10.66299 $ & $ i$\\
$ 55126.96254 $ & $   0.00778 $ & $   0.00104 $ & $  10.66474 $ & $ i$\\
$ 55126.96290 $ & $   0.01142 $ & $   0.00105 $ & $  10.66794 $ & $ i$\\
$ 55126.96346 $ & $   0.00889 $ & $   0.00105 $ & $  10.66717 $ & $ i$\\
$ 55126.96383 $ & $   0.00788 $ & $   0.00105 $ & $  10.66380 $ & $ i$\\
$ 55126.96419 $ & $   0.00404 $ & $   0.00105 $ & $  10.66180 $ & $ i$\\
$ 55126.96472 $ & $   0.00507 $ & $   0.00105 $ & $  10.66228 $ & $ i$\\
$ 55126.96508 $ & $   0.00521 $ & $   0.00105 $ & $  10.66351 $ & $ i$\\
$ 55126.96544 $ & $   0.00176 $ & $   0.00104 $ & $  10.65966 $ & $ i$\\
$ 55126.96601 $ & $   0.00433 $ & $   0.00105 $ & $  10.66391 $ & $ i$\\
$ 55126.96638 $ & $   0.00033 $ & $   0.00104 $ & $  10.65825 $ & $ i$\\
$ 55126.96675 $ & $   0.00225 $ & $   0.00104 $ & $  10.65914 $ & $ i$\\
$ 55126.96731 $ & $  -0.00111 $ & $   0.00104 $ & $  10.65649 $ & $ i$\\
$ 55126.96768 $ & $  -0.00239 $ & $   0.00104 $ & $  10.65555 $ & $ i$\\
$ 55126.96805 $ & $   0.00581 $ & $   0.00105 $ & $  10.66374 $ & $ i$\\
$ 55126.96864 $ & $   0.00407 $ & $   0.00105 $ & $  10.66154 $ & $ i$\\
$ 55126.96900 $ & $   0.00358 $ & $   0.00105 $ & $  10.66090 $ & $ i$\\
$ 55126.96938 $ & $   0.00275 $ & $   0.00105 $ & $  10.66098 $ & $ i$\\
$ 55126.96993 $ & $  -0.00321 $ & $   0.00104 $ & $  10.65506 $ & $ i$\\
$ 55126.97029 $ & $  -0.00090 $ & $   0.00105 $ & $  10.65824 $ & $ i$\\
$ 55126.97064 $ & $   0.00329 $ & $   0.00105 $ & $  10.66030 $ & $ i$\\
$ 55126.97119 $ & $   0.00154 $ & $   0.00105 $ & $  10.65984 $ & $ i$\\
$ 55126.97156 $ & $   0.00165 $ & $   0.00105 $ & $  10.66068 $ & $ i$\\
$ 55126.97194 $ & $   0.00062 $ & $   0.00105 $ & $  10.65905 $ & $ i$\\
$ 55126.97248 $ & $  -0.00083 $ & $   0.00105 $ & $  10.65766 $ & $ i$\\
$ 55126.97284 $ & $  -0.00103 $ & $   0.00104 $ & $  10.65690 $ & $ i$\\
$ 55126.97320 $ & $  -0.00093 $ & $   0.00105 $ & $  10.65761 $ & $ i$\\
$ 55126.97374 $ & $  -0.00124 $ & $   0.00104 $ & $  10.65711 $ & $ i$\\
$ 55126.97411 $ & $  -0.00048 $ & $   0.00105 $ & $  10.65891 $ & $ i$\\
$ 55126.97448 $ & $   0.00095 $ & $   0.00105 $ & $  10.65897 $ & $ i$\\
$ 55126.97506 $ & $  -0.00091 $ & $   0.00104 $ & $  10.65706 $ & $ i$\\
$ 55126.97541 $ & $   0.00320 $ & $   0.00105 $ & $  10.66122 $ & $ i$\\
$ 55126.97578 $ & $  -0.00011 $ & $   0.00105 $ & $  10.65933 $ & $ i$\\
$ 55126.97632 $ & $  -0.00187 $ & $   0.00104 $ & $  10.65619 $ & $ i$\\
$ 55126.97669 $ & $  -0.00318 $ & $   0.00104 $ & $  10.65583 $ & $ i$\\
$ 55126.97708 $ & $   0.00059 $ & $   0.00105 $ & $  10.65841 $ & $ i$\\
$ 55126.97763 $ & $  -0.00169 $ & $   0.00105 $ & $  10.65649 $ & $ i$\\
$ 55126.97799 $ & $   0.00294 $ & $   0.00105 $ & $  10.66245 $ & $ i$\\
$ 55126.97835 $ & $   0.00015 $ & $   0.00104 $ & $  10.65862 $ & $ i$\\
$ 55126.97892 $ & $  -0.00386 $ & $   0.00104 $ & $  10.65408 $ & $ i$\\
$ 55126.97927 $ & $  -0.00007 $ & $   0.00105 $ & $  10.65892 $ & $ i$\\
$ 55126.97962 $ & $   0.00185 $ & $   0.00105 $ & $  10.66093 $ & $ i$\\
$ 55126.98018 $ & $   0.00188 $ & $   0.00105 $ & $  10.65850 $ & $ i$\\
$ 55126.98054 $ & $  -0.00186 $ & $   0.00104 $ & $  10.65445 $ & $ i$\\
$ 55126.98089 $ & $   0.00231 $ & $   0.00105 $ & $  10.66079 $ & $ i$\\
$ 55126.98145 $ & $   0.00029 $ & $   0.00104 $ & $  10.65793 $ & $ i$\\
$ 55126.98182 $ & $   0.00134 $ & $   0.00105 $ & $  10.65999 $ & $ i$\\
$ 55126.98218 $ & $  -0.00149 $ & $   0.00105 $ & $  10.65830 $ & $ i$\\
$ 55126.98275 $ & $  -0.00433 $ & $   0.00104 $ & $  10.65379 $ & $ i$\\
$ 55126.98312 $ & $  -0.00242 $ & $   0.00104 $ & $  10.65467 $ & $ i$\\
$ 55126.98348 $ & $   0.00146 $ & $   0.00104 $ & $  10.65844 $ & $ i$\\
$ 55126.98402 $ & $   0.00198 $ & $   0.00105 $ & $  10.65956 $ & $ i$\\
$ 55126.98438 $ & $  -0.00052 $ & $   0.00105 $ & $  10.65727 $ & $ i$\\
$ 55126.98473 $ & $  -0.00078 $ & $   0.00104 $ & $  10.65797 $ & $ i$\\
$ 55126.98529 $ & $  -0.00183 $ & $   0.00104 $ & $  10.65621 $ & $ i$\\
$ 55126.98565 $ & $   0.00059 $ & $   0.00104 $ & $  10.65743 $ & $ i$\\
$ 55126.98602 $ & $   0.00262 $ & $   0.00105 $ & $  10.66082 $ & $ i$\\
$ 55126.98658 $ & $  -0.00002 $ & $   0.00104 $ & $  10.65676 $ & $ i$\\
$ 55126.98695 $ & $  -0.00371 $ & $   0.00104 $ & $  10.65420 $ & $ i$\\
$ 55126.98734 $ & $  -0.00135 $ & $   0.00105 $ & $  10.65817 $ & $ i$\\
$ 55126.98789 $ & $  -0.00123 $ & $   0.00104 $ & $  10.65614 $ & $ i$\\
$ 55126.98826 $ & $  -0.00195 $ & $   0.00104 $ & $  10.65568 $ & $ i$\\
$ 55126.98863 $ & $  -0.00087 $ & $   0.00105 $ & $  10.65711 $ & $ i$\\
$ 55126.98918 $ & $   0.00252 $ & $   0.00105 $ & $  10.66193 $ & $ i$\\
$ 55126.98954 $ & $   0.00080 $ & $   0.00105 $ & $  10.65919 $ & $ i$\\
$ 55126.98991 $ & $  -0.00105 $ & $   0.00104 $ & $  10.65629 $ & $ i$\\
$ 55126.99047 $ & $   0.00060 $ & $   0.00105 $ & $  10.65866 $ & $ i$\\
$ 55126.99084 $ & $  -0.00037 $ & $   0.00105 $ & $  10.65851 $ & $ i$\\
$ 55126.99121 $ & $   0.00240 $ & $   0.00105 $ & $  10.66184 $ & $ i$\\
$ 55126.99176 $ & $  -0.00062 $ & $   0.00105 $ & $  10.65821 $ & $ i$\\
$ 55126.99212 $ & $   0.00120 $ & $   0.00105 $ & $  10.66075 $ & $ i$\\
$ 55126.99251 $ & $  -0.00108 $ & $   0.00104 $ & $  10.65608 $ & $ i$\\
$ 55126.99306 $ & $   0.00099 $ & $   0.00105 $ & $  10.65993 $ & $ i$\\
$ 55126.99343 $ & $  -0.00173 $ & $   0.00105 $ & $  10.65723 $ & $ i$\\
$ 55126.99380 $ & $   0.00215 $ & $   0.00105 $ & $  10.66119 $ & $ i$\\
$ 55126.99435 $ & $  -0.00118 $ & $   0.00105 $ & $  10.65794 $ & $ i$\\
$ 55126.99469 $ & $   0.00375 $ & $   0.00105 $ & $  10.66322 $ & $ i$\\
$ 55126.99506 $ & $   0.00308 $ & $   0.00105 $ & $  10.66284 $ & $ i$\\
$ 55126.99564 $ & $  -0.00257 $ & $   0.00105 $ & $  10.65685 $ & $ i$\\
$ 55126.99601 $ & $  -0.00026 $ & $   0.00105 $ & $  10.65867 $ & $ i$\\
$ 55126.99694 $ & $   0.00362 $ & $   0.00105 $ & $  10.66143 $ & $ i$\\
$ 55126.99730 $ & $   0.00123 $ & $   0.00105 $ & $  10.65986 $ & $ i$\\
$ 55126.99767 $ & $  -0.00240 $ & $   0.00105 $ & $  10.65454 $ & $ i$\\
$ 55126.99822 $ & $   0.00173 $ & $   0.00105 $ & $  10.66090 $ & $ i$\\
$ 55126.99858 $ & $  -0.00075 $ & $   0.00105 $ & $  10.65705 $ & $ i$\\
$ 55126.99895 $ & $   0.00071 $ & $   0.00105 $ & $  10.65971 $ & $ i$\\
$ 55126.99948 $ & $   0.00033 $ & $   0.00105 $ & $  10.65929 $ & $ i$\\
$ 55126.99984 $ & $   0.00019 $ & $   0.00105 $ & $  10.65797 $ & $ i$\\
$ 55127.00021 $ & $   0.00063 $ & $   0.00105 $ & $  10.65956 $ & $ i$\\
$ 55127.00077 $ & $  -0.00050 $ & $   0.00105 $ & $  10.65787 $ & $ i$\\
$ 55127.00113 $ & $   0.00046 $ & $   0.00105 $ & $  10.65835 $ & $ i$\\
$ 55127.00149 $ & $   0.00052 $ & $   0.00105 $ & $  10.65874 $ & $ i$\\
$ 55127.00205 $ & $  -0.00084 $ & $   0.00105 $ & $  10.65795 $ & $ i$\\
$ 55127.00243 $ & $   0.00151 $ & $   0.00105 $ & $  10.65901 $ & $ i$\\
$ 55127.00278 $ & $   0.00025 $ & $   0.00105 $ & $  10.65869 $ & $ i$\\
$ 55127.00335 $ & $  -0.00077 $ & $   0.00105 $ & $  10.65785 $ & $ i$\\
$ 55127.00372 $ & $  -0.00057 $ & $   0.00105 $ & $  10.65748 $ & $ i$\\
$ 55127.00408 $ & $  -0.00186 $ & $   0.00105 $ & $  10.65734 $ & $ i$\\
$ 55127.00464 $ & $   0.00141 $ & $   0.00105 $ & $  10.65918 $ & $ i$\\
$ 55127.00498 $ & $   0.00225 $ & $   0.00105 $ & $  10.66106 $ & $ i$\\
$ 55127.00534 $ & $   0.00075 $ & $   0.00105 $ & $  10.65845 $ & $ i$\\
$ 55127.00590 $ & $  -0.00007 $ & $   0.00105 $ & $  10.65840 $ & $ i$\\
$ 55127.00626 $ & $   0.00129 $ & $   0.00105 $ & $  10.65872 $ & $ i$\\
$ 55127.00663 $ & $   0.00138 $ & $   0.00105 $ & $  10.66053 $ & $ i$\\
$ 55127.00718 $ & $  -0.00023 $ & $   0.00105 $ & $  10.65935 $ & $ i$\\
$ 55127.00754 $ & $  -0.00108 $ & $   0.00105 $ & $  10.65805 $ & $ i$\\
$ 55127.00790 $ & $   0.00331 $ & $   0.00105 $ & $  10.66199 $ & $ i$\\
$ 55127.00846 $ & $   0.00003 $ & $   0.00105 $ & $  10.65966 $ & $ i$\\
$ 55127.00880 $ & $  -0.00023 $ & $   0.00105 $ & $  10.65822 $ & $ i$\\
$ 55127.00917 $ & $   0.00044 $ & $   0.00105 $ & $  10.65908 $ & $ i$\\
$ 55127.00973 $ & $  -0.00084 $ & $   0.00105 $ & $  10.65825 $ & $ i$\\
$ 55127.01008 $ & $   0.00130 $ & $   0.00105 $ & $  10.65964 $ & $ i$\\
$ 55127.01043 $ & $  -0.00168 $ & $   0.00105 $ & $  10.65641 $ & $ i$\\
$ 55127.01098 $ & $  -0.00052 $ & $   0.00105 $ & $  10.65964 $ & $ i$\\
$ 55127.01134 $ & $   0.00205 $ & $   0.00105 $ & $  10.66070 $ & $ i$\\
$ 55127.01171 $ & $   0.00041 $ & $   0.00105 $ & $  10.66010 $ & $ i$\\
$ 55127.01225 $ & $  -0.00181 $ & $   0.00105 $ & $  10.65851 $ & $ i$\\
$ 55127.01261 $ & $  -0.00181 $ & $   0.00105 $ & $  10.65651 $ & $ i$\\
$ 55127.01298 $ & $  -0.00055 $ & $   0.00105 $ & $  10.65791 $ & $ i$\\
$ 55127.01353 $ & $  -0.00084 $ & $   0.00105 $ & $  10.65940 $ & $ i$\\
$ 55127.01390 $ & $   0.00089 $ & $   0.00105 $ & $  10.65988 $ & $ i$\\
$ 55127.01427 $ & $  -0.00120 $ & $   0.00105 $ & $  10.65854 $ & $ i$\\
$ 55127.01482 $ & $   0.00222 $ & $   0.00105 $ & $  10.66216 $ & $ i$\\
$ 55127.01519 $ & $  -0.00167 $ & $   0.00105 $ & $  10.65693 $ & $ i$\\
$ 55127.01555 $ & $   0.00079 $ & $   0.00105 $ & $  10.65962 $ & $ i$\\
$ 55127.01613 $ & $   0.00158 $ & $   0.00105 $ & $  10.66053 $ & $ i$\\
$ 55127.01649 $ & $  -0.00176 $ & $   0.00105 $ & $  10.65771 $ & $ i$\\
$ 55127.01685 $ & $  -0.00318 $ & $   0.00105 $ & $  10.65770 $ & $ i$\\
$ 55127.01739 $ & $   0.00020 $ & $   0.00105 $ & $  10.65986 $ & $ i$\\
$ 55127.01775 $ & $  -0.00031 $ & $   0.00105 $ & $  10.65821 $ & $ i$\\
$ 55127.01811 $ & $  -0.00300 $ & $   0.00105 $ & $  10.65651 $ & $ i$\\
$ 55127.01866 $ & $   0.00257 $ & $   0.00105 $ & $  10.66175 $ & $ i$\\
$ 55127.01902 $ & $   0.00316 $ & $   0.00105 $ & $  10.66286 $ & $ i$\\
$ 55127.01937 $ & $  -0.00167 $ & $   0.00105 $ & $  10.65922 $ & $ i$\\
$ 55127.01993 $ & $  -0.00111 $ & $   0.00105 $ & $  10.65913 $ & $ i$\\
$ 55127.02029 $ & $  -0.00036 $ & $   0.00105 $ & $  10.65987 $ & $ i$\\
$ 55127.02066 $ & $  -0.00008 $ & $   0.00105 $ & $  10.65924 $ & $ i$\\
$ 55127.02120 $ & $  -0.00186 $ & $   0.00105 $ & $  10.65873 $ & $ i$\\


==> HTR267-010_phfu_tab_short.tex <==
$ 54902.59749 $ & $  -0.00169 $ & $   0.00075 $ & $  10.66286 $ & $ i$\\
$ 54902.59799 $ & $  -0.00139 $ & $   0.00075 $ & $  10.66200 $ & $ i$\\
$ 54902.59848 $ & $  -0.00469 $ & $   0.00075 $ & $  10.65893 $ & $ i$\\
$ 54902.59919 $ & $   0.00281 $ & $   0.00075 $ & $  10.66596 $ & $ i$\\
$ 54902.59970 $ & $  -0.00108 $ & $   0.00075 $ & $  10.66316 $ & $ i$\\
$ 54902.60020 $ & $   0.00141 $ & $   0.00075 $ & $  10.66524 $ & $ i$\\
$ 54902.60089 $ & $   0.00440 $ & $   0.00075 $ & $  10.66726 $ & $ i$\\
$ 54902.60139 $ & $   0.00040 $ & $   0.00075 $ & $  10.66424 $ & $ i$\\
$ 54902.60190 $ & $  -0.00064 $ & $   0.00075 $ & $  10.66234 $ & $ i$\\
$ 54902.60259 $ & $  -0.00009 $ & $   0.00075 $ & $  10.66388 $ & $ i$\\


==> HTR267-010_rvtable.tex <==
$ 934.84149 $ \dotfill & $ -1139.51 $ & $     2.94 $ & \nodata      & \nodata      & \nodata      & \nodata     \\
$ 954.82485 $ \dotfill & \nodata      & \nodata      & $    -8.00 $ & $     3.22 $ & $     2.051 $ & $     0.075 $\\
$ 954.83175 $ \dotfill & $  -942.88 $ & $     2.24 $ & $   -18.65 $ & $     8.02 $ & $     2.900 $ & $     0.035 $\\
$ 956.80481 $ \dotfill & $  1092.32 $ & $     2.28 $ & $   -42.21 $ & $    10.81 $ & $     3.305 $ & $     0.018 $\\
$ 983.73851 $ \dotfill & $ -1151.02 $ & $     2.39 $ & $    18.53 $ & $     4.51 $ & $     2.853 $ & $     0.016 $\\
$ 984.74064 $ \dotfill & $   328.09 $ & $     2.14 $ & $     6.85 $ & $     6.11 $ & $     2.879 $ & $     0.016 $\\
$ 986.74296 $ \dotfill & $ -1225.77 $ & $     2.34 $ & $    15.28 $ & $     7.78 $ & $     2.588 $ & $     0.029 $\\
$ 1107.15226 $ \dotfill & $  -870.02 $ & $     4.89 $ & $    10.00 $ & $    17.65 $ & $     1.352 $ & $     0.043 $\\
$ 1109.05752 $ \dotfill & $  1233.55 $ & $     3.76 $ & $    -1.23 $ & $     7.66 $ & $     2.783 $ & $     0.018 $\\
$ 1191.10274 $ \dotfill & $ -1147.72 $ & $     2.07 $ & $    14.55 $ & $     6.16 $ & $     3.412 $ & $     0.016 $\\
$ 1192.11754 $ \dotfill & $  1100.72 $ & $     2.12 $ & $     4.88 $ & $     2.83 $ & $     3.346 $ & $     0.015 $\\


==> HTR341-004_phfu_tab.tex <==
$ 54632.73784 $ & $   0.02143 $ & $   0.00111 $ & $  10.98360 $ & $ i$\\
$ 54632.73870 $ & $   0.01830 $ & $   0.00116 $ & $  10.98170 $ & $ i$\\
$ 54632.73954 $ & $   0.01503 $ & $   0.00115 $ & $  10.97810 $ & $ i$\\
$ 54632.74039 $ & $   0.01859 $ & $   0.00115 $ & $  10.98340 $ & $ i$\\
$ 54632.74125 $ & $   0.01123 $ & $   0.00111 $ & $  10.97530 $ & $ i$\\
$ 54632.74208 $ & $   0.02006 $ & $   0.00109 $ & $  10.98390 $ & $ i$\\
$ 54632.74295 $ & $   0.01831 $ & $   0.00111 $ & $  10.98220 $ & $ i$\\
$ 54632.74381 $ & $   0.01766 $ & $   0.00114 $ & $  10.97840 $ & $ i$\\
$ 54632.74637 $ & $   0.02025 $ & $   0.00117 $ & $  10.99540 $ & $ i$\\
$ 54632.74722 $ & $   0.01556 $ & $   0.00112 $ & $  10.97990 $ & $ i$\\
$ 54632.74808 $ & $   0.01724 $ & $   0.00116 $ & $  10.98280 $ & $ i$\\
$ 54632.74895 $ & $   0.01475 $ & $   0.00109 $ & $  10.98060 $ & $ i$\\
$ 54632.74980 $ & $   0.01321 $ & $   0.00108 $ & $  10.97650 $ & $ i$\\
$ 54632.75065 $ & $   0.01507 $ & $   0.00112 $ & $  10.97880 $ & $ i$\\
$ 54632.75151 $ & $   0.01296 $ & $   0.00110 $ & $  10.97740 $ & $ i$\\
$ 54632.75234 $ & $   0.01438 $ & $   0.00108 $ & $  10.97970 $ & $ i$\\
$ 54632.75320 $ & $   0.01762 $ & $   0.00110 $ & $  10.98270 $ & $ i$\\
$ 54632.75403 $ & $   0.01104 $ & $   0.00114 $ & $  10.97500 $ & $ i$\\
$ 54632.75490 $ & $   0.01512 $ & $   0.00111 $ & $  10.97920 $ & $ i$\\
$ 54632.75574 $ & $   0.01700 $ & $   0.00108 $ & $  10.98170 $ & $ i$\\
$ 54632.75661 $ & $   0.01283 $ & $   0.00109 $ & $  10.97720 $ & $ i$\\
$ 54632.75743 $ & $   0.01697 $ & $   0.00117 $ & $  10.98140 $ & $ i$\\
$ 54632.75828 $ & $   0.01450 $ & $   0.00109 $ & $  10.98140 $ & $ i$\\
$ 54632.75914 $ & $   0.01598 $ & $   0.00107 $ & $  10.98020 $ & $ i$\\
$ 54632.75999 $ & $   0.01976 $ & $   0.00113 $ & $  10.98490 $ & $ i$\\
$ 54632.76085 $ & $   0.01389 $ & $   0.00108 $ & $  10.97820 $ & $ i$\\
$ 54632.76170 $ & $   0.01581 $ & $   0.00108 $ & $  10.98010 $ & $ i$\\
$ 54632.76255 $ & $   0.01369 $ & $   0.00106 $ & $  10.97850 $ & $ i$\\
$ 54632.76340 $ & $   0.01714 $ & $   0.00106 $ & $  10.98110 $ & $ i$\\
$ 54632.76426 $ & $   0.01521 $ & $   0.00107 $ & $  10.98010 $ & $ i$\\
$ 54632.76511 $ & $   0.00909 $ & $   0.00106 $ & $  10.97470 $ & $ i$\\
$ 54632.76595 $ & $   0.01176 $ & $   0.00111 $ & $  10.97760 $ & $ i$\\
$ 54632.76681 $ & $   0.01449 $ & $   0.00106 $ & $  10.98040 $ & $ i$\\
$ 54632.76764 $ & $   0.01143 $ & $   0.00106 $ & $  10.97520 $ & $ i$\\
$ 54632.76851 $ & $   0.01226 $ & $   0.00105 $ & $  10.97780 $ & $ i$\\
$ 54632.76934 $ & $   0.01304 $ & $   0.00105 $ & $  10.97760 $ & $ i$\\
$ 54632.77020 $ & $   0.00825 $ & $   0.00106 $ & $  10.97360 $ & $ i$\\
$ 54632.77105 $ & $   0.00947 $ & $   0.00104 $ & $  10.97460 $ & $ i$\\
$ 54632.77191 $ & $   0.00774 $ & $   0.00106 $ & $  10.97270 $ & $ i$\\
$ 54632.77277 $ & $   0.00702 $ & $   0.00104 $ & $  10.97060 $ & $ i$\\
$ 54632.77362 $ & $   0.00306 $ & $   0.00103 $ & $  10.96800 $ & $ i$\\
$ 54632.77448 $ & $   0.00161 $ & $   0.00104 $ & $  10.96700 $ & $ i$\\
$ 54632.77533 $ & $   0.00490 $ & $   0.00104 $ & $  10.97030 $ & $ i$\\
$ 54632.77619 $ & $   0.00031 $ & $   0.00106 $ & $  10.96480 $ & $ i$\\
$ 54632.77704 $ & $  -0.00155 $ & $   0.00103 $ & $  10.96350 $ & $ i$\\
$ 54632.77791 $ & $   0.00291 $ & $   0.00104 $ & $  10.96860 $ & $ i$\\
$ 54632.77876 $ & $   0.00162 $ & $   0.00106 $ & $  10.96590 $ & $ i$\\
$ 54632.77962 $ & $   0.00074 $ & $   0.00102 $ & $  10.96580 $ & $ i$\\
$ 54632.78049 $ & $   0.00396 $ & $   0.00103 $ & $  10.96940 $ & $ i$\\
$ 54632.78133 $ & $   0.00224 $ & $   0.00103 $ & $  10.96650 $ & $ i$\\
$ 54632.78220 $ & $   0.00264 $ & $   0.00102 $ & $  10.96700 $ & $ i$\\
$ 54632.78305 $ & $  -0.00070 $ & $   0.00102 $ & $  10.96510 $ & $ i$\\
$ 54632.78391 $ & $   0.00148 $ & $   0.00106 $ & $  10.96640 $ & $ i$\\
$ 54632.78478 $ & $  -0.00058 $ & $   0.00103 $ & $  10.96570 $ & $ i$\\
$ 54632.78565 $ & $   0.00331 $ & $   0.00102 $ & $  10.96930 $ & $ i$\\
$ 54632.78650 $ & $   0.00100 $ & $   0.00099 $ & $  10.96550 $ & $ i$\\
$ 54632.78734 $ & $  -0.00105 $ & $   0.00100 $ & $  10.96460 $ & $ i$\\
$ 54632.78820 $ & $  -0.00081 $ & $   0.00101 $ & $  10.96510 $ & $ i$\\
$ 54632.78903 $ & $  -0.00069 $ & $   0.00100 $ & $  10.96560 $ & $ i$\\
$ 54632.78989 $ & $   0.00253 $ & $   0.00100 $ & $  10.96760 $ & $ i$\\
$ 54632.79073 $ & $  -0.00012 $ & $   0.00100 $ & $  10.96490 $ & $ i$\\
$ 54632.79159 $ & $   0.00211 $ & $   0.00100 $ & $  10.96790 $ & $ i$\\
$ 54632.79246 $ & $  -0.00089 $ & $   0.00099 $ & $  10.96460 $ & $ i$\\
$ 54632.79330 $ & $   0.00008 $ & $   0.00101 $ & $  10.96570 $ & $ i$\\
$ 54632.79415 $ & $  -0.00045 $ & $   0.00100 $ & $  10.96460 $ & $ i$\\
$ 54632.79499 $ & $   0.00041 $ & $   0.00099 $ & $  10.96530 $ & $ i$\\
$ 54632.79587 $ & $   0.00104 $ & $   0.00099 $ & $  10.96720 $ & $ i$\\
$ 54632.79673 $ & $  -0.00196 $ & $   0.00099 $ & $  10.96320 $ & $ i$\\
$ 54632.79757 $ & $   0.00045 $ & $   0.00100 $ & $  10.96600 $ & $ i$\\
$ 54632.79843 $ & $   0.00198 $ & $   0.00099 $ & $  10.96720 $ & $ i$\\
$ 54632.79929 $ & $  -0.00132 $ & $   0.00100 $ & $  10.96460 $ & $ i$\\
$ 54632.80013 $ & $   0.00283 $ & $   0.00101 $ & $  10.96880 $ & $ i$\\
$ 54632.80100 $ & $  -0.00079 $ & $   0.00100 $ & $  10.96480 $ & $ i$\\
$ 54632.80187 $ & $  -0.00036 $ & $   0.00099 $ & $  10.96510 $ & $ i$\\
$ 54632.80270 $ & $  -0.00233 $ & $   0.00099 $ & $  10.96350 $ & $ i$\\
$ 54632.80355 $ & $  -0.00133 $ & $   0.00100 $ & $  10.96440 $ & $ i$\\
$ 54632.80439 $ & $   0.00386 $ & $   0.00099 $ & $  10.96880 $ & $ i$\\
$ 54632.80525 $ & $  -0.00010 $ & $   0.00098 $ & $  10.96620 $ & $ i$\\
$ 54632.80611 $ & $  -0.00212 $ & $   0.00099 $ & $  10.96420 $ & $ i$\\
$ 54632.80696 $ & $   0.00028 $ & $   0.00099 $ & $  10.96620 $ & $ i$\\
$ 54632.80782 $ & $  -0.00085 $ & $   0.00099 $ & $  10.96430 $ & $ i$\\
$ 54632.80867 $ & $  -0.00127 $ & $   0.00099 $ & $  10.96510 $ & $ i$\\
$ 54632.80952 $ & $   0.00059 $ & $   0.00100 $ & $  10.96540 $ & $ i$\\
$ 54632.81039 $ & $  -0.00070 $ & $   0.00099 $ & $  10.96550 $ & $ i$\\
$ 54632.81124 $ & $   0.00171 $ & $   0.00098 $ & $  10.96700 $ & $ i$\\
$ 54632.81209 $ & $   0.00043 $ & $   0.00098 $ & $  10.96590 $ & $ i$\\
$ 54632.81294 $ & $  -0.00091 $ & $   0.00098 $ & $  10.96440 $ & $ i$\\
$ 54632.81378 $ & $   0.00155 $ & $   0.00098 $ & $  10.96640 $ & $ i$\\
$ 54632.81466 $ & $   0.00290 $ & $   0.00098 $ & $  10.96780 $ & $ i$\\
$ 54632.81549 $ & $  -0.00082 $ & $   0.00098 $ & $  10.96450 $ & $ i$\\
$ 54632.81635 $ & $   0.00033 $ & $   0.00097 $ & $  10.96590 $ & $ i$\\
$ 54632.81720 $ & $  -0.00083 $ & $   0.00097 $ & $  10.96440 $ & $ i$\\
$ 54632.81806 $ & $  -0.00026 $ & $   0.00098 $ & $  10.96490 $ & $ i$\\
$ 54632.81891 $ & $  -0.00150 $ & $   0.00097 $ & $  10.96290 $ & $ i$\\
$ 54632.81976 $ & $   0.00000 $ & $   0.00097 $ & $  10.96400 $ & $ i$\\
$ 54632.82061 $ & $   0.00030 $ & $   0.00097 $ & $  10.96490 $ & $ i$\\
$ 54632.82144 $ & $   0.00081 $ & $   0.00097 $ & $  10.96420 $ & $ i$\\
$ 54632.82231 $ & $   0.00001 $ & $   0.00096 $ & $  10.96400 $ & $ i$\\
$ 54632.82316 $ & $  -0.00103 $ & $   0.00098 $ & $  10.96390 $ & $ i$\\
$ 54632.82401 $ & $   0.00023 $ & $   0.00098 $ & $  10.96440 $ & $ i$\\
$ 54632.82484 $ & $  -0.00185 $ & $   0.00097 $ & $  10.96300 $ & $ i$\\
$ 54632.82570 $ & $  -0.00302 $ & $   0.00096 $ & $  10.96090 $ & $ i$\\
$ 54632.82654 $ & $   0.00050 $ & $   0.00097 $ & $  10.96500 $ & $ i$\\
$ 54632.82738 $ & $   0.00198 $ & $   0.00096 $ & $  10.96660 $ & $ i$\\
$ 54632.82825 $ & $   0.00012 $ & $   0.00097 $ & $  10.96520 $ & $ i$\\
$ 54632.82909 $ & $  -0.00113 $ & $   0.00097 $ & $  10.96390 $ & $ i$\\
$ 54632.82995 $ & $   0.00025 $ & $   0.00097 $ & $  10.96470 $ & $ i$\\
$ 54632.83079 $ & $  -0.00121 $ & $   0.00096 $ & $  10.96390 $ & $ i$\\
$ 54632.83166 $ & $  -0.00298 $ & $   0.00095 $ & $  10.96220 $ & $ i$\\
$ 54632.83252 $ & $  -0.00086 $ & $   0.00096 $ & $  10.96400 $ & $ i$\\
$ 54632.83336 $ & $   0.00066 $ & $   0.00096 $ & $  10.96570 $ & $ i$\\
$ 54632.83421 $ & $   0.00125 $ & $   0.00097 $ & $  10.96610 $ & $ i$\\
$ 54632.83505 $ & $   0.00121 $ & $   0.00097 $ & $  10.96640 $ & $ i$\\
$ 54632.83591 $ & $   0.00065 $ & $   0.00097 $ & $  10.96520 $ & $ i$\\
$ 54632.83675 $ & $  -0.00010 $ & $   0.00096 $ & $  10.96400 $ & $ i$\\
$ 54632.83762 $ & $  -0.00143 $ & $   0.00096 $ & $  10.96340 $ & $ i$\\
$ 54632.83848 $ & $  -0.00243 $ & $   0.00096 $ & $  10.96310 $ & $ i$\\
$ 54632.83932 $ & $  -0.00043 $ & $   0.00096 $ & $  10.96450 $ & $ i$\\
$ 54632.84018 $ & $  -0.00249 $ & $   0.00095 $ & $  10.96190 $ & $ i$\\
$ 54632.84104 $ & $  -0.00137 $ & $   0.00096 $ & $  10.96330 $ & $ i$\\
$ 54632.84190 $ & $  -0.00047 $ & $   0.00096 $ & $  10.96450 $ & $ i$\\
$ 54632.84274 $ & $  -0.00212 $ & $   0.00096 $ & $  10.96190 $ & $ i$\\
$ 54632.84361 $ & $  -0.00140 $ & $   0.00095 $ & $  10.96360 $ & $ i$\\
$ 54632.84447 $ & $   0.00072 $ & $   0.00095 $ & $  10.96550 $ & $ i$\\
$ 54632.84533 $ & $  -0.00043 $ & $   0.00095 $ & $  10.96370 $ & $ i$\\
$ 54632.84619 $ & $   0.00067 $ & $   0.00096 $ & $  10.96450 $ & $ i$\\
$ 54632.84704 $ & $  -0.00012 $ & $   0.00096 $ & $  10.96420 $ & $ i$\\
$ 54632.84793 $ & $  -0.00036 $ & $   0.00096 $ & $  10.96400 $ & $ i$\\
$ 54632.84878 $ & $   0.00004 $ & $   0.00095 $ & $  10.96430 $ & $ i$\\
$ 54632.84964 $ & $   0.00213 $ & $   0.00095 $ & $  10.96580 $ & $ i$\\
$ 54632.85050 $ & $  -0.00059 $ & $   0.00095 $ & $  10.96350 $ & $ i$\\
$ 54632.85140 $ & $   0.00164 $ & $   0.00096 $ & $  10.96540 $ & $ i$\\
$ 54632.85225 $ & $   0.00228 $ & $   0.00095 $ & $  10.96630 $ & $ i$\\
$ 54632.85311 $ & $   0.00091 $ & $   0.00095 $ & $  10.96380 $ & $ i$\\
$ 54632.85399 $ & $  -0.00082 $ & $   0.00096 $ & $  10.96320 $ & $ i$\\
$ 54632.85484 $ & $   0.00254 $ & $   0.00095 $ & $  10.96560 $ & $ i$\\
$ 54632.85570 $ & $  -0.00164 $ & $   0.00096 $ & $  10.96180 $ & $ i$\\
$ 54632.85656 $ & $  -0.00039 $ & $   0.00095 $ & $  10.96360 $ & $ i$\\
$ 54632.85743 $ & $   0.00197 $ & $   0.00096 $ & $  10.96580 $ & $ i$\\
$ 54632.85829 $ & $  -0.00108 $ & $   0.00096 $ & $  10.96260 $ & $ i$\\
$ 54632.85915 $ & $  -0.00247 $ & $   0.00095 $ & $  10.96150 $ & $ i$\\
$ 54632.85998 $ & $   0.00170 $ & $   0.00095 $ & $  10.96510 $ & $ i$\\
$ 54632.86082 $ & $  -0.00034 $ & $   0.00096 $ & $  10.96380 $ & $ i$\\
$ 54632.86168 $ & $   0.00080 $ & $   0.00095 $ & $  10.96490 $ & $ i$\\
$ 54632.86253 $ & $  -0.00082 $ & $   0.00095 $ & $  10.96290 $ & $ i$\\
$ 54632.86339 $ & $   0.00316 $ & $   0.00095 $ & $  10.96660 $ & $ i$\\
$ 54718.66507 $ & $   0.00010 $ & $   0.00084 $ & $  10.66080 $ & $ i$\\
$ 54718.66871 $ & $  -0.00031 $ & $   0.00086 $ & $  10.65910 $ & $ i$\\
$ 54718.66957 $ & $  -0.00086 $ & $   0.00085 $ & $  10.65980 $ & $ i$\\
$ 54718.67040 $ & $  -0.00173 $ & $   0.00085 $ & $  10.65890 $ & $ i$\\
$ 54718.67127 $ & $   0.00079 $ & $   0.00085 $ & $  10.66090 $ & $ i$\\
$ 54718.67210 $ & $  -0.00111 $ & $   0.00086 $ & $  10.65900 $ & $ i$\\
$ 54718.67297 $ & $  -0.00100 $ & $   0.00086 $ & $  10.65860 $ & $ i$\\
$ 54718.67381 $ & $  -0.00043 $ & $   0.00086 $ & $  10.65950 $ & $ i$\\
$ 54718.67467 $ & $   0.00083 $ & $   0.00085 $ & $  10.66040 $ & $ i$\\
$ 54718.67553 $ & $  -0.00200 $ & $   0.00086 $ & $  10.65810 $ & $ i$\\
$ 54718.67637 $ & $   0.00097 $ & $   0.00085 $ & $  10.66110 $ & $ i$\\
$ 54718.67725 $ & $  -0.00123 $ & $   0.00085 $ & $  10.65850 $ & $ i$\\
$ 54718.67808 $ & $  -0.00060 $ & $   0.00085 $ & $  10.65940 $ & $ i$\\
$ 54718.67893 $ & $   0.00105 $ & $   0.00085 $ & $  10.66140 $ & $ i$\\
$ 54718.67978 $ & $   0.00053 $ & $   0.00085 $ & $  10.66020 $ & $ i$\\
$ 54718.68065 $ & $   0.00044 $ & $   0.00086 $ & $  10.65950 $ & $ i$\\
$ 54718.68152 $ & $  -0.00042 $ & $   0.00086 $ & $  10.65950 $ & $ i$\\
$ 54718.68237 $ & $  -0.00114 $ & $   0.00085 $ & $  10.65910 $ & $ i$\\
$ 54718.68321 $ & $  -0.00018 $ & $   0.00085 $ & $  10.65990 $ & $ i$\\
$ 54718.68407 $ & $  -0.00287 $ & $   0.00086 $ & $  10.65750 $ & $ i$\\
$ 54718.68492 $ & $   0.00116 $ & $   0.00086 $ & $  10.66120 $ & $ i$\\
$ 54718.68608 $ & $   0.00378 $ & $   0.00086 $ & $  10.66280 $ & $ i$\\
$ 54718.68900 $ & $   0.00050 $ & $   0.00086 $ & $  10.65890 $ & $ i$\\
$ 54718.68985 $ & $   0.00104 $ & $   0.00087 $ & $  10.65930 $ & $ i$\\
$ 54718.69072 $ & $   0.00144 $ & $   0.00086 $ & $  10.65990 $ & $ i$\\
$ 54718.69158 $ & $  -0.00034 $ & $   0.00086 $ & $  10.65820 $ & $ i$\\
$ 54718.69241 $ & $   0.00082 $ & $   0.00087 $ & $  10.65930 $ & $ i$\\
$ 54718.69329 $ & $   0.00187 $ & $   0.00086 $ & $  10.66090 $ & $ i$\\
$ 54718.69412 $ & $  -0.00089 $ & $   0.00086 $ & $  10.65740 $ & $ i$\\
$ 54718.69498 $ & $  -0.00002 $ & $   0.00086 $ & $  10.65860 $ & $ i$\\
$ 54718.69585 $ & $  -0.00186 $ & $   0.00085 $ & $  10.65740 $ & $ i$\\
$ 54718.69673 $ & $   0.00077 $ & $   0.00087 $ & $  10.65960 $ & $ i$\\
$ 54718.69757 $ & $  -0.00026 $ & $   0.00087 $ & $  10.65840 $ & $ i$\\
$ 54718.69842 $ & $   0.00219 $ & $   0.00086 $ & $  10.66060 $ & $ i$\\
$ 54718.69929 $ & $  -0.00236 $ & $   0.00087 $ & $  10.65670 $ & $ i$\\
$ 54718.70013 $ & $   0.00015 $ & $   0.00085 $ & $  10.65900 $ & $ i$\\
$ 54718.70098 $ & $   0.00065 $ & $   0.00086 $ & $  10.65910 $ & $ i$\\
$ 54718.70183 $ & $   0.00162 $ & $   0.00086 $ & $  10.66000 $ & $ i$\\
$ 54718.70268 $ & $   0.00055 $ & $   0.00085 $ & $  10.65880 $ & $ i$\\
$ 54718.70354 $ & $  -0.00032 $ & $   0.00087 $ & $  10.65850 $ & $ i$\\
$ 54718.70441 $ & $   0.00103 $ & $   0.00088 $ & $  10.65800 $ & $ i$\\
$ 54718.70526 $ & $   0.00197 $ & $   0.00088 $ & $  10.65820 $ & $ i$\\
$ 54718.70669 $ & $  -0.00148 $ & $   0.00087 $ & $  10.65570 $ & $ i$\\
$ 54718.70755 $ & $   0.00041 $ & $   0.00088 $ & $  10.65770 $ & $ i$\\
$ 54718.70842 $ & $   0.00007 $ & $   0.00089 $ & $  10.65750 $ & $ i$\\
$ 54718.70927 $ & $  -0.00006 $ & $   0.00088 $ & $  10.65730 $ & $ i$\\
$ 54718.71014 $ & $  -0.00078 $ & $   0.00086 $ & $  10.65670 $ & $ i$\\
$ 54718.71099 $ & $   0.00193 $ & $   0.00087 $ & $  10.65920 $ & $ i$\\
$ 54718.71183 $ & $  -0.00135 $ & $   0.00087 $ & $  10.65700 $ & $ i$\\
$ 54718.71270 $ & $  -0.00055 $ & $   0.00088 $ & $  10.65740 $ & $ i$\\
$ 54718.71354 $ & $   0.00012 $ & $   0.00087 $ & $  10.65810 $ & $ i$\\
$ 54718.71439 $ & $   0.00014 $ & $   0.00087 $ & $  10.65820 $ & $ i$\\
$ 54718.71522 $ & $   0.00187 $ & $   0.00087 $ & $  10.65990 $ & $ i$\\
$ 54718.71609 $ & $   0.00128 $ & $   0.00087 $ & $  10.65890 $ & $ i$\\
$ 54718.71694 $ & $  -0.00123 $ & $   0.00088 $ & $  10.65740 $ & $ i$\\
$ 54718.71779 $ & $   0.00009 $ & $   0.00088 $ & $  10.65920 $ & $ i$\\
$ 54718.71864 $ & $   0.00036 $ & $   0.00087 $ & $  10.65900 $ & $ i$\\
$ 54718.71951 $ & $   0.00101 $ & $   0.00087 $ & $  10.65900 $ & $ i$\\
$ 54718.72034 $ & $  -0.00262 $ & $   0.00088 $ & $  10.65670 $ & $ i$\\
$ 54718.72121 $ & $   0.00120 $ & $   0.00087 $ & $  10.66000 $ & $ i$\\
$ 54718.72206 $ & $  -0.00046 $ & $   0.00087 $ & $  10.65760 $ & $ i$\\
$ 54718.72292 $ & $  -0.00070 $ & $   0.00086 $ & $  10.65780 $ & $ i$\\
$ 54718.72511 $ & $  -0.00069 $ & $   0.00087 $ & $  10.65800 $ & $ i$\\
$ 54718.72597 $ & $  -0.00206 $ & $   0.00086 $ & $  10.65600 $ & $ i$\\
$ 54718.72684 $ & $  -0.00020 $ & $   0.00086 $ & $  10.65880 $ & $ i$\\
$ 54718.72769 $ & $  -0.00087 $ & $   0.00086 $ & $  10.65720 $ & $ i$\\
$ 54718.72854 $ & $   0.00065 $ & $   0.00088 $ & $  10.65850 $ & $ i$\\
$ 54718.72941 $ & $   0.00337 $ & $   0.00087 $ & $  10.66190 $ & $ i$\\
$ 54718.73026 $ & $  -0.00097 $ & $   0.00085 $ & $  10.65730 $ & $ i$\\
$ 54718.73110 $ & $   0.00051 $ & $   0.00087 $ & $  10.65880 $ & $ i$\\
$ 54718.73196 $ & $   0.00179 $ & $   0.00087 $ & $  10.65950 $ & $ i$\\
$ 54718.73280 $ & $  -0.00203 $ & $   0.00087 $ & $  10.65660 $ & $ i$\\
$ 54718.73366 $ & $   0.00031 $ & $   0.00086 $ & $  10.65860 $ & $ i$\\
$ 54718.73453 $ & $  -0.00018 $ & $   0.00087 $ & $  10.65870 $ & $ i$\\
$ 54718.73537 $ & $   0.00048 $ & $   0.00087 $ & $  10.65880 $ & $ i$\\
$ 54718.73622 $ & $  -0.00101 $ & $   0.00087 $ & $  10.65710 $ & $ i$\\
$ 54718.73709 $ & $   0.00105 $ & $   0.00087 $ & $  10.65970 $ & $ i$\\
$ 54718.73793 $ & $  -0.00069 $ & $   0.00086 $ & $  10.65790 $ & $ i$\\
$ 54718.73878 $ & $   0.00058 $ & $   0.00086 $ & $  10.65890 $ & $ i$\\
$ 54718.73963 $ & $  -0.00103 $ & $   0.00086 $ & $  10.65830 $ & $ i$\\
$ 54718.74048 $ & $  -0.00242 $ & $   0.00087 $ & $  10.65640 $ & $ i$\\
$ 54718.74132 $ & $   0.00060 $ & $   0.00087 $ & $  10.65870 $ & $ i$\\
$ 54718.74215 $ & $   0.00005 $ & $   0.00087 $ & $  10.65850 $ & $ i$\\
$ 54718.74302 $ & $   0.00016 $ & $   0.00086 $ & $  10.65890 $ & $ i$\\
$ 54718.74384 $ & $   0.00009 $ & $   0.00087 $ & $  10.65880 $ & $ i$\\
$ 54718.74469 $ & $   0.00200 $ & $   0.00086 $ & $  10.66070 $ & $ i$\\
$ 54718.74554 $ & $   0.00087 $ & $   0.00086 $ & $  10.65930 $ & $ i$\\
$ 54718.74638 $ & $  -0.00192 $ & $   0.00086 $ & $  10.65680 $ & $ i$\\
$ 54718.74725 $ & $   0.00004 $ & $   0.00087 $ & $  10.65860 $ & $ i$\\
$ 54718.74811 $ & $   0.00039 $ & $   0.00086 $ & $  10.65880 $ & $ i$\\
$ 54718.74896 $ & $  -0.00016 $ & $   0.00087 $ & $  10.65870 $ & $ i$\\
$ 54718.74983 $ & $  -0.00122 $ & $   0.00086 $ & $  10.65800 $ & $ i$\\
$ 54718.75066 $ & $  -0.00028 $ & $   0.00086 $ & $  10.65860 $ & $ i$\\
$ 54718.75153 $ & $  -0.00069 $ & $   0.00086 $ & $  10.65780 $ & $ i$\\
$ 54718.75237 $ & $  -0.00051 $ & $   0.00086 $ & $  10.65910 $ & $ i$\\
$ 54718.75322 $ & $  -0.00111 $ & $   0.00086 $ & $  10.65820 $ & $ i$\\
$ 54718.75408 $ & $   0.00058 $ & $   0.00086 $ & $  10.65990 $ & $ i$\\
$ 54718.75493 $ & $   0.00145 $ & $   0.00086 $ & $  10.66040 $ & $ i$\\
$ 54718.75576 $ & $   0.00248 $ & $   0.00085 $ & $  10.66130 $ & $ i$\\
$ 54718.75663 $ & $   0.00024 $ & $   0.00086 $ & $  10.65880 $ & $ i$\\
$ 54718.75748 $ & $  -0.00148 $ & $   0.00087 $ & $  10.65790 $ & $ i$\\
$ 54718.75833 $ & $   0.00034 $ & $   0.00087 $ & $  10.66000 $ & $ i$\\
$ 54718.75919 $ & $  -0.00014 $ & $   0.00086 $ & $  10.65880 $ & $ i$\\
$ 54718.76005 $ & $   0.00084 $ & $   0.00086 $ & $  10.66000 $ & $ i$\\
$ 54718.76089 $ & $  -0.00068 $ & $   0.00085 $ & $  10.65880 $ & $ i$\\
$ 54718.76176 $ & $  -0.00156 $ & $   0.00086 $ & $  10.65690 $ & $ i$\\
$ 54718.76259 $ & $  -0.00039 $ & $   0.00086 $ & $  10.65810 $ & $ i$\\
$ 54718.76343 $ & $  -0.00165 $ & $   0.00087 $ & $  10.65700 $ & $ i$\\
$ 54718.76429 $ & $   0.00064 $ & $   0.00085 $ & $  10.65940 $ & $ i$\\
$ 54718.76516 $ & $   0.00234 $ & $   0.00087 $ & $  10.66080 $ & $ i$\\
$ 54718.76601 $ & $  -0.00154 $ & $   0.00086 $ & $  10.65700 $ & $ i$\\
$ 54718.76686 $ & $   0.00115 $ & $   0.00088 $ & $  10.65960 $ & $ i$\\
$ 54718.76772 $ & $  -0.00059 $ & $   0.00086 $ & $  10.65810 $ & $ i$\\
$ 54718.76858 $ & $   0.00222 $ & $   0.00087 $ & $  10.66070 $ & $ i$\\
$ 54718.76941 $ & $  -0.00022 $ & $   0.00087 $ & $  10.65820 $ & $ i$\\
$ 54718.77028 $ & $   0.00049 $ & $   0.00088 $ & $  10.65890 $ & $ i$\\
$ 54718.77112 $ & $   0.00107 $ & $   0.00086 $ & $  10.65870 $ & $ i$\\
$ 54718.77197 $ & $   0.00236 $ & $   0.00087 $ & $  10.66070 $ & $ i$\\
$ 54718.77281 $ & $   0.00259 $ & $   0.00087 $ & $  10.66090 $ & $ i$\\
$ 54718.77368 $ & $   0.00058 $ & $   0.00086 $ & $  10.65900 $ & $ i$\\
$ 54718.77453 $ & $   0.00026 $ & $   0.00087 $ & $  10.65920 $ & $ i$\\
$ 54718.77537 $ & $  -0.00128 $ & $   0.00087 $ & $  10.65740 $ & $ i$\\
$ 54718.77774 $ & $  -0.00031 $ & $   0.00088 $ & $  10.65810 $ & $ i$\\
$ 54718.77999 $ & $  -0.00154 $ & $   0.00088 $ & $  10.65610 $ & $ i$\\
$ 54718.78081 $ & $   0.00009 $ & $   0.00087 $ & $  10.65830 $ & $ i$\\
$ 54718.78167 $ & $   0.00052 $ & $   0.00086 $ & $  10.65810 $ & $ i$\\
$ 54718.78252 $ & $  -0.00354 $ & $   0.00085 $ & $  10.65460 $ & $ i$\\
$ 54718.78337 $ & $   0.00079 $ & $   0.00088 $ & $  10.65870 $ & $ i$\\
$ 54718.78421 $ & $   0.00015 $ & $   0.00087 $ & $  10.65780 $ & $ i$\\
$ 54718.78508 $ & $  -0.00193 $ & $   0.00087 $ & $  10.65620 $ & $ i$\\
$ 54718.78593 $ & $  -0.00153 $ & $   0.00086 $ & $  10.65580 $ & $ i$\\
$ 54718.78679 $ & $   0.00240 $ & $   0.00089 $ & $  10.65950 $ & $ i$\\
$ 54718.78765 $ & $  -0.00072 $ & $   0.00088 $ & $  10.65710 $ & $ i$\\
$ 54718.78847 $ & $  -0.00073 $ & $   0.00088 $ & $  10.65640 $ & $ i$\\
$ 54718.78932 $ & $   0.00139 $ & $   0.00087 $ & $  10.65900 $ & $ i$\\
$ 54718.79017 $ & $   0.00047 $ & $   0.00089 $ & $  10.65790 $ & $ i$\\
$ 54718.79102 $ & $  -0.00079 $ & $   0.00089 $ & $  10.65640 $ & $ i$\\
$ 54718.79191 $ & $   0.00048 $ & $   0.00087 $ & $  10.65810 $ & $ i$\\
$ 54718.79275 $ & $  -0.00174 $ & $   0.00089 $ & $  10.65590 $ & $ i$\\
$ 54718.79361 $ & $  -0.00001 $ & $   0.00087 $ & $  10.65720 $ & $ i$\\
$ 54718.79445 $ & $  -0.00053 $ & $   0.00088 $ & $  10.65640 $ & $ i$\\
$ 54718.79531 $ & $   0.00095 $ & $   0.00088 $ & $  10.65770 $ & $ i$\\
$ 54718.79616 $ & $  -0.00053 $ & $   0.00087 $ & $  10.65640 $ & $ i$\\
$ 54718.79702 $ & $   0.00134 $ & $   0.00087 $ & $  10.65880 $ & $ i$\\
$ 54718.79787 $ & $  -0.00129 $ & $   0.00088 $ & $  10.65600 $ & $ i$\\
$ 54718.79873 $ & $  -0.00114 $ & $   0.00087 $ & $  10.65660 $ & $ i$\\
$ 54718.79958 $ & $   0.00080 $ & $   0.00089 $ & $  10.65790 $ & $ i$\\
$ 54718.80043 $ & $  -0.00228 $ & $   0.00088 $ & $  10.65530 $ & $ i$\\
$ 54718.80128 $ & $   0.00011 $ & $   0.00087 $ & $  10.65830 $ & $ i$\\
$ 54718.80213 $ & $  -0.00398 $ & $   0.00086 $ & $  10.65410 $ & $ i$\\
$ 54718.80297 $ & $   0.00135 $ & $   0.00086 $ & $  10.65880 $ & $ i$\\
$ 54718.80384 $ & $  -0.00033 $ & $   0.00088 $ & $  10.65730 $ & $ i$\\
$ 54718.80469 $ & $   0.00145 $ & $   0.00087 $ & $  10.65880 $ & $ i$\\
$ 54718.80553 $ & $   0.00209 $ & $   0.00087 $ & $  10.65940 $ & $ i$\\
$ 54718.80639 $ & $   0.00340 $ & $   0.00088 $ & $  10.66160 $ & $ i$\\
$ 54718.80722 $ & $   0.00497 $ & $   0.00088 $ & $  10.66200 $ & $ i$\\
$ 54718.80809 $ & $   0.00813 $ & $   0.00089 $ & $  10.66600 $ & $ i$\\
$ 54718.80893 $ & $   0.00590 $ & $   0.00087 $ & $  10.66360 $ & $ i$\\
$ 54718.80978 $ & $   0.00722 $ & $   0.00088 $ & $  10.66500 $ & $ i$\\
$ 54718.81065 $ & $   0.01331 $ & $   0.00088 $ & $  10.67040 $ & $ i$\\
$ 54718.81149 $ & $   0.01268 $ & $   0.00087 $ & $  10.67020 $ & $ i$\\
$ 54718.81237 $ & $   0.01266 $ & $   0.00088 $ & $  10.67050 $ & $ i$\\
$ 54718.81324 $ & $   0.01557 $ & $   0.00088 $ & $  10.67380 $ & $ i$\\
$ 54718.81408 $ & $   0.01406 $ & $   0.00088 $ & $  10.67210 $ & $ i$\\
$ 54718.81495 $ & $   0.01211 $ & $   0.00088 $ & $  10.67000 $ & $ i$\\
$ 54718.81580 $ & $   0.01269 $ & $   0.00088 $ & $  10.67100 $ & $ i$\\
$ 54718.81665 $ & $   0.01543 $ & $   0.00089 $ & $  10.67310 $ & $ i$\\
$ 54718.81750 $ & $   0.01514 $ & $   0.00089 $ & $  10.67280 $ & $ i$\\
$ 54718.81834 $ & $   0.01648 $ & $   0.00088 $ & $  10.67340 $ & $ i$\\
$ 54718.81920 $ & $   0.01618 $ & $   0.00088 $ & $  10.67400 $ & $ i$\\
$ 54718.82006 $ & $   0.01710 $ & $   0.00088 $ & $  10.67390 $ & $ i$\\
$ 54718.82091 $ & $   0.01448 $ & $   0.00088 $ & $  10.67200 $ & $ i$\\
$ 54718.82178 $ & $   0.01931 $ & $   0.00089 $ & $  10.67740 $ & $ i$\\
$ 54718.82264 $ & $   0.01896 $ & $   0.00088 $ & $  10.67670 $ & $ i$\\
$ 54718.82350 $ & $   0.01645 $ & $   0.00089 $ & $  10.67440 $ & $ i$\\
$ 54718.82434 $ & $   0.01433 $ & $   0.00088 $ & $  10.67240 $ & $ i$\\
$ 54718.82519 $ & $   0.01806 $ & $   0.00087 $ & $  10.67570 $ & $ i$\\
$ 54718.82605 $ & $   0.01470 $ & $   0.00089 $ & $  10.67250 $ & $ i$\\
$ 54718.82691 $ & $   0.01572 $ & $   0.00088 $ & $  10.67360 $ & $ i$\\
$ 54718.82778 $ & $   0.01787 $ & $   0.00088 $ & $  10.67590 $ & $ i$\\
$ 54718.82863 $ & $   0.01653 $ & $   0.00089 $ & $  10.67440 $ & $ i$\\
$ 54718.82947 $ & $   0.01646 $ & $   0.00089 $ & $  10.67530 $ & $ i$\\
$ 54718.83033 $ & $   0.01768 $ & $   0.00089 $ & $  10.67550 $ & $ i$\\
$ 54718.83119 $ & $   0.01698 $ & $   0.00088 $ & $  10.67450 $ & $ i$\\
$ 54718.83203 $ & $   0.01654 $ & $   0.00089 $ & $  10.67490 $ & $ i$\\
$ 54718.83290 $ & $   0.01727 $ & $   0.00089 $ & $  10.67560 $ & $ i$\\
$ 54718.83374 $ & $   0.01505 $ & $   0.00089 $ & $  10.67300 $ & $ i$\\
$ 54718.83460 $ & $   0.01853 $ & $   0.00089 $ & $  10.67630 $ & $ i$\\
$ 54718.83545 $ & $   0.01794 $ & $   0.00089 $ & $  10.67570 $ & $ i$\\
$ 54718.83629 $ & $   0.01740 $ & $   0.00089 $ & $  10.67520 $ & $ i$\\
$ 54718.83715 $ & $   0.01635 $ & $   0.00088 $ & $  10.67470 $ & $ i$\\
$ 54718.83801 $ & $   0.01598 $ & $   0.00089 $ & $  10.67310 $ & $ i$\\
$ 54718.83886 $ & $   0.01616 $ & $   0.00090 $ & $  10.67420 $ & $ i$\\
$ 54718.83971 $ & $   0.01368 $ & $   0.00089 $ & $  10.67150 $ & $ i$\\
$ 54718.84056 $ & $   0.01957 $ & $   0.00089 $ & $  10.67660 $ & $ i$\\
$ 54718.84143 $ & $   0.01652 $ & $   0.00090 $ & $  10.67390 $ & $ i$\\
$ 54718.84225 $ & $   0.01708 $ & $   0.00090 $ & $  10.67430 $ & $ i$\\
$ 54718.84310 $ & $   0.01693 $ & $   0.00089 $ & $  10.67450 $ & $ i$\\
$ 54718.84396 $ & $   0.01903 $ & $   0.00090 $ & $  10.67700 $ & $ i$\\
$ 54718.84482 $ & $   0.01645 $ & $   0.00090 $ & $  10.67400 $ & $ i$\\
$ 54718.84567 $ & $   0.01783 $ & $   0.00090 $ & $  10.67650 $ & $ i$\\
$ 54718.84652 $ & $   0.01710 $ & $   0.00090 $ & $  10.67410 $ & $ i$\\
$ 54718.84737 $ & $   0.01863 $ & $   0.00091 $ & $  10.67690 $ & $ i$\\
$ 54718.84823 $ & $   0.01777 $ & $   0.00090 $ & $  10.67570 $ & $ i$\\
$ 54718.84908 $ & $   0.01732 $ & $   0.00090 $ & $  10.67430 $ & $ i$\\
$ 54718.84995 $ & $   0.01648 $ & $   0.00090 $ & $  10.67330 $ & $ i$\\
$ 54718.85081 $ & $   0.01593 $ & $   0.00091 $ & $  10.67330 $ & $ i$\\
$ 54718.85249 $ & $   0.01843 $ & $   0.00091 $ & $  10.67630 $ & $ i$\\
$ 54718.85419 $ & $   0.01562 $ & $   0.00092 $ & $  10.67170 $ & $ i$\\
$ 54718.85504 $ & $   0.01534 $ & $   0.00090 $ & $  10.67230 $ & $ i$\\
$ 54718.85589 $ & $   0.01780 $ & $   0.00091 $ & $  10.67520 $ & $ i$\\
$ 54718.85676 $ & $   0.01808 $ & $   0.00092 $ & $  10.67620 $ & $ i$\\
$ 54718.85759 $ & $   0.01561 $ & $   0.00091 $ & $  10.67370 $ & $ i$\\
$ 54718.85846 $ & $   0.01835 $ & $   0.00092 $ & $  10.67560 $ & $ i$\\
$ 54718.85928 $ & $   0.01893 $ & $   0.00092 $ & $  10.67650 $ & $ i$\\
$ 54718.86015 $ & $   0.01605 $ & $   0.00092 $ & $  10.67350 $ & $ i$\\
$ 54718.86098 $ & $   0.01646 $ & $   0.00092 $ & $  10.67400 $ & $ i$\\
$ 54718.86184 $ & $   0.01582 $ & $   0.00092 $ & $  10.67220 $ & $ i$\\
$ 54718.86268 $ & $   0.01554 $ & $   0.00092 $ & $  10.67420 $ & $ i$\\
$ 54718.86355 $ & $   0.01820 $ & $   0.00093 $ & $  10.67440 $ & $ i$\\
$ 54718.86439 $ & $   0.01658 $ & $   0.00091 $ & $  10.67390 $ & $ i$\\
$ 54718.86525 $ & $   0.01775 $ & $   0.00091 $ & $  10.67380 $ & $ i$\\
$ 54718.86611 $ & $   0.01965 $ & $   0.00091 $ & $  10.67740 $ & $ i$\\
$ 54718.86695 $ & $   0.01722 $ & $   0.00092 $ & $  10.67400 $ & $ i$\\
$ 54718.86781 $ & $   0.01630 $ & $   0.00092 $ & $  10.67400 $ & $ i$\\
$ 54718.86868 $ & $   0.01795 $ & $   0.00093 $ & $  10.67520 $ & $ i$\\
$ 54718.86952 $ & $   0.01669 $ & $   0.00093 $ & $  10.67360 $ & $ i$\\
$ 54718.87039 $ & $   0.01258 $ & $   0.00092 $ & $  10.67070 $ & $ i$\\
$ 54718.87122 $ & $   0.01374 $ & $   0.00093 $ & $  10.67170 $ & $ i$\\
$ 54718.87208 $ & $   0.01552 $ & $   0.00093 $ & $  10.67170 $ & $ i$\\
$ 54718.87294 $ & $   0.01729 $ & $   0.00092 $ & $  10.67380 $ & $ i$\\
$ 54718.87377 $ & $   0.01641 $ & $   0.00093 $ & $  10.67400 $ & $ i$\\
$ 54718.87464 $ & $   0.01244 $ & $   0.00094 $ & $  10.66900 $ & $ i$\\
$ 54718.87547 $ & $   0.01341 $ & $   0.00093 $ & $  10.67210 $ & $ i$\\
$ 54718.87633 $ & $   0.01336 $ & $   0.00092 $ & $  10.67060 $ & $ i$\\
$ 54718.87717 $ & $   0.01498 $ & $   0.00094 $ & $  10.67220 $ & $ i$\\
$ 54718.87804 $ & $   0.01475 $ & $   0.00092 $ & $  10.67200 $ & $ i$\\
$ 54718.87888 $ & $   0.01330 $ & $   0.00094 $ & $  10.66930 $ & $ i$\\
$ 54718.87973 $ & $   0.01590 $ & $   0.00092 $ & $  10.67280 $ & $ i$\\
$ 54718.88057 $ & $   0.01455 $ & $   0.00093 $ & $  10.67110 $ & $ i$\\
$ 54718.88142 $ & $   0.01315 $ & $   0.00094 $ & $  10.67070 $ & $ i$\\
$ 54718.88315 $ & $   0.01056 $ & $   0.00094 $ & $  10.66640 $ & $ i$\\
$ 54718.88556 $ & $   0.01029 $ & $   0.00094 $ & $  10.66130 $ & $ i$\\
$ 54718.88902 $ & $   0.00231 $ & $   0.00095 $ & $  10.61780 $ & $ i$\\
$ 54723.64023 $ & $  -0.00375 $ & $   0.00108 $ & $  10.66230 $ & $ i$\\
$ 54723.64107 $ & $  -0.00020 $ & $   0.00111 $ & $  10.66630 $ & $ i$\\
$ 54723.64194 $ & $  -0.00283 $ & $   0.00111 $ & $  10.66390 $ & $ i$\\
$ 54723.64281 $ & $  -0.00115 $ & $   0.00110 $ & $  10.66540 $ & $ i$\\
$ 54723.64365 $ & $  -0.00223 $ & $   0.00110 $ & $  10.66450 $ & $ i$\\
$ 54723.64452 $ & $  -0.00289 $ & $   0.00108 $ & $  10.66290 $ & $ i$\\
$ 54723.64535 $ & $  -0.00437 $ & $   0.00111 $ & $  10.66160 $ & $ i$\\
$ 54723.64621 $ & $   0.00174 $ & $   0.00110 $ & $  10.66730 $ & $ i$\\
$ 54723.64706 $ & $   0.00174 $ & $   0.00108 $ & $  10.66850 $ & $ i$\\
$ 54723.64791 $ & $  -0.00168 $ & $   0.00110 $ & $  10.66480 $ & $ i$\\
$ 54723.64876 $ & $  -0.00126 $ & $   0.00109 $ & $  10.66590 $ & $ i$\\
$ 54723.64960 $ & $  -0.00098 $ & $   0.00109 $ & $  10.66530 $ & $ i$\\
$ 54723.65046 $ & $   0.00092 $ & $   0.00110 $ & $  10.66810 $ & $ i$\\
$ 54723.65131 $ & $   0.00157 $ & $   0.00106 $ & $  10.66860 $ & $ i$\\
$ 54723.65218 $ & $  -0.00165 $ & $   0.00104 $ & $  10.66470 $ & $ i$\\
$ 54723.65305 $ & $   0.00090 $ & $   0.00105 $ & $  10.66840 $ & $ i$\\
$ 54723.65390 $ & $  -0.00125 $ & $   0.00097 $ & $  10.66460 $ & $ i$\\
$ 54723.65475 $ & $   0.00407 $ & $   0.00097 $ & $  10.67060 $ & $ i$\\
$ 54723.65560 $ & $   0.00205 $ & $   0.00098 $ & $  10.66850 $ & $ i$\\
$ 54723.65645 $ & $   0.00463 $ & $   0.00099 $ & $  10.67190 $ & $ i$\\
$ 54723.65731 $ & $   0.00475 $ & $   0.00102 $ & $  10.67250 $ & $ i$\\
$ 54723.65817 $ & $   0.00629 $ & $   0.00104 $ & $  10.67290 $ & $ i$\\
$ 54723.65902 $ & $   0.00739 $ & $   0.00105 $ & $  10.67430 $ & $ i$\\
$ 54723.65989 $ & $   0.00957 $ & $   0.00106 $ & $  10.67720 $ & $ i$\\
$ 54723.66075 $ & $   0.00989 $ & $   0.00109 $ & $  10.67610 $ & $ i$\\
$ 54723.66159 $ & $   0.01127 $ & $   0.00109 $ & $  10.67810 $ & $ i$\\
$ 54723.66246 $ & $   0.01326 $ & $   0.00096 $ & $  10.67940 $ & $ i$\\
$ 54723.66328 $ & $   0.01485 $ & $   0.00090 $ & $  10.68120 $ & $ i$\\
$ 54723.66416 $ & $   0.01548 $ & $   0.00092 $ & $  10.68170 $ & $ i$\\
$ 54723.66505 $ & $   0.01748 $ & $   0.00094 $ & $  10.68330 $ & $ i$\\
$ 54723.66590 $ & $   0.01428 $ & $   0.00093 $ & $  10.68050 $ & $ i$\\
$ 54723.66677 $ & $   0.01589 $ & $   0.00092 $ & $  10.68200 $ & $ i$\\
$ 54723.66761 $ & $   0.01392 $ & $   0.00092 $ & $  10.68060 $ & $ i$\\
$ 54723.66848 $ & $   0.01630 $ & $   0.00093 $ & $  10.68280 $ & $ i$\\
$ 54723.66931 $ & $   0.01556 $ & $   0.00093 $ & $  10.68170 $ & $ i$\\
$ 54723.67017 $ & $   0.01508 $ & $   0.00093 $ & $  10.68110 $ & $ i$\\
$ 54723.67102 $ & $   0.01881 $ & $   0.00091 $ & $  10.68480 $ & $ i$\\
$ 54723.67187 $ & $   0.01597 $ & $   0.00094 $ & $  10.68240 $ & $ i$\\
$ 54723.67274 $ & $   0.01744 $ & $   0.00093 $ & $  10.68400 $ & $ i$\\
$ 54723.67358 $ & $   0.01680 $ & $   0.00093 $ & $  10.68260 $ & $ i$\\
$ 54723.67445 $ & $   0.01465 $ & $   0.00092 $ & $  10.68090 $ & $ i$\\
$ 54723.67531 $ & $   0.01585 $ & $   0.00092 $ & $  10.68220 $ & $ i$\\
$ 54723.67617 $ & $   0.01687 $ & $   0.00093 $ & $  10.68370 $ & $ i$\\
$ 54723.67704 $ & $   0.01520 $ & $   0.00093 $ & $  10.68150 $ & $ i$\\
$ 54723.67790 $ & $   0.01662 $ & $   0.00093 $ & $  10.68240 $ & $ i$\\
$ 54723.67873 $ & $   0.01642 $ & $   0.00093 $ & $  10.68280 $ & $ i$\\
$ 54723.67959 $ & $   0.01653 $ & $   0.00090 $ & $  10.68250 $ & $ i$\\
$ 54723.68043 $ & $   0.01250 $ & $   0.00094 $ & $  10.67970 $ & $ i$\\
$ 54723.68129 $ & $   0.01546 $ & $   0.00093 $ & $  10.68260 $ & $ i$\\
$ 54723.68214 $ & $   0.01661 $ & $   0.00092 $ & $  10.68320 $ & $ i$\\
$ 54723.68299 $ & $   0.01410 $ & $   0.00093 $ & $  10.68050 $ & $ i$\\
$ 54723.68386 $ & $   0.01403 $ & $   0.00092 $ & $  10.68080 $ & $ i$\\
$ 54723.68469 $ & $   0.01363 $ & $   0.00093 $ & $  10.67990 $ & $ i$\\
$ 54723.68555 $ & $   0.01747 $ & $   0.00093 $ & $  10.68420 $ & $ i$\\
$ 54723.68641 $ & $   0.01421 $ & $   0.00093 $ & $  10.68080 $ & $ i$\\
$ 54723.68725 $ & $   0.01543 $ & $   0.00092 $ & $  10.68190 $ & $ i$\\
$ 54723.68811 $ & $   0.01770 $ & $   0.00092 $ & $  10.68350 $ & $ i$\\
$ 54723.68899 $ & $   0.01695 $ & $   0.00093 $ & $  10.68330 $ & $ i$\\
$ 54723.68983 $ & $   0.01570 $ & $   0.00092 $ & $  10.68160 $ & $ i$\\
$ 54723.69068 $ & $   0.01560 $ & $   0.00092 $ & $  10.68220 $ & $ i$\\
$ 54723.69291 $ & $   0.01873 $ & $   0.00094 $ & $  10.68570 $ & $ i$\\
$ 54723.69377 $ & $   0.01540 $ & $   0.00094 $ & $  10.68140 $ & $ i$\\
$ 54723.69461 $ & $   0.01541 $ & $   0.00094 $ & $  10.68220 $ & $ i$\\
$ 54723.69547 $ & $   0.01820 $ & $   0.00094 $ & $  10.68420 $ & $ i$\\
$ 54723.69634 $ & $   0.01834 $ & $   0.00092 $ & $  10.68430 $ & $ i$\\
$ 54723.69717 $ & $   0.01798 $ & $   0.00092 $ & $  10.68360 $ & $ i$\\
$ 54723.69803 $ & $   0.01860 $ & $   0.00092 $ & $  10.68470 $ & $ i$\\
$ 54723.69887 $ & $   0.01782 $ & $   0.00093 $ & $  10.68420 $ & $ i$\\
$ 54723.69972 $ & $   0.01687 $ & $   0.00091 $ & $  10.68260 $ & $ i$\\
$ 54723.70060 $ & $   0.01734 $ & $   0.00093 $ & $  10.68420 $ & $ i$\\
$ 54723.70146 $ & $   0.01615 $ & $   0.00092 $ & $  10.68280 $ & $ i$\\
$ 54723.70232 $ & $   0.01875 $ & $   0.00094 $ & $  10.68510 $ & $ i$\\
$ 54723.70318 $ & $   0.01826 $ & $   0.00092 $ & $  10.68370 $ & $ i$\\
$ 54723.70404 $ & $   0.01601 $ & $   0.00093 $ & $  10.68200 $ & $ i$\\
$ 54723.70489 $ & $   0.01566 $ & $   0.00094 $ & $  10.68200 $ & $ i$\\
$ 54723.70574 $ & $   0.01888 $ & $   0.00093 $ & $  10.68440 $ & $ i$\\
$ 54723.70661 $ & $   0.01673 $ & $   0.00093 $ & $  10.68220 $ & $ i$\\
$ 54723.70748 $ & $   0.01844 $ & $   0.00094 $ & $  10.68350 $ & $ i$\\
$ 54723.70831 $ & $   0.01790 $ & $   0.00096 $ & $  10.68320 $ & $ i$\\
$ 54723.70918 $ & $   0.01788 $ & $   0.00095 $ & $  10.68370 $ & $ i$\\
$ 54723.71004 $ & $   0.01797 $ & $   0.00095 $ & $  10.68390 $ & $ i$\\
$ 54723.71088 $ & $   0.01517 $ & $   0.00095 $ & $  10.68070 $ & $ i$\\
$ 54723.71174 $ & $   0.01654 $ & $   0.00093 $ & $  10.68150 $ & $ i$\\
$ 54723.71259 $ & $   0.01637 $ & $   0.00097 $ & $  10.68210 $ & $ i$\\
$ 54723.71345 $ & $   0.01698 $ & $   0.00093 $ & $  10.68190 $ & $ i$\\
$ 54723.71431 $ & $   0.01744 $ & $   0.00095 $ & $  10.68360 $ & $ i$\\
$ 54723.71515 $ & $   0.01517 $ & $   0.00096 $ & $  10.68130 $ & $ i$\\
$ 54723.71601 $ & $   0.01587 $ & $   0.00095 $ & $  10.68160 $ & $ i$\\
$ 54723.71686 $ & $   0.01624 $ & $   0.00093 $ & $  10.68240 $ & $ i$\\
$ 54723.71772 $ & $   0.01565 $ & $   0.00096 $ & $  10.68160 $ & $ i$\\
$ 54723.71857 $ & $   0.01447 $ & $   0.00093 $ & $  10.67990 $ & $ i$\\
$ 54723.71943 $ & $   0.01601 $ & $   0.00097 $ & $  10.68180 $ & $ i$\\
$ 54723.72028 $ & $   0.01700 $ & $   0.00097 $ & $  10.68350 $ & $ i$\\
$ 54723.72113 $ & $   0.01523 $ & $   0.00095 $ & $  10.68060 $ & $ i$\\
$ 54723.72199 $ & $   0.01703 $ & $   0.00093 $ & $  10.68300 $ & $ i$\\
$ 54723.72285 $ & $   0.01528 $ & $   0.00092 $ & $  10.68050 $ & $ i$\\
$ 54723.72370 $ & $   0.01483 $ & $   0.00096 $ & $  10.68000 $ & $ i$\\
$ 54723.72455 $ & $   0.01500 $ & $   0.00092 $ & $  10.68040 $ & $ i$\\
$ 54723.72542 $ & $   0.01550 $ & $   0.00095 $ & $  10.68060 $ & $ i$\\
$ 54723.72625 $ & $   0.01442 $ & $   0.00094 $ & $  10.68030 $ & $ i$\\
$ 54723.72713 $ & $   0.01563 $ & $   0.00094 $ & $  10.68210 $ & $ i$\\
$ 54723.72798 $ & $   0.01489 $ & $   0.00096 $ & $  10.68180 $ & $ i$\\
$ 54723.72883 $ & $   0.01317 $ & $   0.00096 $ & $  10.67960 $ & $ i$\\
$ 54723.72968 $ & $   0.01038 $ & $   0.00096 $ & $  10.67690 $ & $ i$\\
$ 54723.73054 $ & $   0.01413 $ & $   0.00095 $ & $  10.68040 $ & $ i$\\
$ 54723.73139 $ & $   0.01282 $ & $   0.00097 $ & $  10.67940 $ & $ i$\\
$ 54723.73223 $ & $   0.01154 $ & $   0.00094 $ & $  10.67710 $ & $ i$\\
$ 54723.73309 $ & $   0.01040 $ & $   0.00093 $ & $  10.67740 $ & $ i$\\
$ 54723.73395 $ & $   0.01143 $ & $   0.00096 $ & $  10.67730 $ & $ i$\\
$ 54723.73479 $ & $   0.01317 $ & $   0.00097 $ & $  10.67980 $ & $ i$\\
$ 54723.73565 $ & $   0.01217 $ & $   0.00094 $ & $  10.67820 $ & $ i$\\
$ 54723.73651 $ & $   0.00967 $ & $   0.00096 $ & $  10.67680 $ & $ i$\\
$ 54723.73736 $ & $   0.00915 $ & $   0.00096 $ & $  10.67520 $ & $ i$\\
$ 54723.73821 $ & $   0.00958 $ & $   0.00096 $ & $  10.67670 $ & $ i$\\
$ 54723.73908 $ & $   0.00537 $ & $   0.00096 $ & $  10.67220 $ & $ i$\\
$ 54723.73992 $ & $   0.00336 $ & $   0.00095 $ & $  10.67060 $ & $ i$\\
$ 54723.74076 $ & $   0.00639 $ & $   0.00096 $ & $  10.67280 $ & $ i$\\
$ 54723.74162 $ & $   0.00424 $ & $   0.00095 $ & $  10.67100 $ & $ i$\\
$ 54723.74247 $ & $   0.00211 $ & $   0.00095 $ & $  10.66810 $ & $ i$\\
$ 54723.74334 $ & $  -0.00136 $ & $   0.00094 $ & $  10.66530 $ & $ i$\\
$ 54723.74431 $ & $  -0.00030 $ & $   0.00092 $ & $  10.66640 $ & $ i$\\
$ 54723.74518 $ & $   0.00414 $ & $   0.00095 $ & $  10.67010 $ & $ i$\\
$ 54723.74600 $ & $  -0.00059 $ & $   0.00094 $ & $  10.66570 $ & $ i$\\
$ 54723.74685 $ & $   0.00384 $ & $   0.00095 $ & $  10.67030 $ & $ i$\\
$ 54723.74770 $ & $  -0.00185 $ & $   0.00095 $ & $  10.66430 $ & $ i$\\
$ 54723.74854 $ & $   0.00018 $ & $   0.00091 $ & $  10.66690 $ & $ i$\\
$ 54723.74942 $ & $   0.00107 $ & $   0.00095 $ & $  10.66830 $ & $ i$\\
$ 54723.75027 $ & $   0.00043 $ & $   0.00095 $ & $  10.66700 $ & $ i$\\
$ 54723.75115 $ & $   0.00011 $ & $   0.00096 $ & $  10.66660 $ & $ i$\\
$ 54723.75202 $ & $   0.00161 $ & $   0.00093 $ & $  10.66820 $ & $ i$\\
$ 54723.75286 $ & $  -0.00042 $ & $   0.00095 $ & $  10.66570 $ & $ i$\\
$ 54723.75372 $ & $   0.00115 $ & $   0.00094 $ & $  10.66790 $ & $ i$\\
$ 54723.75457 $ & $   0.00101 $ & $   0.00095 $ & $  10.66810 $ & $ i$\\
$ 54723.75544 $ & $  -0.00202 $ & $   0.00093 $ & $  10.66470 $ & $ i$\\
$ 54723.75631 $ & $   0.00258 $ & $   0.00094 $ & $  10.66860 $ & $ i$\\
$ 54723.75714 $ & $  -0.00047 $ & $   0.00094 $ & $  10.66560 $ & $ i$\\
$ 54723.75800 $ & $   0.00058 $ & $   0.00094 $ & $  10.66720 $ & $ i$\\
$ 54723.75887 $ & $  -0.00056 $ & $   0.00094 $ & $  10.66590 $ & $ i$\\
$ 54723.75970 $ & $  -0.00060 $ & $   0.00093 $ & $  10.66630 $ & $ i$\\
$ 54723.76057 $ & $   0.00094 $ & $   0.00093 $ & $  10.66610 $ & $ i$\\
$ 54723.76141 $ & $  -0.00009 $ & $   0.00095 $ & $  10.66700 $ & $ i$\\
$ 54723.76228 $ & $   0.00205 $ & $   0.00094 $ & $  10.66930 $ & $ i$\\
$ 54723.76314 $ & $   0.00247 $ & $   0.00092 $ & $  10.66920 $ & $ i$\\
$ 54723.76398 $ & $  -0.00091 $ & $   0.00092 $ & $  10.66580 $ & $ i$\\
$ 54723.76483 $ & $  -0.00128 $ & $   0.00094 $ & $  10.66520 $ & $ i$\\
$ 54723.76570 $ & $   0.00089 $ & $   0.00093 $ & $  10.66830 $ & $ i$\\
$ 54723.76655 $ & $  -0.00172 $ & $   0.00094 $ & $  10.66540 $ & $ i$\\
$ 54723.76741 $ & $   0.00138 $ & $   0.00095 $ & $  10.66830 $ & $ i$\\
$ 54723.76826 $ & $  -0.00046 $ & $   0.00094 $ & $  10.66690 $ & $ i$\\
$ 54723.76911 $ & $   0.00032 $ & $   0.00096 $ & $  10.66760 $ & $ i$\\
$ 54723.76997 $ & $  -0.00151 $ & $   0.00093 $ & $  10.66580 $ & $ i$\\
$ 54723.77081 $ & $   0.00332 $ & $   0.00094 $ & $  10.67050 $ & $ i$\\
$ 54723.77167 $ & $  -0.00003 $ & $   0.00094 $ & $  10.66870 $ & $ i$\\
$ 54723.77251 $ & $   0.00208 $ & $   0.00094 $ & $  10.67000 $ & $ i$\\
$ 54723.77337 $ & $   0.00044 $ & $   0.00093 $ & $  10.66850 $ & $ i$\\
$ 54723.77424 $ & $  -0.00247 $ & $   0.00093 $ & $  10.66600 $ & $ i$\\
$ 54723.77508 $ & $  -0.00100 $ & $   0.00094 $ & $  10.66740 $ & $ i$\\
$ 54723.77593 $ & $  -0.00383 $ & $   0.00094 $ & $  10.66390 $ & $ i$\\
$ 54723.77677 $ & $   0.00125 $ & $   0.00095 $ & $  10.66940 $ & $ i$\\
$ 54723.77764 $ & $  -0.00347 $ & $   0.00094 $ & $  10.66520 $ & $ i$\\
$ 54723.77848 $ & $  -0.00147 $ & $   0.00095 $ & $  10.66650 $ & $ i$\\
$ 54723.77935 $ & $  -0.00094 $ & $   0.00094 $ & $  10.66780 $ & $ i$\\
$ 54723.78019 $ & $  -0.00295 $ & $   0.00093 $ & $  10.66540 $ & $ i$\\
$ 54723.78105 $ & $   0.00003 $ & $   0.00094 $ & $  10.66890 $ & $ i$\\
$ 54723.78190 $ & $  -0.00104 $ & $   0.00095 $ & $  10.66740 $ & $ i$\\
$ 54723.78274 $ & $  -0.00309 $ & $   0.00094 $ & $  10.66560 $ & $ i$\\
$ 54723.78361 $ & $  -0.00039 $ & $   0.00096 $ & $  10.66830 $ & $ i$\\
$ 54723.78446 $ & $   0.00086 $ & $   0.00094 $ & $  10.67010 $ & $ i$\\
$ 54723.78530 $ & $   0.00119 $ & $   0.00097 $ & $  10.67090 $ & $ i$\\
$ 54723.78617 $ & $  -0.00088 $ & $   0.00095 $ & $  10.66880 $ & $ i$\\
$ 54723.78703 $ & $   0.00231 $ & $   0.00096 $ & $  10.67070 $ & $ i$\\
$ 54723.78787 $ & $   0.00097 $ & $   0.00093 $ & $  10.66920 $ & $ i$\\
$ 54723.78873 $ & $   0.00056 $ & $   0.00097 $ & $  10.66900 $ & $ i$\\
$ 54723.78956 $ & $   0.00160 $ & $   0.00097 $ & $  10.67040 $ & $ i$\\
$ 54723.79041 $ & $  -0.00078 $ & $   0.00095 $ & $  10.66890 $ & $ i$\\
$ 54723.79128 $ & $   0.00154 $ & $   0.00094 $ & $  10.67000 $ & $ i$\\
$ 54723.79214 $ & $   0.00136 $ & $   0.00095 $ & $  10.67040 $ & $ i$\\
$ 54723.79300 $ & $  -0.00056 $ & $   0.00096 $ & $  10.66860 $ & $ i$\\
$ 54723.79387 $ & $  -0.00062 $ & $   0.00096 $ & $  10.66770 $ & $ i$\\
$ 54723.79471 $ & $  -0.00187 $ & $   0.00094 $ & $  10.66680 $ & $ i$\\
$ 54723.80091 $ & $  -0.00015 $ & $   0.00095 $ & $  10.66890 $ & $ i$\\
$ 54723.80177 $ & $  -0.00185 $ & $   0.00098 $ & $  10.66570 $ & $ i$\\
$ 54723.80263 $ & $   0.00182 $ & $   0.00095 $ & $  10.67100 $ & $ i$\\
$ 54723.80351 $ & $   0.00253 $ & $   0.00097 $ & $  10.67090 $ & $ i$\\
$ 54723.80435 $ & $   0.00059 $ & $   0.00096 $ & $  10.66920 $ & $ i$\\
$ 54723.80520 $ & $   0.00318 $ & $   0.00098 $ & $  10.67160 $ & $ i$\\
$ 54723.80605 $ & $   0.00235 $ & $   0.00096 $ & $  10.67110 $ & $ i$\\
$ 54723.80692 $ & $   0.00028 $ & $   0.00097 $ & $  10.66890 $ & $ i$\\
$ 54723.80778 $ & $  -0.00134 $ & $   0.00096 $ & $  10.66690 $ & $ i$\\
$ 54723.80861 $ & $   0.00144 $ & $   0.00096 $ & $  10.66970 $ & $ i$\\
$ 54723.80948 $ & $  -0.00243 $ & $   0.00096 $ & $  10.66580 $ & $ i$\\
$ 54723.81035 $ & $   0.00226 $ & $   0.00099 $ & $  10.67070 $ & $ i$\\
$ 54723.81120 $ & $   0.00439 $ & $   0.00095 $ & $  10.67140 $ & $ i$\\
$ 54723.81204 $ & $   0.00350 $ & $   0.00098 $ & $  10.67120 $ & $ i$\\
$ 54723.81290 $ & $   0.00007 $ & $   0.00100 $ & $  10.66790 $ & $ i$\\
$ 54723.81375 $ & $  -0.00187 $ & $   0.00097 $ & $  10.66640 $ & $ i$\\
$ 54723.81459 $ & $  -0.00106 $ & $   0.00097 $ & $  10.66710 $ & $ i$\\
$ 54723.81544 $ & $   0.00088 $ & $   0.00100 $ & $  10.66910 $ & $ i$\\
$ 54723.81630 $ & $  -0.00250 $ & $   0.00097 $ & $  10.66540 $ & $ i$\\
$ 54723.81714 $ & $  -0.00154 $ & $   0.00096 $ & $  10.66690 $ & $ i$\\
$ 54723.81800 $ & $   0.00053 $ & $   0.00099 $ & $  10.66870 $ & $ i$\\
$ 54723.81885 $ & $  -0.00010 $ & $   0.00101 $ & $  10.66750 $ & $ i$\\
$ 54723.81971 $ & $   0.00037 $ & $   0.00099 $ & $  10.66820 $ & $ i$\\
$ 54723.82054 $ & $   0.00187 $ & $   0.00098 $ & $  10.66830 $ & $ i$\\
$ 54723.82140 $ & $  -0.00267 $ & $   0.00099 $ & $  10.66440 $ & $ i$\\
$ 54723.82224 $ & $   0.00051 $ & $   0.00098 $ & $  10.66830 $ & $ i$\\
$ 54723.82310 $ & $  -0.00195 $ & $   0.00100 $ & $  10.66530 $ & $ i$\\
$ 54723.82396 $ & $  -0.00204 $ & $   0.00097 $ & $  10.66580 $ & $ i$\\
$ 54723.82479 $ & $  -0.00277 $ & $   0.00098 $ & $  10.66460 $ & $ i$\\
$ 54723.82566 $ & $  -0.00149 $ & $   0.00099 $ & $  10.66730 $ & $ i$\\
$ 54723.82650 $ & $   0.00042 $ & $   0.00098 $ & $  10.66740 $ & $ i$\\
$ 54723.82735 $ & $  -0.00169 $ & $   0.00101 $ & $  10.66680 $ & $ i$\\
$ 54723.82819 $ & $  -0.00006 $ & $   0.00098 $ & $  10.66750 $ & $ i$\\
$ 54723.82906 $ & $  -0.00107 $ & $   0.00101 $ & $  10.66560 $ & $ i$\\
$ 54723.82992 $ & $   0.00202 $ & $   0.00101 $ & $  10.67010 $ & $ i$\\
$ 54723.83077 $ & $  -0.00109 $ & $   0.00101 $ & $  10.66680 $ & $ i$\\
$ 54723.83164 $ & $  -0.00169 $ & $   0.00103 $ & $  10.66590 $ & $ i$\\
$ 54723.83249 $ & $   0.00045 $ & $   0.00100 $ & $  10.66880 $ & $ i$\\
$ 54723.83333 $ & $  -0.00272 $ & $   0.00097 $ & $  10.66450 $ & $ i$\\
$ 54723.83421 $ & $   0.00032 $ & $   0.00100 $ & $  10.66830 $ & $ i$\\
$ 54723.83504 $ & $  -0.00088 $ & $   0.00100 $ & $  10.66690 $ & $ i$\\
$ 54723.83591 $ & $   0.00184 $ & $   0.00099 $ & $  10.66960 $ & $ i$\\
$ 54723.83675 $ & $  -0.00286 $ & $   0.00101 $ & $  10.66470 $ & $ i$\\
$ 54723.83759 $ & $  -0.00034 $ & $   0.00099 $ & $  10.66700 $ & $ i$\\
$ 54723.83845 $ & $   0.00003 $ & $   0.00100 $ & $  10.66780 $ & $ i$\\
$ 54723.83929 $ & $   0.00374 $ & $   0.00103 $ & $  10.67060 $ & $ i$\\
$ 54723.84016 $ & $   0.00007 $ & $   0.00102 $ & $  10.66810 $ & $ i$\\
$ 54723.84100 $ & $  -0.00035 $ & $   0.00102 $ & $  10.66720 $ & $ i$\\
$ 54723.84185 $ & $   0.00095 $ & $   0.00099 $ & $  10.66810 $ & $ i$\\
$ 54723.84272 $ & $   0.00094 $ & $   0.00098 $ & $  10.66840 $ & $ i$\\
$ 54723.84357 $ & $   0.00167 $ & $   0.00103 $ & $  10.66960 $ & $ i$\\
$ 54723.84442 $ & $   0.00191 $ & $   0.00102 $ & $  10.66990 $ & $ i$\\
$ 54723.84529 $ & $  -0.00225 $ & $   0.00102 $ & $  10.66490 $ & $ i$\\
$ 54723.84612 $ & $   0.00213 $ & $   0.00104 $ & $  10.66900 $ & $ i$\\
$ 54723.84695 $ & $   0.00145 $ & $   0.00099 $ & $  10.66890 $ & $ i$\\
$ 54723.84782 $ & $  -0.00252 $ & $   0.00101 $ & $  10.66600 $ & $ i$\\
$ 54723.84867 $ & $   0.00038 $ & $   0.00101 $ & $  10.66830 $ & $ i$\\
$ 54723.84952 $ & $  -0.00066 $ & $   0.00102 $ & $  10.66710 $ & $ i$\\
$ 54723.85037 $ & $  -0.00009 $ & $   0.00104 $ & $  10.66720 $ & $ i$\\
$ 54723.85124 $ & $  -0.00096 $ & $   0.00104 $ & $  10.66700 $ & $ i$\\
$ 54723.85393 $ & $  -0.00313 $ & $   0.00100 $ & $  10.66430 $ & $ i$\\
$ 54723.85478 $ & $   0.00181 $ & $   0.00103 $ & $  10.66930 $ & $ i$\\
$ 54723.85563 $ & $   0.00237 $ & $   0.00103 $ & $  10.67070 $ & $ i$\\
$ 54723.85648 $ & $  -0.00193 $ & $   0.00103 $ & $  10.66690 $ & $ i$\\
$ 54723.85733 $ & $  -0.00085 $ & $   0.00104 $ & $  10.66630 $ & $ i$\\
$ 54723.85819 $ & $  -0.00298 $ & $   0.00102 $ & $  10.66540 $ & $ i$\\
$ 54723.85904 $ & $   0.00195 $ & $   0.00105 $ & $  10.67000 $ & $ i$\\
$ 54723.85990 $ & $   0.00085 $ & $   0.00102 $ & $  10.66880 $ & $ i$\\
$ 54723.86073 $ & $   0.00200 $ & $   0.00106 $ & $  10.66990 $ & $ i$\\
$ 54723.86159 $ & $   0.00127 $ & $   0.00103 $ & $  10.66870 $ & $ i$\\
$ 54723.86245 $ & $   0.00183 $ & $   0.00105 $ & $  10.66820 $ & $ i$\\
$ 54723.86331 $ & $   0.00004 $ & $   0.00103 $ & $  10.66820 $ & $ i$\\
$ 54723.86415 $ & $   0.00214 $ & $   0.00104 $ & $  10.66990 $ & $ i$\\
$ 54723.86502 $ & $   0.00043 $ & $   0.00103 $ & $  10.66860 $ & $ i$\\
$ 54723.86589 $ & $  -0.00055 $ & $   0.00104 $ & $  10.66770 $ & $ i$\\
$ 54723.86672 $ & $  -0.00243 $ & $   0.00104 $ & $  10.66500 $ & $ i$\\
$ 54723.86759 $ & $  -0.00031 $ & $   0.00104 $ & $  10.66710 $ & $ i$\\
$ 54723.86843 $ & $  -0.00396 $ & $   0.00104 $ & $  10.66280 $ & $ i$\\
$ 54723.86928 $ & $  -0.00053 $ & $   0.00110 $ & $  10.66690 $ & $ i$\\
$ 54723.87013 $ & $   0.00074 $ & $   0.00107 $ & $  10.66850 $ & $ i$\\
$ 54723.87099 $ & $   0.00171 $ & $   0.00104 $ & $  10.67060 $ & $ i$\\
$ 54723.87185 $ & $  -0.00227 $ & $   0.00107 $ & $  10.66580 $ & $ i$\\
$ 54723.87270 $ & $   0.00483 $ & $   0.00109 $ & $  10.67300 $ & $ i$\\
$ 54723.87354 $ & $   0.00069 $ & $   0.00107 $ & $  10.66850 $ & $ i$\\
$ 54723.87441 $ & $  -0.00157 $ & $   0.00103 $ & $  10.66800 $ & $ i$\\
$ 54774.56600 $ & $   0.00175 $ & $   0.00092 $ & $  10.80680 $ & $ i$\\
$ 54774.56807 $ & $   0.00106 $ & $   0.00090 $ & $  10.80570 $ & $ i$\\
$ 54774.57016 $ & $  -0.00206 $ & $   0.00090 $ & $  10.80370 $ & $ i$\\
$ 54774.57724 $ & $  -0.00005 $ & $   0.00089 $ & $  10.80700 $ & $ i$\\
$ 54774.57827 $ & $  -0.00084 $ & $   0.00088 $ & $  10.80530 $ & $ i$\\
$ 54774.58033 $ & $   0.00066 $ & $   0.00088 $ & $  10.80710 $ & $ i$\\
$ 54774.58135 $ & $  -0.00197 $ & $   0.00088 $ & $  10.80390 $ & $ i$\\
$ 54774.58238 $ & $   0.00104 $ & $   0.00088 $ & $  10.80670 $ & $ i$\\
$ 54774.58343 $ & $   0.00006 $ & $   0.00088 $ & $  10.80580 $ & $ i$\\
$ 54774.58446 $ & $  -0.00063 $ & $   0.00088 $ & $  10.80630 $ & $ i$\\
$ 54774.58551 $ & $  -0.00030 $ & $   0.00089 $ & $  10.80550 $ & $ i$\\
$ 54774.58759 $ & $  -0.00010 $ & $   0.00089 $ & $  10.80600 $ & $ i$\\
$ 54774.58861 $ & $   0.00087 $ & $   0.00090 $ & $  10.80720 $ & $ i$\\
$ 54774.59172 $ & $   0.00089 $ & $   0.00089 $ & $  10.80750 $ & $ i$\\
$ 54774.59276 $ & $  -0.00023 $ & $   0.00089 $ & $  10.80610 $ & $ i$\\
$ 54774.59586 $ & $   0.00007 $ & $   0.00090 $ & $  10.80750 $ & $ i$\\
$ 54774.59688 $ & $   0.00305 $ & $   0.00089 $ & $  10.80910 $ & $ i$\\
$ 54774.59790 $ & $   0.00293 $ & $   0.00089 $ & $  10.80910 $ & $ i$\\
$ 54774.62255 $ & $   0.01924 $ & $   0.00090 $ & $  10.82290 $ & $ i$\\
$ 54774.62360 $ & $   0.01449 $ & $   0.00089 $ & $  10.81910 $ & $ i$\\
$ 54774.62462 $ & $   0.01654 $ & $   0.00089 $ & $  10.82070 $ & $ i$\\
$ 54774.62668 $ & $   0.01661 $ & $   0.00089 $ & $  10.82170 $ & $ i$\\
$ 54774.63079 $ & $   0.01761 $ & $   0.00089 $ & $  10.82280 $ & $ i$\\
$ 54774.63390 $ & $   0.01875 $ & $   0.00089 $ & $  10.82400 $ & $ i$\\
$ 54774.63492 $ & $   0.01929 $ & $   0.00089 $ & $  10.82390 $ & $ i$\\
$ 54774.63596 $ & $   0.01828 $ & $   0.00089 $ & $  10.82300 $ & $ i$\\
$ 54774.63699 $ & $   0.01639 $ & $   0.00089 $ & $  10.82080 $ & $ i$\\
$ 54774.63802 $ & $   0.01820 $ & $   0.00089 $ & $  10.82300 $ & $ i$\\
$ 54774.63903 $ & $   0.01923 $ & $   0.00089 $ & $  10.82360 $ & $ i$\\
$ 54774.64008 $ & $   0.01740 $ & $   0.00089 $ & $  10.82190 $ & $ i$\\
$ 54774.64109 $ & $   0.01429 $ & $   0.00089 $ & $  10.82010 $ & $ i$\\
$ 54774.64211 $ & $   0.01547 $ & $   0.00089 $ & $  10.82110 $ & $ i$\\
$ 54774.64315 $ & $   0.01602 $ & $   0.00089 $ & $  10.82150 $ & $ i$\\
$ 54774.64418 $ & $   0.01620 $ & $   0.00089 $ & $  10.82110 $ & $ i$\\
$ 54774.64520 $ & $   0.01744 $ & $   0.00089 $ & $  10.82250 $ & $ i$\\
$ 54774.64623 $ & $   0.01532 $ & $   0.00089 $ & $  10.82040 $ & $ i$\\
$ 54774.64727 $ & $   0.01675 $ & $   0.00090 $ & $  10.82200 $ & $ i$\\
$ 54774.64831 $ & $   0.01627 $ & $   0.00090 $ & $  10.82120 $ & $ i$\\
$ 54774.64935 $ & $   0.01570 $ & $   0.00089 $ & $  10.82070 $ & $ i$\\
$ 54774.65038 $ & $   0.01630 $ & $   0.00089 $ & $  10.82060 $ & $ i$\\
$ 54774.65140 $ & $   0.01687 $ & $   0.00090 $ & $  10.82080 $ & $ i$\\
$ 54774.65244 $ & $   0.01466 $ & $   0.00089 $ & $  10.81930 $ & $ i$\\
$ 54774.65352 $ & $   0.01559 $ & $   0.00089 $ & $  10.81930 $ & $ i$\\
$ 54774.65456 $ & $   0.01626 $ & $   0.00090 $ & $  10.82050 $ & $ i$\\
$ 54774.65560 $ & $   0.01594 $ & $   0.00089 $ & $  10.82050 $ & $ i$\\
$ 54774.65662 $ & $   0.01751 $ & $   0.00089 $ & $  10.82210 $ & $ i$\\
$ 54774.65767 $ & $   0.01637 $ & $   0.00090 $ & $  10.82000 $ & $ i$\\
$ 54774.65870 $ & $   0.01403 $ & $   0.00090 $ & $  10.81840 $ & $ i$\\
$ 54774.65975 $ & $   0.01499 $ & $   0.00090 $ & $  10.82000 $ & $ i$\\
$ 54774.66079 $ & $   0.01664 $ & $   0.00090 $ & $  10.82180 $ & $ i$\\
$ 54774.66184 $ & $   0.01466 $ & $   0.00090 $ & $  10.81920 $ & $ i$\\
$ 54774.66287 $ & $   0.01376 $ & $   0.00090 $ & $  10.81800 $ & $ i$\\
$ 54774.66389 $ & $   0.01584 $ & $   0.00090 $ & $  10.82030 $ & $ i$\\
$ 54774.66492 $ & $   0.01571 $ & $   0.00090 $ & $  10.82010 $ & $ i$\\
$ 54774.66595 $ & $   0.01562 $ & $   0.00090 $ & $  10.82070 $ & $ i$\\
$ 54774.66699 $ & $   0.01658 $ & $   0.00090 $ & $  10.82080 $ & $ i$\\
$ 54774.66802 $ & $   0.01598 $ & $   0.00090 $ & $  10.82120 $ & $ i$\\
$ 54774.66905 $ & $   0.01694 $ & $   0.00090 $ & $  10.82240 $ & $ i$\\
$ 54774.67006 $ & $   0.01528 $ & $   0.00090 $ & $  10.82110 $ & $ i$\\
$ 54774.67110 $ & $   0.01727 $ & $   0.00090 $ & $  10.82230 $ & $ i$\\
$ 54774.67215 $ & $   0.01436 $ & $   0.00090 $ & $  10.81970 $ & $ i$\\
$ 54774.67319 $ & $   0.01664 $ & $   0.00091 $ & $  10.82120 $ & $ i$\\
$ 54774.67421 $ & $   0.01260 $ & $   0.00090 $ & $  10.81780 $ & $ i$\\
$ 54774.67525 $ & $   0.01479 $ & $   0.00090 $ & $  10.82000 $ & $ i$\\
$ 54774.67629 $ & $   0.01206 $ & $   0.00090 $ & $  10.81760 $ & $ i$\\
$ 54774.67732 $ & $   0.01082 $ & $   0.00090 $ & $  10.81650 $ & $ i$\\
$ 54774.67835 $ & $   0.00900 $ & $   0.00090 $ & $  10.81370 $ & $ i$\\
$ 54774.67938 $ & $   0.00702 $ & $   0.00090 $ & $  10.81210 $ & $ i$\\
$ 54774.68041 $ & $   0.00767 $ & $   0.00090 $ & $  10.81350 $ & $ i$\\
$ 54774.68143 $ & $   0.00637 $ & $   0.00090 $ & $  10.81210 $ & $ i$\\
$ 54774.68247 $ & $   0.00436 $ & $   0.00090 $ & $  10.81040 $ & $ i$\\
$ 54774.68349 $ & $   0.00131 $ & $   0.00090 $ & $  10.80650 $ & $ i$\\
$ 54774.68453 $ & $  -0.00020 $ & $   0.00090 $ & $  10.80560 $ & $ i$\\
$ 54774.68556 $ & $  -0.00006 $ & $   0.00090 $ & $  10.80600 $ & $ i$\\
$ 54774.68662 $ & $   0.00064 $ & $   0.00090 $ & $  10.80730 $ & $ i$\\
$ 54774.68764 $ & $   0.00072 $ & $   0.00090 $ & $  10.80660 $ & $ i$\\
$ 54774.68867 $ & $  -0.00049 $ & $   0.00090 $ & $  10.80530 $ & $ i$\\
$ 54774.68971 $ & $  -0.00159 $ & $   0.00090 $ & $  10.80470 $ & $ i$\\
$ 54774.69172 $ & $  -0.00006 $ & $   0.00091 $ & $  10.80610 $ & $ i$\\
$ 54774.69275 $ & $  -0.00017 $ & $   0.00091 $ & $  10.80490 $ & $ i$\\
$ 54774.69378 $ & $   0.00103 $ & $   0.00090 $ & $  10.80670 $ & $ i$\\
$ 54774.69481 $ & $   0.00126 $ & $   0.00091 $ & $  10.80670 $ & $ i$\\
$ 54774.69583 $ & $  -0.00271 $ & $   0.00091 $ & $  10.80360 $ & $ i$\\
$ 54774.69687 $ & $  -0.00134 $ & $   0.00092 $ & $  10.80480 $ & $ i$\\
$ 54774.69791 $ & $  -0.00083 $ & $   0.00091 $ & $  10.80500 $ & $ i$\\
$ 54774.69893 $ & $  -0.00033 $ & $   0.00092 $ & $  10.80540 $ & $ i$\\
$ 54774.69995 $ & $   0.00067 $ & $   0.00092 $ & $  10.80660 $ & $ i$\\
$ 54774.70099 $ & $   0.00183 $ & $   0.00092 $ & $  10.80730 $ & $ i$\\
$ 54774.70203 $ & $  -0.00152 $ & $   0.00091 $ & $  10.80450 $ & $ i$\\
$ 54774.70304 $ & $  -0.00105 $ & $   0.00092 $ & $  10.80550 $ & $ i$\\
$ 54941.91431 $ & $   0.00237 $ & $   0.00105 $ & $  11.82210 $ & $ g$\\
$ 54941.91601 $ & $  -0.00024 $ & $   0.00106 $ & $  11.82160 $ & $ g$\\
$ 54941.91772 $ & $  -0.00021 $ & $   0.00105 $ & $  11.82180 $ & $ g$\\
$ 54941.91944 $ & $  -0.00028 $ & $   0.00104 $ & $  11.82050 $ & $ g$\\
$ 54941.92115 $ & $  -0.00348 $ & $   0.00106 $ & $  11.81630 $ & $ g$\\
$ 54941.92288 $ & $   0.00045 $ & $   0.00105 $ & $  11.82140 $ & $ g$\\
$ 54941.92460 $ & $   0.00057 $ & $   0.00104 $ & $  11.82010 $ & $ g$\\
$ 54941.92632 $ & $  -0.00150 $ & $   0.00104 $ & $  11.81920 $ & $ g$\\
$ 54941.92804 $ & $   0.00035 $ & $   0.00104 $ & $  11.82120 $ & $ g$\\
$ 54941.92975 $ & $   0.00132 $ & $   0.00107 $ & $  11.81920 $ & $ g$\\
$ 54941.93149 $ & $   0.00028 $ & $   0.00104 $ & $  11.82090 $ & $ g$\\
$ 54941.93320 $ & $   0.00107 $ & $   0.00103 $ & $  11.82090 $ & $ g$\\
$ 54941.93492 $ & $   0.00084 $ & $   0.00103 $ & $  11.82190 $ & $ g$\\
$ 54941.93662 $ & $   0.00036 $ & $   0.00104 $ & $  11.82230 $ & $ g$\\
$ 54941.93834 $ & $  -0.00314 $ & $   0.00103 $ & $  11.81690 $ & $ g$\\
$ 54941.94007 $ & $  -0.00017 $ & $   0.00103 $ & $  11.81990 $ & $ g$\\
$ 54941.94179 $ & $  -0.00009 $ & $   0.00102 $ & $  11.82100 $ & $ g$\\
$ 54941.94351 $ & $  -0.00026 $ & $   0.00102 $ & $  11.81900 $ & $ g$\\
$ 54941.94522 $ & $   0.00068 $ & $   0.00103 $ & $  11.82040 $ & $ g$\\
$ 54941.94694 $ & $   0.00105 $ & $   0.00102 $ & $  11.82080 $ & $ g$\\
$ 54941.94869 $ & $   0.00093 $ & $   0.00101 $ & $  11.82090 $ & $ g$\\
$ 54941.95041 $ & $   0.00120 $ & $   0.00103 $ & $  11.82160 $ & $ g$\\
$ 54941.95212 $ & $  -0.00104 $ & $   0.00102 $ & $  11.82000 $ & $ g$\\
$ 54941.95384 $ & $  -0.00114 $ & $   0.00102 $ & $  11.81840 $ & $ g$\\
$ 54941.95555 $ & $   0.00102 $ & $   0.00101 $ & $  11.82090 $ & $ g$\\
$ 54941.95729 $ & $  -0.00057 $ & $   0.00102 $ & $  11.81910 $ & $ g$\\
$ 54941.95900 $ & $   0.00025 $ & $   0.00101 $ & $  11.82080 $ & $ g$\\
$ 54941.96072 $ & $  -0.00043 $ & $   0.00101 $ & $  11.81990 $ & $ g$\\
$ 54941.96245 $ & $   0.00033 $ & $   0.00101 $ & $  11.82020 $ & $ g$\\
$ 54941.96415 $ & $  -0.00101 $ & $   0.00100 $ & $  11.81760 $ & $ g$\\
$ 54941.96590 $ & $  -0.00031 $ & $   0.00100 $ & $  11.82040 $ & $ g$\\
$ 54941.96761 $ & $   0.00041 $ & $   0.00100 $ & $  11.82070 $ & $ g$\\
$ 54941.96932 $ & $  -0.00093 $ & $   0.00101 $ & $  11.81850 $ & $ g$\\
$ 54941.97104 $ & $   0.00195 $ & $   0.00102 $ & $  11.82210 $ & $ g$\\
$ 54941.97276 $ & $  -0.00042 $ & $   0.00101 $ & $  11.81870 $ & $ g$\\
$ 54941.97450 $ & $   0.00188 $ & $   0.00101 $ & $  11.82160 $ & $ g$\\
$ 54941.97621 $ & $   0.00205 $ & $   0.00101 $ & $  11.82200 $ & $ g$\\
$ 54941.97794 $ & $   0.00484 $ & $   0.00101 $ & $  11.82380 $ & $ g$\\
$ 54941.97966 $ & $   0.00653 $ & $   0.00100 $ & $  11.82650 $ & $ g$\\
$ 54941.98137 $ & $   0.01221 $ & $   0.00102 $ & $  11.83230 $ & $ g$\\
$ 54941.98312 $ & $   0.01271 $ & $   0.00102 $ & $  11.83140 $ & $ g$\\
$ 54941.98485 $ & $   0.01331 $ & $   0.00101 $ & $  11.83290 $ & $ g$\\
$ 54941.98662 $ & $   0.01390 $ & $   0.00103 $ & $  11.83440 $ & $ g$\\
$ 54941.98832 $ & $   0.01460 $ & $   0.00104 $ & $  11.83430 $ & $ g$\\
$ 54941.99003 $ & $   0.01308 $ & $   0.00106 $ & $  11.83240 $ & $ g$\\
$ 54941.99178 $ & $   0.01642 $ & $   0.00110 $ & $  11.83550 $ & $ g$\\
$ 55026.84405 $ & $   0.00228 $ & $   0.00204 $ & $  11.43930 $ & $ i$\\
$ 55026.84489 $ & $   0.00341 $ & $   0.00202 $ & $  11.43450 $ & $ i$\\
$ 55026.84576 $ & $   0.00020 $ & $   0.00213 $ & $  11.43330 $ & $ i$\\
$ 55026.84660 $ & $  -0.00494 $ & $   0.00215 $ & $  11.42570 $ & $ i$\\
$ 55026.84746 $ & $  -0.00004 $ & $   0.00186 $ & $  11.43410 $ & $ i$\\
$ 55026.84832 $ & $  -0.00023 $ & $   0.00188 $ & $  11.43360 $ & $ i$\\
$ 55026.84917 $ & $  -0.00218 $ & $   0.00167 $ & $  11.43060 $ & $ i$\\
$ 55026.85002 $ & $  -0.00135 $ & $   0.00167 $ & $  11.43290 $ & $ i$\\
$ 55026.85087 $ & $  -0.00078 $ & $   0.00158 $ & $  11.43330 $ & $ i$\\
$ 55026.85173 $ & $   0.00187 $ & $   0.00151 $ & $  11.43650 $ & $ i$\\
$ 55026.85260 $ & $   0.00069 $ & $   0.00149 $ & $  11.43480 $ & $ i$\\
$ 55026.85346 $ & $   0.00068 $ & $   0.00150 $ & $  11.43250 $ & $ i$\\
$ 55026.85548 $ & $   0.00007 $ & $   0.00135 $ & $  11.43190 $ & $ i$\\
$ 55026.85632 $ & $   0.00066 $ & $   0.00137 $ & $  11.43230 $ & $ i$\\
$ 55026.85735 $ & $   0.00155 $ & $   0.00145 $ & $  11.42860 $ & $ i$\\
$ 55026.85820 $ & $  -0.00407 $ & $   0.00152 $ & $  11.42470 $ & $ i$\\
$ 55026.85923 $ & $  -0.00328 $ & $   0.00144 $ & $  11.42820 $ & $ i$\\
$ 55026.86008 $ & $   0.00073 $ & $   0.00140 $ & $  11.43100 $ & $ i$\\
$ 55026.86111 $ & $  -0.00162 $ & $   0.00134 $ & $  11.42970 $ & $ i$\\
$ 55026.86196 $ & $  -0.00115 $ & $   0.00137 $ & $  11.43010 $ & $ i$\\
$ 55026.86298 $ & $   0.00039 $ & $   0.00136 $ & $  11.42990 $ & $ i$\\
$ 55026.86383 $ & $  -0.00023 $ & $   0.00142 $ & $  11.43130 $ & $ i$\\
$ 55026.86489 $ & $  -0.00142 $ & $   0.00143 $ & $  11.42940 $ & $ i$\\
$ 55026.86574 $ & $   0.00352 $ & $   0.00148 $ & $  11.43590 $ & $ i$\\
$ 55026.86675 $ & $   0.00317 $ & $   0.00159 $ & $  11.43370 $ & $ i$\\
$ 55026.86759 $ & $  -0.00052 $ & $   0.00155 $ & $  11.43250 $ & $ i$\\
$ 55026.86862 $ & $   0.00158 $ & $   0.00144 $ & $  11.43390 $ & $ i$\\
$ 55026.86949 $ & $   0.00020 $ & $   0.00136 $ & $  11.43390 $ & $ i$\\
$ 55026.87052 $ & $   0.00218 $ & $   0.00143 $ & $  11.43680 $ & $ i$\\
$ 55026.87138 $ & $  -0.00325 $ & $   0.00153 $ & $  11.43020 $ & $ i$\\
$ 55026.87241 $ & $   0.00213 $ & $   0.00134 $ & $  11.43320 $ & $ i$\\
$ 55026.87325 $ & $  -0.00034 $ & $   0.00129 $ & $  11.43040 $ & $ i$\\
$ 55026.87430 $ & $  -0.00039 $ & $   0.00121 $ & $  11.43120 $ & $ i$\\
$ 55026.87515 $ & $   0.00248 $ & $   0.00119 $ & $  11.43340 $ & $ i$\\
$ 55026.87618 $ & $   0.00248 $ & $   0.00124 $ & $  11.43170 $ & $ i$\\
$ 55026.87704 $ & $   0.00293 $ & $   0.00125 $ & $  11.43120 $ & $ i$\\
$ 55026.87807 $ & $   0.00554 $ & $   0.00127 $ & $  11.43550 $ & $ i$\\
$ 55026.87894 $ & $   0.00051 $ & $   0.00127 $ & $  11.43040 $ & $ i$\\
$ 55026.87996 $ & $   0.00791 $ & $   0.00127 $ & $  11.43720 $ & $ i$\\
$ 55026.88080 $ & $   0.01007 $ & $   0.00121 $ & $  11.43720 $ & $ i$\\
$ 55026.88181 $ & $   0.00983 $ & $   0.00120 $ & $  11.43850 $ & $ i$\\
$ 55026.88266 $ & $   0.01130 $ & $   0.00120 $ & $  11.44160 $ & $ i$\\
$ 55026.88371 $ & $   0.01051 $ & $   0.00117 $ & $  11.44040 $ & $ i$\\
$ 55026.88456 $ & $   0.01166 $ & $   0.00119 $ & $  11.44130 $ & $ i$\\
$ 55026.88558 $ & $   0.01290 $ & $   0.00123 $ & $  11.44250 $ & $ i$\\
$ 55026.88643 $ & $   0.01306 $ & $   0.00126 $ & $  11.44100 $ & $ i$\\
$ 55026.88746 $ & $   0.01461 $ & $   0.00128 $ & $  11.44280 $ & $ i$\\
$ 55026.88832 $ & $   0.01540 $ & $   0.00127 $ & $  11.44560 $ & $ i$\\
$ 55026.88935 $ & $   0.01637 $ & $   0.00127 $ & $  11.44520 $ & $ i$\\
$ 55026.89022 $ & $   0.01345 $ & $   0.00128 $ & $  11.44310 $ & $ i$\\
$ 55026.89124 $ & $   0.01178 $ & $   0.00119 $ & $  11.44130 $ & $ i$\\
$ 55026.89209 $ & $   0.01492 $ & $   0.00119 $ & $  11.44550 $ & $ i$\\
$ 55026.89313 $ & $   0.01680 $ & $   0.00120 $ & $  11.44610 $ & $ i$\\
$ 55026.89397 $ & $   0.01635 $ & $   0.00118 $ & $  11.44470 $ & $ i$\\
$ 55026.89501 $ & $   0.01501 $ & $   0.00122 $ & $  11.44400 $ & $ i$\\
$ 55026.89587 $ & $   0.01378 $ & $   0.00125 $ & $  11.44230 $ & $ i$\\
$ 55026.89690 $ & $   0.01620 $ & $   0.00127 $ & $  11.44490 $ & $ i$\\
$ 55026.89777 $ & $   0.01707 $ & $   0.00127 $ & $  11.44680 $ & $ i$\\
$ 55026.89880 $ & $   0.01604 $ & $   0.00128 $ & $  11.44500 $ & $ i$\\
$ 55026.89964 $ & $   0.01460 $ & $   0.00123 $ & $  11.44310 $ & $ i$\\
$ 55026.90067 $ & $   0.01904 $ & $   0.00120 $ & $  11.44880 $ & $ i$\\
$ 55026.90151 $ & $   0.01587 $ & $   0.00119 $ & $  11.44660 $ & $ i$\\
$ 55026.90367 $ & $   0.01683 $ & $   0.00118 $ & $  11.44790 $ & $ i$\\
$ 55026.90452 $ & $   0.01823 $ & $   0.00119 $ & $  11.44850 $ & $ i$\\
$ 55026.90556 $ & $   0.01279 $ & $   0.00126 $ & $  11.44400 $ & $ i$\\
$ 55026.90642 $ & $   0.01582 $ & $   0.00128 $ & $  11.44600 $ & $ i$\\
$ 55026.90743 $ & $   0.01619 $ & $   0.00119 $ & $  11.44670 $ & $ i$\\
$ 55026.90830 $ & $   0.01477 $ & $   0.00124 $ & $  11.44470 $ & $ i$\\
$ 55026.90932 $ & $   0.01949 $ & $   0.00127 $ & $  11.44980 $ & $ i$\\
$ 55026.91015 $ & $   0.01844 $ & $   0.00121 $ & $  11.44760 $ & $ i$\\
$ 55026.91117 $ & $   0.01432 $ & $   0.00118 $ & $  11.44440 $ & $ i$\\
$ 55026.91202 $ & $   0.01686 $ & $   0.00118 $ & $  11.44760 $ & $ i$\\
$ 55026.91306 $ & $   0.01643 $ & $   0.00119 $ & $  11.44640 $ & $ i$\\
$ 55026.91390 $ & $   0.01583 $ & $   0.00124 $ & $  11.44630 $ & $ i$\\
$ 55026.91493 $ & $   0.01600 $ & $   0.00130 $ & $  11.44500 $ & $ i$\\
$ 55026.91578 $ & $   0.01497 $ & $   0.00119 $ & $  11.44480 $ & $ i$\\
$ 55026.91681 $ & $   0.01871 $ & $   0.00118 $ & $  11.44870 $ & $ i$\\
$ 55026.91768 $ & $   0.01772 $ & $   0.00118 $ & $  11.44810 $ & $ i$\\
$ 55026.91871 $ & $   0.01830 $ & $   0.00121 $ & $  11.44760 $ & $ i$\\
$ 55026.91956 $ & $   0.01488 $ & $   0.00126 $ & $  11.44430 $ & $ i$\\
$ 55026.92059 $ & $   0.01628 $ & $   0.00124 $ & $  11.44420 $ & $ i$\\
$ 55026.92146 $ & $   0.01694 $ & $   0.00118 $ & $  11.44720 $ & $ i$\\
$ 55026.92251 $ & $   0.01620 $ & $   0.00124 $ & $  11.44420 $ & $ i$\\
$ 55026.92337 $ & $   0.01720 $ & $   0.00124 $ & $  11.44580 $ & $ i$\\
$ 55026.92440 $ & $   0.01518 $ & $   0.00124 $ & $  11.44290 $ & $ i$\\
$ 55026.92525 $ & $   0.01874 $ & $   0.00118 $ & $  11.44700 $ & $ i$\\
$ 55026.92625 $ & $   0.01694 $ & $   0.00118 $ & $  11.44560 $ & $ i$\\
$ 55026.92712 $ & $   0.01689 $ & $   0.00120 $ & $  11.44590 $ & $ i$\\
$ 55026.92814 $ & $   0.01990 $ & $   0.00126 $ & $  11.44720 $ & $ i$\\
$ 55026.92898 $ & $   0.01699 $ & $   0.00121 $ & $  11.44350 $ & $ i$\\
$ 55026.93000 $ & $   0.01950 $ & $   0.00118 $ & $  11.44730 $ & $ i$\\
$ 55026.93085 $ & $   0.01704 $ & $   0.00118 $ & $  11.44570 $ & $ i$\\
$ 55026.93189 $ & $   0.01875 $ & $   0.00120 $ & $  11.44670 $ & $ i$\\
$ 55026.93273 $ & $   0.01696 $ & $   0.00125 $ & $  11.44310 $ & $ i$\\
$ 55026.93375 $ & $   0.01554 $ & $   0.00119 $ & $  11.44450 $ & $ i$\\
$ 55026.93461 $ & $   0.01760 $ & $   0.00118 $ & $  11.44720 $ & $ i$\\
$ 55026.93564 $ & $   0.01745 $ & $   0.00122 $ & $  11.44530 $ & $ i$\\
$ 55026.93651 $ & $   0.01789 $ & $   0.00127 $ & $  11.44510 $ & $ i$\\
$ 55026.93753 $ & $   0.01612 $ & $   0.00119 $ & $  11.44370 $ & $ i$\\
$ 55026.93838 $ & $   0.01386 $ & $   0.00119 $ & $  11.44340 $ & $ i$\\
$ 55026.93939 $ & $   0.01864 $ & $   0.00123 $ & $  11.44690 $ & $ i$\\
$ 55026.94024 $ & $   0.01349 $ & $   0.00128 $ & $  11.44260 $ & $ i$\\
$ 55026.94127 $ & $   0.01649 $ & $   0.00120 $ & $  11.44690 $ & $ i$\\
$ 55026.94211 $ & $   0.01377 $ & $   0.00119 $ & $  11.44320 $ & $ i$\\
$ 55026.94313 $ & $   0.01568 $ & $   0.00120 $ & $  11.44660 $ & $ i$\\
$ 55026.94397 $ & $   0.01483 $ & $   0.00126 $ & $  11.44420 $ & $ i$\\
$ 55026.94500 $ & $   0.01729 $ & $   0.00124 $ & $  11.44750 $ & $ i$\\
$ 55026.94586 $ & $   0.01349 $ & $   0.00120 $ & $  11.44510 $ & $ i$\\
$ 55026.94689 $ & $   0.01506 $ & $   0.00123 $ & $  11.44510 $ & $ i$\\
$ 55026.94775 $ & $   0.01375 $ & $   0.00129 $ & $  11.44390 $ & $ i$\\
$ 55026.94877 $ & $   0.01759 $ & $   0.00132 $ & $  11.44740 $ & $ i$\\
$ 55026.94961 $ & $   0.01640 $ & $   0.00122 $ & $  11.44690 $ & $ i$\\
$ 55026.95068 $ & $   0.01299 $ & $   0.00120 $ & $  11.44470 $ & $ i$\\
$ 55026.95153 $ & $   0.01176 $ & $   0.00120 $ & $  11.44420 $ & $ i$\\
$ 55026.95255 $ & $   0.01335 $ & $   0.00129 $ & $  11.44520 $ & $ i$\\
$ 55026.95341 $ & $   0.01447 $ & $   0.00127 $ & $  11.44570 $ & $ i$\\
$ 55026.95445 $ & $   0.01540 $ & $   0.00121 $ & $  11.44890 $ & $ i$\\
$ 55026.95531 $ & $   0.01238 $ & $   0.00121 $ & $  11.44530 $ & $ i$\\
$ 55026.95634 $ & $   0.01227 $ & $   0.00123 $ & $  11.44450 $ & $ i$\\
$ 55026.95719 $ & $   0.00988 $ & $   0.00130 $ & $  11.44160 $ & $ i$\\
$ 55026.95821 $ & $   0.00806 $ & $   0.00129 $ & $  11.43810 $ & $ i$\\
$ 55026.95907 $ & $   0.00358 $ & $   0.00121 $ & $  11.43650 $ & $ i$\\
$ 55026.96012 $ & $   0.00490 $ & $   0.00123 $ & $  11.43760 $ & $ i$\\
$ 55026.96096 $ & $   0.00682 $ & $   0.00129 $ & $  11.43690 $ & $ i$\\
$ 55026.96197 $ & $   0.00653 $ & $   0.00135 $ & $  11.43760 $ & $ i$\\
$ 55026.96281 $ & $   0.00451 $ & $   0.00134 $ & $  11.43440 $ & $ i$\\
$ 55026.96382 $ & $   0.00297 $ & $   0.00123 $ & $  11.43710 $ & $ i$\\
$ 55026.96469 $ & $   0.00234 $ & $   0.00121 $ & $  11.43740 $ & $ i$\\
$ 55026.96571 $ & $  -0.00024 $ & $   0.00123 $ & $  11.43400 $ & $ i$\\
$ 55026.96657 $ & $   0.00427 $ & $   0.00132 $ & $  11.43940 $ & $ i$\\
$ 55026.96757 $ & $  -0.00017 $ & $   0.00136 $ & $  11.43080 $ & $ i$\\
$ 55026.96842 $ & $  -0.00125 $ & $   0.00136 $ & $  11.43000 $ & $ i$\\
$ 55026.96947 $ & $   0.00135 $ & $   0.00132 $ & $  11.43440 $ & $ i$\\
$ 55026.97032 $ & $  -0.00035 $ & $   0.00124 $ & $  11.43450 $ & $ i$\\
$ 55026.97134 $ & $   0.00096 $ & $   0.00130 $ & $  11.43160 $ & $ i$\\
$ 55026.97219 $ & $  -0.00010 $ & $   0.00135 $ & $  11.43130 $ & $ i$\\
$ 55026.97323 $ & $   0.00234 $ & $   0.00137 $ & $  11.43140 $ & $ i$\\
$ 55026.97410 $ & $   0.00018 $ & $   0.00131 $ & $  11.43060 $ & $ i$\\
$ 55026.97514 $ & $  -0.00005 $ & $   0.00123 $ & $  11.43470 $ & $ i$\\
$ 55026.97599 $ & $  -0.00373 $ & $   0.00132 $ & $  11.42720 $ & $ i$\\
$ 55026.97701 $ & $  -0.00201 $ & $   0.00137 $ & $  11.42820 $ & $ i$\\
$ 55026.97785 $ & $   0.00092 $ & $   0.00139 $ & $  11.42930 $ & $ i$\\
$ 55026.97892 $ & $   0.00111 $ & $   0.00127 $ & $  11.43290 $ & $ i$\\
$ 55026.97979 $ & $  -0.00096 $ & $   0.00124 $ & $  11.43200 $ & $ i$\\
$ 55026.98082 $ & $  -0.00015 $ & $   0.00126 $ & $  11.43270 $ & $ i$\\
$ 55026.98167 $ & $   0.00044 $ & $   0.00134 $ & $  11.42960 $ & $ i$\\
$ 55026.98269 $ & $   0.00005 $ & $   0.00139 $ & $  11.42950 $ & $ i$\\
$ 55026.98441 $ & $  -0.00261 $ & $   0.00137 $ & $  11.42790 $ & $ i$\\
$ 55026.98525 $ & $  -0.00033 $ & $   0.00142 $ & $  11.42920 $ & $ i$\\


==> HTR341-004_phfu_tab_short.tex <==
$ 54632.73784 $ & $   0.02143 $ & $   0.00111 $ & $  10.98360 $ & $ i$\\
$ 54632.73870 $ & $   0.01830 $ & $   0.00116 $ & $  10.98170 $ & $ i$\\
$ 54632.73954 $ & $   0.01503 $ & $   0.00115 $ & $  10.97810 $ & $ i$\\
$ 54632.74039 $ & $   0.01859 $ & $   0.00115 $ & $  10.98340 $ & $ i$\\
$ 54632.74125 $ & $   0.01123 $ & $   0.00111 $ & $  10.97530 $ & $ i$\\
$ 54632.74208 $ & $   0.02006 $ & $   0.00109 $ & $  10.98390 $ & $ i$\\
$ 54632.74295 $ & $   0.01831 $ & $   0.00111 $ & $  10.98220 $ & $ i$\\
$ 54632.74381 $ & $   0.01766 $ & $   0.00114 $ & $  10.97840 $ & $ i$\\
$ 54632.74637 $ & $   0.02025 $ & $   0.00117 $ & $  10.99540 $ & $ i$\\
$ 54632.74722 $ & $   0.01556 $ & $   0.00112 $ & $  10.97990 $ & $ i$\\


==> HTR341-004_rvtable.tex <==
$ 638.09243 $ \dotfill & \nodata      & \nodata      & $    -4.89 $ & $     4.59 $ & $     1.170 $ & $     0.020 $\\
$ 638.10601 $ \dotfill & $  -137.90 $ & $     4.49 $ & $    -0.45 $ & $     5.22 $ & $     0.797 $ & $     0.006 $\\
$ 674.91404 $ \dotfill & $   374.64 $ & $     5.15 $ & $   -10.71 $ & $     3.99 $ & $     0.794 $ & $     0.006 $\\
$ 723.78719 $ \dotfill & $  -209.16 $ & $     5.55 $ & $    -1.68 $ & $    13.38 $ & $     0.738 $ & $     0.006 $\\
$ 725.85309 $ \dotfill & $   329.57 $ & $     6.18 $ & $    12.86 $ & $     6.55 $ & $     0.749 $ & $     0.006 $\\
$ 726.87976 $ \dotfill & $   277.98 $ & $     4.20 $ & $   -26.82 $ & $     6.17 $ & $     0.770 $ & $     0.005 $\\
$ 727.76247 $ \dotfill & $  -210.01 $ & $     4.81 $ & $   -35.11 $ & $     5.18 $ & $     0.811 $ & $     0.006 $\\
$ 727.89619 $ \dotfill & $   -19.91 $ & $     4.77 $ & $   -30.29 $ & $     5.05 $ & $     0.795 $ & $     0.005 $\\
$ 777.82189 $ \dotfill & $   214.73 $ & $     4.54 $ & $   -12.64 $ & $     4.43 $ & $     0.754 $ & $     0.005 $\\
$ 810.72960 $ \dotfill & $   290.22 $ & $     5.63 $ & $   -13.57 $ & $     5.59 $ & $     0.726 $ & $     0.006 $\\
$ 955.04676 $ \dotfill & $   388.82 $ & $     4.74 $ & $   -15.76 $ & $     3.57 $ & $     0.761 $ & $     0.006 $\\
$ 985.99494 $ \dotfill & $  -369.93 $ & $     4.42 $ & $   -19.69 $ & $     5.06 $ & $     0.718 $ & $     0.006 $\\
$ 1192.70812 $ \dotfill & $   348.01 $ & $     4.40 $ & $   -14.40 $ & $     4.53 $ & $     0.726 $ & $     0.005 $\\
$ 1193.71080 $ \dotfill & $    83.68 $ & $     4.57 $ & $   -20.67 $ & $     4.23 $ & $     0.825 $ & $     0.008 $\\


==> Makefile <==
TARGET=main
PRINTER=cfa_ssplx

all: $(TARGET).pdf $(TARGET).txt

SUB=submit_v1

.PHONY: all clean save print

$(TARGET).dvi: *.tex *.cls
	latex $(TARGET).tex
	latex $(TARGET).tex
	latex $(TARGET).tex

$(TARGET).ps: $(TARGET).dvi
	dvips -t letter $(TARGET).dvi -o

$(TARGET).pdf: $(TARGET).ps
	ps2pdf $< $@
	
$(TARGET).txt: $(TARGET).dvi
	dvi2tty $< -o$@ -w120

save:
	tar cvf $(TARGET).tar *
	gzip $(TARGET).tar
	mv $(TARGET).tar.gz $(TARGET).tgz

sub:
	test -d $(SUB) || mkdir $(SUB)
	test -d $(SUB)/img || mkdir $(SUB)/img
	cp $(TARGET).tex $(SUB)/hatpxx.tex
	cp img/*.eps $(SUB)/img

clean:
	rm -f $(TARGET).dvi $(TARGET).ps $(TARGET).pdf $(TARGET).txt \
		$(TARGET).aux $(TARGET).log

print: $(TARGET).ps
	lpr -P$(PRINTER) $<
	

